Litmus: Fair Pricing for Serverless Computing

Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times. This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2% price difference on average, in a heavily congested system.

==> 07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/00_abstract.tex <==
\begin{abstract}

% Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While the providers can utilize their machines more efficiently, the tenants only need to pay for the resources they consume. However, a serverless system co-runs thousands of short-living functions concurrently to maximize resource utilization, bearing frequent state shifts. Meanwhile, when the system gets too congested, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants are also charged higher costs when experiencing slowdowns since all commercial serverless platforms determine the tenants' costs proportional to their execution times.
Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times.

% This paper argues that the cloud providers should compensate the tenants for their loss when the server is over-provisioned. However, estimating the tenant's loss is challenging when there is no pre-profiled information about the function. Prior studies showed assessing the tenant's loss introduces heavy overheads. Instead, this paper proposes a new pricing model, Litmus pricing, which offers discounts based on the machine's state while presuming the tenant's loss under the state. To monitor the machine state correctly, Litmus pricing frequently conducts Litmus tests, an effectively lightweight solution to measure system congestion. Our experiments show that Litmus pricing can detect the impact of system congestion and offer near-ideal prices, with only a 0.38\% price difference. 
This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2\% price difference on average, in a heavily congested system.

\end{abstract}


==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Serverless computing is growing fast, satisfying today's high demands for better programmability. It allows tenants to develop their programs as stateless functions in high-level languages such as Python, Go, and JavaScript without concerns with low-level resource management and task scheduling~\cite{serverless2,serverless1,schall2022lukewarm,schall2023warming,mohammad2020SerInWild}. This advantage attracts cloud users, helping them to deploy their programs quickly with minimal effort. Recent reports note that over 50-70\% of cloud users have adopted serverless computing for their tasks~\cite{serverless1}.

% Serverless computing claims a pay-as-you-go pricing model where users only pay for the resources used by their functions. This requires the service provider to monitor and estimate the fine-grained resource usage by each user accurately. However, today's high-performance systems maximize resource efficiency by accommodating multiple applications simultaneously and allowing the resources to be shared by them. Such a shared system raises two major challenges. First, tracking a user's resource usage is a challenging task. While being shared, the system tracks the total usage but not a single user's. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress. These inferences between the applications not only make the system hard to track resource usage, but the users may get charged unfairly due to the delayed execution time.
Serverless computing also benefits tenants financially. Unlike traditional cloud platforms that require tenants to purchase the hardware resources needed to deploy their servers regardless of actual usage~\cite{amazonEC2Pricing}, serverless computing claims a pay-as-you-go pricing model, where tenants only pay for the resources consumed during the execution of their functions, facilitating significant cost savings. Meanwhile, this pricing requires service providers to accurately monitor and estimate each user's fine-grained resource usage~\cite{microsoftAzurePricing,awsLambdaPricing,googleCloudFunctionPricing}. 

% However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared system raises two major challenges. First, tracking a tenant's resource usage is a challenging task. While being shared, the system can only monitor a tenant's use of specific resources. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference between the applications not only makes the system hard to track resource usage, but the tenants may get charged unfairly due to the extended execution time~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}. 
However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared serverless system raises two major challenges. First, tracking a tenant's resource usage becomes challenging, as the system can only monitor a tenant's use of exclusively dedicated resources while the system is shared. Second, and more importantly, co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference not only complicates tracking resource usage but also leads to tenants being charged unfairly due to delayed execution times~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}.

% A serverless platform should provide an isolated runtime environment to a user. Otherwise, we argue that the platform provider must compensate a tenant's loss as a discount when it is not achievable. Therefore, we define a charged fee as fair when it reflects the tenant's slowdowns due to the resource sharing. The following two methods can be used to estimate a fair price under a multi-tenant environment. 
A serverless platform should provide a user with an isolated runtime environment. Otherwise, we argue that the platform provider should compensate a tenant's loss as a discount when the isolation is not achievable. Thus, we define a charged fee as fair when it reflects the tenant's slowdowns caused by resource sharing. The following two methods can be used to offer a fair price in a multi-tenant environment.

% First, strict resource partitioning can divide shared resources into multiple partitions, each assigned to a user exclusively. The user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strictly partitioned resources are well known to cancel the opportunities to utilize the given resource efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delayed execution directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources when requesting them. 
First, strict resource partitioning can divide shared resources into multiple partitions, each assigned exclusively to a user. This means the user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strict partitioning is known to cancel opportunities to utilize resources efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delay directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources they need when requested. 

% Alternatively, a discount-based scheme estimates a user's price relative to its slowdown, discounting from the price when run without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources. Thus, the providers can maximize their hardware utilization and earn more money with given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns or interference they get from co-running tasks without overpaying for exclusive resources.
% The tenants also can get a discount reasonably proportional to the amount of their slowdown when their jobs suffer from interference rather than endeavoring to secure necessary resources exclusively.
Alternatively, a discount-based scheme estimates a user's price relative to the slowdown experienced, discounting from the price when running the task without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources, enabling providers to maximize hardware utilization and generate more revenue with the given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns they experience due to co-running tasks, preventing them from overpaying for lowered service quality.

% While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Even if the platform can measure its execution time, computing the slowdown still requires knowing its baseline, which can be gained when executing it alone. The cloud platform could not pre-profile users' applications for reasons such as mandated privacy when processing confidential information. Even if the platform has such information, the function could operate differently when receiving different inputs. That is to say, online profiling is necessary, which unfortunately requires expensive runtime sampling, as proposed in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. All co-running tasks must be stalled when estimating a task's baseline performance. Massive short-living serverless functions make such a sampling-based solution even more impractical. Frequently sampling the baseline performance of thousands of co-running functions is unrealistic. This motivates a new practical solution that can be adopted in commercial platforms. 
While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Although the platform can measure its execution time, determining the slowdown requires knowing its baseline performance, which can be obtained when it runs without interference. However, such profiling is often prohibited due to security concerns, particularly when the function processes confidential information. Additionally, the function may behave differently, with varying inputs each time it runs. That is to say, online profiling is necessary. Unfortunately, this requires expensive runtime sampling, as presented in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. When assessing baseline performance, all co-running tasks must be stalled. Hundreds to thousands of concurrent short-lived functions make this approach indeed impractical, as frequently sampling the baseline performance of such numerous functions is unrealistic. Thus, a new, practical solution that can be adopted in serverless platforms is needed.

%In either approach, a tenant or a service provider bears the problem's complexity alone. Resource partitioning demands the tenant to know the needed resources while losing opportunities to utilize the resources better. Discounting demands a service provider to estimate the task's slowdown with heavy sampling overheads. Accordingly, both approaches complicate the problem while sacrificing the machine's efficiency. Instead, we claim this problem becomes simpler when both entities participate and carry a portion of the responsibilities. 

% Litmus addresses this challenge by imposing the responsibility on both entities. With Litmus, the serverless platform measures the system congestion that may delay a function's execution when every tenant's function starts. The service provider needs to determine a discount rate for a corresponding congestion state. Meanwhile, the tenant needs to know about a possible slowdown and a corresponding discount. 

% We highlight that both partitioning and sampling complicate the problem while sacrificing the machine's efficiency and can hardly be employed in serverless computing. The approaches in serverless must be lightweight and frequent to deal with the fast-changing environment with thousands of concurrent functions. This paper proposes Litmus pricing that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening the system performance. 
We highlight that both partitioning-based and sampling-based approaches complicate the problem, either sacrificing the machine's efficiency or appearing impractical for serverless computing. Approaches in serverless computing must be lightweight, frequent, and sensitive enough to deal with quickly changing environments with numerous concurrent functions. This paper proposes Litmus pricing, a method that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening system performance. 

% \hl{Measuring the server's congestion status is challenging work. Here, Litmus relies on our key observation that, although not limited, function implementation in serverless computing largely relies on high-level programming languages such as Python and GoLang, which require a relatively long startup. This startup overhead has been considered one of the major challenges in serverless computing. However, Litmus utilizes this startup to measure the system's congestion state. Our analysis of Python and GoLang observed that the activities during the startups are almost identical, with plenty of memory operations, regardless of the functions. Thus, we claim that the startup performance can be an index of the system state.}

% \hl{The Litmus test is based on our insight that the serverless functions perform broadly identical operations, with plenty of memory operations, during their long startups, preparing the runtime environment for the functions. Leveraging this observation, the platform can assess the system's congestion level, which hints at the tenant's discount amount. Additionally, Litmus pricing exploits our second insight that the performance of two resources, private and shared, are affected differently by the congestion. In particular, its impact on private resources is minor and predictable, while many functions significantly rely on them, spending most of their execution time with them. }

% During the execution of every function, Litmus pricing conducts a Litmus test, which measures the level of system congestion with no extra overhead using the function's startup process. The Litmus test is based on the observation that serverless functions perform largely identical operations during their startup time. Those operations usually prepare the runtime and include a large amount of memory access to shared hardware resources. In addition, Litmus pricing splits the hardware resources into "private" and "shared" and proposes charging different ratios on each. This further improves the accuracy of the discount calculation.
During each function's execution, Litmus pricing conducts a Litmus test, which measures the level of system congestion without adding extra overhead, using the function's startup process. Litmus test is based on the observation that serverless functions perform largely identical operations during their startup, typically involving significant memory accesses. Additionally, Litmus pricing splits the hardware resources into "private" and "shared" categories, proposing different charging ratios for each. This approach further enhances the accuracy of the discount calculation.

% In our experiments, the Litmus pricing estimates a tenant's price to be nearly ideal, with a \hl{0.38\%} difference from the ideal price, which discounts tenants proportional to their slowdowns.
% This study investigates Litmus pricing across different environments, ranging from restricted to crowded settings. We verify that crowded environments pose additional challenges. Despite this, Litmus pricing accurately estimates a tenant's price, deviating by only 0.26\% from the ideal price, discounting tenants proportional to their slowdowns.
This study investigates Litmus pricing across diverse environments with varying levels of system congestion. We confirm that crowded environments pose complex challenges. Despite this, Litmus pricing accurately estimates a tenant's cost, deviating by only 0.2\% on average from the ideal price that discounts tenants proportional to slowdowns.



==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/02_background.tex <==
\section{Background}
\label{sec:background}

% \textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while the service providers handle back-end implementation~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers, which are later invoked upon associated events~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. The serverless platform guarantees security by executing the tenant's function in a sandbox such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.
\textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while leaving back-end implementation managed by service providers~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. These functions are later invoked upon associated events. The serverless platform ensures security by executing the tenant's function in a sandbox, such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.

% Each tenant's function is stateless and expected to be short~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using the short-lived functions, the tenant can easily scale by invoking many of the functions without provisioning needed resources for themselves, relying on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. Inherently, massive short-living serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. The tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and clients mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Later, under the pay-as-you-go pricing, the tenant is charged for the consumed resources, typically the product of time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
Each tenant's function is stateless and expected to be short-lived~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using these short-lived functions, tenants can easily scale by invoking many functions without provisioning the needed resources for themselves, relying instead on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. In serverless computing, numerous short-lived serverless workloads run together on a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. Tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and tenants mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% In the traditional cloud, tenants purchase hardware resources for the contracted term to support their applications, which are often expected to be large in a server form. Thus, tenants must pay for the agreed period regardless of actual use. Instead, serverless workloads are generally small and launched on-demand as short-living event handlers. This workload difference develops a unique pricing policy, pay-as-you-go pricing. The tenant is charged only for the consumed resources during the execution, typically the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
In traditional cloud computing, tenants purchase hardware resources for a contracted term to support their applications, which are typically large servers. Thus, tenants must pay for the agreed period regardless of actual usage. In contrast, serverless workloads are generally small and launched on-demand as short-lived event handlers. This difference leads to a unique pricing policy known as pay-as-you-go. Under this model, tenants are charged only for the resources consumed during execution, typically calculated as the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, where Python is utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Also, over 90\% of organizations choose Python and Node.js for their AWS services. Other popular language runtimes are Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer a high level of abstraction from machine codes with good programmability and portability, improving the programmer's productivity. As a result, they have been adopted widely by serverless users. However, such high-level languages typically rely on runtime interpretation, which results in a slow start of program execution with extra launching steps. For instance, in the case of Python, when an application is launched, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the codes are compiled and executed. Once the execution is complete, the Python program is terminated, and all assigned resources are released~\cite{pythonUsage}.
\textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python used in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Over 90\% of organizations choose Python and Node.js for their AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer significant abstraction from machine code with good programmability and portability, which in turn improves programmer productivity. Consequently, they are widely adopted by serverless users. However, high-level languages typically rely on runtime interpretation, leading to slower program startup due to extra launching steps. For example, when an application is launched in Python, the interpreter is first prepared. It then parses command-line arguments and imports necessary modules. Afterward, the codes are compiled and executed. Upon completion, the Python program terminates, and all allocated resources are released~\cite{pythonUsage}.

 
% list of pricing models? 
% Amazon? 
% Google?
% The price is calculated by duration time multiplies to the unit price plus the request charges. The duration time is from the time user's code begins executing until it returns or terminates. The unit price depends on the amount of memory the user allocate to their function. The request charges is based on how many times the function has been invoked minus the free requests~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% may need service agreement here, contention impact

%\textbf{Traditional cloud platforms:} In the context of traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage, data transfer, etc. The instance type is the combination of Virtual CPUs(VCPUs), RAM, storage and network performances. The time unit price will be higher with more powerful instance type. Typically, more powerful instance types have higher time unit prices. There are two main pricing options: On-Demand and Reserved Instances. On-demand instance let the customers pay for compute capacity by the hour or second based on the actual usage with no long-term commitments. Reserved Instances, on the other hand, require a commitment to a specific instance type for a contract term and offer cost savings compared to On-Demand pricing. Storage and data transfer for the VM instance can also impact the pricing. The more storage space a customer uses or the more data they transfer, the higher their costs will be. The traditional cloud platform can also be affected by the co-running applications~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} In traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage space, data bandwidth, etc. The instance type includes virtual CPUs, RAM, storage, and network performances. Typically, more powerful instance types charge higher prices. Also, two pricing options are commonly offered: on-demand and reserved instances. On-demand instances allow tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved instances require a commitment to a specific instance type for an agreed term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period. Storage space and data bandwidth for the VM instance also influence the price. Demanding more storage space or more data transfer raises the cost~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} 

% The price of traditional cloud platforms is determined by computing capabilities such as processor type, memory capacity, and network bandwidth. While more and better resources typically charge higher prices, two pricing options are commonly offered: on-demand and reserved instances. On-demand pricing allows tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved pricing requires a commitment to specific resources for an agreed-upon term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period~\cite{amazonEC2Pricing}. 

% There are several differences between traditional cloud platforms and serverless platform. 
% Firstly, the roles of customers in the execution environment differ between traditional and serverless platforms. In the traditional cloud, customers are responsible for configuring and maintaining virtual machines (VMs), setting up networking, and managing databases~\cite{amazonEC2Pricing}. And it's the customers's responsibility to detact and update the configurations to balance their expenses and performance. On the other hand, in serverless platforms, users only provide a single file to indicate their system and library requirement, while the service provider handles the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. This feature enables users to focus solely on their actual workload without the burden of managing the infrastructures. Additionally, the platform can automatically scale the resources for the users based on the current demand of the application to guarantee the customer satisfaction~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% There are apparent differences between traditional and serverless cloud platforms. First, tenants are responsible for managing hardware resources in traditional platforms. The tenants need to configure and maintain virtual machines, set up networking, and manage databases~\cite{amazonEC2Pricing}. Also, tenants should study the optimal configurations to balance their expenses and performance. Meanwhile, in serverless platforms, tenants only provide a single file to specify their system requirements while the cloud provider prepares the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. The platform provisions or scales the needed resources on demand. Consequently, the serverless platforms encourage tenants to focus solely on their front-end workloads without the burden of managing the low-level back-ends~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% Secondly, there are notable differences in compute power and memory size options between the two platforms. For traditional cloud, the granularity usually 1 VCPU and 1GB memory. But, for serverless platform, the smallest memory size is 128 MB~\cite{awsLambdaApiGateWay,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Thirdly, the characteristics of workloads on these platforms set them apart. Serverless applications are generally small and executed on-demand, resulting in very short workload durations~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can complete in less than one second. In contrast, traditional cloud applications tend to be larger and may require hours to complete. Additionally, the number of co-located applications on a single computing node is smaller in traditional cloud setups, making their execution environment less dynamic compared to serverless platforms.
% Lastly, the billing periods differ significantly between traditional cloud and serverless platforms. Traditional cloud users are charged for the allocated time period. Regardless of whether they are actively running tasks on the machine, they are still need to pay for the allocated time period. However, serverless customers are only billed for the actual execution time of their tasks on the platform.

% Second, the workloads are expected to be small in serverless computing. Serverless workloads are generally small and launched on-demand as short-living event handlers~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can be completed in less than one second, unlike traditional cloud applications that are often expected to be large in a server form. Inherently, massive serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. This workload difference develops a unique pricing policy in serverless computing, pay-as-you-go pricing. In the traditional cloud, the tenants purchase hardware resources for the contracted term. Regardless of actual use, they need to pay for the agreed period. However, the serverless platforms bill their tenants for the actual execution time of their tasks.


% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python being utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Furthermore, over 90\% of organizations leverage Python and Node.js alongside AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer numerous advantages for programmers, such as user-friendliness, portability, reduced error risks, and thriving ecosystems. As a result, they have garnered widespread acceptance within serverless platforms. High-level programming languages typically follow a fixed execution procedure. For instance, in Python, when an application is executed, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the code is compiled and executed. Once the execution is complete, the Python program is terminated, and all resources used by the program are released. Due to the consistency of the operating system and Python version, the beginning of the execution process remains the same each time~\cite{pythonUsage}.



% \textbf{Resource based discount vs. Slowdown based discount:} To fully utilize the available resources, service providers often run as many applications as they can in one computing node within the service agreement requirement. However, this may lead to resource congestion and cause slowdowns for users, which can be unfair, since the customers are paying more money for the worse experiences. The intuitionistic solution could be for the service provider to track the resource usage of each application and offer discounts to users who consume fewer resources. However, serverless applications are typically very small, and contention can affect different applications differently, making this approach less practical. A more suitable solution for serverless platforms could involve offering slowdown-based discounts. In this approach, the service provider dynamically updates unit prices based on the level of system congestion. When there is less contention, users normally stiffed with the experiences and pay the regular price. However, during periods of high congestion, when the system is under heavy load, users could receive discounted prices as compensation for potential slowdowns. This approach would align pricing with the actual performance experienced by users, ensuring a fair and responsive pricing model.


==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/03_methodology.tex <==
\section{Methodology}
\label{sec:method}

% \textbf{Hardware Infrastructure:} All the experiments are performed on a dual-socket server platform. Each socket has 16 simultaneous multithreading(SMT) cores. The CPU model is Intel Xeon Gold 5218(Cascade Lake). The maximum frequency of the machine is 3.9GHz. Each core has a 32KB L1 instruction cache, a 32KB L1 data cache and a 1MB L2 cache. The 32 virtual cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The computer node runs the latest Ubuntu server version(Ubuntu 22.04 LTS) with kernel version 5.15.0. For consistency in the results, the core frequency was set to 3.0GHz using the 'cpupower frequency-set' command. We use linux perf~\cite{perfWiki} to collect the performance counters for each experiment. To analyze the startup status, we use -I 1 option to obtain count deltas at one-millisecond intervals. By utilizing interpolation, we can know the performance counters of each execution period. 

% In this study, we test today's server systems with serverless functions. This section describes our test configuration. 
This section outlines our test setup for evaluating serverless functions in this study.

% % original version
% \textbf{Hardware Infrastructure:} All experiments are performed on a dual-socket server platform with two Intel Xeon Gold 5218 (Cascade Lake). The CPU offers 16 simultaneous multithreading (SMT) cores with 3.9 GHz maximum frequency. We pin the core frequency at 3.0GHz for our tests. Each core has 32KB L1 instruction/data caches and 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The machine runs the Ubuntu server OS (Ubuntu 22.04 LTS) with a kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to collect the performance counters, which are collected at every one-millisecond interval. 
\textbf{Hardware Infrastructure:} All experiments are conducted on a dual-socket server platform equipped with two Intel Xeon Gold 5218 processors based on the Cascade Lake architecture. Each CPU provides 16 cores that support simultaneous multithreading (SMT) with a maximum frequency of 3.9 GHz. Every core features 32KB of L1 instruction/data caches and a 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets collectively have access to 384GB of main memory. The server operates on Ubuntu Server OS, version 22.04 LTS, with kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to gather performance counters.

% The CPU frequency is a key performance/energy factor, significantly affecting a function's execution time and energy consumption. A CPU's frequency can be altered in software or hardware based on its power and thermal budget, configuring it for better energy efficiency or performance. However, varying frequencies cause the system performance/energy to be unsettled, making system management intractable. For this reason, commercial systems such as Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. In our tests, when the frequency is not fixed by software, Intel's Turbo technology alters the frequency occasionally but mainly employs 2.8GHz. We will discuss this further in the sensitivity section.
The CPU frequency is a critical factor influencing both performance and energy consumption, significantly affecting a function's execution time and energy usage. A CPU's frequency can be adjusted through software or hardware based on power and thermal budget, optimizing for either energy efficiency or performance. However, varying frequencies can cause instability in system performance and energy usage, complicating system management. For this reason, commercial systems like Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. If we do not fix the frequency through software, Intel's Turbo technology occasionally adjusts it, but it mostly remains at 2.8 GHz during our tests. We will provide more details on this in Section~\ref{sec:sensitivity}.

% \textbf{Stressing Programs:} We used two stressing programs to investigate how applications and the startup portion of the high level languages behave in a resource contention environment. FigureXXX illustrates the number of instructions, L3 accesses, and L3 misses that the stressing programs can generate in five seconds as the stressing levels increase. By combining different stress levels of these stress-testing programs, we can simulate various resource-congested environments. The XXX-stressor(lineXXX)  generates more L3 accesses with a high L3 hit rate. While XXX-stressor(lineXXX), in each stressing level, generates fewer L3 accesses but more L3 misses. With these two stressors and different stressing levels, we can simulate the system with varying contentions to the shared resources by creating various  L3 accesses and L3 misses. In figureXXX we can see that the L3 accesses generated from the L2-stressor (update name later) begin to decrease after reaching stressing level 20.  However, during this period, the L3 misses continue to increase. The reason behind this trend is that, after stressing level 20, the heightened L3 miss rate starts to impact the stressor's performance, leading to a decline in the committed instruction count. Consequently, the stressor generates fewer L3 accesses and more L3 misses. 

% \begin{table}[h]
%     \begin{center}
%     % \vspace{-1.0em}
%         \caption{Serverless Benchmarks \& Runtimes}
%         \label{tb:benchmarks}
%         % \vspace{-1.0em}
%         \begin{tabular}{|l l||l l|} \hline
%             Function & Abbr. & Function & Abbr. \\ \hline \hline
%             \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  & \multicolumn{2}{c|}{\textbf{Hotel Reservation~\cite{gan2019open}}} \\ \hline
%             Dyn HTML & dyn-py & Geo & geo-go* \\ \hline
%             Thumbnail & thum-py* & Profile & profile-go \\ \hline
%             Compression & compre-py & Rate & rate-go \\ \hline
%             Image Recogn & recogn-py* & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
%             Graph Rank & pager-py & Currency & cur-nj* \\ \hline
%             Graph Mst & mst-py & Payment & pay-nj \\ \hline
%             Graph Bfs & bfs-py* & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
%             DNA Visual & visual-py* & Authen & auth-py/nj/go \\ \hline
%             \multicolumn{2}{|c||}{\textbf{Function Bench~\cite{kim2019functionbench}}} & Fibonacci & fib-py/nj/go* \\ \hline
%             Chameleon & chame-py & AES & aes-py/nj/go \\ \hline
%             FloatOp & float-py* & & \\ \hline
%             % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
%         \end{tabular}
%     \end{center}
%     % \vspace{-1.5em}
% \end{table}

\begin{table}[h]
    \begin{center}
    % \vspace{-1.0em}
        \caption{Serverless Benchmarks \& Language Runtimes (py, nj, go)}
        \label{tb:benchmarks}
        % \vspace{-1.0em}
        \begin{tabular}{|l l||l l|} \hline
            Function & Abbr. & Function & Abbr. \\ \hline \hline
            \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  &  \multicolumn{2}{|c|}{\textbf{Function Bench~\cite{kim2019functionbench}}}\\ \hline
            Dyn HTML & dyn-py & Chameleon & chame-py \\ \hline
            Thumbnail & thum-py* & FloatOp & float-py \\ \hline
            Compression & compre-py & Gzip & gzip-py* \\ \hline
            Image Recogn & recogn-py & RandDisk & randDisk-py* \\ \hline
            Graph Rank & pager-py & SequenDisk & seqDisk-py \\ \hline
            Graph Mst & mst-py & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
            Graph Bfs & bfs-py* & Currency & cur-nj* \\ \hline
            DNA Visual & visual-py* & Payment & pay-nj \\ \hline
            \multicolumn{2}{|c||}{\textbf{Hotel Reservation~\cite{gan2019open}}} & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
            Geo & geo-go & Authen & auth-py*/nj/go \\ \hline
            Profile & profile-go* & Fibonacci & fib-py*/nj*/go* \\ \hline
            Rate & rate-go & AES & aes-py/nj*/go* \\ \hline
            % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
        \end{tabular}
    \end{center}
    % \vspace{-1.5em}
\end{table}

% revision version
% \textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we select 27 distinct serverless functions from different benchmark suites, including AWS' authentication serverless functions~\cite{awsLambdaApiGateWay}, Hotel Reservation from the DeathStarBench suite~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and SeBS serverless benchmark suite~\cite{copik2021sebs}. The three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating 3 separate test cases per function. Among them, we pick 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. The functions are implemented using three languages: Python, Nodejs, and Go. We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. 
\textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we selected 27 distinct serverless functions from various benchmark suites, including AWS authentication serverless functions~\cite{awsLambdaApiGateWay}, the Hotel Reservation from DeathStarBench~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and the SeBS serverless benchmark suite~\cite{copik2021sebs}. The functions are implemented using three languages: Python, Nodejs, and Go. Notably, the three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating three separate test cases per function. 
% This comprehensive language support ensures that our test coverage is thorough and representative of the diverse language preferences in the serverless computing community. 
We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. Additionally, we selected 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. 


%\hl{The benchmarks we choose include I/O-bound, memory-bound, and compute-bound functions. For an experiment, we put the testing function in core 0 to core 4. We also put 50 other functions in core 0-4 to let the application co-running with 10 other applications to observe the impact of context switching.}

% \hl{We select benchmarks with mixed performance characteristics: I/O, memory, and compute-bound. Also, to replicate the congested commercial systems, we located a testing function with 50 other functions and tied them to selected 5 cores, Core 0 to 4. During our evaluation, those functions run simultaneously and compete to secure any core among the five.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
\caption{(a) L2 misses and (b) L3 misses of traffic generators, both normalized with the average L2 and L3 misses of serverless applications listed in Table~\ref{tb:benchmarks}}
% \vspace{-0.5em}
\label{fig:stressing_specs}
\end{figure}

% \textbf{Traffic Generator:} We divide the CPU's shared resources into two distinct categories: resources before and after the L3 caches. To pressure each resource group individually, we developed two separate traffic generators aimed at generating traffic and congestion in these resources. The first traffic generator, CT-Gen, applies pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another traffic generator, MB-Gen, induces massive L3 misses that stress the resources after the L3 cache, mainly the off-chip memory bandwidth and L3 cache spaces.
\textbf{Traffic Generator:} We categorize the CPU's shared resources into two groups: those before the L3 caches and those after. To stress each group independently, we developed two separate traffic generators designed to generate traffic and congestion within these resources. The first generator, CT-Gen, exerts pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another generator, MB-Gen, induces massive L3 misses, which stress the resources beyond the L3 cache, primarily targeting off-chip memory bandwidth and L3 cache spaces.

% Both traffic generators are multi-threaded, governing the volume of traffic by adjusting the number of threads they spawn. Each thread spawned by the traffic generator is pinned on each core to prevent conflicts between threads; consequently, this setup allows us to vary the stress level across our 32-core processors, ranging from level 1 to 31. Figure~\ref{fig:stressing_specs} shows each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), for every thread count increment, CT-Gen makes massive L2 misses. The CT-Gen's L2 misses are ended with L3 hits, as shown in Figure~\ref{fig:stressing_specs}(b). Meanwhile, MB-Gen creates huge L2 and L3 misses, as implemented. Interestingly, its L2 misses are fewer than CT-Gen's because MB-Gen is slowed by its L3 misses, suffering from a self-created bandwidth bottleneck. 
Both traffic generators are multi-threaded and govern the amount of traffic by adjusting the number of threads they spawn. Each thread is pinned to a specific core to avoid conflicts between threads, allowing us to vary the stress level on our 32-core processors from level 1 to 31. Figure~\ref{fig:stressing_specs} illustrates each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), with each increase in thread count, CT-Gen generates substantial L2 cache misses. These L2 misses by CT-Gen are ended with L3 cache hits, as shown in Figure~\ref{fig:stressing_specs}(b). In contrast, MB-Gen produces significant L2 and L3 cache misses. Interestingly, MB-Gen's L2 misses are fewer than those of CT-Gen because MB-Gen is hindered by its L3 misses, suffering from a self-imposed performance bottleneck.



==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/04_motivation.tex <==
\section{The Need for Fair Pricing}
\label{sec:motivation}

% Offering fairness appears in different approaches in cloud computing when multiple tenants share hardware resources. One standard is SLA, which defines the level of services the cloud provider furnishes while a tenant sets their expectation. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving unfairness between tenants. Although serverless computing highlights the pay-as-you-go pricing model, such unfairness still exists.
Fairness in cloud computing, especially when multiple tenants share hardware resources, is addressed through various approaches. One standard method is the Service Level Agreement (SLA), which specifies the level of service the cloud provider must deliver and the tenants' expectations. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving fairness issues. Despite serverless computing's emphasis on a pay-as-you-go pricing model, unfairness among tenants still exists.

% Unfortunately, modern systems are designed to maximize hardware efficiency by co-running multiple applications; the function's execution time can be affected by co-scheduled applications with conflicts when using shared resources. Ironically, whenever the service provider squeezes their resources further for better profit by accommodating more functions into a single machine, each function's execution time increases, charging them a higher cost for the same workload. However, in serverless computing, tenants lack control and insights into how their software is executed and billed for the cost of convenience. 
Unfortunately, modern systems are designed to maximize hardware efficiency by running multiple applications concurrently. This results in conflicts over shared resources, affecting each function's execution time. Ironically, when service providers optimize for profit by packing more functions into a single machine, the execution time for each function increases, resulting in higher costs for the same workload. In serverless computing, tenants have no control or visibility over how their software is executed, leading to potential inefficiencies and higher costs for the sake of convenience.

% Genuine pay-as-you-go pricing can be achieved when there is no interference. However, that is not desired by the providers who expect to utilize their resources to maximize profits. In serverless, although each function runs virtually exclusively in a sandbox with private resources, it still shares a few resources with other co-running functions, such as shared caches and memory bandwidth. Resource partitioning, a traditional solution that eliminates interference, can promise exclusively dedicated resources to a tenant but cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 
In serverless computing, although each function runs exclusively in a virtual sandbox with private resources, it still shares certain resources like caches and memory bandwidth with other functions. Resource partitioning, a traditional solution that eliminates interference by dedicating resources exclusively to a tenant, cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 

\begin{figure}[h]
\centering
% \vspace{-0.7 em}
\includegraphics[width=1\columnwidth]{./fig/normalizedCPIRunWith26Rev}\\
% \vspace{-1 em}
\caption{Execution time of applications that run with 26 others, normalized to the execution time when running alone}
% \vspace{-0.4 em}
\label{fig:normalizedCPIRunWith26Rev}
\end{figure}

% Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed down when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. \hl{Whenever a function finishes, another function is randomly launched to maintain a total of 26 co-running functions.} The figure shows a function's performance drops by up to 35\%, and most functions are significantly influenced by the co-running functions. Compared to when an isolated environment is offered, the function performs 11.5\% slower on average, charging 11.5\% more to users. We highlight that the function runs only with 26 other functions, which is tiny compared to massively crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.
Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. Whenever a function finishes, a new randomly-selected function is launched to maintain a total of 26 co-running functions. The figure shows a function's performance can drop by up to 35\%, with most functions significantly impacted by the co-running functions. On average, functions perform 11.5\% slower in this shared environment compared to an isolated one, resulting in users being charged 11.5\% more. We highlight that this scenario involves only 26 co-running functions, which is tiny compared to heavily crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.

% Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} attempted to offer price discounts if it has a slowdown, compensating for the slowdowns. To provide the discount, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount reflecting the slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all the responsibilities of the contentions between co-running functions, guaranteeing all tenants an invariant price for their use. Any unexpected slowdowns that a tenant experiences are returned with a discount. However, sampling is an expensive operation, requiring all co-running processes to stall during the sampling. Moreover, accurate measurement requires frequent sampling when its system environment quickly alters, making the approach impossible in a fast-shifting environment like a serverless platform.   
Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} offers price discounts to compensate for slowdowns. To provide these discounts, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount based on the observed slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all responsibilities related to contentions from resource sharing, ensuring tenants pay a consistent price for their usage. Any unexpected slowdowns that a tenant experiences are compensated with a discount. However, sampling is an expensive operation that requires stalling all co-running processes during the sampling. Moreover, accurate measurement necessitates frequent sampling, especially in rapidly changing environments, making the approach impractical for dynamic environments like serverless platforms.


% A tenant needs a new pricing model based on more than just execution time. However, prior approaches have limitations, burdening cloud participants too heavily; it is unsuitable for \hl{thousands} of concurrent short-lived functions in serverless computing. This motivates us to propose a new solution, Litmus pricing, that discounts prices based on the system state but offers lightweight with no overheads.
Overall, tenants need a new pricing model that considers more than just execution time. Prior approaches have limitations, excessively burdening cloud participants and being unsuitable for the many short-lived functions typical in serverless computing. This motivates us to propose a new solution: Litmus pricing, which discounts prices based on the system congestion while remaining lightweight and imposing no additional overhead.


==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/05_design.tex <==
\section{Litmus Pricing}
\subsection{Overview}

% The estimated prices of serverless functions should reflect the congestion level of the system inside their machines. With the massive short-living functions, the serverless system's state can dramatically change in a short time. Accordingly, the system state can be congested at any moment and also resolved in a short time. However, such a temporary traffic jam may significantly impact the performance of short-living functions. Therefore, assessing the congestion must be lightweight, quick, and on time. However, a prior approach, POPPA\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling with considerable performance overheads, preventing them from wide adoption. Instead, we propose a new scheme, Litmus pricing, that quickly estimates system congestion at the start of every function and reflects the estimation into pricing the function. 
The estimated prices of serverless functions should reflect the system's congestion state. The presence of numerous small transient functions within the serverless system can rapidly alter its congestion state, causing sudden congestion or swift resolution. Nevertheless, such transient traffic jams can significantly impact the performance of short-lived functions. Thus, assessing the congestion must be lightweight, quick, and timely. However, a prior approach, POPPA~\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling, which incurs considerable performance costs, thereby limiting its widespread adoption. Alternatively, this study introduces Litmus pricing, which promptly gauges system congestion at the onset of each function and reflects the estimated congestion level into pricing the function.

% Like the prior approach~\cite{tiwari2013enabling,alex2013ScFairPrice}, Litmus pricing suggests that the service provider discounts when a tenant's functions are intervened, compensating for the performance loss. To determine the discount ratio, Litmus measures system congestion level, which can also help service providers evaluate remaining resources and make decisions on job scheduling. 
Like the prior approach, Litmus pricing suggests that service providers should offer discounts when a tenant's functions experience interference, thus compensating for the performance loss. Litmus pricing determines the discount rate based on the system's congestion level. Evaluating congestion also assists providers in estimating remaining resources and making informed decisions regarding job scheduling.

%Nevertheless, the Litmus pricing does not quantify each function's slowdown; the discount amount is determined only by the severity of the measured congestion. The impact of the congestion on distinct functions appears differently despite facing the same congestion level, and precisely estimating a function's performance loss is a complex problem. That's why the prior approach had to rely on expensive sampling. Instead, the Litmus pricing avoids the overheads and limits the service provider's responsibility to measure the current congestion. 
However, Litmus pricing does not quantify the slowdown of each individual function; the discount amount is solely determined by the severity of the measured congestion. Even though different functions face the same congestion level, their respective impacts can vary, making precise estimation of each function's performance loss a challenging task. This complexity necessitated the expensive sampling relied upon by the previous approach. Instead, Litmus pricing circumvents such overheads and lightens the service provider's burden solely to measure ongoing congestion levels.

% Litmus pricing embodies the varying value of shared resources across different system conditions by applying equal discounts to all functions under the same system condition, although the functions experience different slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that a function that is slowed more than others demands the over-crowded resources more while exacerbating the adverse over-crowded conditions. Litmus pricing does not provide additional compensation for their extra loss compared to others due to their heavy use of shared resources.
Litmus pricing captures the dynamic significance of shared resources under varying system conditions by offering uniform discounts to all functions under the same system congestion, regardless of their individual slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that functions experiencing larger slowdowns tend to demand more of the crowded resources, thereby exacerbating adverse overcrowded conditions. However, Litmus pricing does not offer additional compensation for the larger loss experienced by functions that use shared resources more heavily than others.

% As a result, Litmus inherently incentivizes users who use shared resources sparingly. When over-crowded, functions with minimal needs for shared resources still enjoy discounts but encounter slight slowdowns. This implies that users may take advantage of this policy by minimizing their use of shared resources, receiving substantial discounts despite enduring only minor slowdowns. Such a trade-off is considered acceptable because the user's shared resource usage reduces their contribution to congestion, thereby benefiting the overall system over the other users.
As a result, Litmus inherently incentivizes users who use shared resources sparingly. During periods of overcrowding, functions with minimal needs for shared resources still enjoy discounts but with only slight slowdowns. This implies that users may take advantage of this policy by minimizing their reliance on shared resources, receiving substantial discounts despite only experiencing minor slowdowns. This trade-off is considered acceptable because reduced shared resource usage by users helps mitigate congestion, thereby benefiting the overall system and other users.
% Lastly, the system refrains from scheduling a function if the congestion level exceeds a predetermined threshold, thus preventing resource thrashing.


\subsection{Pricing Model}
\label{pricing model}

% Developing Litmus pricing raises two challenges. First, Litmus needs a new pricing model to estimate a function's price. Second, Litmus needs a way to measure the system's congestion state. Due to the serverless's fast-shifting environment, assessing the congestion must be lightweight and frequent at the right time. Nevertheless, all present commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants must pay more with prolonged execution time when using over-crowded resources. Rather than simply imposing a price by multiplying the main memory usage and a function's total execution time, Litmus suggests the price as a sum of two distinct price components as follows.
Developing Litmus pricing raises two challenges. First, it needs a new model to estimate a function's price. Second, it needs a way to measure the system's congestion state. Due to the rapidly changing environment in serverless computing, assessing congestion must be lightweight and timely. Commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants end up paying more for prolonged execution time when using over-crowded resources. Rather than simply imposing the price by multiplying the main memory usage and a function's execution time, Litmus pricing determines the price as a sum of two distinct pricing components as follows.

\begin{equation} 
P = P_{private} + P_{shared}
\end{equation}

% In this equation, \(P\) denotes the total price tenants need to pay to execute their functions. Litmus pricing divides the tenant's price into two pricing components, each with a different resource type. \(P_{private}\) represents the price the tenant needs to pay for private resources, which are entirely assigned to a tenant. \(P_{shared}\) is the price the tenant needs to pay for the shared resources. Each price component is measured proportional to a user's time to occupy the corresponding resources. However, such occupied time can be extended when contention disturbs a process's execution in the shared resources. This delayed time increases a tenant's price unfairly. 
In this equation, \(P\) denotes the total price tenants must pay to execute their functions. Litmus pricing divides this cost into two pricing components, each associated with a different resource type. \(P_{private}\) is the cost for private resources, which are entirely assigned to a single tenant. \(P_{shared}\) is the cost for shared resources. Each pricing component is measured proportional to the time users occupy the respective resources. However, if contention disturbs a process's execution in the shared resources, the occupied time will be extended. This delay unfairly increases the tenant's cost. 


\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/slowdownRunwith26Rev}\\
\caption{\(T_{private}\) and \(T_{shared}\) of applications that run with 26 others, normalized to those when running alone}
\vspace{-0.5em}
\label{fig:slowdownRunwith26Rev}
\end{figure}

% Using Perf, we measure the delays due to the shared resources and split a function's execution time into two distinct slices: one slice, \(T_{private}\), which is time spent on private resources and another slice, \(T_{shared}\), which is time spent on shared resources. Figure~\ref{fig:normalizedTcore&Tuncore-runWith16} shows the impact of the contentions on each time slice, where we normalize \(T_{private}\) per instruction and \(T_{shared}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 207\% on average and 364\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions. 

% We observe that the system congestion influences the occupied time for each resource type differently. The time to hold private resources is slightly affected, with minor changes, even under heavy congestion. Meanwhile, the time due to shared resources is broadly affected, showing significant differences. Thus, we separately measure the two delays and charge their use with a different rule.
We observed that system congestion influences the occupied time for each resource type differently. The time to use private resources is only slightly affected, with minor changes, even under heavy congestion. In contrast, the time spent on shared resources is broadly affected, showing significant differences. Thus, we separately measure the delays for the two resource types and apply different charging rules for their use. 

% Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where we normalize \(T_{shared}\) per instruction and \(T_{private}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 181\% on average and 488\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions.
Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is calculated as the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where \(T_{shared}\) per instruction and \(T_{private}\) per instruction are normalized to the same tests when running alone. The figure shows that \(T_{shared}\) is significantly affected by system congestion compared to \(T_{private}\). On average, \(T_{shared}\) increases by 181\%, with a maximum increase of 488\%. Meanwhile, \(T_{private}\) increases by only 4\%, with minor variance between functions.

% This figure gives insights into two key factors. First, the congestion in the shared resources does not impact the performance of private resources. Accordingly, when the system gets congested, the degree of a function's dependence on the shared resources determines the function's performance. If the \(T_{shared}\) takes a minor portion of a function's execution, severe congestion still barely influences its overall execution. Second, hardware PMUs available in modern CPUs, and profiling tools such as Linux Perf are widely available and can be used to distinguish the usage of shared and private resources. Across the paper, we will take advantage of such tools to develop Litmus pricing.
This figure highlights two key factors. First, congestion in shared resources has a negligible impact on the performance of private resources. Accordingly, when the system gets congested, the extent of a function's reliance on shared resources determines its performance. If \(T_{shared}\) constitutes a minor portion of a function's execution, even severe congestion will have minimal impact on its overall execution. Second, hardware Performance Monitoring Units (PMUs) in modern CPUs and profiling tools like Linux Perf are widely available and can be utilized to differentiate between the use of shared and private resources. Throughout this paper, we will leverage these tools to develop Litmus pricing.

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/TpriTshardDistriRev}\\
% \caption{\(T_{private}\) and \(T_{shared}\) distribution when they run alone}
\caption{Execution time distribution of \(T_{private}\) and \(T_{shared}\)}
\vspace{-0.5em}
\label{fig:TpriTshardDistriRev}
\end{figure}

% Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) in a function's execution. The compute-intensive workloads (e.g., fib-py, float-py) have a substantial \(T_{private}\) portion that can reach 99.96\% of the execution time. However, the portion decreases when running memory-intensive workloads such as fib-nj. This distribution indicates how much other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase float-py's \(T_{shared}\), its total execution time, $T_{private}+T_{shared}$, will undergo minor change.
Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) during a function's execution. Compute-intensive workloads (e.g., fib-py, float-py) exhibit a substantial \(T_{private}\) portion, accounting for up to 99.96\% of the execution time. However, this portion decreases when running memory-intensive workloads such as fib-nj. This distribution reflects how other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase its \(T_{shared}\), the total execution time, $T_{private}+T_{shared}$, will undergo only a minor change.

% For each pricing component, we calculate the price by multiplying its charging rate with its time distribution. Thus we can further update the pricing equation.
After collecting the time slices spent on each resource, Litmus calculates each pricing component by multiplying two different charging rates with corresponding slices. Consequently, a new pricing equation emerges as follows:

\begin{equation} 
P = R_{private} * T_{private}  + R_{shared} * T_{shared}
\end{equation}

% \(T_{shared}\) is the cycles stalled due to L2 misses. It is measured from the perf counter, STALLS\_L2\_Misses. \(T_{private}\) is the total execution minus STALLS\_L2\_Misses. 
% Using Perf, Litmus collects\(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total cycles to complete the application minus \(T_{shared}\). 
% While Litmus returns the system's congestion state, the service provider still needs to determine reasonable prices charged for a service when having different congestion levels. 

% \(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. Again, the two charging rates are necessary since each component is affected differently, directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from the crowded execution environment. Thus, the charging rates should be measured as follows.
\(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. These two charging rates are necessary because each component is affected differently, either directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from a crowded execution environment. Thus, the charging rates should be measured as follows:

\begin{equation} 
R = R_{base} * \frac{T_{solo}}{T_{congestion}}
\end{equation}

% In this equation, \(R\) is the charging rate for executions on either private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free execution environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is the execution time when the function runs alone, and \(T_{congestion}\) is its execution time in the congested environment. Again, we should collect a separate \(T_{solo}\) and \(T_{congestion}\) for each pricing component. To measure \(T_{solo}\), \hl{the prior work}~\cite{alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. Litmus pricing avoids such a costly approach but presumes the function's \textit{solo} performance by examining reference workloads on the system.
In this equation, \(R\) represents the charging rate for executions on private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free runtime environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is its non-interfered execution time when the function runs alone, and \(T_{congestion}\) is its execution time in a congested environment. We need to collect separate \(T_{solo}\) and \(T_{congestion}\) values for each pricing component. To measure \(T_{solo}\), the prior study~\cite{tiwari2013enabling,alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. However, Litmus pricing avoids such a costly approach by presuming the function's solo performance through reference workloads on the system.

% Litmus pricing requires both providers and tenants to be involved in the price decision. The providers need to decide on reasonable rates for each resource use by analyzing the selected representative functions running on the system. To offer reasonable discounts, the providers must choose the functions analyzed carefully, collecting the functions representing the system. The tenants must also know the consequences when their tasks heavily rely on any of the shared resources. Unfortunately, their tasks may get delayed more than the provider's expectation while still receiving the discount rate up to the expectation. 
Litmus pricing requires both providers and tenants to be involved in the price decision process. Providers need to establish reasonable rates for each resource usage by analyzing selected representative functions. To offer fair discounts, providers must carefully choose the functions to be analyzed, ensuring the functions accurately represent the system condition. Tenants must also know the consequences when their tasks heavily rely on shared resources. Unfortunately, their tasks may get delayed more than the provider's expectations while still receiving the expected discount rate. 

% Here, the Litmus pricing reflects the varying value of the shared resources when the system's congestion level changes; the importance of shared resources becomes more valuable when congested. 



==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/06_design_details.tex <==
\section{Estimating prices with Litmus}
\label{sec:designDetails}

% The providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}, before using Litmus pricing. The numbers in both tables are the slowdowns of codes while testing the system congestion. Shortly, the congestion table is filled with the slowdowns of startup codes, and the performance table is filled with the slowdowns of reference benchmarks. Litmus pricing needs three steps to charge the final price with a discount. First, the providers assess the system's congestion at multiple levels and range them in a table. This step completes the congestion table. Second, the providers study the impact of congestion on tenants' functions and complete the performance table. Lastly, the service provider determines a tenant's price based on the two tables. 
Before using Litmus pricing, service providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}. The congestion table lists the slowdowns during the startup phases, whereas the performance table lists the slowdowns of reference functions. Litmus pricing needs three steps to determine the final price with a discount. First, providers assess system congestion at multiple levels and record the results in the congestion table. Second, providers analyze the impact of congestion on reference functions and fill out the performance table. Lastly, providers determine a tenant's price based on the data from both tables.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tables}\\
\caption{Congestion and performance tables: numbers in both tables indicate the slowdowns of startup codes and reference functions, collected with CT-Gen and MB-Gen}
\vspace{-0.7em}
\label{fig:litmust_tables}
\end{figure}

\textbf{Step 1, Defining Congestion Levels:} We manage the system's congestion levels using two traffic generators that create a range of congestion states by stressing shared resources differently. The traffic generator is multi-threaded, creating traffic in shared resources to incur congestion, with each thread running on a separate core. We rank the stress levels from 1 to 32 by changing the number of active threads running on distinct cores. Entries from top to bottom in the congestion table indicate increasing stress levels.

% \begin{figure}[h]
% \centering
% \vspace{-1.5em}
% \includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
% \vspace{-1em}
% \caption{stressing program's instruction, L3 accesses and L3 misses }
% \vspace{-0.5em}
% \label{fig:stressing_specs}
% \end{figure}

% \textbf{Step 2. Measuring System Congestion:} Measuring the current level of system congestion that may influence a function's performance is a crucial challenge. If we assume that the platform does not have pre-profiled information about a function's performance, the platform cannot figure out whether co-running functions influenced the function. Additionally, the serverless platform's fast-changing states with massive short-living functions make the assessment even more complicated, requiring quick and frequent examinations.

% Meanwhile, measuring the amount of a system's congestion and its impact on performance is a crucial challenge. This challenge particularly stands apparent when being demanded to quantify the impact of the congestion on a running application without pre-profiled information about the application. Moreover, the serverless platform's fast-changing system states with \hl{numerous} short-lived functions make the assessment even more complicated, requiring quick and frequent performance examinations.
Measuring the amount of system congestion and its impact on performance is a crucial challenge. This challenge becomes particularly pronounced when trying to quantify the impact of the congestion on a running application without pre-profiled information about the application. The fast-changing system states of a serverless platform, with numerous short-lived functions, further complicate the assessment, necessitating quick and frequent performance examinations.

% Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. The proposal is based on the observation that high-level languages, such as Python and Node.js, used in serverless computing have long startup times to accommodate their runtime environments. Since the inception of serverless computing, these startups have been recognized as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests leverage these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests further validated that all tested functions exhibited similar performance characteristics during their startups. 
Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. This method leverages our observation that high-level languages like Python and Node.js, commonly used in serverless computing, have lengthy startup phases to accommodate their runtime environments. Since the inception of serverless computing, these startup delays have been identified as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests exploit these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests have validated that tested functions exhibit similar performance characteristics during startup phases. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_all}\\
% \caption{IPC for serverless applications with different runtimes in the first 100 milliseconds of their execution}
% \vspace{-0.5em}
% \label{fig:startupIPC_all}
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped}\\
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-1}\\
\includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-3}\\
% \caption{IPC for serverless applications grouped by language runtime in the first 100 milliseconds of their execution}
\caption{IPC of serverless applications based on languages (Go, Python, and NodeJS) during their startup phase}
% \vspace{-0.7em}
\label{fig:startupIPC_grouped}
\end{figure}

% Figure~\ref{fig:startupIPC_grouped} depicts the fluctuation in IPC (Instructions Per Cycle) of a function during the first milliseconds of its execution. The x-axis shows a time flow since the beginning; every tick indicates a millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language, and the throughput of each group is represented in separate figures. Although figures exhibit different patterns, functions in the same figure display notable similarities. The figures imply that functions written in the same language have nearly identical startups.
Figure~\ref{fig:startupIPC_grouped} depicts a function's fluctuation in IPC (Instructions Per Cycle) during its startup phases. The x-axis represents the time elapsed since the beginning, with each tick indicating one millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language runtime, and the IPC of each group is presented in separate figures. As shown in these figures, functions in the same figure show notable similarities. This implies that functions written in the same language have nearly identical startups.

% The startup of a runtime usually includes bursts of memory reads to load images and libraries, which can probe the traffic in the shared resources. By conducting a Litmus test before executing every tenant's codes, the providers can observe the system state for the function. Meanwhile, the providers also need to study how the startup codes perform in different system states. They complete the congestion tables by performing the Litmus tests with the startups written in three languages while varying the congestion levels. To this end, the information in the congestion table is looked up when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}. 
% estimating the system's state upon receiving a result of a function's Litmus test. 
The startup of a runtime typically includes bursts of memory reads to load images and libraries, which can be used to probe the traffic in shared resources. By conducting a Litmus test before executing a tenant's function, providers can assess the system state. Meanwhile, providers also need to study how startup phases perform under different system states. They complete the congestion tables by conducting the Litmus tests with startups written in three languages while varying congestion levels. This information from the congestion table is then referenced when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tests}\\
\caption{Progress of serverless applications on four cores with Litmus tests (dotted arrows) over time}
% \vspace{-0.5em}
\label{fig:Litmus_tests}
\end{figure}

% Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests. The Litmus tests examine the level of system congestion with every function startup. \hl{Many} concurrent functions in serverless offer frequent test opportunities. Function\#1 is a memory-intensive function that raises a congestion level. While active, Litmus tests measure the congestion level above 8. After Function\#1's completion, the next Litmus test detects a non-congested system with a congestion level below 3. However, with the start of another heavy function, function\#2, the Litmus tests measure the new congestion in the system.
Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests, which examine the level of system congestion during each function's startup. Many concurrent functions in serverless offer frequent opportunities for testing. Function \#1, which is memory-intensive, causes congestion levels to rise above 8 during its execution. A Litmus test in Core 3 detects this congestion. After Function \#1 is complete, a subsequent Litmus test indicates a non-congested system with a congestion level below 3. However, during another resource-intensive function, Function \#2, the Litmus test identifies new system congestion with a level above 9.  

% \textbf{Step 2. Measuring the Impact of Congestion:} Although discerning the system congestion through the Litmus test, estimating its impact on a user's application is another challenge. This work proposes a discount based on the pre-studied impacts on reference functions, assuming the user's functions are alike. For this, the service providers need to select reference functions that represent users' functions running on their systems. In this work, we select the workloads in \hl{Section 2} as our reference applications. 
\textbf{Step 2, Measuring the Impact of Congestion:} Discerning system congestion through the Litmus test solves only one of the two challenges; the other is determining its impact on a tenant's function. Different tenants' functions could experience varying degrees of slowdown under the same congestion level. To address this, we propose using pre-selected reference functions to analyze these impacts, thereby avoiding the cost of runtime profiling. For this, providers need to carefully select reference functions that represent tenants' functions operating on the systems, as these selections influence the overall accuracy of congestion measurement. Later, in Section~\ref{sec:evaluation}, our tests will show that pre-selected reference functions can effectively represent unknown user applications. For this study, the selected reference applications (* marked) are listed in  Table~\ref{tb:benchmarks}. 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/refSlowdownStressing14}\\
% \includegraphics[width=1\columnwidth]{./fig/slowdownStressing16}\\
\caption{\(T_{private}\), \(T_{shared}\), and \(T_{total}\) of serverless applications that run with MB-Gen at stress level 14, normalized to their execution time when they run alone}
% \vspace{-0.5em}
\label{fig:refSlowdownStressing14}
\end{figure}

% Once the reference functions are ready, the providers study the slowdowns of the reference functions while varying different congestion levels again. This study completes the performance table in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. Again, our two traffic generators create two separate sub-tables. All entries in this table are 1-to-1 mapped to entries in the congestion table. The providers estimate a general function's slowdown when having a certain congestion level using this 1-to-1 mapping.
Once the reference functions are ready, providers analyze their slowdowns under varying congestion levels. This analysis completes the performance table shown in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. With two traffic generators, providers can complete another set of two sub-tables for the performance table. All entries in this table are mapped 1-to-1 to entries in the congestion table. Providers can estimate a general function's slowdown at a given congestion level using this one-to-one mapping.

% Figure~\ref{fig:refSlowdownStressing14} shows the reference functions' slowdowns when stressing the system. The X-axis shows different functions, each consisting of three bars: the first two bars show the CPI during each time slice, \(T_{private}\) and \(T_{shared}\), and the last bar shows the CPI of an entire execution. The figure shows that the tested functions suffer from different amounts of slowdowns, although the tests maintain consistent stress levels. \hl{The last group} shows the gmean of all the slowdowns, which is used when providers estimate a function's slowdown later. 
Figure~\ref{fig:refSlowdownStressing14} shows an example of the reference functions' slowdowns when stressing the system. The X-axis shows tested functions, each depicted with three bars: the first two bars show \(T_{private}\) and \(T_{shared}\), while the last bar shows the total execution time, all normalized to their execution time when running alone without interference. The figure shows that the tested functions experience varying degrees of slowdown despite consistent stress levels maintained during the tests. The next-to-last group shows the gmean of all the slowdowns, which providers use to estimate a function's slowdown later.

% \hl{This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/referenceStartupSlowdownRev}\\
\caption{The correlation between the slowdown of Python's startup phase and the slowdown of reference applications. From left, (a) \(T_{private}\), (b) \(T_{shared}\), and (c) \(T_{total}\), normalized to the execution time when running alone}
\label{fig:referenceStartupSlowdownRev}
\end{figure}

% \textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while a range of congestion levels is continuous, the tables only contain a few slowdowns in discrete intervals. Thus, providers need a model that returns an estimated slowdown when receiving a congestion level as an input. In our tests, we employ a linear regression to achieve the model.
\textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while congestion levels vary continuously, the tables only contain slowdowns at discrete intervals. Therefore, providers need a model that estimates the slowdown for any given congestion level. In our tests, we employ linear regression to develop the model.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/interpolation}\\
\caption{Estimating a function's slowdown with logarithmic interpolation}
\label{fig:interpolation}
\end{figure}

% Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding references' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). We employed two traffic generators to extrapolate a more precise congestion level, yielding two sub-tables in both the congestion and the performance tables. Consequently, the figure presents two linear regression models, each associated with a different traffic generator. 
Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding reference applications' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). To extrapolate a precise congestion level, we created two sub-tables within both the congestion and performance tables using two distinct traffic generators. As a result, the figure depicts two linear regression lines (red and blue dotted lines), each associated with a different traffic generator.

% The provider needs to estimate the function's slowdown to uncover its price. However, the above two regression models return two vastly different slowdowns. Then, the providers need to determine which model is close to the current environment. We think the two models reflect two extreme congestions that the traffic generators create, one before the L3 and one after the L3. CT-Gen creates massive traffic from the core to the L3 cache, which filters the traffic, preventing the operations from consuming the memory bandwidth. MB-Gen also creates huge traffic but consumes the memory bandwidth and replaces L3 blocks. Since each traffic generator creates an extreme case, the machine state could be intermediate with congestion in the range between the two congestions created by CT-Gen and MB-Gen. However, Litmus pricing cannot answer this question with only the startup's slowdown. 

% To address this question, we note that the system's L3 misses are a critical indicator closely related to a function's performance. Functions suffer more when the system experiences more L3 misses, which stresses the cache space and off-chip memory bandwidth. Accordingly, Litmus test collects the system's L3 miss count as a supplementary index, which tells more about the crowdedness of shared resources.

These regression models return two different slowdowns. To estimate a function's slowdown, providers must determine which model reflects the current environment more accurately. The traffic generators create two extreme congestion scenarios: one before the L3 cache and one after. CT-Gen generates substantial traffic from the core to the L3 cache that filters the traffic and prevents operations from consuming memory bandwidth. Conversely, MB-Gen also generates massive traffic but consumes memory bandwidth and repeatedly evicts L3 cache blocks. Because each traffic generator represents a distinct extreme case, the actual machine state could fall somewhere between the two congestion levels created by CT-Gen and MB-Gen. However, Litmus pricing requires more than just the startup slowdown to identify the machine's state in these models. Thus, we have enabled Litmus tests to gather the system's L3 miss count as a supplementary metric that offers deeper insights into the crowdedness of shared resources.


% \hl{Figure 1} shows how to use the L3 cache misses with the performance sub-tables. The two traffic generators make the upper and lower boundary of the L3 miss rates. When performing a Litmus test, if the test's L3 miss rate is XXX, close to the L3 misses with CT-Gen, we can conclude that the congestion occurs before the L3 cache and select the expected slowdown of XXX. On the contrary, we choose XXX, in case the L3 miss rate is XXX, close to the L3 misses with MB-Gen. If the test's L3 miss rate is in-between, we interpolate the two slowdowns based on the L3 misses, assuming congestion in both resources. 
% Finally, we determine the Rprivate and Rshared based on the expected slowdown from its performance table. Calculating Rprivate and Rshared takes the same steps. The final discount price is computed using the equation with the computed rates. 

% Figure~\ref{fig:interpolation} shows how we employ the L3 misses when estimating the slowdown. The two traffic generators make the upper and lower boundary of the L3 misses. If a Litmus test reports the L3 miss count is 10, close to the L3 misses with CT-Gen, \textcircled{1}Litmus pricing estimates the discount (=expected slowdown) of the function to be near 1\%. This indicates that the congestion happens before the L3, as what CT-Gen creates. On the contrary, in case the L3 misses are 1000, close to the L3 misses with MB-Gen, \textcircled{2}Litmus pricing estimates the function's discount rate close to 6\%. Meanwhile, if the Litmus test reports the L3 misses as 100, we interpolate the two extreme discounts, 1 and 6, based on the L3 misses, assuming current congestion to stand in between the two extreme congestions. The congestion model in the figure shows how we interpolate with logarithmic interpolation. In this figure, \textcircled{3}applying the logarithmic interpolation to the L3 miss count returns the half-point between CT-Gen's 1\% and MB-Gen's 6\%, which is 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 
Figure~\ref{fig:interpolation} shows our approach to using L3 misses to estimate slowdowns. We created two figures illustrating separate regression models. The left figure (a) is derived from the startup slowdowns and L3 misses with logarithmic regression, indicating L3 misses at specific congestion levels. The right figure (b) is derived from the performance table with linear regression, displaying discounts at specific congestion levels. Each figure depicts two regression lines associated with different traffic generators.

The two traffic generators set the upper and lower boundaries for L3 misses. For instance, if a Litmus test reports 10 L3 misses, close to what CT-Gen generates: \textcircled{1}This suggests congestion occurs before reaching the L3 cache, similar to CT-Gen's scenario. Thus, Litmus pricing estimates the function's discount to be around 1\%. Conversely, if the Litmus test reports 1000 L3 misses, close to MB-Gen's results: \textcircled{2}Litmus pricing estimates the function's discount rate to be approximately 6\%, indicating congestion similar to MB-Gen, where memory bandwidth is heavily consumed and L3 cache blocks are frequently evicted. When the Litmus test reports 100 L3 misses, an interpolation between these extremes is applied: \textcircled{3}Using logarithmic interpolation, Litmus pricing estimates the function's discount rate to be midway between CT-Gen's 1\% and MB-Gen's 6\%, resulting in approximately 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 



==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/08_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \textbf{Litmus price \& error:}
% We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, and the other consists of selected reference applications to obtain the linear regression models for Litmus pricing. The discount models plug into the Litmus pricing used in our tests. For this experiment, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown.
We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, while the other consists of chosen reference applications to derive linear regression models for Litmus pricing. The discount models plug into the Litmus pricing employed in the tests. In this study, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown. 

% % original version
% We maintain the congestion state consistent across all tests, co-running each function with 26 other functions. Using Perf~\cite{perfWiki}, we collect the three key stats: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup, which implies the congestion level in these tests, as well as the discount rates that every function receives. We execute every function 100 times and collect the average of the function's \(T_{private}\) and \(T_{shared}\). Finally, we compute each function's \(P_{private}\), \(P_{shared}\), and \(P\), the total price, by summing \(P_{private}\) and \(P_{shared}\).  

\subsection{One Function Per Core}

% revision version
% We maintain consistent congestion states across all tests by co-running each function with 26 other functions. Using Perf, we collect the three key statistics: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup. These metrics hint at the congestion level during the tests as well as the discount rates that a function receives. Each function is executed 30 times, and the average of its \(T_{private}\) and \(T_{shared}\) is collected. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).
We maintain consistent congestion levels across all tests by co-running each function with 26 other functions. As outlined in Section~\ref{sec:motivation}, whenever a function finishes, another is randomly launched to keep a total of 26 co-running functions. Using Perf~\cite{perfWiki}, we collect three key statistics: \(T_{private}\), \(T_{shared}\), and the machine's L3 misses during the first 45 million instructions of the Python startup. Through these metrics, Litmus pricing estimates the level of system congestion and the discount rates a function receives. Each function is executed 30 times, and we average its \(T_{private}\) and \(T_{shared}\) values. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice26Rev}\\
% \caption{The total price for functions computed via Litmus pricing and ideal prices when co-running with 26 other functions normalized to the commercial price that offers no discount}
\caption{Prices computed via Litmus pricing and ideal prices when co-running with 26 other functions, normalized to the commercial price that offers no discount}
\label{fig:normalizedPrice26Rev}
\end{figure}

% In Figure~\ref{fig:normalizedPrice26}, we can see a minimal difference in the discount rate between the Litmus price and the Ideal price. The average Litmus discount rate stands at 11.5\%, which is only marginally larger by 0.6\% than the average Ideal discount rate of 10.9\%. Also, we can see that the difference between the Litmus price and Ideal price are different among the applications. Certain applications exhibit higher Litmus prices compared to the Ideal price, while conversely, some applications demonstrate smaller Litmus prices. 
 %Figure~\ref{fig:priceErrorRunwith26} shows further details, analyzing the errors in each pricing component. 

% Figure~\ref{fig:normalizedPrice26Rev} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{10.66\%}, which is only marginally larger by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{10.28\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice26Rev} illustrates estimated prices derived from Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices to offset delays in a congested execution environment. The figure shows minimal disparities between the two prices, implying that Litmus pricing offers a reasonable discount. The average discount from Litmus pricing across all functions is 10.7\%, which is only marginally higher by 0.4\% compared to the average slowdown experienced by functions, which stands at 10.3\%, as depicted by the ideal price.

% However, the discount rates per slowdown differ among functions. For instance, float-py's ideal discount rate is \hl{0.05\%}, but it enjoys a \hl{4.31\%} discount with the Litmus pricing. Meanwhile, pager-py's performance drops by \hl{15.63\%} while receiving a \hl{13.87\%} discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more easily affected than the reference when congested. In contrast, float-py runs mostly with private resources, receiving a minor impact from the execution environment. Figure~\ref{fig:priceErrorRunwith26Rev} shows further details, analyzing the differences in each pricing component.
However, the discounts per slowdown differ among functions. For instance, float-py's ideal discount rate is 0.05\%, but it benefits from a 4.3\% discount with Litmus pricing. Conversely, pager-py encounters a 15.6\% performance decline while receiving only a 13.9\% discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more susceptible to congestion than the references. In contrast, float-py predominantly utilizes private resources, resulting in minimal impact from the execution environment. Further insights into these variations in each pricing component are presented in Figure~\ref{fig:priceErrorRunwith26Rev}.


% From figure~\ref{fig:tcore\(T_{private}\)Distr}, we know that \(T_{private}\) dominates the execution time among all applications. The impact from \(T_{private}\) error has a bigger impact on the overall error. The slowdowns due to congestion in private resources are small. Theoretically, there should be no slowdowns when using private resources, but we observed that the congestion still influences it. The observed slowdown is 000, a small difference from an ideal slowdown. Meanwhile, the slowdowns in shared resources are significant. We observe that 

% % \[  Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}}\]

% \[Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{TotalIdealPrice}\]
% \[TotalIdealPrice = R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}\]

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/priceErrorRunwith26Rev}\\
\caption{Weighted errors in prices derived from Litmus pricing, which are compared to ideal prices}
% \vspace{-1em}
\label{fig:priceErrorRunwith26Rev}
\end{figure}

%%% We discuss error
% In figure~\ref{fig:priceErrorRunwith26} we can see that there are some applications receive positive errors and some receive negative errors.  A negative error indicates that our estimated slowdown for that application is higher than its actual slowdown, resulting in greater compensation than the observed performance losses. On the other hand, a positive error indicates that the compensation is smaller than its real slowdown. For most applications, the Litmus price is slightly higher than the Ideal price, with minimal differences. The highest price error is 0.0389 for auth-nj, while the lowest error is 0.007 for dyn-py. The geometric mean of the absolute error is 0.018. 
% Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors that each function experiences. The error rate is computed as the difference between the estimated and the ideal prices over the ideal price. The first two bars show the errors in \(P_{private}\) and \(P_{shared}\), which are weighted by their corresponding ratio in the execution time, considering their impacts, as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. The functions can have two different errors: positive and negative. A positive error indicates that the Litmus-estimated price is higher than its ideal price, implying that it receives smaller compensation than its performance losses. In other words, Litmus pricing estimates its slowdown to be less than its actual slowdown. A negative error implies the opposite; a function's compensation is higher than its slowdown. This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others. Meanwhile, the tenants need to acknowledge the consequences if their functions differ vastly from the reference workloads, heavily relying on shared memory.
Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors each function experiences. The error rate is computed by comparing the estimated prices with the ideal prices and dividing the difference by the ideal prices. The first two bars show errors in \(P_{private}\) and \(P_{shared}\), weighted by their corresponding ratios in execution time, reflecting their impacts as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. Functions may have two types of errors: positive and negative. A positive error means that the estimated price exceeds its ideal price, implying that the compensation received is less than the performance loss incurred. In other words, Litmus pricing underestimates the slowdown relative to the actual slowdown. Conversely, a negative error indicates the opposite; a function's compensation exceeds its slowdown. This discrepancy indicates Litmus pricing may offer varying advantages to different functions, favoring those with lesser slowdowns. Meanwhile, tenants must recognize the consequences if their functions differ vastly from the references, particularly those heavily reliant on shared resources.

% Delete the followings
% This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.

% The largest absolute error is \hl{0.0723} for rate-go, while the smallest absolute error is \hl{0.0039} for \hl{mst-py}. Overall, the Litmus pricing shows minor errors with an average of \hl{0.0231}. With further details, the Litmus pricing accurately estimates the slowdowns in \(P_{private}\) with \hl{0.0175} of an average weighted error rate. \(P_{private}\)'s highest weighted error rate is \hl{0.079}, yet minor, while the lowest rate is only \hl{0.0008}. The weighted error rate for the estimated \(P_{shared}\) is also small. The average error rate for \(P_{shared}\) is \hl{0.0068}, even lower than for \(P_{private}\). \(P_{shared}\)'s highest error rate is \hl{0.0404}.
% The largest absolute error is 0.072, which occurs with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, the Litmus pricing exhibits minor errors, averaging 0.023, \hl{with the estimated discount differing by 22.5\% over the ideal discount.} With more details, Litmus pricing accurately estimates slowdowns in \(P_{private}\), with an average weighted error rate of 0.018. \(P_{private}\)'s highest weighted error rate is 0.08, yet minor, while the lowest rate is only 0.0008. The weighted error rate for estimated \(P_{shared}\) is similarly small, averaging at 0.0068, even lower than for \(P_{private}\). The highest error rate for \(P_{shared}\) stands at 0.04.
The largest absolute error is 0.072, occurring with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, Litmus pricing exhibits minor errors, averaging 0.023. Thus, the estimated discount deviates by 22.5\% from the ideal discount. Note that Litmus pricing aims to match the average discount across all functions by applying a system-wide discount based on the system's congestion level rather than adjusting the discount for each function individually. Consequently, individual functions may experience either positive or negative errors. However, it is noteworthy that the average discount between Litmus and ideal pricing differs by just 0.4\%, as illustrated in Figure~\ref{fig:normalizedPrice26Rev}, satisfying its objectives.
% This policy may incentivize some functions while penalizing others based on shared resource usage. 
Specifically, Litmus pricing estimates slowdowns in \(P_{private}\) with an average weighted error rate of 0.018. The highest for \(P_{private}\) is 0.079, while the lowest is just 0.001. For \(P_{shared}\), the average weighted error rate is even lower, at 0.007. The highest for \(P_{shared}\) is 0.040.


% Litmus employs the average performance of applications to determine the discount rate applied universally. In this context, an application encounters a positive error when its speedup is less than the estimated average speedup across all applications. Also, the error rate depends on the difference between the actual speedup and the estimated average speedup, with larger differences resulting in more significant errors for the given application.
% As discussed in Figure~\ref{fig:TpriTshardDistri}, \(T_{private}\) dominates the execution time across all applications, implying that a small error in the estimated \(T_{private}\) largely influences the execution time. This explains why, for functions that demand little shared resources, such as float-py and chame-py, the error in P is almost identical to that in \(T_{private}\), and errors with \(T_{shared}\) can be overlooked. In contrast, for functions with a larger \(T_{shared}\) ratio, such as pager-py and mst-py, errors in \(T_{shared}\) meaningfully affect the total execution time. Note that the Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price.  

Litmus pricing estimates each pricing component separately with an individual discount rate. For functions that demand minimal shared resources, such as float-py, the errors in P are nearly identical to those in \(T_{private}\), and the errors in \(T_{shared}\) can be overlooked. As shown in Figure~\ref{fig:TpriTshardDistriRev}, \(T_{private}\) dominates the execution time across many applications. While even a small error in the estimated \(T_{private}\) influences the function's execution time, substantial errors in \(T_{shared}\) likely have limited impacts, except for functions that have a relatively meaningful \(T_{shared}\) ratio, such as pager-py and mst-py, whose errors in \(T_{shared}\) are observable in the total price. 

% We emphasize that Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price. We observe that functions have similar slowdowns in \(T_{private}\) with slight variation when congested. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, also estimating reliable total prices since \(T_{private}\) mostly dominates the execution time. The \(T_{shared}\) fluctuates more dynamically across functions with a relatively large error, but the error's impact is little, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}. 
We emphasize that Litmus pricing cannot avoid producing a certain degree of error since it relies on estimation using a few metrics. However, the figure proves that Litmus pricing effectively captures a congested environment and reflects that environment in the price. Under the same congestion level, \(T_{private}\) values of all functions are delayed similarly with a little variation. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, leading to reliable total price estimates since \(T_{private}\) generally dominates execution time. \(T_{shared}\) fluctuates more dynamically across functions and has a relatively larger error, but the impact of this error is minimal, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}.

\begin{figure}[h]
\centering
% \vspace{-5em}
 \includegraphics[width=1\columnwidth]{./fig/normTprivtTshared26Rev}\\
% \vspace{-5.5em}
\caption{\(T_{private}\) \& \(T_{shared}\) of applications when co-running with 26 others, normalized to those when they run alone. The top(black) and bottom(blue) lines are discount rates from Litmus pricing for \(T_{private}\) and \(T_{shared}\)}
% \vspace{-1em}
\label{fig:normTprivtTshared26Rev}
\end{figure}

% To further investigate the price error differences, in igure~\ref{fig:normTprivtTshared}, we explore the \(T_{private}\) speedups across various serverless applications.  
% Notably, the difference between the Litmus discount (L-Discount) and the average speedup is merely 0.006.  This minute difference explains why Litmus can attains such high accuracy. 
%Furthermore, when comparing with figure~\ref{fig:priceErrorRunwith26}, a correlation between the error rate and the speedup differences becomes apparent. 
%For instance, float-py, with the most substantial difference above the Litmus discount, also experiences the most significant negative error rate. 
%Conversely, aes-go, with the smallest speedup, experiences the highest positive error rate.
% % original version
% Figure~\ref{fig:normTprivtTshared} shows the execution time of the baseline normalized to the execution time of each run under congestion. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the functions spend only 3.67\% more time on private resources, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, resulting in precise estimation with a Litmus test. 

% Figure~\ref{fig:normTprivtTshared26Rev} shows the execution time of each function run under congestion normalized to the execution time of the baseline. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the interferences in private resources extend the function execution time only by 5.3\%, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, enabling precise estimation with a Litmus test.
Figure~\ref{fig:normTprivtTshared26Rev} shows the \(T_{private}\) and \(T_{shared}\) of each function, normalized to the same time components of the baseline. The gap between the bar and 1 represents the amount of slowdown that should be translated into ideal discounts. The top (black) and bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that interferences in private resources extend the function execution time by only 5.3\%, implying the performance of the private resources is marginally affected by congestion. Additionally, all functions exhibit similar \(T_{private}\) values with little dispersion, helping precise estimation with Litmus tests.

% Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors are still in an acceptable range since their impacts are small. Functions that have a considerable \(T_{shared}\) ratio become more sensitive to system congestion. Instead, a function, such as float-py, with negligible \(T_{shared}\) ratio gains huge benefits with high discounts while its performance remains firm. This shows that Litmus pricing reflects the dynamically changing values of shared resources when the congestion level alters and encourages functions to be developed to use more private resources. 
Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors remain within an acceptable range as their impacts are minor. Functions that have a considerable \(T_{shared}\) ratio are more sensitive to system congestion. Conversely, a function like float-py, which has a negligible \(T_{shared}\) ratio, gains huge benefits from high discounts while maintaining stable performance under congestion. This shows that Litmus pricing accurately reflects the dynamic values of shared resources when the congestion level changes and incentivizes functions to be developed to use less shared resources. 

% \textbf{Litmus pricing under high congestion:} We test our Litmus pricing under a heavily congested environment to verify its pricing of functions with large slowdowns. To create a crowded environment, we concurrently execute 60 instances of Fibonacci-go, which produces the most L2 misses among our tested functions. 
% We raise the congestion level significantly with 60 co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo} shows the results from the same tests of Figure 11. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.8\%, which is only a 1.7\% difference from the ideal discount of 27.1\% with 2.48\% of an average absolute error. In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.151 and 4.299, which are only 2.45\% and 7.83\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. 
% \textbf{Litmus pricing under high congestion:} We raise the congestion level significantly with \hl{500} co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo500} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.1\%, which is only a 1\% difference from the ideal discount of 27.1\% with 0.088\% of an average absolute error. Litmus pricing discounts slightly more than an actual slowdown, leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% % \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
% \caption{The normalized total price for the applications calculated by using Litmus pricing and ideal prices when co-running with 500 Fibonacci-go}
% \label{fig:normalizedPriceCongested320}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\columnwidth]{./fig/diffStartupPortion-2Rev}\\
%\caption{The slowdown of Python's startup with 25 and 15 million instructions (X-axis) and the slowdown of reference applications (Y-axis). From left, \(T_{private}\), \(T_{shared}\), and \(T_{total}\), normalized to those when running alone}
%\label{fig:diffStartupPortion}
%\end{figure}

% \textbf{Instructions in Startup:} Litmus tests react differently to congestion when performed with different numbers of instructions from the startup phase. For example, Python's startup involves about 45 million instructions. While we have conducted Litmus tests using all these instructions, Figure~\ref{fig:diffStartupPortion} shows the response of these tests when running with the first 15 and 25 million instructions from this set. The figure shows the startups' \(T_{private}\), \(T_{shared}\), and \(T_{total}\) with two traffic generators, as depicted in Figure~\ref{fig:referenceStartupSlowdownRev}. Tests with fewer instructions are more sensitive to cold cache misses but less to interference in the L3 cache. Therefore, as the instruction count in Litmus tests decreases, they become less susceptible to conflicts in shared resources, especially from traffic by MB-Gen. As a result, tests with 25 million instructions exhibit reduced slowdowns. This trend becomes more apparent when running the tests with 15 million instructions, depicting that slowdowns when co-running with MB-Gen become nearly identical to those with CT-Gen. 

%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%







% \textbf{Instructions in Startup:} Python's whole startup phase contains about 45 million instructions. We can further divide the startup phase into smaller pieces with 10 million instructions code chunks. And each code chunk would have its characteristics. They react differently in the same congested environment. In section XXX we use the whole Python's startup portion's slowdown to indexsing the serverless application's slowdown. But, since the co-relationship between these two slowdown in different congestion source are different, one startup \(T_{private}\) slowdown may indicate two application's slowdown. By carefully picking the code chunks we can mitigate the difference between the two normalized slowdowns of the guidance application that correlated to the same startup phase slowdown. 

% Figure~\ref{fig:diffStartupPortion} depicts the correlation between the performance changes in the reference applications and distinct segments of Python's startup phase. From the figure, we see that selecting the first 15 million instructions as our startup phase results in the normalized \(T_{uncore}PerInst\) of the guidance application aligning nearly into a singular trendline. However, there are substantial gaps in the case of \(T_{core}PerInst\) with this code segment. Thus, we should pick xxx-xxx as our startup phase representation code for the normalized \(T_{core}PerInst\). We think that this can be used to mitigate the differences. But, we should be careful to use the small code chunks for the following reasons: First, only measuring the small portion can be a problem. The results might be too dynamic. Second, since we only measure this small portion there might be a huge execution period that cannot be covered.

% Continue to work from here

\subsection{Temporal CPU Sharing}
\label{sec:temporalCPUSharing}

The previous evaluation assumes an isolated environment where a CPU is assigned exclusively to an active function during execution, disallowing temporal sharing between functions through context-switching. While this setup ensures strict performance isolation, it inherently limits resource utilization. Conversely, enhancing utilization by permitting temporal CPU sharing among functions complicates price estimation. We explore how Litmus pricing can be applied in a less restrictive environment that permits sharing, where functions can temporarily share the same CPU and are not bound exclusively to specific cores. 

In this section, we deploy a testing function to co-run with 160 other functions across 16 cores without exclusive core assignments, assuming an average of 10 functions share a core. The reduction in the number of cores tested was necessitated by our system's memory limitations, as certain functions require significant memory space.

% \textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, the subsequent function clears the displaced one's cached data. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, the slowdown with extra sharing financially benefits the provider; we thereby argue that the extent of sharing should be factored into Litmus pricing as another discount factor.
\textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, a subsequent function evicts the cached data of the displaced one. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, delayed execution due to extra sharing financially benefits the providers. Thus, we argue that the extent of temporal sharing should be incorporated into Litmus pricing as another discount factor.

Figure~\ref{fig:csImpactor} depicts the switching overheads as concurrently running functions increase. The figure demonstrates that the sharing overhead follows a logarithmic growth pattern and stabilizes at around 20 co-running functions. Furthermore, we discovered that the switching overheads predominantly affect \(T_{private}\). Consequently, Litmus pricing needs to calibrate \(T_{private}\) to account for the impacts of sharing before estimating the slowdown using the performance table.

Figure~\ref{fig:normalizedPrice160Method1} illustrates the discounted price reflecting this adjustment. In our configuration, with an average of 10 functions per core, we divide \(T_{private}\) by 1.025 before estimating the slowdown. In this figure, Litmus pricing estimates an average discount of 14.5\%, which falls 2.9\% short of the ideal discount of 17.4\%. While most benchmarks receive discounts lower than ideal, aes-py stands out with the largest error of 9.9\%, which is 6.9\% less than its ideal discount of 16.8\%.

\begin{figure}
\centering
% \includegraphics[width=1\columnwidth]{./fig/csImpactor}\\
\includegraphics[width=1\columnwidth]{./fig/csImpactor2}\\
\caption{\(T_{private}\) of functions over different co-running counts in the same core, normalized to when running alone}
% \vspace{-1em}
\label{fig:csImpactor}
\end{figure}

\begin{figure}
\centering
% \vspace{-1.2em}
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160Method1}\\
\caption{Prices derived from Litmus pricing (Method 1) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
% \vspace{-0.5em}
\label{fig:normalizedPrice160Method1}
\end{figure}

% In Figure~\ref{fig:normalizedPrice160Method1} we use the the same congestion and performance tables that we collected in the restricted environment. When checking the tables instead of using the original startup slowdown of tcore we use an adjusted slowdown by dividing the context switch impact factor. From figure~\ref{fig:normalizedPrice160Method1} we can see that the average Litums discount is 14.65\%, 3.01\% less than what they should receive compared to the ideal discount of 17.67\%. Most applications receive a smaller discount than the ideal price. The largest error is on aes-py with Litmus discount of 9.85\%, 6.87\% smaller than the ideal discount of 16.72\%. The smallest error is on dyn-py. It's Litmus discount is 22.45\%, only 0.47\% larger than the ideal discount of 21.97\%.

\textbf{Method 2, Updating Performance Tables:} Rather than reusing the performance/congestion tables designed for restrictive environments, arranging new tables for the sharing-enabled environments returns better accuracy. Although the notion of preparing separate tables for various sharing levels may seem challenging, we argue that only one or a few extra tables for heavily crowded systems would suffice, given that commercial systems are typically heavily crowded. Again, we emphasize that the impact of function co-placement stabilizes above a certain co-placement count, as shown in Figure~\ref{fig:csImpactor}.

For this test, we prepared new performance/congestion tables for the environment described above, where a testing function is assumed to co-locate and compete for a core with 9 other functions. Moreover, considering the scenario where a switched-out function has a low chance of being rescheduled to the same core, instead of assigning 10 functions to a specific core, we ran 50 functions across 5 dedicated cores; each can run on any of the 5 cores. We managed the congestion levels in shared resources using traffic generators on the other cores, as outlined in Section~\ref{sec:designDetails}.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPrice160}
% \vspace{-0.6em}
\end{figure}

% Figure~\ref{fig:normalizedPrice160} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{17.29\%}, which is only marginally smaller by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{17.67\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice160} shows the prices obtained from Litmus pricing with the new tables, which are normalized to those from commercial sources. Once more, as in Figure~\ref{fig:normalizedPrice26Rev}, the figure reveals marginal distinctions between the two price points, suggesting that Litmus pricing continues to offer a reasonable discount. Across all functions, the average discount provided by Litmus pricing stands at 17.2\%, merely 0.2\% less than the ideal discount of 17.4\%.


==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/09_sensitivity.tex <==
\section{Sensitivity}
\label{sec:sensitivity}

While the aforementioned tests highlight Litmus's potential, we recognize the need for more compelling results. This section expands our analysis and examines Litmus pricing from various angles across diverse system environments.

% \textbf{Heavy Congestions:} We raise the congestion level significantly with 320 co-running applications to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. The Litmus pricing is still close to the ideal price, discounting the price by 20.00\%, which is only a 1.46\% difference from the ideal discount of 21.46\%. The highest Litmus discount is 26.01\% for dyn-py. It has an error of 2.83\% compared with the ideal discount.
\textbf{Heavy Congestion:} We significantly escalate the congestion level to verify Litmus pricing under conditions of substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} presents the outcomes of the same tests depicted in Figure~\ref{fig:normalizedPrice160} but with 320 co-running functions. Not only did we increase the function count, but we also specifically selected 8 memory-intensive functions, aes-py, compre-py, thum-py, bfs-py, auth-py, fib-go, geo-go, and profile-go, that produce the most L2 cache misses among the tested functions to create heavy congestion in shared resources deliberately. Even under such intensified congestion, Litmus pricing produces results remarkably close to the ideal price, discounting the price by 20.0\%, which deviates by merely 1.5\% from the ideal discount of 21.5\%. The highest discount by Litmus pricing is 26.0\% for dyn-py, a minor error of 2.8\% compared to the ideal discount.


% leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 320 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPriceCongested320}
% \vspace{-1em}
\end{figure}

\textbf{CPU Frequency:} Modern CPUs feature dynamic CPU frequency adjustments, which are controlled via software or hardware. A hardware technique like Intel Turbo Technology autonomously adjusts the CPU frequency based on the CPU's power and thermal budgets, allowing the CPU to operate at higher frequencies when conditions permit and lower frequencies under heavy load. Prior tests assumed that the frequencies were fixed and strictly managed by service providers who had knowledge of when and to what extent frequency adjustments were necessary. Also, we evaluated Litmus pricing under the other scenarios where CPU frequencies were not fixed, providing more dynamic perspectives.

% Figure~\ref{fig:normalizedPrice160unset} illustrates the prices from the Litmus pricing and the ideal price, which are normalized to commercial prices. We tested it under the configuration in Section 7.2 with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, the Litmus pricing's discount is lowered from 17.16\% to 16.84\%, while the ideal discount rate is decreased from 17.42\% to 17.31\%. Still, the discount rate difference from the ideal price is only 0.47\% without setting the CPU frequency. We observed that the CPU frequency changes rarely when the system runs with 160 functions. Overall, the varying frequency made a minor impact on performance as well as the pricing scheme. 
Figure~\ref{fig:normalizedPrice160unset} illustrates the prices derived from Litmus pricing alongside the ideal prices, both normalized to commercial prices. This evaluation was conducted under the configuration outlined in Section~\ref{sec:temporalCPUSharing} with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, we observe a slight decrease in Litmus pricing's discount, from 17.2\% to 16.8\%, while the ideal discount rate decreases from 17.4\% to 17.3\%. Still, even without fixed CPU frequencies, the difference in the discount rate from the ideal price is only 0.5\%. We noted that CPU frequency changes were infrequent when the system operated with 160 functions. Overall, the variation in frequency had a negligible impact on Litmus pricing.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160unset}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others with unfixed CPU frequencies, both normalized to commercial prices}
\label{fig:normalizedPrice160unset}
% \vspace{-1em}
\end{figure}

% All the above experiments are done on Intel Xeon Gold 5218(Cascade Lake). We also perform our scheme on another CPU architecture, Intel Xeon Silver 4314(Ice Lake-SP). 
\textbf{CPU Architecture:} Ensuring the validity of Litmus pricing across different architectures is crucial. Our Litmus tests rely on the performance counter that measures a stall count due to L2 cache misses (cycle\_activity.stalls\_L2\_miss)~\cite{perfMonEvents}, supported by Intel's CPUs. Unfortunately, other vendors like AMD do not yet offer the same performance counter~\cite{amdPMC}, restricting our tests to Intel CPUs. Alternatively, we conducted tests on another Intel CPU based on the Ice Lake architecture, Xeon Silver 4314, to broaden the scope of our analysis.

\begin{figure}[b]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun70kiwi}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 70 others on Xeon Silver 4314, both normalized to commercial prices}
\label{fig:normalizedPriceCorun70kiwi}
\end{figure}

% Because of the limitation of our memory size, we test Limtmus with 70 co-running applications. In this test, we use method 2 introduced in section~\ref{sec:temporalCPUSharing}. We first conduct the congestion and performance tables with 50 applications running in the first 5 cores. Then for the evaluation, we run 70 applications in the first 7 cores to let our testing application compete with 9 other applications for a core.  Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus discounting the tenant only pays 82.52\% commercial price. It's 0.696\% less than with the ideal discount.
Once again, this evaluation was conducted following the configuration outlined in Section~\ref{sec:temporalCPUSharing}, albeit with 70 co-running functions, limited by the main memory capacity of 128GB. Following Method 2, we constructed new congestion and performance tables with 50 functions running across 5 cores. Then, we ran 70 functions across 7 cores to match the competition count, averaging 10 functions per core. Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus pricing, the tenant only pays 82.5\% of the commercial prices, which is merely 0.7\% less than the ideal price.

% \textbf{Per-core Function Count:} When altering the co-located applications in each core the performance of the application can also be influenced. In this test, we put 240 applications in the first 16 cores. The testing application is competing with 14 other applications. We used the same congestion and performance tables from section~\ref{sec:temporalCPUSharing} method 2. Figure~\ref{fig:normalizedPriceCorun15} presents the results. The error of Litmus pricing is 1.23\% with The average discount of 16.69\%. The ideal discount is 17.92\%. The mean price of Litmus is larger than the ideal price because we are using the tables that are made based on 10 applications per-core. The context-switching overhead is larger. But, from figure~\ref{fig:csImpactor} we know that there is a diminishing impact of per-core application count. The error of the Litmus pricing is still under control when we increase the per-core application count.
\textbf{CPU Sharing Overhead:} The co-located function count determines the level of interference, impacting a function's performance differently. To assess Litmus pricing under various co-running function counts, we increased the function count to 240 from the configuration outlined in Section~\ref{sec:temporalCPUSharing}, making an average of 15 functions running on each core. However, we reused the performance and congestion tables generated in Section~\ref{sec:temporalCPUSharing}. Figure~\ref{fig:normalizedPriceCorun15} illustrates the results, where the Litmus pricing's error is 1.2\% with an average discount of 16.7\%, compared to the ideal of 17.9\%. Despite reusing the tables constructed for 10 co-running functions per core, the error remains negligible. This outcome aligns with Figure~\ref{fig:csImpactor}, which highlights the diminishing impact of temporal sharing when running more than 10 co-running functions. Given the perpetual overcrowding of commercial systems, any configuration gap between the environment where constructing the tables and where conducting tests is expected to remain minor and easily manageable.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun15}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 15 functions per core and reusing tables, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun15}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun160smt}
\end{figure}

\textbf{Simultaneous Multithreading (SMT):} SMT is a technique aimed at maximizing resource utilization by enabling multiple threads to execute concurrently on the same core, extending the shared resource domain across the entire processor. However, while SMT enhances resource utilization, it significantly complicates the measurement of interference impact. Moreover, SMT introduces additional side channels, thereby increasing the processor's vulnerability to security attacks. Due to these concerns, serverless platforms like Amazon Lambda disable SMT in their systems~\cite{schall2023warming,agache2020firecracker,schall2022lukewarm}. Nonetheless, we have conducted a study to assess the impact of SMT on our Litmus pricing methodology.

% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
% \caption{Prices computed via Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, normalized to the commercial prices}
% \vspace{-0.5em}
% \label{fig:normalizedPriceCorun160smt}
% \end{figure}

% To generate the performance/congestion tables, we executed 50 applications across 5 dedicated physical cores. In this way, the testing function is co-located with 9 other applications in the same virtual core and 19 other applications in the same physical core. Fiugre~\ref{fig:normalizedPriceCorun160smt} illustrates the results. The first thing we notice is that the normalized price is much smaller compared with the setups without SMT turned on. The average discount of Litmus is 45.42\% which is 1.9\% smaller than the average ideal discount of 47.32\%.
To construct the performance and congestion tables, we executed 50 applications across 5 physically separated cores, allowing an average of 10 functions to share two virtual cores. Figure~\ref{fig:normalizedPriceCorun160smt} illustrates the results,  presenting prices derived from Litmus pricing and ideal prices, both normalized to commercial prices without discounts. The normalized price experiences a significant drop compared to other configurations, highlighting the impact of heavy congestion within a physical core. The ideal price, which assumes no interference, stands at 47.3\% of the commercial price. Meanwhile, Litmus pricing offers a discount of 45.4\%, which is only 1.9\% less, confirming the effectiveness of Litmus pricing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Node JS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Nodejs Startup:}NodeJs is another well-adopted language in serverless platforms besides Python. It's one of the earliest languages to be supported by AWS Lambda ~\cite{serverless1}. From Section~\ref{sec:designDetails} we see that NodeJs has a long startup phase which makes it a great candidate when we need to pick a language startup phase for the Litmus test. 

%\begin{figure}[h]
%\centering
%\vspace{-0.5em}
%\includegraphics[width=1\columnwidth]{./fig/njReferenceStartupSlowdown}\\
%\vspace{-1em}
%\caption{The correlation between the normalized NodeJs's startup phase and the normalized reference applications.}
%\vspace{-0.5em}
%\label{fig:njReferenceStartupSlowdown}
%\end{figure}

%Figure~\ref{fig:njReferenceStartupSlowdown} shows the correlation between NodeJs startup phases and reference applications. After applying the Litmus test with NodeJs applications, with this figure, we can use the slowdown of the NodeJs startup phase to find the corresponding system congestion level and the discount rate for both private and shared resources. NodeJs has a longer startup phase compared with Python. It gives us more room when picking the most suitable portions of the startup phase. We can choose the language to be used for the Litmus test based on the density of the startup phase. 


==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/10_related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Serverless:} Many works address the performance bottleneck of serverless execution~\cite{du2020catalyzer}~\cite{agarwal2021reinforcement}~\cite{roy2022icebreaker}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Schall et al.~\cite{schall2022lukewarm} record and reload the instructions to reduce the front-end stalls when reaccessing the same application. Jovan et al.~\cite{stojkovic2023specfaas} focus on the performance of an application chain. They break the execution flow and speculative execute the functions. However, we are focusing on the price which is one of the most important potions of the cloud ecosystem.

% For the cloud providers, accommodating more tenants in a machine is a key strategy, gaining higher profits by maximizing the utilization of their machines. However, the approach inevitably introduces interference between tenants, slowing down applications unpredictably. Thus, prior researchers solved this challenge by allowing the tenants more non-biased, predictable, quality services~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed a clustering-based cache partitioning to remove unfairness between tenants. Rohan et al.~\cite{roy2021satori} simultaneously control multiple architectural resources to aim for both fairness and throughput. However, offering fairness inevitably sacrifices resource utilization. Thus, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} solve the unfairness uniquely by adjusting their prices while leaving the unfairness at a certain degree. This paper follows this direction but explores a more practical solution in serverless computing. 

Cloud providers strive to maximize profits by accommodating more tenants on their machines, which inevitably introduces interference between tenants, leading to unpredictable application slowdowns. To address this challenge, prior researchers have focused on providing tenants with a more unbiased and predictable quality of service~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed clustering-based cache partitioning to mitigate unfairness between tenants. Rohan et al.~\cite{roy2021satori} aimed for both fairness and throughput by simultaneously controlling multiple architectural resources. However, achieving fairness comes at the cost of sacrificing resource utilization. In contrast, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} addressed the unfairness by adjusting their prices while accepting a certain degree of unfairness. Our study follows a similar direction but explores a more practical solution within the context of serverless computing.

% delete the following section: the approaches are against our scheme. 
% \textbf{Serverless Computing:} Many studies focus on reducing the latencies of serverless applications~\cite{cadden2020seuss,oakes2018sock,wang2019replayable,jia2021boki}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Ustiugov et al.~\cite{ustiugov2021benchmarking} record and prefetches the functions’ stable working set of guest memory pages to further reduce the function's startup time. Wei et al.~\cite{wei2023no} remote forking the serverless functions to reduce the cold start latency while limiting the resource usage. Schall et al. record and reload the instructions~\cite{schall2022lukewarm} or the BTB entries ~\cite{schall2023warming} to reduce the front-end stalls when reaccessing the same application. 
% \hl{Litmus is orthogonal to these approaches and can be adopted together.}

==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Serverless computing is a key technology in present cloud computing, offering numerous advantages. One primary advantage is its effective cost-saving, as tenants only pay for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion. While tenants suffer slowdowns, they also have to pay more for the slowdowns. Unlike prior approaches that aim to maintain quality of service, this paper discounts the tenant's cost to compensate for the loss. Litmus pricing proposed in this work monitors the machine states and adjusts the tenants' costs. The congestion level can be frequently gauged before every function using the proposed Litmus test, an effectively lightweight testing approach. Our tests show that Litmus offers near-ideal prices with a 0.38\% difference, compared to the ideal price that discounts proportional to its slowdown. 
Serverless computing is a key technology in contemporary cloud computing, offering a range of benefits. One primary advantage is effective cost-saving, as tenants are billed only for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion, which not only results in slowdowns but also higher costs for tenants. Rather than aiming to maintain service quality, this paper suggests discounting tenants' costs to compensate for performance losses. Litmus pricing proposed in this work monitors machine states through Litmus tests and adjusts tenant costs accordingly. The Litmus test is a lightweight testing approach for serverless platforms, which assesses the machine's congestion level before starting a user's function. Our tests prove that Litmus pricing offers nearly ideal prices in heavily congested environments, with an average deviation of just 0.2\% from the ideal price that adjusts discounts in proportion to the slowdown experienced.


==> 2024_ASPLOS_-_Litmus__Fair_Pricing_for_Serverless_Computing/12_ack.tex <==
\section{Acknowledgment}
\label{ack}

We would like to thank our reviewers for their valuable feedback to improve this paper. This work was supported by NSF CAREER Award CCF-2146475.


==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/00_abstract.tex <==
\begin{abstract}

% Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While the providers can utilize their machines more efficiently, the tenants only need to pay for the resources they consume. However, a serverless system co-runs thousands of short-living functions concurrently to maximize resource utilization, bearing frequent state shifts. Meanwhile, when the system gets too congested, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants are also charged higher costs when experiencing slowdowns since all commercial serverless platforms determine the tenants' costs proportional to their execution times.
Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times.

% This paper argues that the cloud providers should compensate the tenants for their loss when the server is over-provisioned. However, estimating the tenant's loss is challenging when there is no pre-profiled information about the function. Prior studies showed assessing the tenant's loss introduces heavy overheads. Instead, this paper proposes a new pricing model, Litmus pricing, which offers discounts based on the machine's state while presuming the tenant's loss under the state. To monitor the machine state correctly, Litmus pricing frequently conducts Litmus tests, an effectively lightweight solution to measure system congestion. Our experiments show that Litmus pricing can detect the impact of system congestion and offer near-ideal prices, with only a 0.38\% price difference. 
This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2\% price difference on average, in a heavily congested system.

\end{abstract}


==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Serverless computing is growing fast, satisfying today's high demands for better programmability. It allows tenants to develop their programs as stateless functions in high-level languages such as Python, Go, and JavaScript without concerns with low-level resource management and task scheduling~\cite{serverless2,serverless1,schall2022lukewarm,schall2023warming,mohammad2020SerInWild}. This advantage attracts cloud users, helping them to deploy their programs quickly with minimal effort. Recent reports note that over 50-70\% of cloud users have adopted serverless computing for their tasks~\cite{serverless1}.

% Serverless computing claims a pay-as-you-go pricing model where users only pay for the resources used by their functions. This requires the service provider to monitor and estimate the fine-grained resource usage by each user accurately. However, today's high-performance systems maximize resource efficiency by accommodating multiple applications simultaneously and allowing the resources to be shared by them. Such a shared system raises two major challenges. First, tracking a user's resource usage is a challenging task. While being shared, the system tracks the total usage but not a single user's. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress. These inferences between the applications not only make the system hard to track resource usage, but the users may get charged unfairly due to the delayed execution time.
Serverless computing also benefits tenants financially. Unlike traditional cloud platforms that require tenants to purchase the hardware resources needed to deploy their servers regardless of actual usage~\cite{amazonEC2Pricing}, serverless computing claims a pay-as-you-go pricing model, where tenants only pay for the resources consumed during the execution of their functions, facilitating significant cost savings. Meanwhile, this pricing requires service providers to accurately monitor and estimate each user's fine-grained resource usage~\cite{microsoftAzurePricing,awsLambdaPricing,googleCloudFunctionPricing}. 

% However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared system raises two major challenges. First, tracking a tenant's resource usage is a challenging task. While being shared, the system can only monitor a tenant's use of specific resources. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference between the applications not only makes the system hard to track resource usage, but the tenants may get charged unfairly due to the extended execution time~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}. 
However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared serverless system raises two major challenges. First, tracking a tenant's resource usage becomes challenging, as the system can only monitor a tenant's use of exclusively dedicated resources while the system is shared. Second, and more importantly, co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference not only complicates tracking resource usage but also leads to tenants being charged unfairly due to delayed execution times~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}.

% A serverless platform should provide an isolated runtime environment to a user. Otherwise, we argue that the platform provider must compensate a tenant's loss as a discount when it is not achievable. Therefore, we define a charged fee as fair when it reflects the tenant's slowdowns due to the resource sharing. The following two methods can be used to estimate a fair price under a multi-tenant environment. 
A serverless platform should provide a user with an isolated runtime environment. Otherwise, we argue that the platform provider should compensate a tenant's loss as a discount when the isolation is not achievable. Thus, we define a charged fee as fair when it reflects the tenant's slowdowns caused by resource sharing. The following two methods can be used to offer a fair price in a multi-tenant environment.

% First, strict resource partitioning can divide shared resources into multiple partitions, each assigned to a user exclusively. The user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strictly partitioned resources are well known to cancel the opportunities to utilize the given resource efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delayed execution directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources when requesting them. 
First, strict resource partitioning can divide shared resources into multiple partitions, each assigned exclusively to a user. This means the user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strict partitioning is known to cancel opportunities to utilize resources efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delay directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources they need when requested. 

% Alternatively, a discount-based scheme estimates a user's price relative to its slowdown, discounting from the price when run without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources. Thus, the providers can maximize their hardware utilization and earn more money with given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns or interference they get from co-running tasks without overpaying for exclusive resources.
% The tenants also can get a discount reasonably proportional to the amount of their slowdown when their jobs suffer from interference rather than endeavoring to secure necessary resources exclusively.
Alternatively, a discount-based scheme estimates a user's price relative to the slowdown experienced, discounting from the price when running the task without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources, enabling providers to maximize hardware utilization and generate more revenue with the given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns they experience due to co-running tasks, preventing them from overpaying for lowered service quality.

% While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Even if the platform can measure its execution time, computing the slowdown still requires knowing its baseline, which can be gained when executing it alone. The cloud platform could not pre-profile users' applications for reasons such as mandated privacy when processing confidential information. Even if the platform has such information, the function could operate differently when receiving different inputs. That is to say, online profiling is necessary, which unfortunately requires expensive runtime sampling, as proposed in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. All co-running tasks must be stalled when estimating a task's baseline performance. Massive short-living serverless functions make such a sampling-based solution even more impractical. Frequently sampling the baseline performance of thousands of co-running functions is unrealistic. This motivates a new practical solution that can be adopted in commercial platforms. 
While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Although the platform can measure its execution time, determining the slowdown requires knowing its baseline performance, which can be obtained when it runs without interference. However, such profiling is often prohibited due to security concerns, particularly when the function processes confidential information. Additionally, the function may behave differently, with varying inputs each time it runs. That is to say, online profiling is necessary. Unfortunately, this requires expensive runtime sampling, as presented in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. When assessing baseline performance, all co-running tasks must be stalled. Hundreds to thousands of concurrent short-lived functions make this approach indeed impractical, as frequently sampling the baseline performance of such numerous functions is unrealistic. Thus, a new, practical solution that can be adopted in serverless platforms is needed.

%In either approach, a tenant or a service provider bears the problem's complexity alone. Resource partitioning demands the tenant to know the needed resources while losing opportunities to utilize the resources better. Discounting demands a service provider to estimate the task's slowdown with heavy sampling overheads. Accordingly, both approaches complicate the problem while sacrificing the machine's efficiency. Instead, we claim this problem becomes simpler when both entities participate and carry a portion of the responsibilities. 

% Litmus addresses this challenge by imposing the responsibility on both entities. With Litmus, the serverless platform measures the system congestion that may delay a function's execution when every tenant's function starts. The service provider needs to determine a discount rate for a corresponding congestion state. Meanwhile, the tenant needs to know about a possible slowdown and a corresponding discount. 

% We highlight that both partitioning and sampling complicate the problem while sacrificing the machine's efficiency and can hardly be employed in serverless computing. The approaches in serverless must be lightweight and frequent to deal with the fast-changing environment with thousands of concurrent functions. This paper proposes Litmus pricing that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening the system performance. 
We highlight that both partitioning-based and sampling-based approaches complicate the problem, either sacrificing the machine's efficiency or appearing impractical for serverless computing. Approaches in serverless computing must be lightweight, frequent, and sensitive enough to deal with quickly changing environments with numerous concurrent functions. This paper proposes Litmus pricing, a method that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening system performance. 

% \hl{Measuring the server's congestion status is challenging work. Here, Litmus relies on our key observation that, although not limited, function implementation in serverless computing largely relies on high-level programming languages such as Python and GoLang, which require a relatively long startup. This startup overhead has been considered one of the major challenges in serverless computing. However, Litmus utilizes this startup to measure the system's congestion state. Our analysis of Python and GoLang observed that the activities during the startups are almost identical, with plenty of memory operations, regardless of the functions. Thus, we claim that the startup performance can be an index of the system state.}

% \hl{The Litmus test is based on our insight that the serverless functions perform broadly identical operations, with plenty of memory operations, during their long startups, preparing the runtime environment for the functions. Leveraging this observation, the platform can assess the system's congestion level, which hints at the tenant's discount amount. Additionally, Litmus pricing exploits our second insight that the performance of two resources, private and shared, are affected differently by the congestion. In particular, its impact on private resources is minor and predictable, while many functions significantly rely on them, spending most of their execution time with them. }

% During the execution of every function, Litmus pricing conducts a Litmus test, which measures the level of system congestion with no extra overhead using the function's startup process. The Litmus test is based on the observation that serverless functions perform largely identical operations during their startup time. Those operations usually prepare the runtime and include a large amount of memory access to shared hardware resources. In addition, Litmus pricing splits the hardware resources into "private" and "shared" and proposes charging different ratios on each. This further improves the accuracy of the discount calculation.
During each function's execution, Litmus pricing conducts a Litmus test, which measures the level of system congestion without adding extra overhead, using the function's startup process. Litmus test is based on the observation that serverless functions perform largely identical operations during their startup, typically involving significant memory accesses. Additionally, Litmus pricing splits the hardware resources into "private" and "shared" categories, proposing different charging ratios for each. This approach further enhances the accuracy of the discount calculation.

% In our experiments, the Litmus pricing estimates a tenant's price to be nearly ideal, with a \hl{0.38\%} difference from the ideal price, which discounts tenants proportional to their slowdowns.
% This study investigates Litmus pricing across different environments, ranging from restricted to crowded settings. We verify that crowded environments pose additional challenges. Despite this, Litmus pricing accurately estimates a tenant's price, deviating by only 0.26\% from the ideal price, discounting tenants proportional to their slowdowns.
This study investigates Litmus pricing across diverse environments with varying levels of system congestion. We confirm that crowded environments pose complex challenges. Despite this, Litmus pricing accurately estimates a tenant's cost, deviating by only 0.2\% on average from the ideal price that discounts tenants proportional to slowdowns.



==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/02_background.tex <==
\section{Background}
\label{sec:background}

% \textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while the service providers handle back-end implementation~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers, which are later invoked upon associated events~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. The serverless platform guarantees security by executing the tenant's function in a sandbox such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.
\textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while leaving back-end implementation managed by service providers~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. These functions are later invoked upon associated events. The serverless platform ensures security by executing the tenant's function in a sandbox, such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.

% Each tenant's function is stateless and expected to be short~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using the short-lived functions, the tenant can easily scale by invoking many of the functions without provisioning needed resources for themselves, relying on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. Inherently, massive short-living serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. The tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and clients mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Later, under the pay-as-you-go pricing, the tenant is charged for the consumed resources, typically the product of time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
Each tenant's function is stateless and expected to be short-lived~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using these short-lived functions, tenants can easily scale by invoking many functions without provisioning the needed resources for themselves, relying instead on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. In serverless computing, numerous short-lived serverless workloads run together on a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. Tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and tenants mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% In the traditional cloud, tenants purchase hardware resources for the contracted term to support their applications, which are often expected to be large in a server form. Thus, tenants must pay for the agreed period regardless of actual use. Instead, serverless workloads are generally small and launched on-demand as short-living event handlers. This workload difference develops a unique pricing policy, pay-as-you-go pricing. The tenant is charged only for the consumed resources during the execution, typically the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
In traditional cloud computing, tenants purchase hardware resources for a contracted term to support their applications, which are typically large servers. Thus, tenants must pay for the agreed period regardless of actual usage. In contrast, serverless workloads are generally small and launched on-demand as short-lived event handlers. This difference leads to a unique pricing policy known as pay-as-you-go. Under this model, tenants are charged only for the resources consumed during execution, typically calculated as the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, where Python is utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Also, over 90\% of organizations choose Python and Node.js for their AWS services. Other popular language runtimes are Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer a high level of abstraction from machine codes with good programmability and portability, improving the programmer's productivity. As a result, they have been adopted widely by serverless users. However, such high-level languages typically rely on runtime interpretation, which results in a slow start of program execution with extra launching steps. For instance, in the case of Python, when an application is launched, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the codes are compiled and executed. Once the execution is complete, the Python program is terminated, and all assigned resources are released~\cite{pythonUsage}.
\textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python used in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Over 90\% of organizations choose Python and Node.js for their AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer significant abstraction from machine code with good programmability and portability, which in turn improves programmer productivity. Consequently, they are widely adopted by serverless users. However, high-level languages typically rely on runtime interpretation, leading to slower program startup due to extra launching steps. For example, when an application is launched in Python, the interpreter is first prepared. It then parses command-line arguments and imports necessary modules. Afterward, the codes are compiled and executed. Upon completion, the Python program terminates, and all allocated resources are released~\cite{pythonUsage}.

 
% list of pricing models? 
% Amazon? 
% Google?
% The price is calculated by duration time multiplies to the unit price plus the request charges. The duration time is from the time user's code begins executing until it returns or terminates. The unit price depends on the amount of memory the user allocate to their function. The request charges is based on how many times the function has been invoked minus the free requests~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% may need service agreement here, contention impact

%\textbf{Traditional cloud platforms:} In the context of traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage, data transfer, etc. The instance type is the combination of Virtual CPUs(VCPUs), RAM, storage and network performances. The time unit price will be higher with more powerful instance type. Typically, more powerful instance types have higher time unit prices. There are two main pricing options: On-Demand and Reserved Instances. On-demand instance let the customers pay for compute capacity by the hour or second based on the actual usage with no long-term commitments. Reserved Instances, on the other hand, require a commitment to a specific instance type for a contract term and offer cost savings compared to On-Demand pricing. Storage and data transfer for the VM instance can also impact the pricing. The more storage space a customer uses or the more data they transfer, the higher their costs will be. The traditional cloud platform can also be affected by the co-running applications~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} In traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage space, data bandwidth, etc. The instance type includes virtual CPUs, RAM, storage, and network performances. Typically, more powerful instance types charge higher prices. Also, two pricing options are commonly offered: on-demand and reserved instances. On-demand instances allow tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved instances require a commitment to a specific instance type for an agreed term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period. Storage space and data bandwidth for the VM instance also influence the price. Demanding more storage space or more data transfer raises the cost~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} 

% The price of traditional cloud platforms is determined by computing capabilities such as processor type, memory capacity, and network bandwidth. While more and better resources typically charge higher prices, two pricing options are commonly offered: on-demand and reserved instances. On-demand pricing allows tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved pricing requires a commitment to specific resources for an agreed-upon term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period~\cite{amazonEC2Pricing}. 

% There are several differences between traditional cloud platforms and serverless platform. 
% Firstly, the roles of customers in the execution environment differ between traditional and serverless platforms. In the traditional cloud, customers are responsible for configuring and maintaining virtual machines (VMs), setting up networking, and managing databases~\cite{amazonEC2Pricing}. And it's the customers's responsibility to detact and update the configurations to balance their expenses and performance. On the other hand, in serverless platforms, users only provide a single file to indicate their system and library requirement, while the service provider handles the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. This feature enables users to focus solely on their actual workload without the burden of managing the infrastructures. Additionally, the platform can automatically scale the resources for the users based on the current demand of the application to guarantee the customer satisfaction~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% There are apparent differences between traditional and serverless cloud platforms. First, tenants are responsible for managing hardware resources in traditional platforms. The tenants need to configure and maintain virtual machines, set up networking, and manage databases~\cite{amazonEC2Pricing}. Also, tenants should study the optimal configurations to balance their expenses and performance. Meanwhile, in serverless platforms, tenants only provide a single file to specify their system requirements while the cloud provider prepares the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. The platform provisions or scales the needed resources on demand. Consequently, the serverless platforms encourage tenants to focus solely on their front-end workloads without the burden of managing the low-level back-ends~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% Secondly, there are notable differences in compute power and memory size options between the two platforms. For traditional cloud, the granularity usually 1 VCPU and 1GB memory. But, for serverless platform, the smallest memory size is 128 MB~\cite{awsLambdaApiGateWay,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Thirdly, the characteristics of workloads on these platforms set them apart. Serverless applications are generally small and executed on-demand, resulting in very short workload durations~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can complete in less than one second. In contrast, traditional cloud applications tend to be larger and may require hours to complete. Additionally, the number of co-located applications on a single computing node is smaller in traditional cloud setups, making their execution environment less dynamic compared to serverless platforms.
% Lastly, the billing periods differ significantly between traditional cloud and serverless platforms. Traditional cloud users are charged for the allocated time period. Regardless of whether they are actively running tasks on the machine, they are still need to pay for the allocated time period. However, serverless customers are only billed for the actual execution time of their tasks on the platform.

% Second, the workloads are expected to be small in serverless computing. Serverless workloads are generally small and launched on-demand as short-living event handlers~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can be completed in less than one second, unlike traditional cloud applications that are often expected to be large in a server form. Inherently, massive serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. This workload difference develops a unique pricing policy in serverless computing, pay-as-you-go pricing. In the traditional cloud, the tenants purchase hardware resources for the contracted term. Regardless of actual use, they need to pay for the agreed period. However, the serverless platforms bill their tenants for the actual execution time of their tasks.


% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python being utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Furthermore, over 90\% of organizations leverage Python and Node.js alongside AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer numerous advantages for programmers, such as user-friendliness, portability, reduced error risks, and thriving ecosystems. As a result, they have garnered widespread acceptance within serverless platforms. High-level programming languages typically follow a fixed execution procedure. For instance, in Python, when an application is executed, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the code is compiled and executed. Once the execution is complete, the Python program is terminated, and all resources used by the program are released. Due to the consistency of the operating system and Python version, the beginning of the execution process remains the same each time~\cite{pythonUsage}.



% \textbf{Resource based discount vs. Slowdown based discount:} To fully utilize the available resources, service providers often run as many applications as they can in one computing node within the service agreement requirement. However, this may lead to resource congestion and cause slowdowns for users, which can be unfair, since the customers are paying more money for the worse experiences. The intuitionistic solution could be for the service provider to track the resource usage of each application and offer discounts to users who consume fewer resources. However, serverless applications are typically very small, and contention can affect different applications differently, making this approach less practical. A more suitable solution for serverless platforms could involve offering slowdown-based discounts. In this approach, the service provider dynamically updates unit prices based on the level of system congestion. When there is less contention, users normally stiffed with the experiences and pay the regular price. However, during periods of high congestion, when the system is under heavy load, users could receive discounted prices as compensation for potential slowdowns. This approach would align pricing with the actual performance experienced by users, ensuring a fair and responsive pricing model.


==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/03_methodology.tex <==
\section{Methodology}
\label{sec:method}

% \textbf{Hardware Infrastructure:} All the experiments are performed on a dual-socket server platform. Each socket has 16 simultaneous multithreading(SMT) cores. The CPU model is Intel Xeon Gold 5218(Cascade Lake). The maximum frequency of the machine is 3.9GHz. Each core has a 32KB L1 instruction cache, a 32KB L1 data cache and a 1MB L2 cache. The 32 virtual cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The computer node runs the latest Ubuntu server version(Ubuntu 22.04 LTS) with kernel version 5.15.0. For consistency in the results, the core frequency was set to 3.0GHz using the 'cpupower frequency-set' command. We use linux perf~\cite{perfWiki} to collect the performance counters for each experiment. To analyze the startup status, we use -I 1 option to obtain count deltas at one-millisecond intervals. By utilizing interpolation, we can know the performance counters of each execution period. 

% In this study, we test today's server systems with serverless functions. This section describes our test configuration. 
This section outlines our test setup for evaluating serverless functions in this study.

% % original version
% \textbf{Hardware Infrastructure:} All experiments are performed on a dual-socket server platform with two Intel Xeon Gold 5218 (Cascade Lake). The CPU offers 16 simultaneous multithreading (SMT) cores with 3.9 GHz maximum frequency. We pin the core frequency at 3.0GHz for our tests. Each core has 32KB L1 instruction/data caches and 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The machine runs the Ubuntu server OS (Ubuntu 22.04 LTS) with a kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to collect the performance counters, which are collected at every one-millisecond interval. 
\textbf{Hardware Infrastructure:} All experiments are conducted on a dual-socket server platform equipped with two Intel Xeon Gold 5218 processors based on the Cascade Lake architecture. Each CPU provides 16 cores that support simultaneous multithreading (SMT) with a maximum frequency of 3.9 GHz. Every core features 32KB of L1 instruction/data caches and a 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets collectively have access to 384GB of main memory. The server operates on Ubuntu Server OS, version 22.04 LTS, with kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to gather performance counters.

% The CPU frequency is a key performance/energy factor, significantly affecting a function's execution time and energy consumption. A CPU's frequency can be altered in software or hardware based on its power and thermal budget, configuring it for better energy efficiency or performance. However, varying frequencies cause the system performance/energy to be unsettled, making system management intractable. For this reason, commercial systems such as Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. In our tests, when the frequency is not fixed by software, Intel's Turbo technology alters the frequency occasionally but mainly employs 2.8GHz. We will discuss this further in the sensitivity section.
The CPU frequency is a critical factor influencing both performance and energy consumption, significantly affecting a function's execution time and energy usage. A CPU's frequency can be adjusted through software or hardware based on power and thermal budget, optimizing for either energy efficiency or performance. However, varying frequencies can cause instability in system performance and energy usage, complicating system management. For this reason, commercial systems like Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. If we do not fix the frequency through software, Intel's Turbo technology occasionally adjusts it, but it mostly remains at 2.8 GHz during our tests. We will provide more details on this in Section~\ref{sec:sensitivity}.

% \textbf{Stressing Programs:} We used two stressing programs to investigate how applications and the startup portion of the high level languages behave in a resource contention environment. FigureXXX illustrates the number of instructions, L3 accesses, and L3 misses that the stressing programs can generate in five seconds as the stressing levels increase. By combining different stress levels of these stress-testing programs, we can simulate various resource-congested environments. The XXX-stressor(lineXXX)  generates more L3 accesses with a high L3 hit rate. While XXX-stressor(lineXXX), in each stressing level, generates fewer L3 accesses but more L3 misses. With these two stressors and different stressing levels, we can simulate the system with varying contentions to the shared resources by creating various  L3 accesses and L3 misses. In figureXXX we can see that the L3 accesses generated from the L2-stressor (update name later) begin to decrease after reaching stressing level 20.  However, during this period, the L3 misses continue to increase. The reason behind this trend is that, after stressing level 20, the heightened L3 miss rate starts to impact the stressor's performance, leading to a decline in the committed instruction count. Consequently, the stressor generates fewer L3 accesses and more L3 misses. 

% \begin{table}[h]
%     \begin{center}
%     % \vspace{-1.0em}
%         \caption{Serverless Benchmarks \& Runtimes}
%         \label{tb:benchmarks}
%         % \vspace{-1.0em}
%         \begin{tabular}{|l l||l l|} \hline
%             Function & Abbr. & Function & Abbr. \\ \hline \hline
%             \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  & \multicolumn{2}{c|}{\textbf{Hotel Reservation~\cite{gan2019open}}} \\ \hline
%             Dyn HTML & dyn-py & Geo & geo-go* \\ \hline
%             Thumbnail & thum-py* & Profile & profile-go \\ \hline
%             Compression & compre-py & Rate & rate-go \\ \hline
%             Image Recogn & recogn-py* & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
%             Graph Rank & pager-py & Currency & cur-nj* \\ \hline
%             Graph Mst & mst-py & Payment & pay-nj \\ \hline
%             Graph Bfs & bfs-py* & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
%             DNA Visual & visual-py* & Authen & auth-py/nj/go \\ \hline
%             \multicolumn{2}{|c||}{\textbf{Function Bench~\cite{kim2019functionbench}}} & Fibonacci & fib-py/nj/go* \\ \hline
%             Chameleon & chame-py & AES & aes-py/nj/go \\ \hline
%             FloatOp & float-py* & & \\ \hline
%             % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
%         \end{tabular}
%     \end{center}
%     % \vspace{-1.5em}
% \end{table}

\begin{table}[h]
    \begin{center}
    % \vspace{-1.0em}
        \caption{Serverless Benchmarks \& Language Runtimes (py, nj, go)}
        \label{tb:benchmarks}
        % \vspace{-1.0em}
        \begin{tabular}{|l l||l l|} \hline
            Function & Abbr. & Function & Abbr. \\ \hline \hline
            \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  &  \multicolumn{2}{|c|}{\textbf{Function Bench~\cite{kim2019functionbench}}}\\ \hline
            Dyn HTML & dyn-py & Chameleon & chame-py \\ \hline
            Thumbnail & thum-py* & FloatOp & float-py \\ \hline
            Compression & compre-py & Gzip & gzip-py* \\ \hline
            Image Recogn & recogn-py & RandDisk & randDisk-py* \\ \hline
            Graph Rank & pager-py & SequenDisk & seqDisk-py \\ \hline
            Graph Mst & mst-py & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
            Graph Bfs & bfs-py* & Currency & cur-nj* \\ \hline
            DNA Visual & visual-py* & Payment & pay-nj \\ \hline
            \multicolumn{2}{|c||}{\textbf{Hotel Reservation~\cite{gan2019open}}} & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
            Geo & geo-go & Authen & auth-py*/nj/go \\ \hline
            Profile & profile-go* & Fibonacci & fib-py*/nj*/go* \\ \hline
            Rate & rate-go & AES & aes-py/nj*/go* \\ \hline
            % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
        \end{tabular}
    \end{center}
    % \vspace{-1.5em}
\end{table}

% revision version
% \textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we select 27 distinct serverless functions from different benchmark suites, including AWS' authentication serverless functions~\cite{awsLambdaApiGateWay}, Hotel Reservation from the DeathStarBench suite~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and SeBS serverless benchmark suite~\cite{copik2021sebs}. The three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating 3 separate test cases per function. Among them, we pick 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. The functions are implemented using three languages: Python, Nodejs, and Go. We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. 
\textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we selected 27 distinct serverless functions from various benchmark suites, including AWS authentication serverless functions~\cite{awsLambdaApiGateWay}, the Hotel Reservation from DeathStarBench~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and the SeBS serverless benchmark suite~\cite{copik2021sebs}. The functions are implemented using three languages: Python, Nodejs, and Go. Notably, the three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating three separate test cases per function. 
% This comprehensive language support ensures that our test coverage is thorough and representative of the diverse language preferences in the serverless computing community. 
We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. Additionally, we selected 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. 


%\hl{The benchmarks we choose include I/O-bound, memory-bound, and compute-bound functions. For an experiment, we put the testing function in core 0 to core 4. We also put 50 other functions in core 0-4 to let the application co-running with 10 other applications to observe the impact of context switching.}

% \hl{We select benchmarks with mixed performance characteristics: I/O, memory, and compute-bound. Also, to replicate the congested commercial systems, we located a testing function with 50 other functions and tied them to selected 5 cores, Core 0 to 4. During our evaluation, those functions run simultaneously and compete to secure any core among the five.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
\caption{(a) L2 misses and (b) L3 misses of traffic generators, both normalized with the average L2 and L3 misses of serverless applications listed in Table~\ref{tb:benchmarks}}
% \vspace{-0.5em}
\label{fig:stressing_specs}
\end{figure}

% \textbf{Traffic Generator:} We divide the CPU's shared resources into two distinct categories: resources before and after the L3 caches. To pressure each resource group individually, we developed two separate traffic generators aimed at generating traffic and congestion in these resources. The first traffic generator, CT-Gen, applies pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another traffic generator, MB-Gen, induces massive L3 misses that stress the resources after the L3 cache, mainly the off-chip memory bandwidth and L3 cache spaces.
\textbf{Traffic Generator:} We categorize the CPU's shared resources into two groups: those before the L3 caches and those after. To stress each group independently, we developed two separate traffic generators designed to generate traffic and congestion within these resources. The first generator, CT-Gen, exerts pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another generator, MB-Gen, induces massive L3 misses, which stress the resources beyond the L3 cache, primarily targeting off-chip memory bandwidth and L3 cache spaces.

% Both traffic generators are multi-threaded, governing the volume of traffic by adjusting the number of threads they spawn. Each thread spawned by the traffic generator is pinned on each core to prevent conflicts between threads; consequently, this setup allows us to vary the stress level across our 32-core processors, ranging from level 1 to 31. Figure~\ref{fig:stressing_specs} shows each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), for every thread count increment, CT-Gen makes massive L2 misses. The CT-Gen's L2 misses are ended with L3 hits, as shown in Figure~\ref{fig:stressing_specs}(b). Meanwhile, MB-Gen creates huge L2 and L3 misses, as implemented. Interestingly, its L2 misses are fewer than CT-Gen's because MB-Gen is slowed by its L3 misses, suffering from a self-created bandwidth bottleneck. 
Both traffic generators are multi-threaded and govern the amount of traffic by adjusting the number of threads they spawn. Each thread is pinned to a specific core to avoid conflicts between threads, allowing us to vary the stress level on our 32-core processors from level 1 to 31. Figure~\ref{fig:stressing_specs} illustrates each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), with each increase in thread count, CT-Gen generates substantial L2 cache misses. These L2 misses by CT-Gen are ended with L3 cache hits, as shown in Figure~\ref{fig:stressing_specs}(b). In contrast, MB-Gen produces significant L2 and L3 cache misses. Interestingly, MB-Gen's L2 misses are fewer than those of CT-Gen because MB-Gen is hindered by its L3 misses, suffering from a self-imposed performance bottleneck.



==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/04_motivation.tex <==
\section{The Need for Fair Pricing}
\label{sec:motivation}

% Offering fairness appears in different approaches in cloud computing when multiple tenants share hardware resources. One standard is SLA, which defines the level of services the cloud provider furnishes while a tenant sets their expectation. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving unfairness between tenants. Although serverless computing highlights the pay-as-you-go pricing model, such unfairness still exists.
Fairness in cloud computing, especially when multiple tenants share hardware resources, is addressed through various approaches. One standard method is the Service Level Agreement (SLA), which specifies the level of service the cloud provider must deliver and the tenants' expectations. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving fairness issues. Despite serverless computing's emphasis on a pay-as-you-go pricing model, unfairness among tenants still exists.

% Unfortunately, modern systems are designed to maximize hardware efficiency by co-running multiple applications; the function's execution time can be affected by co-scheduled applications with conflicts when using shared resources. Ironically, whenever the service provider squeezes their resources further for better profit by accommodating more functions into a single machine, each function's execution time increases, charging them a higher cost for the same workload. However, in serverless computing, tenants lack control and insights into how their software is executed and billed for the cost of convenience. 
Unfortunately, modern systems are designed to maximize hardware efficiency by running multiple applications concurrently. This results in conflicts over shared resources, affecting each function's execution time. Ironically, when service providers optimize for profit by packing more functions into a single machine, the execution time for each function increases, resulting in higher costs for the same workload. In serverless computing, tenants have no control or visibility over how their software is executed, leading to potential inefficiencies and higher costs for the sake of convenience.

% Genuine pay-as-you-go pricing can be achieved when there is no interference. However, that is not desired by the providers who expect to utilize their resources to maximize profits. In serverless, although each function runs virtually exclusively in a sandbox with private resources, it still shares a few resources with other co-running functions, such as shared caches and memory bandwidth. Resource partitioning, a traditional solution that eliminates interference, can promise exclusively dedicated resources to a tenant but cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 
In serverless computing, although each function runs exclusively in a virtual sandbox with private resources, it still shares certain resources like caches and memory bandwidth with other functions. Resource partitioning, a traditional solution that eliminates interference by dedicating resources exclusively to a tenant, cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 

\begin{figure}[h]
\centering
% \vspace{-0.7 em}
\includegraphics[width=1\columnwidth]{./fig/normalizedCPIRunWith26Rev}\\
% \vspace{-1 em}
\caption{Execution time of applications that run with 26 others, normalized to the execution time when running alone}
% \vspace{-0.4 em}
\label{fig:normalizedCPIRunWith26Rev}
\end{figure}

% Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed down when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. \hl{Whenever a function finishes, another function is randomly launched to maintain a total of 26 co-running functions.} The figure shows a function's performance drops by up to 35\%, and most functions are significantly influenced by the co-running functions. Compared to when an isolated environment is offered, the function performs 11.5\% slower on average, charging 11.5\% more to users. We highlight that the function runs only with 26 other functions, which is tiny compared to massively crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.
Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. Whenever a function finishes, a new randomly-selected function is launched to maintain a total of 26 co-running functions. The figure shows a function's performance can drop by up to 35\%, with most functions significantly impacted by the co-running functions. On average, functions perform 11.5\% slower in this shared environment compared to an isolated one, resulting in users being charged 11.5\% more. We highlight that this scenario involves only 26 co-running functions, which is tiny compared to heavily crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.

% Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} attempted to offer price discounts if it has a slowdown, compensating for the slowdowns. To provide the discount, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount reflecting the slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all the responsibilities of the contentions between co-running functions, guaranteeing all tenants an invariant price for their use. Any unexpected slowdowns that a tenant experiences are returned with a discount. However, sampling is an expensive operation, requiring all co-running processes to stall during the sampling. Moreover, accurate measurement requires frequent sampling when its system environment quickly alters, making the approach impossible in a fast-shifting environment like a serverless platform.   
Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} offers price discounts to compensate for slowdowns. To provide these discounts, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount based on the observed slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all responsibilities related to contentions from resource sharing, ensuring tenants pay a consistent price for their usage. Any unexpected slowdowns that a tenant experiences are compensated with a discount. However, sampling is an expensive operation that requires stalling all co-running processes during the sampling. Moreover, accurate measurement necessitates frequent sampling, especially in rapidly changing environments, making the approach impractical for dynamic environments like serverless platforms.


% A tenant needs a new pricing model based on more than just execution time. However, prior approaches have limitations, burdening cloud participants too heavily; it is unsuitable for \hl{thousands} of concurrent short-lived functions in serverless computing. This motivates us to propose a new solution, Litmus pricing, that discounts prices based on the system state but offers lightweight with no overheads.
Overall, tenants need a new pricing model that considers more than just execution time. Prior approaches have limitations, excessively burdening cloud participants and being unsuitable for the many short-lived functions typical in serverless computing. This motivates us to propose a new solution: Litmus pricing, which discounts prices based on the system congestion while remaining lightweight and imposing no additional overhead.


==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/05_design.tex <==
\section{Litmus Pricing}
\subsection{Overview}

% The estimated prices of serverless functions should reflect the congestion level of the system inside their machines. With the massive short-living functions, the serverless system's state can dramatically change in a short time. Accordingly, the system state can be congested at any moment and also resolved in a short time. However, such a temporary traffic jam may significantly impact the performance of short-living functions. Therefore, assessing the congestion must be lightweight, quick, and on time. However, a prior approach, POPPA\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling with considerable performance overheads, preventing them from wide adoption. Instead, we propose a new scheme, Litmus pricing, that quickly estimates system congestion at the start of every function and reflects the estimation into pricing the function. 
The estimated prices of serverless functions should reflect the system's congestion state. The presence of numerous small transient functions within the serverless system can rapidly alter its congestion state, causing sudden congestion or swift resolution. Nevertheless, such transient traffic jams can significantly impact the performance of short-lived functions. Thus, assessing the congestion must be lightweight, quick, and timely. However, a prior approach, POPPA~\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling, which incurs considerable performance costs, thereby limiting its widespread adoption. Alternatively, this study introduces Litmus pricing, which promptly gauges system congestion at the onset of each function and reflects the estimated congestion level into pricing the function.

% Like the prior approach~\cite{tiwari2013enabling,alex2013ScFairPrice}, Litmus pricing suggests that the service provider discounts when a tenant's functions are intervened, compensating for the performance loss. To determine the discount ratio, Litmus measures system congestion level, which can also help service providers evaluate remaining resources and make decisions on job scheduling. 
Like the prior approach, Litmus pricing suggests that service providers should offer discounts when a tenant's functions experience interference, thus compensating for the performance loss. Litmus pricing determines the discount rate based on the system's congestion level. Evaluating congestion also assists providers in estimating remaining resources and making informed decisions regarding job scheduling.

%Nevertheless, the Litmus pricing does not quantify each function's slowdown; the discount amount is determined only by the severity of the measured congestion. The impact of the congestion on distinct functions appears differently despite facing the same congestion level, and precisely estimating a function's performance loss is a complex problem. That's why the prior approach had to rely on expensive sampling. Instead, the Litmus pricing avoids the overheads and limits the service provider's responsibility to measure the current congestion. 
However, Litmus pricing does not quantify the slowdown of each individual function; the discount amount is solely determined by the severity of the measured congestion. Even though different functions face the same congestion level, their respective impacts can vary, making precise estimation of each function's performance loss a challenging task. This complexity necessitated the expensive sampling relied upon by the previous approach. Instead, Litmus pricing circumvents such overheads and lightens the service provider's burden solely to measure ongoing congestion levels.

% Litmus pricing embodies the varying value of shared resources across different system conditions by applying equal discounts to all functions under the same system condition, although the functions experience different slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that a function that is slowed more than others demands the over-crowded resources more while exacerbating the adverse over-crowded conditions. Litmus pricing does not provide additional compensation for their extra loss compared to others due to their heavy use of shared resources.
Litmus pricing captures the dynamic significance of shared resources under varying system conditions by offering uniform discounts to all functions under the same system congestion, regardless of their individual slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that functions experiencing larger slowdowns tend to demand more of the crowded resources, thereby exacerbating adverse overcrowded conditions. However, Litmus pricing does not offer additional compensation for the larger loss experienced by functions that use shared resources more heavily than others.

% As a result, Litmus inherently incentivizes users who use shared resources sparingly. When over-crowded, functions with minimal needs for shared resources still enjoy discounts but encounter slight slowdowns. This implies that users may take advantage of this policy by minimizing their use of shared resources, receiving substantial discounts despite enduring only minor slowdowns. Such a trade-off is considered acceptable because the user's shared resource usage reduces their contribution to congestion, thereby benefiting the overall system over the other users.
As a result, Litmus inherently incentivizes users who use shared resources sparingly. During periods of overcrowding, functions with minimal needs for shared resources still enjoy discounts but with only slight slowdowns. This implies that users may take advantage of this policy by minimizing their reliance on shared resources, receiving substantial discounts despite only experiencing minor slowdowns. This trade-off is considered acceptable because reduced shared resource usage by users helps mitigate congestion, thereby benefiting the overall system and other users.
% Lastly, the system refrains from scheduling a function if the congestion level exceeds a predetermined threshold, thus preventing resource thrashing.


\subsection{Pricing Model}
\label{pricing model}

% Developing Litmus pricing raises two challenges. First, Litmus needs a new pricing model to estimate a function's price. Second, Litmus needs a way to measure the system's congestion state. Due to the serverless's fast-shifting environment, assessing the congestion must be lightweight and frequent at the right time. Nevertheless, all present commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants must pay more with prolonged execution time when using over-crowded resources. Rather than simply imposing a price by multiplying the main memory usage and a function's total execution time, Litmus suggests the price as a sum of two distinct price components as follows.
Developing Litmus pricing raises two challenges. First, it needs a new model to estimate a function's price. Second, it needs a way to measure the system's congestion state. Due to the rapidly changing environment in serverless computing, assessing congestion must be lightweight and timely. Commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants end up paying more for prolonged execution time when using over-crowded resources. Rather than simply imposing the price by multiplying the main memory usage and a function's execution time, Litmus pricing determines the price as a sum of two distinct pricing components as follows.

\begin{equation} 
P = P_{private} + P_{shared}
\end{equation}

% In this equation, \(P\) denotes the total price tenants need to pay to execute their functions. Litmus pricing divides the tenant's price into two pricing components, each with a different resource type. \(P_{private}\) represents the price the tenant needs to pay for private resources, which are entirely assigned to a tenant. \(P_{shared}\) is the price the tenant needs to pay for the shared resources. Each price component is measured proportional to a user's time to occupy the corresponding resources. However, such occupied time can be extended when contention disturbs a process's execution in the shared resources. This delayed time increases a tenant's price unfairly. 
In this equation, \(P\) denotes the total price tenants must pay to execute their functions. Litmus pricing divides this cost into two pricing components, each associated with a different resource type. \(P_{private}\) is the cost for private resources, which are entirely assigned to a single tenant. \(P_{shared}\) is the cost for shared resources. Each pricing component is measured proportional to the time users occupy the respective resources. However, if contention disturbs a process's execution in the shared resources, the occupied time will be extended. This delay unfairly increases the tenant's cost. 


\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/slowdownRunwith26Rev}\\
\caption{\(T_{private}\) and \(T_{shared}\) of applications that run with 26 others, normalized to those when running alone}
\vspace{-0.5em}
\label{fig:slowdownRunwith26Rev}
\end{figure}

% Using Perf, we measure the delays due to the shared resources and split a function's execution time into two distinct slices: one slice, \(T_{private}\), which is time spent on private resources and another slice, \(T_{shared}\), which is time spent on shared resources. Figure~\ref{fig:normalizedTcore&Tuncore-runWith16} shows the impact of the contentions on each time slice, where we normalize \(T_{private}\) per instruction and \(T_{shared}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 207\% on average and 364\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions. 

% We observe that the system congestion influences the occupied time for each resource type differently. The time to hold private resources is slightly affected, with minor changes, even under heavy congestion. Meanwhile, the time due to shared resources is broadly affected, showing significant differences. Thus, we separately measure the two delays and charge their use with a different rule.
We observed that system congestion influences the occupied time for each resource type differently. The time to use private resources is only slightly affected, with minor changes, even under heavy congestion. In contrast, the time spent on shared resources is broadly affected, showing significant differences. Thus, we separately measure the delays for the two resource types and apply different charging rules for their use. 

% Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where we normalize \(T_{shared}\) per instruction and \(T_{private}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 181\% on average and 488\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions.
Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is calculated as the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where \(T_{shared}\) per instruction and \(T_{private}\) per instruction are normalized to the same tests when running alone. The figure shows that \(T_{shared}\) is significantly affected by system congestion compared to \(T_{private}\). On average, \(T_{shared}\) increases by 181\%, with a maximum increase of 488\%. Meanwhile, \(T_{private}\) increases by only 4\%, with minor variance between functions.

% This figure gives insights into two key factors. First, the congestion in the shared resources does not impact the performance of private resources. Accordingly, when the system gets congested, the degree of a function's dependence on the shared resources determines the function's performance. If the \(T_{shared}\) takes a minor portion of a function's execution, severe congestion still barely influences its overall execution. Second, hardware PMUs available in modern CPUs, and profiling tools such as Linux Perf are widely available and can be used to distinguish the usage of shared and private resources. Across the paper, we will take advantage of such tools to develop Litmus pricing.
This figure highlights two key factors. First, congestion in shared resources has a negligible impact on the performance of private resources. Accordingly, when the system gets congested, the extent of a function's reliance on shared resources determines its performance. If \(T_{shared}\) constitutes a minor portion of a function's execution, even severe congestion will have minimal impact on its overall execution. Second, hardware Performance Monitoring Units (PMUs) in modern CPUs and profiling tools like Linux Perf are widely available and can be utilized to differentiate between the use of shared and private resources. Throughout this paper, we will leverage these tools to develop Litmus pricing.

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/TpriTshardDistriRev}\\
% \caption{\(T_{private}\) and \(T_{shared}\) distribution when they run alone}
\caption{Execution time distribution of \(T_{private}\) and \(T_{shared}\)}
\vspace{-0.5em}
\label{fig:TpriTshardDistriRev}
\end{figure}

% Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) in a function's execution. The compute-intensive workloads (e.g., fib-py, float-py) have a substantial \(T_{private}\) portion that can reach 99.96\% of the execution time. However, the portion decreases when running memory-intensive workloads such as fib-nj. This distribution indicates how much other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase float-py's \(T_{shared}\), its total execution time, $T_{private}+T_{shared}$, will undergo minor change.
Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) during a function's execution. Compute-intensive workloads (e.g., fib-py, float-py) exhibit a substantial \(T_{private}\) portion, accounting for up to 99.96\% of the execution time. However, this portion decreases when running memory-intensive workloads such as fib-nj. This distribution reflects how other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase its \(T_{shared}\), the total execution time, $T_{private}+T_{shared}$, will undergo only a minor change.

% For each pricing component, we calculate the price by multiplying its charging rate with its time distribution. Thus we can further update the pricing equation.
After collecting the time slices spent on each resource, Litmus calculates each pricing component by multiplying two different charging rates with corresponding slices. Consequently, a new pricing equation emerges as follows:

\begin{equation} 
P = R_{private} * T_{private}  + R_{shared} * T_{shared}
\end{equation}

% \(T_{shared}\) is the cycles stalled due to L2 misses. It is measured from the perf counter, STALLS\_L2\_Misses. \(T_{private}\) is the total execution minus STALLS\_L2\_Misses. 
% Using Perf, Litmus collects\(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total cycles to complete the application minus \(T_{shared}\). 
% While Litmus returns the system's congestion state, the service provider still needs to determine reasonable prices charged for a service when having different congestion levels. 

% \(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. Again, the two charging rates are necessary since each component is affected differently, directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from the crowded execution environment. Thus, the charging rates should be measured as follows.
\(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. These two charging rates are necessary because each component is affected differently, either directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from a crowded execution environment. Thus, the charging rates should be measured as follows:

\begin{equation} 
R = R_{base} * \frac{T_{solo}}{T_{congestion}}
\end{equation}

% In this equation, \(R\) is the charging rate for executions on either private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free execution environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is the execution time when the function runs alone, and \(T_{congestion}\) is its execution time in the congested environment. Again, we should collect a separate \(T_{solo}\) and \(T_{congestion}\) for each pricing component. To measure \(T_{solo}\), \hl{the prior work}~\cite{alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. Litmus pricing avoids such a costly approach but presumes the function's \textit{solo} performance by examining reference workloads on the system.
In this equation, \(R\) represents the charging rate for executions on private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free runtime environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is its non-interfered execution time when the function runs alone, and \(T_{congestion}\) is its execution time in a congested environment. We need to collect separate \(T_{solo}\) and \(T_{congestion}\) values for each pricing component. To measure \(T_{solo}\), the prior study~\cite{tiwari2013enabling,alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. However, Litmus pricing avoids such a costly approach by presuming the function's solo performance through reference workloads on the system.

% Litmus pricing requires both providers and tenants to be involved in the price decision. The providers need to decide on reasonable rates for each resource use by analyzing the selected representative functions running on the system. To offer reasonable discounts, the providers must choose the functions analyzed carefully, collecting the functions representing the system. The tenants must also know the consequences when their tasks heavily rely on any of the shared resources. Unfortunately, their tasks may get delayed more than the provider's expectation while still receiving the discount rate up to the expectation. 
Litmus pricing requires both providers and tenants to be involved in the price decision process. Providers need to establish reasonable rates for each resource usage by analyzing selected representative functions. To offer fair discounts, providers must carefully choose the functions to be analyzed, ensuring the functions accurately represent the system condition. Tenants must also know the consequences when their tasks heavily rely on shared resources. Unfortunately, their tasks may get delayed more than the provider's expectations while still receiving the expected discount rate. 

% Here, the Litmus pricing reflects the varying value of the shared resources when the system's congestion level changes; the importance of shared resources becomes more valuable when congested. 



==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/06_design_details.tex <==
\section{Estimating prices with Litmus}
\label{sec:designDetails}

% The providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}, before using Litmus pricing. The numbers in both tables are the slowdowns of codes while testing the system congestion. Shortly, the congestion table is filled with the slowdowns of startup codes, and the performance table is filled with the slowdowns of reference benchmarks. Litmus pricing needs three steps to charge the final price with a discount. First, the providers assess the system's congestion at multiple levels and range them in a table. This step completes the congestion table. Second, the providers study the impact of congestion on tenants' functions and complete the performance table. Lastly, the service provider determines a tenant's price based on the two tables. 
Before using Litmus pricing, service providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}. The congestion table lists the slowdowns during the startup phases, whereas the performance table lists the slowdowns of reference functions. Litmus pricing needs three steps to determine the final price with a discount. First, providers assess system congestion at multiple levels and record the results in the congestion table. Second, providers analyze the impact of congestion on reference functions and fill out the performance table. Lastly, providers determine a tenant's price based on the data from both tables.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tables}\\
\caption{Congestion and performance tables: numbers in both tables indicate the slowdowns of startup codes and reference functions, collected with CT-Gen and MB-Gen}
\vspace{-0.7em}
\label{fig:litmust_tables}
\end{figure}

\textbf{Step 1, Defining Congestion Levels:} We manage the system's congestion levels using two traffic generators that create a range of congestion states by stressing shared resources differently. The traffic generator is multi-threaded, creating traffic in shared resources to incur congestion, with each thread running on a separate core. We rank the stress levels from 1 to 32 by changing the number of active threads running on distinct cores. Entries from top to bottom in the congestion table indicate increasing stress levels.

% \begin{figure}[h]
% \centering
% \vspace{-1.5em}
% \includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
% \vspace{-1em}
% \caption{stressing program's instruction, L3 accesses and L3 misses }
% \vspace{-0.5em}
% \label{fig:stressing_specs}
% \end{figure}

% \textbf{Step 2. Measuring System Congestion:} Measuring the current level of system congestion that may influence a function's performance is a crucial challenge. If we assume that the platform does not have pre-profiled information about a function's performance, the platform cannot figure out whether co-running functions influenced the function. Additionally, the serverless platform's fast-changing states with massive short-living functions make the assessment even more complicated, requiring quick and frequent examinations.

% Meanwhile, measuring the amount of a system's congestion and its impact on performance is a crucial challenge. This challenge particularly stands apparent when being demanded to quantify the impact of the congestion on a running application without pre-profiled information about the application. Moreover, the serverless platform's fast-changing system states with \hl{numerous} short-lived functions make the assessment even more complicated, requiring quick and frequent performance examinations.
Measuring the amount of system congestion and its impact on performance is a crucial challenge. This challenge becomes particularly pronounced when trying to quantify the impact of the congestion on a running application without pre-profiled information about the application. The fast-changing system states of a serverless platform, with numerous short-lived functions, further complicate the assessment, necessitating quick and frequent performance examinations.

% Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. The proposal is based on the observation that high-level languages, such as Python and Node.js, used in serverless computing have long startup times to accommodate their runtime environments. Since the inception of serverless computing, these startups have been recognized as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests leverage these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests further validated that all tested functions exhibited similar performance characteristics during their startups. 
Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. This method leverages our observation that high-level languages like Python and Node.js, commonly used in serverless computing, have lengthy startup phases to accommodate their runtime environments. Since the inception of serverless computing, these startup delays have been identified as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests exploit these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests have validated that tested functions exhibit similar performance characteristics during startup phases. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_all}\\
% \caption{IPC for serverless applications with different runtimes in the first 100 milliseconds of their execution}
% \vspace{-0.5em}
% \label{fig:startupIPC_all}
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped}\\
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-1}\\
\includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-3}\\
% \caption{IPC for serverless applications grouped by language runtime in the first 100 milliseconds of their execution}
\caption{IPC of serverless applications based on languages (Go, Python, and NodeJS) during their startup phase}
% \vspace{-0.7em}
\label{fig:startupIPC_grouped}
\end{figure}

% Figure~\ref{fig:startupIPC_grouped} depicts the fluctuation in IPC (Instructions Per Cycle) of a function during the first milliseconds of its execution. The x-axis shows a time flow since the beginning; every tick indicates a millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language, and the throughput of each group is represented in separate figures. Although figures exhibit different patterns, functions in the same figure display notable similarities. The figures imply that functions written in the same language have nearly identical startups.
Figure~\ref{fig:startupIPC_grouped} depicts a function's fluctuation in IPC (Instructions Per Cycle) during its startup phases. The x-axis represents the time elapsed since the beginning, with each tick indicating one millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language runtime, and the IPC of each group is presented in separate figures. As shown in these figures, functions in the same figure show notable similarities. This implies that functions written in the same language have nearly identical startups.

% The startup of a runtime usually includes bursts of memory reads to load images and libraries, which can probe the traffic in the shared resources. By conducting a Litmus test before executing every tenant's codes, the providers can observe the system state for the function. Meanwhile, the providers also need to study how the startup codes perform in different system states. They complete the congestion tables by performing the Litmus tests with the startups written in three languages while varying the congestion levels. To this end, the information in the congestion table is looked up when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}. 
% estimating the system's state upon receiving a result of a function's Litmus test. 
The startup of a runtime typically includes bursts of memory reads to load images and libraries, which can be used to probe the traffic in shared resources. By conducting a Litmus test before executing a tenant's function, providers can assess the system state. Meanwhile, providers also need to study how startup phases perform under different system states. They complete the congestion tables by conducting the Litmus tests with startups written in three languages while varying congestion levels. This information from the congestion table is then referenced when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tests}\\
\caption{Progress of serverless applications on four cores with Litmus tests (dotted arrows) over time}
% \vspace{-0.5em}
\label{fig:Litmus_tests}
\end{figure}

% Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests. The Litmus tests examine the level of system congestion with every function startup. \hl{Many} concurrent functions in serverless offer frequent test opportunities. Function\#1 is a memory-intensive function that raises a congestion level. While active, Litmus tests measure the congestion level above 8. After Function\#1's completion, the next Litmus test detects a non-congested system with a congestion level below 3. However, with the start of another heavy function, function\#2, the Litmus tests measure the new congestion in the system.
Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests, which examine the level of system congestion during each function's startup. Many concurrent functions in serverless offer frequent opportunities for testing. Function \#1, which is memory-intensive, causes congestion levels to rise above 8 during its execution. A Litmus test in Core 3 detects this congestion. After Function \#1 is complete, a subsequent Litmus test indicates a non-congested system with a congestion level below 3. However, during another resource-intensive function, Function \#2, the Litmus test identifies new system congestion with a level above 9.  

% \textbf{Step 2. Measuring the Impact of Congestion:} Although discerning the system congestion through the Litmus test, estimating its impact on a user's application is another challenge. This work proposes a discount based on the pre-studied impacts on reference functions, assuming the user's functions are alike. For this, the service providers need to select reference functions that represent users' functions running on their systems. In this work, we select the workloads in \hl{Section 2} as our reference applications. 
\textbf{Step 2, Measuring the Impact of Congestion:} Discerning system congestion through the Litmus test solves only one of the two challenges; the other is determining its impact on a tenant's function. Different tenants' functions could experience varying degrees of slowdown under the same congestion level. To address this, we propose using pre-selected reference functions to analyze these impacts, thereby avoiding the cost of runtime profiling. For this, providers need to carefully select reference functions that represent tenants' functions operating on the systems, as these selections influence the overall accuracy of congestion measurement. Later, in Section~\ref{sec:evaluation}, our tests will show that pre-selected reference functions can effectively represent unknown user applications. For this study, the selected reference applications (* marked) are listed in  Table~\ref{tb:benchmarks}. 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/refSlowdownStressing14}\\
% \includegraphics[width=1\columnwidth]{./fig/slowdownStressing16}\\
\caption{\(T_{private}\), \(T_{shared}\), and \(T_{total}\) of serverless applications that run with MB-Gen at stress level 14, normalized to their execution time when they run alone}
% \vspace{-0.5em}
\label{fig:refSlowdownStressing14}
\end{figure}

% Once the reference functions are ready, the providers study the slowdowns of the reference functions while varying different congestion levels again. This study completes the performance table in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. Again, our two traffic generators create two separate sub-tables. All entries in this table are 1-to-1 mapped to entries in the congestion table. The providers estimate a general function's slowdown when having a certain congestion level using this 1-to-1 mapping.
Once the reference functions are ready, providers analyze their slowdowns under varying congestion levels. This analysis completes the performance table shown in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. With two traffic generators, providers can complete another set of two sub-tables for the performance table. All entries in this table are mapped 1-to-1 to entries in the congestion table. Providers can estimate a general function's slowdown at a given congestion level using this one-to-one mapping.

% Figure~\ref{fig:refSlowdownStressing14} shows the reference functions' slowdowns when stressing the system. The X-axis shows different functions, each consisting of three bars: the first two bars show the CPI during each time slice, \(T_{private}\) and \(T_{shared}\), and the last bar shows the CPI of an entire execution. The figure shows that the tested functions suffer from different amounts of slowdowns, although the tests maintain consistent stress levels. \hl{The last group} shows the gmean of all the slowdowns, which is used when providers estimate a function's slowdown later. 
Figure~\ref{fig:refSlowdownStressing14} shows an example of the reference functions' slowdowns when stressing the system. The X-axis shows tested functions, each depicted with three bars: the first two bars show \(T_{private}\) and \(T_{shared}\), while the last bar shows the total execution time, all normalized to their execution time when running alone without interference. The figure shows that the tested functions experience varying degrees of slowdown despite consistent stress levels maintained during the tests. The next-to-last group shows the gmean of all the slowdowns, which providers use to estimate a function's slowdown later.

% \hl{This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/referenceStartupSlowdownRev}\\
\caption{The correlation between the slowdown of Python's startup phase and the slowdown of reference applications. From left, (a) \(T_{private}\), (b) \(T_{shared}\), and (c) \(T_{total}\), normalized to the execution time when running alone}
\label{fig:referenceStartupSlowdownRev}
\end{figure}

% \textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while a range of congestion levels is continuous, the tables only contain a few slowdowns in discrete intervals. Thus, providers need a model that returns an estimated slowdown when receiving a congestion level as an input. In our tests, we employ a linear regression to achieve the model.
\textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while congestion levels vary continuously, the tables only contain slowdowns at discrete intervals. Therefore, providers need a model that estimates the slowdown for any given congestion level. In our tests, we employ linear regression to develop the model.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/interpolation}\\
\caption{Estimating a function's slowdown with logarithmic interpolation}
\label{fig:interpolation}
\end{figure}

% Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding references' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). We employed two traffic generators to extrapolate a more precise congestion level, yielding two sub-tables in both the congestion and the performance tables. Consequently, the figure presents two linear regression models, each associated with a different traffic generator. 
Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding reference applications' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). To extrapolate a precise congestion level, we created two sub-tables within both the congestion and performance tables using two distinct traffic generators. As a result, the figure depicts two linear regression lines (red and blue dotted lines), each associated with a different traffic generator.

% The provider needs to estimate the function's slowdown to uncover its price. However, the above two regression models return two vastly different slowdowns. Then, the providers need to determine which model is close to the current environment. We think the two models reflect two extreme congestions that the traffic generators create, one before the L3 and one after the L3. CT-Gen creates massive traffic from the core to the L3 cache, which filters the traffic, preventing the operations from consuming the memory bandwidth. MB-Gen also creates huge traffic but consumes the memory bandwidth and replaces L3 blocks. Since each traffic generator creates an extreme case, the machine state could be intermediate with congestion in the range between the two congestions created by CT-Gen and MB-Gen. However, Litmus pricing cannot answer this question with only the startup's slowdown. 

% To address this question, we note that the system's L3 misses are a critical indicator closely related to a function's performance. Functions suffer more when the system experiences more L3 misses, which stresses the cache space and off-chip memory bandwidth. Accordingly, Litmus test collects the system's L3 miss count as a supplementary index, which tells more about the crowdedness of shared resources.

These regression models return two different slowdowns. To estimate a function's slowdown, providers must determine which model reflects the current environment more accurately. The traffic generators create two extreme congestion scenarios: one before the L3 cache and one after. CT-Gen generates substantial traffic from the core to the L3 cache that filters the traffic and prevents operations from consuming memory bandwidth. Conversely, MB-Gen also generates massive traffic but consumes memory bandwidth and repeatedly evicts L3 cache blocks. Because each traffic generator represents a distinct extreme case, the actual machine state could fall somewhere between the two congestion levels created by CT-Gen and MB-Gen. However, Litmus pricing requires more than just the startup slowdown to identify the machine's state in these models. Thus, we have enabled Litmus tests to gather the system's L3 miss count as a supplementary metric that offers deeper insights into the crowdedness of shared resources.


% \hl{Figure 1} shows how to use the L3 cache misses with the performance sub-tables. The two traffic generators make the upper and lower boundary of the L3 miss rates. When performing a Litmus test, if the test's L3 miss rate is XXX, close to the L3 misses with CT-Gen, we can conclude that the congestion occurs before the L3 cache and select the expected slowdown of XXX. On the contrary, we choose XXX, in case the L3 miss rate is XXX, close to the L3 misses with MB-Gen. If the test's L3 miss rate is in-between, we interpolate the two slowdowns based on the L3 misses, assuming congestion in both resources. 
% Finally, we determine the Rprivate and Rshared based on the expected slowdown from its performance table. Calculating Rprivate and Rshared takes the same steps. The final discount price is computed using the equation with the computed rates. 

% Figure~\ref{fig:interpolation} shows how we employ the L3 misses when estimating the slowdown. The two traffic generators make the upper and lower boundary of the L3 misses. If a Litmus test reports the L3 miss count is 10, close to the L3 misses with CT-Gen, \textcircled{1}Litmus pricing estimates the discount (=expected slowdown) of the function to be near 1\%. This indicates that the congestion happens before the L3, as what CT-Gen creates. On the contrary, in case the L3 misses are 1000, close to the L3 misses with MB-Gen, \textcircled{2}Litmus pricing estimates the function's discount rate close to 6\%. Meanwhile, if the Litmus test reports the L3 misses as 100, we interpolate the two extreme discounts, 1 and 6, based on the L3 misses, assuming current congestion to stand in between the two extreme congestions. The congestion model in the figure shows how we interpolate with logarithmic interpolation. In this figure, \textcircled{3}applying the logarithmic interpolation to the L3 miss count returns the half-point between CT-Gen's 1\% and MB-Gen's 6\%, which is 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 
Figure~\ref{fig:interpolation} shows our approach to using L3 misses to estimate slowdowns. We created two figures illustrating separate regression models. The left figure (a) is derived from the startup slowdowns and L3 misses with logarithmic regression, indicating L3 misses at specific congestion levels. The right figure (b) is derived from the performance table with linear regression, displaying discounts at specific congestion levels. Each figure depicts two regression lines associated with different traffic generators.

The two traffic generators set the upper and lower boundaries for L3 misses. For instance, if a Litmus test reports 10 L3 misses, close to what CT-Gen generates: \textcircled{1}This suggests congestion occurs before reaching the L3 cache, similar to CT-Gen's scenario. Thus, Litmus pricing estimates the function's discount to be around 1\%. Conversely, if the Litmus test reports 1000 L3 misses, close to MB-Gen's results: \textcircled{2}Litmus pricing estimates the function's discount rate to be approximately 6\%, indicating congestion similar to MB-Gen, where memory bandwidth is heavily consumed and L3 cache blocks are frequently evicted. When the Litmus test reports 100 L3 misses, an interpolation between these extremes is applied: \textcircled{3}Using logarithmic interpolation, Litmus pricing estimates the function's discount rate to be midway between CT-Gen's 1\% and MB-Gen's 6\%, resulting in approximately 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 



==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/08_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \textbf{Litmus price \& error:}
% We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, and the other consists of selected reference applications to obtain the linear regression models for Litmus pricing. The discount models plug into the Litmus pricing used in our tests. For this experiment, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown.
We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, while the other consists of chosen reference applications to derive linear regression models for Litmus pricing. The discount models plug into the Litmus pricing employed in the tests. In this study, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown. 

% % original version
% We maintain the congestion state consistent across all tests, co-running each function with 26 other functions. Using Perf~\cite{perfWiki}, we collect the three key stats: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup, which implies the congestion level in these tests, as well as the discount rates that every function receives. We execute every function 100 times and collect the average of the function's \(T_{private}\) and \(T_{shared}\). Finally, we compute each function's \(P_{private}\), \(P_{shared}\), and \(P\), the total price, by summing \(P_{private}\) and \(P_{shared}\).  

\subsection{One Function Per Core}

% revision version
% We maintain consistent congestion states across all tests by co-running each function with 26 other functions. Using Perf, we collect the three key statistics: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup. These metrics hint at the congestion level during the tests as well as the discount rates that a function receives. Each function is executed 30 times, and the average of its \(T_{private}\) and \(T_{shared}\) is collected. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).
We maintain consistent congestion levels across all tests by co-running each function with 26 other functions. As outlined in Section~\ref{sec:motivation}, whenever a function finishes, another is randomly launched to keep a total of 26 co-running functions. Using Perf~\cite{perfWiki}, we collect three key statistics: \(T_{private}\), \(T_{shared}\), and the machine's L3 misses during the first 45 million instructions of the Python startup. Through these metrics, Litmus pricing estimates the level of system congestion and the discount rates a function receives. Each function is executed 30 times, and we average its \(T_{private}\) and \(T_{shared}\) values. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice26Rev}\\
% \caption{The total price for functions computed via Litmus pricing and ideal prices when co-running with 26 other functions normalized to the commercial price that offers no discount}
\caption{Prices computed via Litmus pricing and ideal prices when co-running with 26 other functions, normalized to the commercial price that offers no discount}
\label{fig:normalizedPrice26Rev}
\end{figure}

% In Figure~\ref{fig:normalizedPrice26}, we can see a minimal difference in the discount rate between the Litmus price and the Ideal price. The average Litmus discount rate stands at 11.5\%, which is only marginally larger by 0.6\% than the average Ideal discount rate of 10.9\%. Also, we can see that the difference between the Litmus price and Ideal price are different among the applications. Certain applications exhibit higher Litmus prices compared to the Ideal price, while conversely, some applications demonstrate smaller Litmus prices. 
 %Figure~\ref{fig:priceErrorRunwith26} shows further details, analyzing the errors in each pricing component. 

% Figure~\ref{fig:normalizedPrice26Rev} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{10.66\%}, which is only marginally larger by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{10.28\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice26Rev} illustrates estimated prices derived from Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices to offset delays in a congested execution environment. The figure shows minimal disparities between the two prices, implying that Litmus pricing offers a reasonable discount. The average discount from Litmus pricing across all functions is 10.7\%, which is only marginally higher by 0.4\% compared to the average slowdown experienced by functions, which stands at 10.3\%, as depicted by the ideal price.

% However, the discount rates per slowdown differ among functions. For instance, float-py's ideal discount rate is \hl{0.05\%}, but it enjoys a \hl{4.31\%} discount with the Litmus pricing. Meanwhile, pager-py's performance drops by \hl{15.63\%} while receiving a \hl{13.87\%} discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more easily affected than the reference when congested. In contrast, float-py runs mostly with private resources, receiving a minor impact from the execution environment. Figure~\ref{fig:priceErrorRunwith26Rev} shows further details, analyzing the differences in each pricing component.
However, the discounts per slowdown differ among functions. For instance, float-py's ideal discount rate is 0.05\%, but it benefits from a 4.3\% discount with Litmus pricing. Conversely, pager-py encounters a 15.6\% performance decline while receiving only a 13.9\% discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more susceptible to congestion than the references. In contrast, float-py predominantly utilizes private resources, resulting in minimal impact from the execution environment. Further insights into these variations in each pricing component are presented in Figure~\ref{fig:priceErrorRunwith26Rev}.


% From figure~\ref{fig:tcore\(T_{private}\)Distr}, we know that \(T_{private}\) dominates the execution time among all applications. The impact from \(T_{private}\) error has a bigger impact on the overall error. The slowdowns due to congestion in private resources are small. Theoretically, there should be no slowdowns when using private resources, but we observed that the congestion still influences it. The observed slowdown is 000, a small difference from an ideal slowdown. Meanwhile, the slowdowns in shared resources are significant. We observe that 

% % \[  Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}}\]

% \[Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{TotalIdealPrice}\]
% \[TotalIdealPrice = R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}\]

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/priceErrorRunwith26Rev}\\
\caption{Weighted errors in prices derived from Litmus pricing, which are compared to ideal prices}
% \vspace{-1em}
\label{fig:priceErrorRunwith26Rev}
\end{figure}

%%% We discuss error
% In figure~\ref{fig:priceErrorRunwith26} we can see that there are some applications receive positive errors and some receive negative errors.  A negative error indicates that our estimated slowdown for that application is higher than its actual slowdown, resulting in greater compensation than the observed performance losses. On the other hand, a positive error indicates that the compensation is smaller than its real slowdown. For most applications, the Litmus price is slightly higher than the Ideal price, with minimal differences. The highest price error is 0.0389 for auth-nj, while the lowest error is 0.007 for dyn-py. The geometric mean of the absolute error is 0.018. 
% Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors that each function experiences. The error rate is computed as the difference between the estimated and the ideal prices over the ideal price. The first two bars show the errors in \(P_{private}\) and \(P_{shared}\), which are weighted by their corresponding ratio in the execution time, considering their impacts, as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. The functions can have two different errors: positive and negative. A positive error indicates that the Litmus-estimated price is higher than its ideal price, implying that it receives smaller compensation than its performance losses. In other words, Litmus pricing estimates its slowdown to be less than its actual slowdown. A negative error implies the opposite; a function's compensation is higher than its slowdown. This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others. Meanwhile, the tenants need to acknowledge the consequences if their functions differ vastly from the reference workloads, heavily relying on shared memory.
Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors each function experiences. The error rate is computed by comparing the estimated prices with the ideal prices and dividing the difference by the ideal prices. The first two bars show errors in \(P_{private}\) and \(P_{shared}\), weighted by their corresponding ratios in execution time, reflecting their impacts as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. Functions may have two types of errors: positive and negative. A positive error means that the estimated price exceeds its ideal price, implying that the compensation received is less than the performance loss incurred. In other words, Litmus pricing underestimates the slowdown relative to the actual slowdown. Conversely, a negative error indicates the opposite; a function's compensation exceeds its slowdown. This discrepancy indicates Litmus pricing may offer varying advantages to different functions, favoring those with lesser slowdowns. Meanwhile, tenants must recognize the consequences if their functions differ vastly from the references, particularly those heavily reliant on shared resources.

% Delete the followings
% This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.

% The largest absolute error is \hl{0.0723} for rate-go, while the smallest absolute error is \hl{0.0039} for \hl{mst-py}. Overall, the Litmus pricing shows minor errors with an average of \hl{0.0231}. With further details, the Litmus pricing accurately estimates the slowdowns in \(P_{private}\) with \hl{0.0175} of an average weighted error rate. \(P_{private}\)'s highest weighted error rate is \hl{0.079}, yet minor, while the lowest rate is only \hl{0.0008}. The weighted error rate for the estimated \(P_{shared}\) is also small. The average error rate for \(P_{shared}\) is \hl{0.0068}, even lower than for \(P_{private}\). \(P_{shared}\)'s highest error rate is \hl{0.0404}.
% The largest absolute error is 0.072, which occurs with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, the Litmus pricing exhibits minor errors, averaging 0.023, \hl{with the estimated discount differing by 22.5\% over the ideal discount.} With more details, Litmus pricing accurately estimates slowdowns in \(P_{private}\), with an average weighted error rate of 0.018. \(P_{private}\)'s highest weighted error rate is 0.08, yet minor, while the lowest rate is only 0.0008. The weighted error rate for estimated \(P_{shared}\) is similarly small, averaging at 0.0068, even lower than for \(P_{private}\). The highest error rate for \(P_{shared}\) stands at 0.04.
The largest absolute error is 0.072, occurring with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, Litmus pricing exhibits minor errors, averaging 0.023. Thus, the estimated discount deviates by 22.5\% from the ideal discount. Note that Litmus pricing aims to match the average discount across all functions by applying a system-wide discount based on the system's congestion level rather than adjusting the discount for each function individually. Consequently, individual functions may experience either positive or negative errors. However, it is noteworthy that the average discount between Litmus and ideal pricing differs by just 0.4\%, as illustrated in Figure~\ref{fig:normalizedPrice26Rev}, satisfying its objectives.
% This policy may incentivize some functions while penalizing others based on shared resource usage. 
Specifically, Litmus pricing estimates slowdowns in \(P_{private}\) with an average weighted error rate of 0.018. The highest for \(P_{private}\) is 0.079, while the lowest is just 0.001. For \(P_{shared}\), the average weighted error rate is even lower, at 0.007. The highest for \(P_{shared}\) is 0.040.


% Litmus employs the average performance of applications to determine the discount rate applied universally. In this context, an application encounters a positive error when its speedup is less than the estimated average speedup across all applications. Also, the error rate depends on the difference between the actual speedup and the estimated average speedup, with larger differences resulting in more significant errors for the given application.
% As discussed in Figure~\ref{fig:TpriTshardDistri}, \(T_{private}\) dominates the execution time across all applications, implying that a small error in the estimated \(T_{private}\) largely influences the execution time. This explains why, for functions that demand little shared resources, such as float-py and chame-py, the error in P is almost identical to that in \(T_{private}\), and errors with \(T_{shared}\) can be overlooked. In contrast, for functions with a larger \(T_{shared}\) ratio, such as pager-py and mst-py, errors in \(T_{shared}\) meaningfully affect the total execution time. Note that the Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price.  

Litmus pricing estimates each pricing component separately with an individual discount rate. For functions that demand minimal shared resources, such as float-py, the errors in P are nearly identical to those in \(T_{private}\), and the errors in \(T_{shared}\) can be overlooked. As shown in Figure~\ref{fig:TpriTshardDistriRev}, \(T_{private}\) dominates the execution time across many applications. While even a small error in the estimated \(T_{private}\) influences the function's execution time, substantial errors in \(T_{shared}\) likely have limited impacts, except for functions that have a relatively meaningful \(T_{shared}\) ratio, such as pager-py and mst-py, whose errors in \(T_{shared}\) are observable in the total price. 

% We emphasize that Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price. We observe that functions have similar slowdowns in \(T_{private}\) with slight variation when congested. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, also estimating reliable total prices since \(T_{private}\) mostly dominates the execution time. The \(T_{shared}\) fluctuates more dynamically across functions with a relatively large error, but the error's impact is little, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}. 
We emphasize that Litmus pricing cannot avoid producing a certain degree of error since it relies on estimation using a few metrics. However, the figure proves that Litmus pricing effectively captures a congested environment and reflects that environment in the price. Under the same congestion level, \(T_{private}\) values of all functions are delayed similarly with a little variation. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, leading to reliable total price estimates since \(T_{private}\) generally dominates execution time. \(T_{shared}\) fluctuates more dynamically across functions and has a relatively larger error, but the impact of this error is minimal, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}.

\begin{figure}[h]
\centering
% \vspace{-5em}
 \includegraphics[width=1\columnwidth]{./fig/normTprivtTshared26Rev}\\
% \vspace{-5.5em}
\caption{\(T_{private}\) \& \(T_{shared}\) of applications when co-running with 26 others, normalized to those when they run alone. The top(black) and bottom(blue) lines are discount rates from Litmus pricing for \(T_{private}\) and \(T_{shared}\)}
% \vspace{-1em}
\label{fig:normTprivtTshared26Rev}
\end{figure}

% To further investigate the price error differences, in igure~\ref{fig:normTprivtTshared}, we explore the \(T_{private}\) speedups across various serverless applications.  
% Notably, the difference between the Litmus discount (L-Discount) and the average speedup is merely 0.006.  This minute difference explains why Litmus can attains such high accuracy. 
%Furthermore, when comparing with figure~\ref{fig:priceErrorRunwith26}, a correlation between the error rate and the speedup differences becomes apparent. 
%For instance, float-py, with the most substantial difference above the Litmus discount, also experiences the most significant negative error rate. 
%Conversely, aes-go, with the smallest speedup, experiences the highest positive error rate.
% % original version
% Figure~\ref{fig:normTprivtTshared} shows the execution time of the baseline normalized to the execution time of each run under congestion. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the functions spend only 3.67\% more time on private resources, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, resulting in precise estimation with a Litmus test. 

% Figure~\ref{fig:normTprivtTshared26Rev} shows the execution time of each function run under congestion normalized to the execution time of the baseline. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the interferences in private resources extend the function execution time only by 5.3\%, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, enabling precise estimation with a Litmus test.
Figure~\ref{fig:normTprivtTshared26Rev} shows the \(T_{private}\) and \(T_{shared}\) of each function, normalized to the same time components of the baseline. The gap between the bar and 1 represents the amount of slowdown that should be translated into ideal discounts. The top (black) and bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that interferences in private resources extend the function execution time by only 5.3\%, implying the performance of the private resources is marginally affected by congestion. Additionally, all functions exhibit similar \(T_{private}\) values with little dispersion, helping precise estimation with Litmus tests.

% Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors are still in an acceptable range since their impacts are small. Functions that have a considerable \(T_{shared}\) ratio become more sensitive to system congestion. Instead, a function, such as float-py, with negligible \(T_{shared}\) ratio gains huge benefits with high discounts while its performance remains firm. This shows that Litmus pricing reflects the dynamically changing values of shared resources when the congestion level alters and encourages functions to be developed to use more private resources. 
Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors remain within an acceptable range as their impacts are minor. Functions that have a considerable \(T_{shared}\) ratio are more sensitive to system congestion. Conversely, a function like float-py, which has a negligible \(T_{shared}\) ratio, gains huge benefits from high discounts while maintaining stable performance under congestion. This shows that Litmus pricing accurately reflects the dynamic values of shared resources when the congestion level changes and incentivizes functions to be developed to use less shared resources. 

% \textbf{Litmus pricing under high congestion:} We test our Litmus pricing under a heavily congested environment to verify its pricing of functions with large slowdowns. To create a crowded environment, we concurrently execute 60 instances of Fibonacci-go, which produces the most L2 misses among our tested functions. 
% We raise the congestion level significantly with 60 co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo} shows the results from the same tests of Figure 11. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.8\%, which is only a 1.7\% difference from the ideal discount of 27.1\% with 2.48\% of an average absolute error. In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.151 and 4.299, which are only 2.45\% and 7.83\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. 
% \textbf{Litmus pricing under high congestion:} We raise the congestion level significantly with \hl{500} co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo500} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.1\%, which is only a 1\% difference from the ideal discount of 27.1\% with 0.088\% of an average absolute error. Litmus pricing discounts slightly more than an actual slowdown, leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% % \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
% \caption{The normalized total price for the applications calculated by using Litmus pricing and ideal prices when co-running with 500 Fibonacci-go}
% \label{fig:normalizedPriceCongested320}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\columnwidth]{./fig/diffStartupPortion-2Rev}\\
%\caption{The slowdown of Python's startup with 25 and 15 million instructions (X-axis) and the slowdown of reference applications (Y-axis). From left, \(T_{private}\), \(T_{shared}\), and \(T_{total}\), normalized to those when running alone}
%\label{fig:diffStartupPortion}
%\end{figure}

% \textbf{Instructions in Startup:} Litmus tests react differently to congestion when performed with different numbers of instructions from the startup phase. For example, Python's startup involves about 45 million instructions. While we have conducted Litmus tests using all these instructions, Figure~\ref{fig:diffStartupPortion} shows the response of these tests when running with the first 15 and 25 million instructions from this set. The figure shows the startups' \(T_{private}\), \(T_{shared}\), and \(T_{total}\) with two traffic generators, as depicted in Figure~\ref{fig:referenceStartupSlowdownRev}. Tests with fewer instructions are more sensitive to cold cache misses but less to interference in the L3 cache. Therefore, as the instruction count in Litmus tests decreases, they become less susceptible to conflicts in shared resources, especially from traffic by MB-Gen. As a result, tests with 25 million instructions exhibit reduced slowdowns. This trend becomes more apparent when running the tests with 15 million instructions, depicting that slowdowns when co-running with MB-Gen become nearly identical to those with CT-Gen. 

%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%







% \textbf{Instructions in Startup:} Python's whole startup phase contains about 45 million instructions. We can further divide the startup phase into smaller pieces with 10 million instructions code chunks. And each code chunk would have its characteristics. They react differently in the same congested environment. In section XXX we use the whole Python's startup portion's slowdown to indexsing the serverless application's slowdown. But, since the co-relationship between these two slowdown in different congestion source are different, one startup \(T_{private}\) slowdown may indicate two application's slowdown. By carefully picking the code chunks we can mitigate the difference between the two normalized slowdowns of the guidance application that correlated to the same startup phase slowdown. 

% Figure~\ref{fig:diffStartupPortion} depicts the correlation between the performance changes in the reference applications and distinct segments of Python's startup phase. From the figure, we see that selecting the first 15 million instructions as our startup phase results in the normalized \(T_{uncore}PerInst\) of the guidance application aligning nearly into a singular trendline. However, there are substantial gaps in the case of \(T_{core}PerInst\) with this code segment. Thus, we should pick xxx-xxx as our startup phase representation code for the normalized \(T_{core}PerInst\). We think that this can be used to mitigate the differences. But, we should be careful to use the small code chunks for the following reasons: First, only measuring the small portion can be a problem. The results might be too dynamic. Second, since we only measure this small portion there might be a huge execution period that cannot be covered.

% Continue to work from here

\subsection{Temporal CPU Sharing}
\label{sec:temporalCPUSharing}

The previous evaluation assumes an isolated environment where a CPU is assigned exclusively to an active function during execution, disallowing temporal sharing between functions through context-switching. While this setup ensures strict performance isolation, it inherently limits resource utilization. Conversely, enhancing utilization by permitting temporal CPU sharing among functions complicates price estimation. We explore how Litmus pricing can be applied in a less restrictive environment that permits sharing, where functions can temporarily share the same CPU and are not bound exclusively to specific cores. 

In this section, we deploy a testing function to co-run with 160 other functions across 16 cores without exclusive core assignments, assuming an average of 10 functions share a core. The reduction in the number of cores tested was necessitated by our system's memory limitations, as certain functions require significant memory space.

% \textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, the subsequent function clears the displaced one's cached data. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, the slowdown with extra sharing financially benefits the provider; we thereby argue that the extent of sharing should be factored into Litmus pricing as another discount factor.
\textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, a subsequent function evicts the cached data of the displaced one. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, delayed execution due to extra sharing financially benefits the providers. Thus, we argue that the extent of temporal sharing should be incorporated into Litmus pricing as another discount factor.

Figure~\ref{fig:csImpactor} depicts the switching overheads as concurrently running functions increase. The figure demonstrates that the sharing overhead follows a logarithmic growth pattern and stabilizes at around 20 co-running functions. Furthermore, we discovered that the switching overheads predominantly affect \(T_{private}\). Consequently, Litmus pricing needs to calibrate \(T_{private}\) to account for the impacts of sharing before estimating the slowdown using the performance table.

Figure~\ref{fig:normalizedPrice160Method1} illustrates the discounted price reflecting this adjustment. In our configuration, with an average of 10 functions per core, we divide \(T_{private}\) by 1.025 before estimating the slowdown. In this figure, Litmus pricing estimates an average discount of 14.5\%, which falls 2.9\% short of the ideal discount of 17.4\%. While most benchmarks receive discounts lower than ideal, aes-py stands out with the largest error of 9.9\%, which is 6.9\% less than its ideal discount of 16.8\%.

\begin{figure}
\centering
% \includegraphics[width=1\columnwidth]{./fig/csImpactor}\\
\includegraphics[width=1\columnwidth]{./fig/csImpactor2}\\
\caption{\(T_{private}\) of functions over different co-running counts in the same core, normalized to when running alone}
% \vspace{-1em}
\label{fig:csImpactor}
\end{figure}

\begin{figure}
\centering
% \vspace{-1.2em}
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160Method1}\\
\caption{Prices derived from Litmus pricing (Method 1) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
% \vspace{-0.5em}
\label{fig:normalizedPrice160Method1}
\end{figure}

% In Figure~\ref{fig:normalizedPrice160Method1} we use the the same congestion and performance tables that we collected in the restricted environment. When checking the tables instead of using the original startup slowdown of tcore we use an adjusted slowdown by dividing the context switch impact factor. From figure~\ref{fig:normalizedPrice160Method1} we can see that the average Litums discount is 14.65\%, 3.01\% less than what they should receive compared to the ideal discount of 17.67\%. Most applications receive a smaller discount than the ideal price. The largest error is on aes-py with Litmus discount of 9.85\%, 6.87\% smaller than the ideal discount of 16.72\%. The smallest error is on dyn-py. It's Litmus discount is 22.45\%, only 0.47\% larger than the ideal discount of 21.97\%.

\textbf{Method 2, Updating Performance Tables:} Rather than reusing the performance/congestion tables designed for restrictive environments, arranging new tables for the sharing-enabled environments returns better accuracy. Although the notion of preparing separate tables for various sharing levels may seem challenging, we argue that only one or a few extra tables for heavily crowded systems would suffice, given that commercial systems are typically heavily crowded. Again, we emphasize that the impact of function co-placement stabilizes above a certain co-placement count, as shown in Figure~\ref{fig:csImpactor}.

For this test, we prepared new performance/congestion tables for the environment described above, where a testing function is assumed to co-locate and compete for a core with 9 other functions. Moreover, considering the scenario where a switched-out function has a low chance of being rescheduled to the same core, instead of assigning 10 functions to a specific core, we ran 50 functions across 5 dedicated cores; each can run on any of the 5 cores. We managed the congestion levels in shared resources using traffic generators on the other cores, as outlined in Section~\ref{sec:designDetails}.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPrice160}
% \vspace{-0.6em}
\end{figure}

% Figure~\ref{fig:normalizedPrice160} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{17.29\%}, which is only marginally smaller by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{17.67\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice160} shows the prices obtained from Litmus pricing with the new tables, which are normalized to those from commercial sources. Once more, as in Figure~\ref{fig:normalizedPrice26Rev}, the figure reveals marginal distinctions between the two price points, suggesting that Litmus pricing continues to offer a reasonable discount. Across all functions, the average discount provided by Litmus pricing stands at 17.2\%, merely 0.2\% less than the ideal discount of 17.4\%.


==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/09_sensitivity.tex <==
\section{Sensitivity}
\label{sec:sensitivity}

While the aforementioned tests highlight Litmus's potential, we recognize the need for more compelling results. This section expands our analysis and examines Litmus pricing from various angles across diverse system environments.

% \textbf{Heavy Congestions:} We raise the congestion level significantly with 320 co-running applications to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. The Litmus pricing is still close to the ideal price, discounting the price by 20.00\%, which is only a 1.46\% difference from the ideal discount of 21.46\%. The highest Litmus discount is 26.01\% for dyn-py. It has an error of 2.83\% compared with the ideal discount.
\textbf{Heavy Congestion:} We significantly escalate the congestion level to verify Litmus pricing under conditions of substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} presents the outcomes of the same tests depicted in Figure~\ref{fig:normalizedPrice160} but with 320 co-running functions. Not only did we increase the function count, but we also specifically selected 8 memory-intensive functions, aes-py, compre-py, thum-py, bfs-py, auth-py, fib-go, geo-go, and profile-go, that produce the most L2 cache misses among the tested functions to create heavy congestion in shared resources deliberately. Even under such intensified congestion, Litmus pricing produces results remarkably close to the ideal price, discounting the price by 20.0\%, which deviates by merely 1.5\% from the ideal discount of 21.5\%. The highest discount by Litmus pricing is 26.0\% for dyn-py, a minor error of 2.8\% compared to the ideal discount.


% leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 320 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPriceCongested320}
% \vspace{-1em}
\end{figure}

\textbf{CPU Frequency:} Modern CPUs feature dynamic CPU frequency adjustments, which are controlled via software or hardware. A hardware technique like Intel Turbo Technology autonomously adjusts the CPU frequency based on the CPU's power and thermal budgets, allowing the CPU to operate at higher frequencies when conditions permit and lower frequencies under heavy load. Prior tests assumed that the frequencies were fixed and strictly managed by service providers who had knowledge of when and to what extent frequency adjustments were necessary. Also, we evaluated Litmus pricing under the other scenarios where CPU frequencies were not fixed, providing more dynamic perspectives.

% Figure~\ref{fig:normalizedPrice160unset} illustrates the prices from the Litmus pricing and the ideal price, which are normalized to commercial prices. We tested it under the configuration in Section 7.2 with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, the Litmus pricing's discount is lowered from 17.16\% to 16.84\%, while the ideal discount rate is decreased from 17.42\% to 17.31\%. Still, the discount rate difference from the ideal price is only 0.47\% without setting the CPU frequency. We observed that the CPU frequency changes rarely when the system runs with 160 functions. Overall, the varying frequency made a minor impact on performance as well as the pricing scheme. 
Figure~\ref{fig:normalizedPrice160unset} illustrates the prices derived from Litmus pricing alongside the ideal prices, both normalized to commercial prices. This evaluation was conducted under the configuration outlined in Section~\ref{sec:temporalCPUSharing} with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, we observe a slight decrease in Litmus pricing's discount, from 17.2\% to 16.8\%, while the ideal discount rate decreases from 17.4\% to 17.3\%. Still, even without fixed CPU frequencies, the difference in the discount rate from the ideal price is only 0.5\%. We noted that CPU frequency changes were infrequent when the system operated with 160 functions. Overall, the variation in frequency had a negligible impact on Litmus pricing.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160unset}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others with unfixed CPU frequencies, both normalized to commercial prices}
\label{fig:normalizedPrice160unset}
% \vspace{-1em}
\end{figure}

% All the above experiments are done on Intel Xeon Gold 5218(Cascade Lake). We also perform our scheme on another CPU architecture, Intel Xeon Silver 4314(Ice Lake-SP). 
\textbf{CPU Architecture:} Ensuring the validity of Litmus pricing across different architectures is crucial. Our Litmus tests rely on the performance counter that measures a stall count due to L2 cache misses (cycle\_activity.stalls\_L2\_miss)~\cite{perfMonEvents}, supported by Intel's CPUs. Unfortunately, other vendors like AMD do not yet offer the same performance counter~\cite{amdPMC}, restricting our tests to Intel CPUs. Alternatively, we conducted tests on another Intel CPU based on the Ice Lake architecture, Xeon Silver 4314, to broaden the scope of our analysis.

\begin{figure}[b]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun70kiwi}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 70 others on Xeon Silver 4314, both normalized to commercial prices}
\label{fig:normalizedPriceCorun70kiwi}
\end{figure}

% Because of the limitation of our memory size, we test Limtmus with 70 co-running applications. In this test, we use method 2 introduced in section~\ref{sec:temporalCPUSharing}. We first conduct the congestion and performance tables with 50 applications running in the first 5 cores. Then for the evaluation, we run 70 applications in the first 7 cores to let our testing application compete with 9 other applications for a core.  Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus discounting the tenant only pays 82.52\% commercial price. It's 0.696\% less than with the ideal discount.
Once again, this evaluation was conducted following the configuration outlined in Section~\ref{sec:temporalCPUSharing}, albeit with 70 co-running functions, limited by the main memory capacity of 128GB. Following Method 2, we constructed new congestion and performance tables with 50 functions running across 5 cores. Then, we ran 70 functions across 7 cores to match the competition count, averaging 10 functions per core. Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus pricing, the tenant only pays 82.5\% of the commercial prices, which is merely 0.7\% less than the ideal price.

% \textbf{Per-core Function Count:} When altering the co-located applications in each core the performance of the application can also be influenced. In this test, we put 240 applications in the first 16 cores. The testing application is competing with 14 other applications. We used the same congestion and performance tables from section~\ref{sec:temporalCPUSharing} method 2. Figure~\ref{fig:normalizedPriceCorun15} presents the results. The error of Litmus pricing is 1.23\% with The average discount of 16.69\%. The ideal discount is 17.92\%. The mean price of Litmus is larger than the ideal price because we are using the tables that are made based on 10 applications per-core. The context-switching overhead is larger. But, from figure~\ref{fig:csImpactor} we know that there is a diminishing impact of per-core application count. The error of the Litmus pricing is still under control when we increase the per-core application count.
\textbf{CPU Sharing Overhead:} The co-located function count determines the level of interference, impacting a function's performance differently. To assess Litmus pricing under various co-running function counts, we increased the function count to 240 from the configuration outlined in Section~\ref{sec:temporalCPUSharing}, making an average of 15 functions running on each core. However, we reused the performance and congestion tables generated in Section~\ref{sec:temporalCPUSharing}. Figure~\ref{fig:normalizedPriceCorun15} illustrates the results, where the Litmus pricing's error is 1.2\% with an average discount of 16.7\%, compared to the ideal of 17.9\%. Despite reusing the tables constructed for 10 co-running functions per core, the error remains negligible. This outcome aligns with Figure~\ref{fig:csImpactor}, which highlights the diminishing impact of temporal sharing when running more than 10 co-running functions. Given the perpetual overcrowding of commercial systems, any configuration gap between the environment where constructing the tables and where conducting tests is expected to remain minor and easily manageable.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun15}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 15 functions per core and reusing tables, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun15}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun160smt}
\end{figure}

\textbf{Simultaneous Multithreading (SMT):} SMT is a technique aimed at maximizing resource utilization by enabling multiple threads to execute concurrently on the same core, extending the shared resource domain across the entire processor. However, while SMT enhances resource utilization, it significantly complicates the measurement of interference impact. Moreover, SMT introduces additional side channels, thereby increasing the processor's vulnerability to security attacks. Due to these concerns, serverless platforms like Amazon Lambda disable SMT in their systems~\cite{schall2023warming,agache2020firecracker,schall2022lukewarm}. Nonetheless, we have conducted a study to assess the impact of SMT on our Litmus pricing methodology.

% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
% \caption{Prices computed via Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, normalized to the commercial prices}
% \vspace{-0.5em}
% \label{fig:normalizedPriceCorun160smt}
% \end{figure}

% To generate the performance/congestion tables, we executed 50 applications across 5 dedicated physical cores. In this way, the testing function is co-located with 9 other applications in the same virtual core and 19 other applications in the same physical core. Fiugre~\ref{fig:normalizedPriceCorun160smt} illustrates the results. The first thing we notice is that the normalized price is much smaller compared with the setups without SMT turned on. The average discount of Litmus is 45.42\% which is 1.9\% smaller than the average ideal discount of 47.32\%.
To construct the performance and congestion tables, we executed 50 applications across 5 physically separated cores, allowing an average of 10 functions to share two virtual cores. Figure~\ref{fig:normalizedPriceCorun160smt} illustrates the results,  presenting prices derived from Litmus pricing and ideal prices, both normalized to commercial prices without discounts. The normalized price experiences a significant drop compared to other configurations, highlighting the impact of heavy congestion within a physical core. The ideal price, which assumes no interference, stands at 47.3\% of the commercial price. Meanwhile, Litmus pricing offers a discount of 45.4\%, which is only 1.9\% less, confirming the effectiveness of Litmus pricing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Node JS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Nodejs Startup:}NodeJs is another well-adopted language in serverless platforms besides Python. It's one of the earliest languages to be supported by AWS Lambda ~\cite{serverless1}. From Section~\ref{sec:designDetails} we see that NodeJs has a long startup phase which makes it a great candidate when we need to pick a language startup phase for the Litmus test. 

%\begin{figure}[h]
%\centering
%\vspace{-0.5em}
%\includegraphics[width=1\columnwidth]{./fig/njReferenceStartupSlowdown}\\
%\vspace{-1em}
%\caption{The correlation between the normalized NodeJs's startup phase and the normalized reference applications.}
%\vspace{-0.5em}
%\label{fig:njReferenceStartupSlowdown}
%\end{figure}

%Figure~\ref{fig:njReferenceStartupSlowdown} shows the correlation between NodeJs startup phases and reference applications. After applying the Litmus test with NodeJs applications, with this figure, we can use the slowdown of the NodeJs startup phase to find the corresponding system congestion level and the discount rate for both private and shared resources. NodeJs has a longer startup phase compared with Python. It gives us more room when picking the most suitable portions of the startup phase. We can choose the language to be used for the Litmus test based on the density of the startup phase. 


==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/10_related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Serverless:} Many works address the performance bottleneck of serverless execution~\cite{du2020catalyzer}~\cite{agarwal2021reinforcement}~\cite{roy2022icebreaker}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Schall et al.~\cite{schall2022lukewarm} record and reload the instructions to reduce the front-end stalls when reaccessing the same application. Jovan et al.~\cite{stojkovic2023specfaas} focus on the performance of an application chain. They break the execution flow and speculative execute the functions. However, we are focusing on the price which is one of the most important potions of the cloud ecosystem.

% For the cloud providers, accommodating more tenants in a machine is a key strategy, gaining higher profits by maximizing the utilization of their machines. However, the approach inevitably introduces interference between tenants, slowing down applications unpredictably. Thus, prior researchers solved this challenge by allowing the tenants more non-biased, predictable, quality services~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed a clustering-based cache partitioning to remove unfairness between tenants. Rohan et al.~\cite{roy2021satori} simultaneously control multiple architectural resources to aim for both fairness and throughput. However, offering fairness inevitably sacrifices resource utilization. Thus, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} solve the unfairness uniquely by adjusting their prices while leaving the unfairness at a certain degree. This paper follows this direction but explores a more practical solution in serverless computing. 

Cloud providers strive to maximize profits by accommodating more tenants on their machines, which inevitably introduces interference between tenants, leading to unpredictable application slowdowns. To address this challenge, prior researchers have focused on providing tenants with a more unbiased and predictable quality of service~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed clustering-based cache partitioning to mitigate unfairness between tenants. Rohan et al.~\cite{roy2021satori} aimed for both fairness and throughput by simultaneously controlling multiple architectural resources. However, achieving fairness comes at the cost of sacrificing resource utilization. In contrast, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} addressed the unfairness by adjusting their prices while accepting a certain degree of unfairness. Our study follows a similar direction but explores a more practical solution within the context of serverless computing.

% delete the following section: the approaches are against our scheme. 
% \textbf{Serverless Computing:} Many studies focus on reducing the latencies of serverless applications~\cite{cadden2020seuss,oakes2018sock,wang2019replayable,jia2021boki}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Ustiugov et al.~\cite{ustiugov2021benchmarking} record and prefetches the functions’ stable working set of guest memory pages to further reduce the function's startup time. Wei et al.~\cite{wei2023no} remote forking the serverless functions to reduce the cold start latency while limiting the resource usage. Schall et al. record and reload the instructions~\cite{schall2022lukewarm} or the BTB entries ~\cite{schall2023warming} to reduce the front-end stalls when reaccessing the same application. 
% \hl{Litmus is orthogonal to these approaches and can be adopted together.}

==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Serverless computing is a key technology in present cloud computing, offering numerous advantages. One primary advantage is its effective cost-saving, as tenants only pay for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion. While tenants suffer slowdowns, they also have to pay more for the slowdowns. Unlike prior approaches that aim to maintain quality of service, this paper discounts the tenant's cost to compensate for the loss. Litmus pricing proposed in this work monitors the machine states and adjusts the tenants' costs. The congestion level can be frequently gauged before every function using the proposed Litmus test, an effectively lightweight testing approach. Our tests show that Litmus offers near-ideal prices with a 0.38\% difference, compared to the ideal price that discounts proportional to its slowdown. 
Serverless computing is a key technology in contemporary cloud computing, offering a range of benefits. One primary advantage is effective cost-saving, as tenants are billed only for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion, which not only results in slowdowns but also higher costs for tenants. Rather than aiming to maintain service quality, this paper suggests discounting tenants' costs to compensate for performance losses. Litmus pricing proposed in this work monitors machine states through Litmus tests and adjusts tenant costs accordingly. The Litmus test is a lightweight testing approach for serverless platforms, which assesses the machine's congestion level before starting a user's function. Our tests prove that Litmus pricing offers nearly ideal prices in heavily congested environments, with an average deviation of just 0.2\% from the ideal price that adjusts discounts in proportion to the slowdown experienced.


==> 2024_ASPLOS_Litmus__Fair_Pricing_for_Serverless_Computing/12_ack.tex <==
\section{Acknowledgment}
\label{ack}

We would like to thank our reviewers for their valuable feedback to improve this paper. This work was supported by NSF CAREER Award CCF-2146475.


==> ASPLOS_2024_litmus/00_abstract.tex <==
\begin{abstract}

% Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While the providers can utilize their machines more efficiently, the tenants only need to pay for the resources they consume. However, a serverless system co-runs thousands of short-living functions concurrently to maximize resource utilization, bearing frequent state shifts. Meanwhile, when the system gets too congested, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants are also charged higher costs when experiencing slowdowns since all commercial serverless platforms determine the tenants' costs proportional to their execution times.
Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times.

% This paper argues that the cloud providers should compensate the tenants for their loss when the server is over-provisioned. However, estimating the tenant's loss is challenging when there is no pre-profiled information about the function. Prior studies showed assessing the tenant's loss introduces heavy overheads. Instead, this paper proposes a new pricing model, Litmus pricing, which offers discounts based on the machine's state while presuming the tenant's loss under the state. To monitor the machine state correctly, Litmus pricing frequently conducts Litmus tests, an effectively lightweight solution to measure system congestion. Our experiments show that Litmus pricing can detect the impact of system congestion and offer near-ideal prices, with only a 0.38\% price difference. 
This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2\% price difference on average, in a heavily congested system.

\end{abstract}


==> ASPLOS_2024_litmus/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Serverless computing is growing fast, satisfying today's high demands for better programmability. It allows tenants to develop their programs as stateless functions in high-level languages such as Python, Go, and JavaScript without concerns with low-level resource management and task scheduling~\cite{serverless2,serverless1,schall2022lukewarm,schall2023warming,mohammad2020SerInWild}. This advantage attracts cloud users, helping them to deploy their programs quickly with minimal effort. Recent reports note that over 50-70\% of cloud users have adopted serverless computing for their tasks~\cite{serverless1}.

% Serverless computing claims a pay-as-you-go pricing model where users only pay for the resources used by their functions. This requires the service provider to monitor and estimate the fine-grained resource usage by each user accurately. However, today's high-performance systems maximize resource efficiency by accommodating multiple applications simultaneously and allowing the resources to be shared by them. Such a shared system raises two major challenges. First, tracking a user's resource usage is a challenging task. While being shared, the system tracks the total usage but not a single user's. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress. These inferences between the applications not only make the system hard to track resource usage, but the users may get charged unfairly due to the delayed execution time.
Serverless computing also benefits tenants financially. Unlike traditional cloud platforms that require tenants to purchase the hardware resources needed to deploy their servers regardless of actual usage~\cite{amazonEC2Pricing}, serverless computing claims a pay-as-you-go pricing model, where tenants only pay for the resources consumed during the execution of their functions, facilitating significant cost savings. Meanwhile, this pricing requires service providers to accurately monitor and estimate each user's fine-grained resource usage~\cite{microsoftAzurePricing,awsLambdaPricing,googleCloudFunctionPricing}. 

% However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared system raises two major challenges. First, tracking a tenant's resource usage is a challenging task. While being shared, the system can only monitor a tenant's use of specific resources. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference between the applications not only makes the system hard to track resource usage, but the tenants may get charged unfairly due to the extended execution time~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}. 
However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared serverless system raises two major challenges. First, tracking a tenant's resource usage becomes challenging, as the system can only monitor a tenant's use of exclusively dedicated resources while the system is shared. Second, and more importantly, co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference not only complicates tracking resource usage but also leads to tenants being charged unfairly due to delayed execution times~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}.

% A serverless platform should provide an isolated runtime environment to a user. Otherwise, we argue that the platform provider must compensate a tenant's loss as a discount when it is not achievable. Therefore, we define a charged fee as fair when it reflects the tenant's slowdowns due to the resource sharing. The following two methods can be used to estimate a fair price under a multi-tenant environment. 
A serverless platform should provide a user with an isolated runtime environment. Otherwise, we argue that the platform provider should compensate a tenant's loss as a discount when the isolation is not achievable. Thus, we define a charged fee as fair when it reflects the tenant's slowdowns caused by resource sharing. The following two methods can be used to offer a fair price in a multi-tenant environment.

% First, strict resource partitioning can divide shared resources into multiple partitions, each assigned to a user exclusively. The user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strictly partitioned resources are well known to cancel the opportunities to utilize the given resource efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delayed execution directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources when requesting them. 
First, strict resource partitioning can divide shared resources into multiple partitions, each assigned exclusively to a user. This means the user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strict partitioning is known to cancel opportunities to utilize resources efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delay directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources they need when requested. 

% Alternatively, a discount-based scheme estimates a user's price relative to its slowdown, discounting from the price when run without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources. Thus, the providers can maximize their hardware utilization and earn more money with given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns or interference they get from co-running tasks without overpaying for exclusive resources.
% The tenants also can get a discount reasonably proportional to the amount of their slowdown when their jobs suffer from interference rather than endeavoring to secure necessary resources exclusively.
Alternatively, a discount-based scheme estimates a user's price relative to the slowdown experienced, discounting from the price when running the task without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources, enabling providers to maximize hardware utilization and generate more revenue with the given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns they experience due to co-running tasks, preventing them from overpaying for lowered service quality.

% While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Even if the platform can measure its execution time, computing the slowdown still requires knowing its baseline, which can be gained when executing it alone. The cloud platform could not pre-profile users' applications for reasons such as mandated privacy when processing confidential information. Even if the platform has such information, the function could operate differently when receiving different inputs. That is to say, online profiling is necessary, which unfortunately requires expensive runtime sampling, as proposed in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. All co-running tasks must be stalled when estimating a task's baseline performance. Massive short-living serverless functions make such a sampling-based solution even more impractical. Frequently sampling the baseline performance of thousands of co-running functions is unrealistic. This motivates a new practical solution that can be adopted in commercial platforms. 
While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Although the platform can measure its execution time, determining the slowdown requires knowing its baseline performance, which can be obtained when it runs without interference. However, such profiling is often prohibited due to security concerns, particularly when the function processes confidential information. Additionally, the function may behave differently, with varying inputs each time it runs. That is to say, online profiling is necessary. Unfortunately, this requires expensive runtime sampling, as presented in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. When assessing baseline performance, all co-running tasks must be stalled. Hundreds to thousands of concurrent short-lived functions make this approach indeed impractical, as frequently sampling the baseline performance of such numerous functions is unrealistic. Thus, a new, practical solution that can be adopted in serverless platforms is needed.

%In either approach, a tenant or a service provider bears the problem's complexity alone. Resource partitioning demands the tenant to know the needed resources while losing opportunities to utilize the resources better. Discounting demands a service provider to estimate the task's slowdown with heavy sampling overheads. Accordingly, both approaches complicate the problem while sacrificing the machine's efficiency. Instead, we claim this problem becomes simpler when both entities participate and carry a portion of the responsibilities. 

% Litmus addresses this challenge by imposing the responsibility on both entities. With Litmus, the serverless platform measures the system congestion that may delay a function's execution when every tenant's function starts. The service provider needs to determine a discount rate for a corresponding congestion state. Meanwhile, the tenant needs to know about a possible slowdown and a corresponding discount. 

% We highlight that both partitioning and sampling complicate the problem while sacrificing the machine's efficiency and can hardly be employed in serverless computing. The approaches in serverless must be lightweight and frequent to deal with the fast-changing environment with thousands of concurrent functions. This paper proposes Litmus pricing that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening the system performance. 
We highlight that both partitioning-based and sampling-based approaches complicate the problem, either sacrificing the machine's efficiency or appearing impractical for serverless computing. Approaches in serverless computing must be lightweight, frequent, and sensitive enough to deal with quickly changing environments with numerous concurrent functions. This paper proposes Litmus pricing, a method that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening system performance. 

% \hl{Measuring the server's congestion status is challenging work. Here, Litmus relies on our key observation that, although not limited, function implementation in serverless computing largely relies on high-level programming languages such as Python and GoLang, which require a relatively long startup. This startup overhead has been considered one of the major challenges in serverless computing. However, Litmus utilizes this startup to measure the system's congestion state. Our analysis of Python and GoLang observed that the activities during the startups are almost identical, with plenty of memory operations, regardless of the functions. Thus, we claim that the startup performance can be an index of the system state.}

% \hl{The Litmus test is based on our insight that the serverless functions perform broadly identical operations, with plenty of memory operations, during their long startups, preparing the runtime environment for the functions. Leveraging this observation, the platform can assess the system's congestion level, which hints at the tenant's discount amount. Additionally, Litmus pricing exploits our second insight that the performance of two resources, private and shared, are affected differently by the congestion. In particular, its impact on private resources is minor and predictable, while many functions significantly rely on them, spending most of their execution time with them. }

% During the execution of every function, Litmus pricing conducts a Litmus test, which measures the level of system congestion with no extra overhead using the function's startup process. The Litmus test is based on the observation that serverless functions perform largely identical operations during their startup time. Those operations usually prepare the runtime and include a large amount of memory access to shared hardware resources. In addition, Litmus pricing splits the hardware resources into "private" and "shared" and proposes charging different ratios on each. This further improves the accuracy of the discount calculation.
During each function's execution, Litmus pricing conducts a Litmus test, which measures the level of system congestion without adding extra overhead, using the function's startup process. Litmus test is based on the observation that serverless functions perform largely identical operations during their startup, typically involving significant memory accesses. Additionally, Litmus pricing splits the hardware resources into "private" and "shared" categories, proposing different charging ratios for each. This approach further enhances the accuracy of the discount calculation.

% In our experiments, the Litmus pricing estimates a tenant's price to be nearly ideal, with a \hl{0.38\%} difference from the ideal price, which discounts tenants proportional to their slowdowns.
% This study investigates Litmus pricing across different environments, ranging from restricted to crowded settings. We verify that crowded environments pose additional challenges. Despite this, Litmus pricing accurately estimates a tenant's price, deviating by only 0.26\% from the ideal price, discounting tenants proportional to their slowdowns.
This study investigates Litmus pricing across diverse environments with varying levels of system congestion. We confirm that crowded environments pose complex challenges. Despite this, Litmus pricing accurately estimates a tenant's cost, deviating by only 0.2\% on average from the ideal price that discounts tenants proportional to slowdowns.



==> ASPLOS_2024_litmus/02_background.tex <==
\section{Background}
\label{sec:background}

% \textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while the service providers handle back-end implementation~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers, which are later invoked upon associated events~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. The serverless platform guarantees security by executing the tenant's function in a sandbox such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.
\textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while leaving back-end implementation managed by service providers~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. These functions are later invoked upon associated events. The serverless platform ensures security by executing the tenant's function in a sandbox, such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.

% Each tenant's function is stateless and expected to be short~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using the short-lived functions, the tenant can easily scale by invoking many of the functions without provisioning needed resources for themselves, relying on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. Inherently, massive short-living serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. The tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and clients mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Later, under the pay-as-you-go pricing, the tenant is charged for the consumed resources, typically the product of time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
Each tenant's function is stateless and expected to be short-lived~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using these short-lived functions, tenants can easily scale by invoking many functions without provisioning the needed resources for themselves, relying instead on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. In serverless computing, numerous short-lived serverless workloads run together on a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. Tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and tenants mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% In the traditional cloud, tenants purchase hardware resources for the contracted term to support their applications, which are often expected to be large in a server form. Thus, tenants must pay for the agreed period regardless of actual use. Instead, serverless workloads are generally small and launched on-demand as short-living event handlers. This workload difference develops a unique pricing policy, pay-as-you-go pricing. The tenant is charged only for the consumed resources during the execution, typically the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
In traditional cloud computing, tenants purchase hardware resources for a contracted term to support their applications, which are typically large servers. Thus, tenants must pay for the agreed period regardless of actual usage. In contrast, serverless workloads are generally small and launched on-demand as short-lived event handlers. This difference leads to a unique pricing policy known as pay-as-you-go. Under this model, tenants are charged only for the resources consumed during execution, typically calculated as the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, where Python is utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Also, over 90\% of organizations choose Python and Node.js for their AWS services. Other popular language runtimes are Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer a high level of abstraction from machine codes with good programmability and portability, improving the programmer's productivity. As a result, they have been adopted widely by serverless users. However, such high-level languages typically rely on runtime interpretation, which results in a slow start of program execution with extra launching steps. For instance, in the case of Python, when an application is launched, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the codes are compiled and executed. Once the execution is complete, the Python program is terminated, and all assigned resources are released~\cite{pythonUsage}.
\textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python used in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Over 90\% of organizations choose Python and Node.js for their AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer significant abstraction from machine code with good programmability and portability, which in turn improves programmer productivity. Consequently, they are widely adopted by serverless users. However, high-level languages typically rely on runtime interpretation, leading to slower program startup due to extra launching steps. For example, when an application is launched in Python, the interpreter is first prepared. It then parses command-line arguments and imports necessary modules. Afterward, the codes are compiled and executed. Upon completion, the Python program terminates, and all allocated resources are released~\cite{pythonUsage}.

 
% list of pricing models? 
% Amazon? 
% Google?
% The price is calculated by duration time multiplies to the unit price plus the request charges. The duration time is from the time user's code begins executing until it returns or terminates. The unit price depends on the amount of memory the user allocate to their function. The request charges is based on how many times the function has been invoked minus the free requests~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% may need service agreement here, contention impact

%\textbf{Traditional cloud platforms:} In the context of traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage, data transfer, etc. The instance type is the combination of Virtual CPUs(VCPUs), RAM, storage and network performances. The time unit price will be higher with more powerful instance type. Typically, more powerful instance types have higher time unit prices. There are two main pricing options: On-Demand and Reserved Instances. On-demand instance let the customers pay for compute capacity by the hour or second based on the actual usage with no long-term commitments. Reserved Instances, on the other hand, require a commitment to a specific instance type for a contract term and offer cost savings compared to On-Demand pricing. Storage and data transfer for the VM instance can also impact the pricing. The more storage space a customer uses or the more data they transfer, the higher their costs will be. The traditional cloud platform can also be affected by the co-running applications~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} In traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage space, data bandwidth, etc. The instance type includes virtual CPUs, RAM, storage, and network performances. Typically, more powerful instance types charge higher prices. Also, two pricing options are commonly offered: on-demand and reserved instances. On-demand instances allow tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved instances require a commitment to a specific instance type for an agreed term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period. Storage space and data bandwidth for the VM instance also influence the price. Demanding more storage space or more data transfer raises the cost~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} 

% The price of traditional cloud platforms is determined by computing capabilities such as processor type, memory capacity, and network bandwidth. While more and better resources typically charge higher prices, two pricing options are commonly offered: on-demand and reserved instances. On-demand pricing allows tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved pricing requires a commitment to specific resources for an agreed-upon term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period~\cite{amazonEC2Pricing}. 

% There are several differences between traditional cloud platforms and serverless platform. 
% Firstly, the roles of customers in the execution environment differ between traditional and serverless platforms. In the traditional cloud, customers are responsible for configuring and maintaining virtual machines (VMs), setting up networking, and managing databases~\cite{amazonEC2Pricing}. And it's the customers's responsibility to detact and update the configurations to balance their expenses and performance. On the other hand, in serverless platforms, users only provide a single file to indicate their system and library requirement, while the service provider handles the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. This feature enables users to focus solely on their actual workload without the burden of managing the infrastructures. Additionally, the platform can automatically scale the resources for the users based on the current demand of the application to guarantee the customer satisfaction~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% There are apparent differences between traditional and serverless cloud platforms. First, tenants are responsible for managing hardware resources in traditional platforms. The tenants need to configure and maintain virtual machines, set up networking, and manage databases~\cite{amazonEC2Pricing}. Also, tenants should study the optimal configurations to balance their expenses and performance. Meanwhile, in serverless platforms, tenants only provide a single file to specify their system requirements while the cloud provider prepares the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. The platform provisions or scales the needed resources on demand. Consequently, the serverless platforms encourage tenants to focus solely on their front-end workloads without the burden of managing the low-level back-ends~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% Secondly, there are notable differences in compute power and memory size options between the two platforms. For traditional cloud, the granularity usually 1 VCPU and 1GB memory. But, for serverless platform, the smallest memory size is 128 MB~\cite{awsLambdaApiGateWay,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Thirdly, the characteristics of workloads on these platforms set them apart. Serverless applications are generally small and executed on-demand, resulting in very short workload durations~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can complete in less than one second. In contrast, traditional cloud applications tend to be larger and may require hours to complete. Additionally, the number of co-located applications on a single computing node is smaller in traditional cloud setups, making their execution environment less dynamic compared to serverless platforms.
% Lastly, the billing periods differ significantly between traditional cloud and serverless platforms. Traditional cloud users are charged for the allocated time period. Regardless of whether they are actively running tasks on the machine, they are still need to pay for the allocated time period. However, serverless customers are only billed for the actual execution time of their tasks on the platform.

% Second, the workloads are expected to be small in serverless computing. Serverless workloads are generally small and launched on-demand as short-living event handlers~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can be completed in less than one second, unlike traditional cloud applications that are often expected to be large in a server form. Inherently, massive serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. This workload difference develops a unique pricing policy in serverless computing, pay-as-you-go pricing. In the traditional cloud, the tenants purchase hardware resources for the contracted term. Regardless of actual use, they need to pay for the agreed period. However, the serverless platforms bill their tenants for the actual execution time of their tasks.


% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python being utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Furthermore, over 90\% of organizations leverage Python and Node.js alongside AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer numerous advantages for programmers, such as user-friendliness, portability, reduced error risks, and thriving ecosystems. As a result, they have garnered widespread acceptance within serverless platforms. High-level programming languages typically follow a fixed execution procedure. For instance, in Python, when an application is executed, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the code is compiled and executed. Once the execution is complete, the Python program is terminated, and all resources used by the program are released. Due to the consistency of the operating system and Python version, the beginning of the execution process remains the same each time~\cite{pythonUsage}.



% \textbf{Resource based discount vs. Slowdown based discount:} To fully utilize the available resources, service providers often run as many applications as they can in one computing node within the service agreement requirement. However, this may lead to resource congestion and cause slowdowns for users, which can be unfair, since the customers are paying more money for the worse experiences. The intuitionistic solution could be for the service provider to track the resource usage of each application and offer discounts to users who consume fewer resources. However, serverless applications are typically very small, and contention can affect different applications differently, making this approach less practical. A more suitable solution for serverless platforms could involve offering slowdown-based discounts. In this approach, the service provider dynamically updates unit prices based on the level of system congestion. When there is less contention, users normally stiffed with the experiences and pay the regular price. However, during periods of high congestion, when the system is under heavy load, users could receive discounted prices as compensation for potential slowdowns. This approach would align pricing with the actual performance experienced by users, ensuring a fair and responsive pricing model.


==> ASPLOS_2024_litmus/03_methodology.tex <==
\section{Methodology}
\label{sec:method}

% \textbf{Hardware Infrastructure:} All the experiments are performed on a dual-socket server platform. Each socket has 16 simultaneous multithreading(SMT) cores. The CPU model is Intel Xeon Gold 5218(Cascade Lake). The maximum frequency of the machine is 3.9GHz. Each core has a 32KB L1 instruction cache, a 32KB L1 data cache and a 1MB L2 cache. The 32 virtual cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The computer node runs the latest Ubuntu server version(Ubuntu 22.04 LTS) with kernel version 5.15.0. For consistency in the results, the core frequency was set to 3.0GHz using the 'cpupower frequency-set' command. We use linux perf~\cite{perfWiki} to collect the performance counters for each experiment. To analyze the startup status, we use -I 1 option to obtain count deltas at one-millisecond intervals. By utilizing interpolation, we can know the performance counters of each execution period. 

% In this study, we test today's server systems with serverless functions. This section describes our test configuration. 
This section outlines our test setup for evaluating serverless functions in this study.

% % original version
% \textbf{Hardware Infrastructure:} All experiments are performed on a dual-socket server platform with two Intel Xeon Gold 5218 (Cascade Lake). The CPU offers 16 simultaneous multithreading (SMT) cores with 3.9 GHz maximum frequency. We pin the core frequency at 3.0GHz for our tests. Each core has 32KB L1 instruction/data caches and 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The machine runs the Ubuntu server OS (Ubuntu 22.04 LTS) with a kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to collect the performance counters, which are collected at every one-millisecond interval. 
\textbf{Hardware Infrastructure:} All experiments are conducted on a dual-socket server platform equipped with two Intel Xeon Gold 5218 processors based on the Cascade Lake architecture. Each CPU provides 16 cores that support simultaneous multithreading (SMT) with a maximum frequency of 3.9 GHz. Every core features 32KB of L1 instruction/data caches and a 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets collectively have access to 384GB of main memory. The server operates on Ubuntu Server OS, version 22.04 LTS, with kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to gather performance counters.

% The CPU frequency is a key performance/energy factor, significantly affecting a function's execution time and energy consumption. A CPU's frequency can be altered in software or hardware based on its power and thermal budget, configuring it for better energy efficiency or performance. However, varying frequencies cause the system performance/energy to be unsettled, making system management intractable. For this reason, commercial systems such as Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. In our tests, when the frequency is not fixed by software, Intel's Turbo technology alters the frequency occasionally but mainly employs 2.8GHz. We will discuss this further in the sensitivity section.
The CPU frequency is a critical factor influencing both performance and energy consumption, significantly affecting a function's execution time and energy usage. A CPU's frequency can be adjusted through software or hardware based on power and thermal budget, optimizing for either energy efficiency or performance. However, varying frequencies can cause instability in system performance and energy usage, complicating system management. For this reason, commercial systems like Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. If we do not fix the frequency through software, Intel's Turbo technology occasionally adjusts it, but it mostly remains at 2.8 GHz during our tests. We will provide more details on this in Section~\ref{sec:sensitivity}.

% \textbf{Stressing Programs:} We used two stressing programs to investigate how applications and the startup portion of the high level languages behave in a resource contention environment. FigureXXX illustrates the number of instructions, L3 accesses, and L3 misses that the stressing programs can generate in five seconds as the stressing levels increase. By combining different stress levels of these stress-testing programs, we can simulate various resource-congested environments. The XXX-stressor(lineXXX)  generates more L3 accesses with a high L3 hit rate. While XXX-stressor(lineXXX), in each stressing level, generates fewer L3 accesses but more L3 misses. With these two stressors and different stressing levels, we can simulate the system with varying contentions to the shared resources by creating various  L3 accesses and L3 misses. In figureXXX we can see that the L3 accesses generated from the L2-stressor (update name later) begin to decrease after reaching stressing level 20.  However, during this period, the L3 misses continue to increase. The reason behind this trend is that, after stressing level 20, the heightened L3 miss rate starts to impact the stressor's performance, leading to a decline in the committed instruction count. Consequently, the stressor generates fewer L3 accesses and more L3 misses. 

% \begin{table}[h]
%     \begin{center}
%     % \vspace{-1.0em}
%         \caption{Serverless Benchmarks \& Runtimes}
%         \label{tb:benchmarks}
%         % \vspace{-1.0em}
%         \begin{tabular}{|l l||l l|} \hline
%             Function & Abbr. & Function & Abbr. \\ \hline \hline
%             \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  & \multicolumn{2}{c|}{\textbf{Hotel Reservation~\cite{gan2019open}}} \\ \hline
%             Dyn HTML & dyn-py & Geo & geo-go* \\ \hline
%             Thumbnail & thum-py* & Profile & profile-go \\ \hline
%             Compression & compre-py & Rate & rate-go \\ \hline
%             Image Recogn & recogn-py* & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
%             Graph Rank & pager-py & Currency & cur-nj* \\ \hline
%             Graph Mst & mst-py & Payment & pay-nj \\ \hline
%             Graph Bfs & bfs-py* & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
%             DNA Visual & visual-py* & Authen & auth-py/nj/go \\ \hline
%             \multicolumn{2}{|c||}{\textbf{Function Bench~\cite{kim2019functionbench}}} & Fibonacci & fib-py/nj/go* \\ \hline
%             Chameleon & chame-py & AES & aes-py/nj/go \\ \hline
%             FloatOp & float-py* & & \\ \hline
%             % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
%         \end{tabular}
%     \end{center}
%     % \vspace{-1.5em}
% \end{table}

\begin{table}[h]
    \begin{center}
    % \vspace{-1.0em}
        \caption{Serverless Benchmarks \& Language Runtimes (py, nj, go)}
        \label{tb:benchmarks}
        % \vspace{-1.0em}
        \begin{tabular}{|l l||l l|} \hline
            Function & Abbr. & Function & Abbr. \\ \hline \hline
            \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  &  \multicolumn{2}{|c|}{\textbf{Function Bench~\cite{kim2019functionbench}}}\\ \hline
            Dyn HTML & dyn-py & Chameleon & chame-py \\ \hline
            Thumbnail & thum-py* & FloatOp & float-py \\ \hline
            Compression & compre-py & Gzip & gzip-py* \\ \hline
            Image Recogn & recogn-py & RandDisk & randDisk-py* \\ \hline
            Graph Rank & pager-py & SequenDisk & seqDisk-py \\ \hline
            Graph Mst & mst-py & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
            Graph Bfs & bfs-py* & Currency & cur-nj* \\ \hline
            DNA Visual & visual-py* & Payment & pay-nj \\ \hline
            \multicolumn{2}{|c||}{\textbf{Hotel Reservation~\cite{gan2019open}}} & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
            Geo & geo-go & Authen & auth-py*/nj/go \\ \hline
            Profile & profile-go* & Fibonacci & fib-py*/nj*/go* \\ \hline
            Rate & rate-go & AES & aes-py/nj*/go* \\ \hline
            % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
        \end{tabular}
    \end{center}
    % \vspace{-1.5em}
\end{table}

% revision version
% \textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we select 27 distinct serverless functions from different benchmark suites, including AWS' authentication serverless functions~\cite{awsLambdaApiGateWay}, Hotel Reservation from the DeathStarBench suite~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and SeBS serverless benchmark suite~\cite{copik2021sebs}. The three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating 3 separate test cases per function. Among them, we pick 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. The functions are implemented using three languages: Python, Nodejs, and Go. We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. 
\textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we selected 27 distinct serverless functions from various benchmark suites, including AWS authentication serverless functions~\cite{awsLambdaApiGateWay}, the Hotel Reservation from DeathStarBench~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and the SeBS serverless benchmark suite~\cite{copik2021sebs}. The functions are implemented using three languages: Python, Nodejs, and Go. Notably, the three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating three separate test cases per function. 
% This comprehensive language support ensures that our test coverage is thorough and representative of the diverse language preferences in the serverless computing community. 
We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. Additionally, we selected 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. 


%\hl{The benchmarks we choose include I/O-bound, memory-bound, and compute-bound functions. For an experiment, we put the testing function in core 0 to core 4. We also put 50 other functions in core 0-4 to let the application co-running with 10 other applications to observe the impact of context switching.}

% \hl{We select benchmarks with mixed performance characteristics: I/O, memory, and compute-bound. Also, to replicate the congested commercial systems, we located a testing function with 50 other functions and tied them to selected 5 cores, Core 0 to 4. During our evaluation, those functions run simultaneously and compete to secure any core among the five.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
\caption{(a) L2 misses and (b) L3 misses of traffic generators, both normalized with the average L2 and L3 misses of serverless applications listed in Table~\ref{tb:benchmarks}}
% \vspace{-0.5em}
\label{fig:stressing_specs}
\end{figure}

% \textbf{Traffic Generator:} We divide the CPU's shared resources into two distinct categories: resources before and after the L3 caches. To pressure each resource group individually, we developed two separate traffic generators aimed at generating traffic and congestion in these resources. The first traffic generator, CT-Gen, applies pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another traffic generator, MB-Gen, induces massive L3 misses that stress the resources after the L3 cache, mainly the off-chip memory bandwidth and L3 cache spaces.
\textbf{Traffic Generator:} We categorize the CPU's shared resources into two groups: those before the L3 caches and those after. To stress each group independently, we developed two separate traffic generators designed to generate traffic and congestion within these resources. The first generator, CT-Gen, exerts pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another generator, MB-Gen, induces massive L3 misses, which stress the resources beyond the L3 cache, primarily targeting off-chip memory bandwidth and L3 cache spaces.

% Both traffic generators are multi-threaded, governing the volume of traffic by adjusting the number of threads they spawn. Each thread spawned by the traffic generator is pinned on each core to prevent conflicts between threads; consequently, this setup allows us to vary the stress level across our 32-core processors, ranging from level 1 to 31. Figure~\ref{fig:stressing_specs} shows each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), for every thread count increment, CT-Gen makes massive L2 misses. The CT-Gen's L2 misses are ended with L3 hits, as shown in Figure~\ref{fig:stressing_specs}(b). Meanwhile, MB-Gen creates huge L2 and L3 misses, as implemented. Interestingly, its L2 misses are fewer than CT-Gen's because MB-Gen is slowed by its L3 misses, suffering from a self-created bandwidth bottleneck. 
Both traffic generators are multi-threaded and govern the amount of traffic by adjusting the number of threads they spawn. Each thread is pinned to a specific core to avoid conflicts between threads, allowing us to vary the stress level on our 32-core processors from level 1 to 31. Figure~\ref{fig:stressing_specs} illustrates each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), with each increase in thread count, CT-Gen generates substantial L2 cache misses. These L2 misses by CT-Gen are ended with L3 cache hits, as shown in Figure~\ref{fig:stressing_specs}(b). In contrast, MB-Gen produces significant L2 and L3 cache misses. Interestingly, MB-Gen's L2 misses are fewer than those of CT-Gen because MB-Gen is hindered by its L3 misses, suffering from a self-imposed performance bottleneck.



==> ASPLOS_2024_litmus/04_motivation.tex <==
\section{The Need for Fair Pricing}
\label{sec:motivation}

% Offering fairness appears in different approaches in cloud computing when multiple tenants share hardware resources. One standard is SLA, which defines the level of services the cloud provider furnishes while a tenant sets their expectation. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving unfairness between tenants. Although serverless computing highlights the pay-as-you-go pricing model, such unfairness still exists.
Fairness in cloud computing, especially when multiple tenants share hardware resources, is addressed through various approaches. One standard method is the Service Level Agreement (SLA), which specifies the level of service the cloud provider must deliver and the tenants' expectations. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving fairness issues. Despite serverless computing's emphasis on a pay-as-you-go pricing model, unfairness among tenants still exists.

% Unfortunately, modern systems are designed to maximize hardware efficiency by co-running multiple applications; the function's execution time can be affected by co-scheduled applications with conflicts when using shared resources. Ironically, whenever the service provider squeezes their resources further for better profit by accommodating more functions into a single machine, each function's execution time increases, charging them a higher cost for the same workload. However, in serverless computing, tenants lack control and insights into how their software is executed and billed for the cost of convenience. 
Unfortunately, modern systems are designed to maximize hardware efficiency by running multiple applications concurrently. This results in conflicts over shared resources, affecting each function's execution time. Ironically, when service providers optimize for profit by packing more functions into a single machine, the execution time for each function increases, resulting in higher costs for the same workload. In serverless computing, tenants have no control or visibility over how their software is executed, leading to potential inefficiencies and higher costs for the sake of convenience.

% Genuine pay-as-you-go pricing can be achieved when there is no interference. However, that is not desired by the providers who expect to utilize their resources to maximize profits. In serverless, although each function runs virtually exclusively in a sandbox with private resources, it still shares a few resources with other co-running functions, such as shared caches and memory bandwidth. Resource partitioning, a traditional solution that eliminates interference, can promise exclusively dedicated resources to a tenant but cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 
In serverless computing, although each function runs exclusively in a virtual sandbox with private resources, it still shares certain resources like caches and memory bandwidth with other functions. Resource partitioning, a traditional solution that eliminates interference by dedicating resources exclusively to a tenant, cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 

\begin{figure}[h]
\centering
% \vspace{-0.7 em}
\includegraphics[width=1\columnwidth]{./fig/normalizedCPIRunWith26Rev}\\
% \vspace{-1 em}
\caption{Execution time of applications that run with 26 others, normalized to the execution time when running alone}
% \vspace{-0.4 em}
\label{fig:normalizedCPIRunWith26Rev}
\end{figure}

% Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed down when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. \hl{Whenever a function finishes, another function is randomly launched to maintain a total of 26 co-running functions.} The figure shows a function's performance drops by up to 35\%, and most functions are significantly influenced by the co-running functions. Compared to when an isolated environment is offered, the function performs 11.5\% slower on average, charging 11.5\% more to users. We highlight that the function runs only with 26 other functions, which is tiny compared to massively crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.
Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. Whenever a function finishes, a new randomly-selected function is launched to maintain a total of 26 co-running functions. The figure shows a function's performance can drop by up to 35\%, with most functions significantly impacted by the co-running functions. On average, functions perform 11.5\% slower in this shared environment compared to an isolated one, resulting in users being charged 11.5\% more. We highlight that this scenario involves only 26 co-running functions, which is tiny compared to heavily crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.

% Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} attempted to offer price discounts if it has a slowdown, compensating for the slowdowns. To provide the discount, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount reflecting the slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all the responsibilities of the contentions between co-running functions, guaranteeing all tenants an invariant price for their use. Any unexpected slowdowns that a tenant experiences are returned with a discount. However, sampling is an expensive operation, requiring all co-running processes to stall during the sampling. Moreover, accurate measurement requires frequent sampling when its system environment quickly alters, making the approach impossible in a fast-shifting environment like a serverless platform.   
Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} offers price discounts to compensate for slowdowns. To provide these discounts, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount based on the observed slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all responsibilities related to contentions from resource sharing, ensuring tenants pay a consistent price for their usage. Any unexpected slowdowns that a tenant experiences are compensated with a discount. However, sampling is an expensive operation that requires stalling all co-running processes during the sampling. Moreover, accurate measurement necessitates frequent sampling, especially in rapidly changing environments, making the approach impractical for dynamic environments like serverless platforms.


% A tenant needs a new pricing model based on more than just execution time. However, prior approaches have limitations, burdening cloud participants too heavily; it is unsuitable for \hl{thousands} of concurrent short-lived functions in serverless computing. This motivates us to propose a new solution, Litmus pricing, that discounts prices based on the system state but offers lightweight with no overheads.
Overall, tenants need a new pricing model that considers more than just execution time. Prior approaches have limitations, excessively burdening cloud participants and being unsuitable for the many short-lived functions typical in serverless computing. This motivates us to propose a new solution: Litmus pricing, which discounts prices based on the system congestion while remaining lightweight and imposing no additional overhead.


==> ASPLOS_2024_litmus/05_design.tex <==
\section{Litmus Pricing}
\subsection{Overview}

% The estimated prices of serverless functions should reflect the congestion level of the system inside their machines. With the massive short-living functions, the serverless system's state can dramatically change in a short time. Accordingly, the system state can be congested at any moment and also resolved in a short time. However, such a temporary traffic jam may significantly impact the performance of short-living functions. Therefore, assessing the congestion must be lightweight, quick, and on time. However, a prior approach, POPPA\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling with considerable performance overheads, preventing them from wide adoption. Instead, we propose a new scheme, Litmus pricing, that quickly estimates system congestion at the start of every function and reflects the estimation into pricing the function. 
The estimated prices of serverless functions should reflect the system's congestion state. The presence of numerous small transient functions within the serverless system can rapidly alter its congestion state, causing sudden congestion or swift resolution. Nevertheless, such transient traffic jams can significantly impact the performance of short-lived functions. Thus, assessing the congestion must be lightweight, quick, and timely. However, a prior approach, POPPA~\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling, which incurs considerable performance costs, thereby limiting its widespread adoption. Alternatively, this study introduces Litmus pricing, which promptly gauges system congestion at the onset of each function and reflects the estimated congestion level into pricing the function.

% Like the prior approach~\cite{tiwari2013enabling,alex2013ScFairPrice}, Litmus pricing suggests that the service provider discounts when a tenant's functions are intervened, compensating for the performance loss. To determine the discount ratio, Litmus measures system congestion level, which can also help service providers evaluate remaining resources and make decisions on job scheduling. 
Like the prior approach, Litmus pricing suggests that service providers should offer discounts when a tenant's functions experience interference, thus compensating for the performance loss. Litmus pricing determines the discount rate based on the system's congestion level. Evaluating congestion also assists providers in estimating remaining resources and making informed decisions regarding job scheduling.

%Nevertheless, the Litmus pricing does not quantify each function's slowdown; the discount amount is determined only by the severity of the measured congestion. The impact of the congestion on distinct functions appears differently despite facing the same congestion level, and precisely estimating a function's performance loss is a complex problem. That's why the prior approach had to rely on expensive sampling. Instead, the Litmus pricing avoids the overheads and limits the service provider's responsibility to measure the current congestion. 
However, Litmus pricing does not quantify the slowdown of each individual function; the discount amount is solely determined by the severity of the measured congestion. Even though different functions face the same congestion level, their respective impacts can vary, making precise estimation of each function's performance loss a challenging task. This complexity necessitated the expensive sampling relied upon by the previous approach. Instead, Litmus pricing circumvents such overheads and lightens the service provider's burden solely to measure ongoing congestion levels.

% Litmus pricing embodies the varying value of shared resources across different system conditions by applying equal discounts to all functions under the same system condition, although the functions experience different slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that a function that is slowed more than others demands the over-crowded resources more while exacerbating the adverse over-crowded conditions. Litmus pricing does not provide additional compensation for their extra loss compared to others due to their heavy use of shared resources.
Litmus pricing captures the dynamic significance of shared resources under varying system conditions by offering uniform discounts to all functions under the same system congestion, regardless of their individual slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that functions experiencing larger slowdowns tend to demand more of the crowded resources, thereby exacerbating adverse overcrowded conditions. However, Litmus pricing does not offer additional compensation for the larger loss experienced by functions that use shared resources more heavily than others.

% As a result, Litmus inherently incentivizes users who use shared resources sparingly. When over-crowded, functions with minimal needs for shared resources still enjoy discounts but encounter slight slowdowns. This implies that users may take advantage of this policy by minimizing their use of shared resources, receiving substantial discounts despite enduring only minor slowdowns. Such a trade-off is considered acceptable because the user's shared resource usage reduces their contribution to congestion, thereby benefiting the overall system over the other users.
As a result, Litmus inherently incentivizes users who use shared resources sparingly. During periods of overcrowding, functions with minimal needs for shared resources still enjoy discounts but with only slight slowdowns. This implies that users may take advantage of this policy by minimizing their reliance on shared resources, receiving substantial discounts despite only experiencing minor slowdowns. This trade-off is considered acceptable because reduced shared resource usage by users helps mitigate congestion, thereby benefiting the overall system and other users.
% Lastly, the system refrains from scheduling a function if the congestion level exceeds a predetermined threshold, thus preventing resource thrashing.


\subsection{Pricing Model}
\label{pricing model}

% Developing Litmus pricing raises two challenges. First, Litmus needs a new pricing model to estimate a function's price. Second, Litmus needs a way to measure the system's congestion state. Due to the serverless's fast-shifting environment, assessing the congestion must be lightweight and frequent at the right time. Nevertheless, all present commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants must pay more with prolonged execution time when using over-crowded resources. Rather than simply imposing a price by multiplying the main memory usage and a function's total execution time, Litmus suggests the price as a sum of two distinct price components as follows.
Developing Litmus pricing raises two challenges. First, it needs a new model to estimate a function's price. Second, it needs a way to measure the system's congestion state. Due to the rapidly changing environment in serverless computing, assessing congestion must be lightweight and timely. Commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants end up paying more for prolonged execution time when using over-crowded resources. Rather than simply imposing the price by multiplying the main memory usage and a function's execution time, Litmus pricing determines the price as a sum of two distinct pricing components as follows.

\begin{equation} 
P = P_{private} + P_{shared}
\end{equation}

% In this equation, \(P\) denotes the total price tenants need to pay to execute their functions. Litmus pricing divides the tenant's price into two pricing components, each with a different resource type. \(P_{private}\) represents the price the tenant needs to pay for private resources, which are entirely assigned to a tenant. \(P_{shared}\) is the price the tenant needs to pay for the shared resources. Each price component is measured proportional to a user's time to occupy the corresponding resources. However, such occupied time can be extended when contention disturbs a process's execution in the shared resources. This delayed time increases a tenant's price unfairly. 
In this equation, \(P\) denotes the total price tenants must pay to execute their functions. Litmus pricing divides this cost into two pricing components, each associated with a different resource type. \(P_{private}\) is the cost for private resources, which are entirely assigned to a single tenant. \(P_{shared}\) is the cost for shared resources. Each pricing component is measured proportional to the time users occupy the respective resources. However, if contention disturbs a process's execution in the shared resources, the occupied time will be extended. This delay unfairly increases the tenant's cost. 


\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/slowdownRunwith26Rev}\\
\caption{\(T_{private}\) and \(T_{shared}\) of applications that run with 26 others, normalized to those when running alone}
\vspace{-0.5em}
\label{fig:slowdownRunwith26Rev}
\end{figure}

% Using Perf, we measure the delays due to the shared resources and split a function's execution time into two distinct slices: one slice, \(T_{private}\), which is time spent on private resources and another slice, \(T_{shared}\), which is time spent on shared resources. Figure~\ref{fig:normalizedTcore&Tuncore-runWith16} shows the impact of the contentions on each time slice, where we normalize \(T_{private}\) per instruction and \(T_{shared}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 207\% on average and 364\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions. 

% We observe that the system congestion influences the occupied time for each resource type differently. The time to hold private resources is slightly affected, with minor changes, even under heavy congestion. Meanwhile, the time due to shared resources is broadly affected, showing significant differences. Thus, we separately measure the two delays and charge their use with a different rule.
We observed that system congestion influences the occupied time for each resource type differently. The time to use private resources is only slightly affected, with minor changes, even under heavy congestion. In contrast, the time spent on shared resources is broadly affected, showing significant differences. Thus, we separately measure the delays for the two resource types and apply different charging rules for their use. 

% Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where we normalize \(T_{shared}\) per instruction and \(T_{private}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 181\% on average and 488\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions.
Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is calculated as the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where \(T_{shared}\) per instruction and \(T_{private}\) per instruction are normalized to the same tests when running alone. The figure shows that \(T_{shared}\) is significantly affected by system congestion compared to \(T_{private}\). On average, \(T_{shared}\) increases by 181\%, with a maximum increase of 488\%. Meanwhile, \(T_{private}\) increases by only 4\%, with minor variance between functions.

% This figure gives insights into two key factors. First, the congestion in the shared resources does not impact the performance of private resources. Accordingly, when the system gets congested, the degree of a function's dependence on the shared resources determines the function's performance. If the \(T_{shared}\) takes a minor portion of a function's execution, severe congestion still barely influences its overall execution. Second, hardware PMUs available in modern CPUs, and profiling tools such as Linux Perf are widely available and can be used to distinguish the usage of shared and private resources. Across the paper, we will take advantage of such tools to develop Litmus pricing.
This figure highlights two key factors. First, congestion in shared resources has a negligible impact on the performance of private resources. Accordingly, when the system gets congested, the extent of a function's reliance on shared resources determines its performance. If \(T_{shared}\) constitutes a minor portion of a function's execution, even severe congestion will have minimal impact on its overall execution. Second, hardware Performance Monitoring Units (PMUs) in modern CPUs and profiling tools like Linux Perf are widely available and can be utilized to differentiate between the use of shared and private resources. Throughout this paper, we will leverage these tools to develop Litmus pricing.

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/TpriTshardDistriRev}\\
% \caption{\(T_{private}\) and \(T_{shared}\) distribution when they run alone}
\caption{Execution time distribution of \(T_{private}\) and \(T_{shared}\)}
\vspace{-0.5em}
\label{fig:TpriTshardDistriRev}
\end{figure}

% Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) in a function's execution. The compute-intensive workloads (e.g., fib-py, float-py) have a substantial \(T_{private}\) portion that can reach 99.96\% of the execution time. However, the portion decreases when running memory-intensive workloads such as fib-nj. This distribution indicates how much other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase float-py's \(T_{shared}\), its total execution time, $T_{private}+T_{shared}$, will undergo minor change.
Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) during a function's execution. Compute-intensive workloads (e.g., fib-py, float-py) exhibit a substantial \(T_{private}\) portion, accounting for up to 99.96\% of the execution time. However, this portion decreases when running memory-intensive workloads such as fib-nj. This distribution reflects how other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase its \(T_{shared}\), the total execution time, $T_{private}+T_{shared}$, will undergo only a minor change.

% For each pricing component, we calculate the price by multiplying its charging rate with its time distribution. Thus we can further update the pricing equation.
After collecting the time slices spent on each resource, Litmus calculates each pricing component by multiplying two different charging rates with corresponding slices. Consequently, a new pricing equation emerges as follows:

\begin{equation} 
P = R_{private} * T_{private}  + R_{shared} * T_{shared}
\end{equation}

% \(T_{shared}\) is the cycles stalled due to L2 misses. It is measured from the perf counter, STALLS\_L2\_Misses. \(T_{private}\) is the total execution minus STALLS\_L2\_Misses. 
% Using Perf, Litmus collects\(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total cycles to complete the application minus \(T_{shared}\). 
% While Litmus returns the system's congestion state, the service provider still needs to determine reasonable prices charged for a service when having different congestion levels. 

% \(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. Again, the two charging rates are necessary since each component is affected differently, directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from the crowded execution environment. Thus, the charging rates should be measured as follows.
\(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. These two charging rates are necessary because each component is affected differently, either directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from a crowded execution environment. Thus, the charging rates should be measured as follows:

\begin{equation} 
R = R_{base} * \frac{T_{solo}}{T_{congestion}}
\end{equation}

% In this equation, \(R\) is the charging rate for executions on either private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free execution environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is the execution time when the function runs alone, and \(T_{congestion}\) is its execution time in the congested environment. Again, we should collect a separate \(T_{solo}\) and \(T_{congestion}\) for each pricing component. To measure \(T_{solo}\), \hl{the prior work}~\cite{alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. Litmus pricing avoids such a costly approach but presumes the function's \textit{solo} performance by examining reference workloads on the system.
In this equation, \(R\) represents the charging rate for executions on private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free runtime environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is its non-interfered execution time when the function runs alone, and \(T_{congestion}\) is its execution time in a congested environment. We need to collect separate \(T_{solo}\) and \(T_{congestion}\) values for each pricing component. To measure \(T_{solo}\), the prior study~\cite{tiwari2013enabling,alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. However, Litmus pricing avoids such a costly approach by presuming the function's solo performance through reference workloads on the system.

% Litmus pricing requires both providers and tenants to be involved in the price decision. The providers need to decide on reasonable rates for each resource use by analyzing the selected representative functions running on the system. To offer reasonable discounts, the providers must choose the functions analyzed carefully, collecting the functions representing the system. The tenants must also know the consequences when their tasks heavily rely on any of the shared resources. Unfortunately, their tasks may get delayed more than the provider's expectation while still receiving the discount rate up to the expectation. 
Litmus pricing requires both providers and tenants to be involved in the price decision process. Providers need to establish reasonable rates for each resource usage by analyzing selected representative functions. To offer fair discounts, providers must carefully choose the functions to be analyzed, ensuring the functions accurately represent the system condition. Tenants must also know the consequences when their tasks heavily rely on shared resources. Unfortunately, their tasks may get delayed more than the provider's expectations while still receiving the expected discount rate. 

% Here, the Litmus pricing reflects the varying value of the shared resources when the system's congestion level changes; the importance of shared resources becomes more valuable when congested. 



==> ASPLOS_2024_litmus/06_design_details.tex <==
\section{Estimating prices with Litmus}
\label{sec:designDetails}

% The providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}, before using Litmus pricing. The numbers in both tables are the slowdowns of codes while testing the system congestion. Shortly, the congestion table is filled with the slowdowns of startup codes, and the performance table is filled with the slowdowns of reference benchmarks. Litmus pricing needs three steps to charge the final price with a discount. First, the providers assess the system's congestion at multiple levels and range them in a table. This step completes the congestion table. Second, the providers study the impact of congestion on tenants' functions and complete the performance table. Lastly, the service provider determines a tenant's price based on the two tables. 
Before using Litmus pricing, service providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}. The congestion table lists the slowdowns during the startup phases, whereas the performance table lists the slowdowns of reference functions. Litmus pricing needs three steps to determine the final price with a discount. First, providers assess system congestion at multiple levels and record the results in the congestion table. Second, providers analyze the impact of congestion on reference functions and fill out the performance table. Lastly, providers determine a tenant's price based on the data from both tables.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tables}\\
\caption{Congestion and performance tables: numbers in both tables indicate the slowdowns of startup codes and reference functions, collected with CT-Gen and MB-Gen}
\vspace{-0.7em}
\label{fig:litmust_tables}
\end{figure}

\textbf{Step 1, Defining Congestion Levels:} We manage the system's congestion levels using two traffic generators that create a range of congestion states by stressing shared resources differently. The traffic generator is multi-threaded, creating traffic in shared resources to incur congestion, with each thread running on a separate core. We rank the stress levels from 1 to 32 by changing the number of active threads running on distinct cores. Entries from top to bottom in the congestion table indicate increasing stress levels.

% \begin{figure}[h]
% \centering
% \vspace{-1.5em}
% \includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
% \vspace{-1em}
% \caption{stressing program's instruction, L3 accesses and L3 misses }
% \vspace{-0.5em}
% \label{fig:stressing_specs}
% \end{figure}

% \textbf{Step 2. Measuring System Congestion:} Measuring the current level of system congestion that may influence a function's performance is a crucial challenge. If we assume that the platform does not have pre-profiled information about a function's performance, the platform cannot figure out whether co-running functions influenced the function. Additionally, the serverless platform's fast-changing states with massive short-living functions make the assessment even more complicated, requiring quick and frequent examinations.

% Meanwhile, measuring the amount of a system's congestion and its impact on performance is a crucial challenge. This challenge particularly stands apparent when being demanded to quantify the impact of the congestion on a running application without pre-profiled information about the application. Moreover, the serverless platform's fast-changing system states with \hl{numerous} short-lived functions make the assessment even more complicated, requiring quick and frequent performance examinations.
Measuring the amount of system congestion and its impact on performance is a crucial challenge. This challenge becomes particularly pronounced when trying to quantify the impact of the congestion on a running application without pre-profiled information about the application. The fast-changing system states of a serverless platform, with numerous short-lived functions, further complicate the assessment, necessitating quick and frequent performance examinations.

% Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. The proposal is based on the observation that high-level languages, such as Python and Node.js, used in serverless computing have long startup times to accommodate their runtime environments. Since the inception of serverless computing, these startups have been recognized as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests leverage these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests further validated that all tested functions exhibited similar performance characteristics during their startups. 
Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. This method leverages our observation that high-level languages like Python and Node.js, commonly used in serverless computing, have lengthy startup phases to accommodate their runtime environments. Since the inception of serverless computing, these startup delays have been identified as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests exploit these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests have validated that tested functions exhibit similar performance characteristics during startup phases. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_all}\\
% \caption{IPC for serverless applications with different runtimes in the first 100 milliseconds of their execution}
% \vspace{-0.5em}
% \label{fig:startupIPC_all}
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped}\\
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-1}\\
\includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped_3}\\
% \caption{IPC for serverless applications grouped by language runtime in the first 100 milliseconds of their execution}
\caption{IPC of serverless applications based on languages (Go, Python, and NodeJS) during their startup phase}
% \vspace{-0.7em}
\label{fig:startupIPC_grouped}
\end{figure}

% Figure~\ref{fig:startupIPC_grouped} depicts the fluctuation in IPC (Instructions Per Cycle) of a function during the first milliseconds of its execution. The x-axis shows a time flow since the beginning; every tick indicates a millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language, and the throughput of each group is represented in separate figures. Although figures exhibit different patterns, functions in the same figure display notable similarities. The figures imply that functions written in the same language have nearly identical startups.
Figure~\ref{fig:startupIPC_grouped} depicts a function's fluctuation in IPC (Instructions Per Cycle) during its startup phases. The x-axis represents the time elapsed since the beginning, with each tick indicating one millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language runtime, and the IPC of each group is presented in separate figures. As shown in these figures, functions in the same figure show notable similarities. This implies that functions written in the same language have nearly identical startups.

% The startup of a runtime usually includes bursts of memory reads to load images and libraries, which can probe the traffic in the shared resources. By conducting a Litmus test before executing every tenant's codes, the providers can observe the system state for the function. Meanwhile, the providers also need to study how the startup codes perform in different system states. They complete the congestion tables by performing the Litmus tests with the startups written in three languages while varying the congestion levels. To this end, the information in the congestion table is looked up when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}. 
% estimating the system's state upon receiving a result of a function's Litmus test. 
The startup of a runtime typically includes bursts of memory reads to load images and libraries, which can be used to probe the traffic in shared resources. By conducting a Litmus test before executing a tenant's function, providers can assess the system state. Meanwhile, providers also need to study how startup phases perform under different system states. They complete the congestion tables by conducting the Litmus tests with startups written in three languages while varying congestion levels. This information from the congestion table is then referenced when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tests}\\
\caption{Progress of serverless applications on four cores with Litmus tests (dotted arrows) over time}
% \vspace{-0.5em}
\label{fig:Litmus_tests}
\end{figure}

% Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests. The Litmus tests examine the level of system congestion with every function startup. \hl{Many} concurrent functions in serverless offer frequent test opportunities. Function\#1 is a memory-intensive function that raises a congestion level. While active, Litmus tests measure the congestion level above 8. After Function\#1's completion, the next Litmus test detects a non-congested system with a congestion level below 3. However, with the start of another heavy function, function\#2, the Litmus tests measure the new congestion in the system.
Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests, which examine the level of system congestion during each function's startup. Many concurrent functions in serverless offer frequent opportunities for testing. Function \#1, which is memory-intensive, causes congestion levels to rise above 8 during its execution. A Litmus test in Core 3 detects this congestion. After Function \#1 is complete, a subsequent Litmus test indicates a non-congested system with a congestion level below 3. However, during another resource-intensive function, Function \#2, the Litmus test identifies new system congestion with a level above 9.  

% \textbf{Step 2. Measuring the Impact of Congestion:} Although discerning the system congestion through the Litmus test, estimating its impact on a user's application is another challenge. This work proposes a discount based on the pre-studied impacts on reference functions, assuming the user's functions are alike. For this, the service providers need to select reference functions that represent users' functions running on their systems. In this work, we select the workloads in \hl{Section 2} as our reference applications. 
\textbf{Step 2, Measuring the Impact of Congestion:} Discerning system congestion through the Litmus test solves only one of the two challenges; the other is determining its impact on a tenant's function. Different tenants' functions could experience varying degrees of slowdown under the same congestion level. To address this, we propose using pre-selected reference functions to analyze these impacts, thereby avoiding the cost of runtime profiling. For this, providers need to carefully select reference functions that represent tenants' functions operating on the systems, as these selections influence the overall accuracy of congestion measurement. Later, in Section~\ref{sec:evaluation}, our tests will show that pre-selected reference functions can effectively represent unknown user applications. For this study, the selected reference applications (* marked) are listed in  Table~\ref{tb:benchmarks}. 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/refSlowdownStressing14}\\
% \includegraphics[width=1\columnwidth]{./fig/slowdownStressing16}\\
\caption{\(T_{private}\), \(T_{shared}\), and \(T_{total}\) of serverless applications that run with MB-Gen at stress level 14, normalized to their execution time when they run alone}
% \vspace{-0.5em}
\label{fig:refSlowdownStressing14}
\end{figure}

% Once the reference functions are ready, the providers study the slowdowns of the reference functions while varying different congestion levels again. This study completes the performance table in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. Again, our two traffic generators create two separate sub-tables. All entries in this table are 1-to-1 mapped to entries in the congestion table. The providers estimate a general function's slowdown when having a certain congestion level using this 1-to-1 mapping.
Once the reference functions are ready, providers analyze their slowdowns under varying congestion levels. This analysis completes the performance table shown in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. With two traffic generators, providers can complete another set of two sub-tables for the performance table. All entries in this table are mapped 1-to-1 to entries in the congestion table. Providers can estimate a general function's slowdown at a given congestion level using this one-to-one mapping.

% Figure~\ref{fig:refSlowdownStressing14} shows the reference functions' slowdowns when stressing the system. The X-axis shows different functions, each consisting of three bars: the first two bars show the CPI during each time slice, \(T_{private}\) and \(T_{shared}\), and the last bar shows the CPI of an entire execution. The figure shows that the tested functions suffer from different amounts of slowdowns, although the tests maintain consistent stress levels. \hl{The last group} shows the gmean of all the slowdowns, which is used when providers estimate a function's slowdown later. 
Figure~\ref{fig:refSlowdownStressing14} shows an example of the reference functions' slowdowns when stressing the system. The X-axis shows tested functions, each depicted with three bars: the first two bars show \(T_{private}\) and \(T_{shared}\), while the last bar shows the total execution time, all normalized to their execution time when running alone without interference. The figure shows that the tested functions experience varying degrees of slowdown despite consistent stress levels maintained during the tests. The next-to-last group shows the gmean of all the slowdowns, which providers use to estimate a function's slowdown later.

% \hl{This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/referenceStartupSlowdownRev}\\
\caption{The correlation between the slowdown of Python's startup phase and the slowdown of reference applications. From left, (a) \(T_{private}\), (b) \(T_{shared}\), and (c) \(T_{total}\), normalized to the execution time when running alone}
\label{fig:referenceStartupSlowdownRev}
\end{figure}

% \textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while a range of congestion levels is continuous, the tables only contain a few slowdowns in discrete intervals. Thus, providers need a model that returns an estimated slowdown when receiving a congestion level as an input. In our tests, we employ a linear regression to achieve the model.
\textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while congestion levels vary continuously, the tables only contain slowdowns at discrete intervals. Therefore, providers need a model that estimates the slowdown for any given congestion level. In our tests, we employ linear regression to develop the model.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/interpolation}\\
\caption{Estimating a function's slowdown with logarithmic interpolation}
\label{fig:interpolation}
\end{figure}

% Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding references' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). We employed two traffic generators to extrapolate a more precise congestion level, yielding two sub-tables in both the congestion and the performance tables. Consequently, the figure presents two linear regression models, each associated with a different traffic generator. 
Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding reference applications' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). To extrapolate a precise congestion level, we created two sub-tables within both the congestion and performance tables using two distinct traffic generators. As a result, the figure depicts two linear regression lines (red and blue dotted lines), each associated with a different traffic generator.

% The provider needs to estimate the function's slowdown to uncover its price. However, the above two regression models return two vastly different slowdowns. Then, the providers need to determine which model is close to the current environment. We think the two models reflect two extreme congestions that the traffic generators create, one before the L3 and one after the L3. CT-Gen creates massive traffic from the core to the L3 cache, which filters the traffic, preventing the operations from consuming the memory bandwidth. MB-Gen also creates huge traffic but consumes the memory bandwidth and replaces L3 blocks. Since each traffic generator creates an extreme case, the machine state could be intermediate with congestion in the range between the two congestions created by CT-Gen and MB-Gen. However, Litmus pricing cannot answer this question with only the startup's slowdown. 

% To address this question, we note that the system's L3 misses are a critical indicator closely related to a function's performance. Functions suffer more when the system experiences more L3 misses, which stresses the cache space and off-chip memory bandwidth. Accordingly, Litmus test collects the system's L3 miss count as a supplementary index, which tells more about the crowdedness of shared resources.

These regression models return two different slowdowns. To estimate a function's slowdown, providers must determine which model reflects the current environment more accurately. The traffic generators create two extreme congestion scenarios: one before the L3 cache and one after. CT-Gen generates substantial traffic from the core to the L3 cache that filters the traffic and prevents operations from consuming memory bandwidth. Conversely, MB-Gen also generates massive traffic but consumes memory bandwidth and repeatedly evicts L3 cache blocks. Because each traffic generator represents a distinct extreme case, the actual machine state could fall somewhere between the two congestion levels created by CT-Gen and MB-Gen. However, Litmus pricing requires more than just the startup slowdown to identify the machine's state in these models. Thus, we have enabled Litmus tests to gather the system's L3 miss count as a supplementary metric that offers deeper insights into the crowdedness of shared resources.


% \hl{Figure 1} shows how to use the L3 cache misses with the performance sub-tables. The two traffic generators make the upper and lower boundary of the L3 miss rates. When performing a Litmus test, if the test's L3 miss rate is XXX, close to the L3 misses with CT-Gen, we can conclude that the congestion occurs before the L3 cache and select the expected slowdown of XXX. On the contrary, we choose XXX, in case the L3 miss rate is XXX, close to the L3 misses with MB-Gen. If the test's L3 miss rate is in-between, we interpolate the two slowdowns based on the L3 misses, assuming congestion in both resources. 
% Finally, we determine the Rprivate and Rshared based on the expected slowdown from its performance table. Calculating Rprivate and Rshared takes the same steps. The final discount price is computed using the equation with the computed rates. 

% Figure~\ref{fig:interpolation} shows how we employ the L3 misses when estimating the slowdown. The two traffic generators make the upper and lower boundary of the L3 misses. If a Litmus test reports the L3 miss count is 10, close to the L3 misses with CT-Gen, \textcircled{1}Litmus pricing estimates the discount (=expected slowdown) of the function to be near 1\%. This indicates that the congestion happens before the L3, as what CT-Gen creates. On the contrary, in case the L3 misses are 1000, close to the L3 misses with MB-Gen, \textcircled{2}Litmus pricing estimates the function's discount rate close to 6\%. Meanwhile, if the Litmus test reports the L3 misses as 100, we interpolate the two extreme discounts, 1 and 6, based on the L3 misses, assuming current congestion to stand in between the two extreme congestions. The congestion model in the figure shows how we interpolate with logarithmic interpolation. In this figure, \textcircled{3}applying the logarithmic interpolation to the L3 miss count returns the half-point between CT-Gen's 1\% and MB-Gen's 6\%, which is 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 
Figure~\ref{fig:interpolation} shows our approach to using L3 misses to estimate slowdowns. We created two figures illustrating separate regression models. The left figure (a) is derived from the startup slowdowns and L3 misses with logarithmic regression, indicating L3 misses at specific congestion levels. The right figure (b) is derived from the performance table with linear regression, displaying discounts at specific congestion levels. Each figure depicts two regression lines associated with different traffic generators.

The two traffic generators set the upper and lower boundaries for L3 misses. For instance, if a Litmus test reports 10 L3 misses, close to what CT-Gen generates: \textcircled{1}This suggests congestion occurs before reaching the L3 cache, similar to CT-Gen's scenario. Thus, Litmus pricing estimates the function's discount to be around 1\%. Conversely, if the Litmus test reports 1000 L3 misses, close to MB-Gen's results: \textcircled{2}Litmus pricing estimates the function's discount rate to be approximately 6\%, indicating congestion similar to MB-Gen, where memory bandwidth is heavily consumed and L3 cache blocks are frequently evicted. When the Litmus test reports 100 L3 misses, an interpolation between these extremes is applied: \textcircled{3}Using logarithmic interpolation, Litmus pricing estimates the function's discount rate to be midway between CT-Gen's 1\% and MB-Gen's 6\%, resulting in approximately 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 



==> ASPLOS_2024_litmus/07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> ASPLOS_2024_litmus/08_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \textbf{Litmus price \& error:}
% We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, and the other consists of selected reference applications to obtain the linear regression models for Litmus pricing. The discount models plug into the Litmus pricing used in our tests. For this experiment, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown.
We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, while the other consists of chosen reference applications to derive linear regression models for Litmus pricing. The discount models plug into the Litmus pricing employed in the tests. In this study, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown. 

% % original version
% We maintain the congestion state consistent across all tests, co-running each function with 26 other functions. Using Perf~\cite{perfWiki}, we collect the three key stats: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup, which implies the congestion level in these tests, as well as the discount rates that every function receives. We execute every function 100 times and collect the average of the function's \(T_{private}\) and \(T_{shared}\). Finally, we compute each function's \(P_{private}\), \(P_{shared}\), and \(P\), the total price, by summing \(P_{private}\) and \(P_{shared}\).  

\subsection{One Function Per Core}

% revision version
% We maintain consistent congestion states across all tests by co-running each function with 26 other functions. Using Perf, we collect the three key statistics: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup. These metrics hint at the congestion level during the tests as well as the discount rates that a function receives. Each function is executed 30 times, and the average of its \(T_{private}\) and \(T_{shared}\) is collected. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).
We maintain consistent congestion levels across all tests by co-running each function with 26 other functions. As outlined in Section~\ref{sec:motivation}, whenever a function finishes, another is randomly launched to keep a total of 26 co-running functions. Using Perf~\cite{perfWiki}, we collect three key statistics: \(T_{private}\), \(T_{shared}\), and the machine's L3 misses during the first 45 million instructions of the Python startup. Through these metrics, Litmus pricing estimates the level of system congestion and the discount rates a function receives. Each function is executed 30 times, and we average its \(T_{private}\) and \(T_{shared}\) values. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice26Rev}\\
% \caption{The total price for functions computed via Litmus pricing and ideal prices when co-running with 26 other functions normalized to the commercial price that offers no discount}
\caption{Prices computed via Litmus pricing and ideal prices when co-running with 26 other functions, normalized to the commercial price that offers no discount}
\label{fig:normalizedPrice26Rev}
\end{figure}

% In Figure~\ref{fig:normalizedPrice26}, we can see a minimal difference in the discount rate between the Litmus price and the Ideal price. The average Litmus discount rate stands at 11.5\%, which is only marginally larger by 0.6\% than the average Ideal discount rate of 10.9\%. Also, we can see that the difference between the Litmus price and Ideal price are different among the applications. Certain applications exhibit higher Litmus prices compared to the Ideal price, while conversely, some applications demonstrate smaller Litmus prices. 
 %Figure~\ref{fig:priceErrorRunwith26} shows further details, analyzing the errors in each pricing component. 

% Figure~\ref{fig:normalizedPrice26Rev} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{10.66\%}, which is only marginally larger by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{10.28\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice26Rev} illustrates estimated prices derived from Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices to offset delays in a congested execution environment. The figure shows minimal disparities between the two prices, implying that Litmus pricing offers a reasonable discount. The average discount from Litmus pricing across all functions is 10.7\%, which is only marginally higher by 0.4\% compared to the average slowdown experienced by functions, which stands at 10.3\%, as depicted by the ideal price.

% However, the discount rates per slowdown differ among functions. For instance, float-py's ideal discount rate is \hl{0.05\%}, but it enjoys a \hl{4.31\%} discount with the Litmus pricing. Meanwhile, pager-py's performance drops by \hl{15.63\%} while receiving a \hl{13.87\%} discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more easily affected than the reference when congested. In contrast, float-py runs mostly with private resources, receiving a minor impact from the execution environment. Figure~\ref{fig:priceErrorRunwith26Rev} shows further details, analyzing the differences in each pricing component.
However, the discounts per slowdown differ among functions. For instance, float-py's ideal discount rate is 0.05\%, but it benefits from a 4.3\% discount with Litmus pricing. Conversely, pager-py encounters a 15.6\% performance decline while receiving only a 13.9\% discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more susceptible to congestion than the references. In contrast, float-py predominantly utilizes private resources, resulting in minimal impact from the execution environment. Further insights into these variations in each pricing component are presented in Figure~\ref{fig:priceErrorRunwith26Rev}.


% From figure~\ref{fig:tcore\(T_{private}\)Distr}, we know that \(T_{private}\) dominates the execution time among all applications. The impact from \(T_{private}\) error has a bigger impact on the overall error. The slowdowns due to congestion in private resources are small. Theoretically, there should be no slowdowns when using private resources, but we observed that the congestion still influences it. The observed slowdown is 000, a small difference from an ideal slowdown. Meanwhile, the slowdowns in shared resources are significant. We observe that 

% % \[  Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}}\]

% \[Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{TotalIdealPrice}\]
% \[TotalIdealPrice = R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}\]

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/priceErrorRunwith26Rev}\\
\caption{Weighted errors in prices derived from Litmus pricing, which are compared to ideal prices}
% \vspace{-1em}
\label{fig:priceErrorRunwith26Rev}
\end{figure}

%%% We discuss error
% In figure~\ref{fig:priceErrorRunwith26} we can see that there are some applications receive positive errors and some receive negative errors.  A negative error indicates that our estimated slowdown for that application is higher than its actual slowdown, resulting in greater compensation than the observed performance losses. On the other hand, a positive error indicates that the compensation is smaller than its real slowdown. For most applications, the Litmus price is slightly higher than the Ideal price, with minimal differences. The highest price error is 0.0389 for auth-nj, while the lowest error is 0.007 for dyn-py. The geometric mean of the absolute error is 0.018. 
% Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors that each function experiences. The error rate is computed as the difference between the estimated and the ideal prices over the ideal price. The first two bars show the errors in \(P_{private}\) and \(P_{shared}\), which are weighted by their corresponding ratio in the execution time, considering their impacts, as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. The functions can have two different errors: positive and negative. A positive error indicates that the Litmus-estimated price is higher than its ideal price, implying that it receives smaller compensation than its performance losses. In other words, Litmus pricing estimates its slowdown to be less than its actual slowdown. A negative error implies the opposite; a function's compensation is higher than its slowdown. This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others. Meanwhile, the tenants need to acknowledge the consequences if their functions differ vastly from the reference workloads, heavily relying on shared memory.
Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors each function experiences. The error rate is computed by comparing the estimated prices with the ideal prices and dividing the difference by the ideal prices. The first two bars show errors in \(P_{private}\) and \(P_{shared}\), weighted by their corresponding ratios in execution time, reflecting their impacts as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. Functions may have two types of errors: positive and negative. A positive error means that the estimated price exceeds its ideal price, implying that the compensation received is less than the performance loss incurred. In other words, Litmus pricing underestimates the slowdown relative to the actual slowdown. Conversely, a negative error indicates the opposite; a function's compensation exceeds its slowdown. This discrepancy indicates Litmus pricing may offer varying advantages to different functions, favoring those with lesser slowdowns. Meanwhile, tenants must recognize the consequences if their functions differ vastly from the references, particularly those heavily reliant on shared resources.

% Delete the followings
% This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.

% The largest absolute error is \hl{0.0723} for rate-go, while the smallest absolute error is \hl{0.0039} for \hl{mst-py}. Overall, the Litmus pricing shows minor errors with an average of \hl{0.0231}. With further details, the Litmus pricing accurately estimates the slowdowns in \(P_{private}\) with \hl{0.0175} of an average weighted error rate. \(P_{private}\)'s highest weighted error rate is \hl{0.079}, yet minor, while the lowest rate is only \hl{0.0008}. The weighted error rate for the estimated \(P_{shared}\) is also small. The average error rate for \(P_{shared}\) is \hl{0.0068}, even lower than for \(P_{private}\). \(P_{shared}\)'s highest error rate is \hl{0.0404}.
% The largest absolute error is 0.072, which occurs with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, the Litmus pricing exhibits minor errors, averaging 0.023, \hl{with the estimated discount differing by 22.5\% over the ideal discount.} With more details, Litmus pricing accurately estimates slowdowns in \(P_{private}\), with an average weighted error rate of 0.018. \(P_{private}\)'s highest weighted error rate is 0.08, yet minor, while the lowest rate is only 0.0008. The weighted error rate for estimated \(P_{shared}\) is similarly small, averaging at 0.0068, even lower than for \(P_{private}\). The highest error rate for \(P_{shared}\) stands at 0.04.
The largest absolute error is 0.072, occurring with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, Litmus pricing exhibits minor errors, averaging 0.023. Thus, the estimated discount deviates by 22.5\% from the ideal discount. Note that Litmus pricing aims to match the average discount across all functions by applying a system-wide discount based on the system's congestion level rather than adjusting the discount for each function individually. Consequently, individual functions may experience either positive or negative errors. However, it is noteworthy that the average discount between Litmus and ideal pricing differs by just 0.4\%, as illustrated in Figure~\ref{fig:normalizedPrice26Rev}, satisfying its objectives.
% This policy may incentivize some functions while penalizing others based on shared resource usage. 
Specifically, Litmus pricing estimates slowdowns in \(P_{private}\) with an average weighted error rate of 0.018. The highest for \(P_{private}\) is 0.079, while the lowest is just 0.001. For \(P_{shared}\), the average weighted error rate is even lower, at 0.007. The highest for \(P_{shared}\) is 0.040.


% Litmus employs the average performance of applications to determine the discount rate applied universally. In this context, an application encounters a positive error when its speedup is less than the estimated average speedup across all applications. Also, the error rate depends on the difference between the actual speedup and the estimated average speedup, with larger differences resulting in more significant errors for the given application.
% As discussed in Figure~\ref{fig:TpriTshardDistri}, \(T_{private}\) dominates the execution time across all applications, implying that a small error in the estimated \(T_{private}\) largely influences the execution time. This explains why, for functions that demand little shared resources, such as float-py and chame-py, the error in P is almost identical to that in \(T_{private}\), and errors with \(T_{shared}\) can be overlooked. In contrast, for functions with a larger \(T_{shared}\) ratio, such as pager-py and mst-py, errors in \(T_{shared}\) meaningfully affect the total execution time. Note that the Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price.  

Litmus pricing estimates each pricing component separately with an individual discount rate. For functions that demand minimal shared resources, such as float-py, the errors in P are nearly identical to those in \(T_{private}\), and the errors in \(T_{shared}\) can be overlooked. As shown in Figure~\ref{fig:TpriTshardDistriRev}, \(T_{private}\) dominates the execution time across many applications. While even a small error in the estimated \(T_{private}\) influences the function's execution time, substantial errors in \(T_{shared}\) likely have limited impacts, except for functions that have a relatively meaningful \(T_{shared}\) ratio, such as pager-py and mst-py, whose errors in \(T_{shared}\) are observable in the total price. 

% We emphasize that Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price. We observe that functions have similar slowdowns in \(T_{private}\) with slight variation when congested. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, also estimating reliable total prices since \(T_{private}\) mostly dominates the execution time. The \(T_{shared}\) fluctuates more dynamically across functions with a relatively large error, but the error's impact is little, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}. 
We emphasize that Litmus pricing cannot avoid producing a certain degree of error since it relies on estimation using a few metrics. However, the figure proves that Litmus pricing effectively captures a congested environment and reflects that environment in the price. Under the same congestion level, \(T_{private}\) values of all functions are delayed similarly with a little variation. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, leading to reliable total price estimates since \(T_{private}\) generally dominates execution time. \(T_{shared}\) fluctuates more dynamically across functions and has a relatively larger error, but the impact of this error is minimal, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}.

\begin{figure}[h]
\centering
% \vspace{-5em}
 \includegraphics[width=1\columnwidth]{./fig/normTprivtTshared26Rev}\\
% \vspace{-5.5em}
\caption{\(T_{private}\) \& \(T_{shared}\) of applications when co-running with 26 others, normalized to those when they run alone. The top(black) and bottom(blue) lines are discount rates from Litmus pricing for \(T_{private}\) and \(T_{shared}\)}
% \vspace{-1em}
\label{fig:normTprivtTshared26Rev}
\end{figure}

% To further investigate the price error differences, in igure~\ref{fig:normTprivtTshared}, we explore the \(T_{private}\) speedups across various serverless applications.  
% Notably, the difference between the Litmus discount (L-Discount) and the average speedup is merely 0.006.  This minute difference explains why Litmus can attains such high accuracy. 
%Furthermore, when comparing with figure~\ref{fig:priceErrorRunwith26}, a correlation between the error rate and the speedup differences becomes apparent. 
%For instance, float-py, with the most substantial difference above the Litmus discount, also experiences the most significant negative error rate. 
%Conversely, aes-go, with the smallest speedup, experiences the highest positive error rate.
% % original version
% Figure~\ref{fig:normTprivtTshared} shows the execution time of the baseline normalized to the execution time of each run under congestion. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the functions spend only 3.67\% more time on private resources, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, resulting in precise estimation with a Litmus test. 

% Figure~\ref{fig:normTprivtTshared26Rev} shows the execution time of each function run under congestion normalized to the execution time of the baseline. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the interferences in private resources extend the function execution time only by 5.3\%, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, enabling precise estimation with a Litmus test.
Figure~\ref{fig:normTprivtTshared26Rev} shows the \(T_{private}\) and \(T_{shared}\) of each function, normalized to the same time components of the baseline. The gap between the bar and 1 represents the amount of slowdown that should be translated into ideal discounts. The top (black) and bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that interferences in private resources extend the function execution time by only 5.3\%, implying the performance of the private resources is marginally affected by congestion. Additionally, all functions exhibit similar \(T_{private}\) values with little dispersion, helping precise estimation with Litmus tests.

% Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors are still in an acceptable range since their impacts are small. Functions that have a considerable \(T_{shared}\) ratio become more sensitive to system congestion. Instead, a function, such as float-py, with negligible \(T_{shared}\) ratio gains huge benefits with high discounts while its performance remains firm. This shows that Litmus pricing reflects the dynamically changing values of shared resources when the congestion level alters and encourages functions to be developed to use more private resources. 
Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors remain within an acceptable range as their impacts are minor. Functions that have a considerable \(T_{shared}\) ratio are more sensitive to system congestion. Conversely, a function like float-py, which has a negligible \(T_{shared}\) ratio, gains huge benefits from high discounts while maintaining stable performance under congestion. This shows that Litmus pricing accurately reflects the dynamic values of shared resources when the congestion level changes and incentivizes functions to be developed to use less shared resources. 

% \textbf{Litmus pricing under high congestion:} We test our Litmus pricing under a heavily congested environment to verify its pricing of functions with large slowdowns. To create a crowded environment, we concurrently execute 60 instances of Fibonacci-go, which produces the most L2 misses among our tested functions. 
% We raise the congestion level significantly with 60 co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo} shows the results from the same tests of Figure 11. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.8\%, which is only a 1.7\% difference from the ideal discount of 27.1\% with 2.48\% of an average absolute error. In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.151 and 4.299, which are only 2.45\% and 7.83\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. 
% \textbf{Litmus pricing under high congestion:} We raise the congestion level significantly with \hl{500} co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo500} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.1\%, which is only a 1\% difference from the ideal discount of 27.1\% with 0.088\% of an average absolute error. Litmus pricing discounts slightly more than an actual slowdown, leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% % \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
% \caption{The normalized total price for the applications calculated by using Litmus pricing and ideal prices when co-running with 500 Fibonacci-go}
% \label{fig:normalizedPriceCongested320}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\columnwidth]{./fig/diffStartupPortion-2Rev}\\
%\caption{The slowdown of Python's startup with 25 and 15 million instructions (X-axis) and the slowdown of reference applications (Y-axis). From left, \(T_{private}\), \(T_{shared}\), and \(T_{total}\), normalized to those when running alone}
%\label{fig:diffStartupPortion}
%\end{figure}

% \textbf{Instructions in Startup:} Litmus tests react differently to congestion when performed with different numbers of instructions from the startup phase. For example, Python's startup involves about 45 million instructions. While we have conducted Litmus tests using all these instructions, Figure~\ref{fig:diffStartupPortion} shows the response of these tests when running with the first 15 and 25 million instructions from this set. The figure shows the startups' \(T_{private}\), \(T_{shared}\), and \(T_{total}\) with two traffic generators, as depicted in Figure~\ref{fig:referenceStartupSlowdownRev}. Tests with fewer instructions are more sensitive to cold cache misses but less to interference in the L3 cache. Therefore, as the instruction count in Litmus tests decreases, they become less susceptible to conflicts in shared resources, especially from traffic by MB-Gen. As a result, tests with 25 million instructions exhibit reduced slowdowns. This trend becomes more apparent when running the tests with 15 million instructions, depicting that slowdowns when co-running with MB-Gen become nearly identical to those with CT-Gen. 

%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%







% \textbf{Instructions in Startup:} Python's whole startup phase contains about 45 million instructions. We can further divide the startup phase into smaller pieces with 10 million instructions code chunks. And each code chunk would have its characteristics. They react differently in the same congested environment. In section XXX we use the whole Python's startup portion's slowdown to indexsing the serverless application's slowdown. But, since the co-relationship between these two slowdown in different congestion source are different, one startup \(T_{private}\) slowdown may indicate two application's slowdown. By carefully picking the code chunks we can mitigate the difference between the two normalized slowdowns of the guidance application that correlated to the same startup phase slowdown. 

% Figure~\ref{fig:diffStartupPortion} depicts the correlation between the performance changes in the reference applications and distinct segments of Python's startup phase. From the figure, we see that selecting the first 15 million instructions as our startup phase results in the normalized \(T_{uncore}PerInst\) of the guidance application aligning nearly into a singular trendline. However, there are substantial gaps in the case of \(T_{core}PerInst\) with this code segment. Thus, we should pick xxx-xxx as our startup phase representation code for the normalized \(T_{core}PerInst\). We think that this can be used to mitigate the differences. But, we should be careful to use the small code chunks for the following reasons: First, only measuring the small portion can be a problem. The results might be too dynamic. Second, since we only measure this small portion there might be a huge execution period that cannot be covered.

% Continue to work from here

\subsection{Temporal CPU Sharing}
\label{sec:temporalCPUSharing}

The previous evaluation assumes an isolated environment where a CPU is assigned exclusively to an active function during execution, disallowing temporal sharing between functions through context-switching. While this setup ensures strict performance isolation, it inherently limits resource utilization. Conversely, enhancing utilization by permitting temporal CPU sharing among functions complicates price estimation. We explore how Litmus pricing can be applied in a less restrictive environment that permits sharing, where functions can temporarily share the same CPU and are not bound exclusively to specific cores. 

In this section, we deploy a testing function to co-run with 160 other functions across 16 cores without exclusive core assignments, assuming an average of 10 functions share a core. The reduction in the number of cores tested was necessitated by our system's memory limitations, as certain functions require significant memory space.

% \textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, the subsequent function clears the displaced one's cached data. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, the slowdown with extra sharing financially benefits the provider; we thereby argue that the extent of sharing should be factored into Litmus pricing as another discount factor.
\textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, a subsequent function evicts the cached data of the displaced one. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, delayed execution due to extra sharing financially benefits the providers. Thus, we argue that the extent of temporal sharing should be incorporated into Litmus pricing as another discount factor.

Figure~\ref{fig:csImpactor} depicts the switching overheads as concurrently running functions increase. The figure demonstrates that the sharing overhead follows a logarithmic growth pattern and stabilizes at around 20 co-running functions. Furthermore, we discovered that the switching overheads predominantly affect \(T_{private}\). Consequently, Litmus pricing needs to calibrate \(T_{private}\) to account for the impacts of sharing before estimating the slowdown using the performance table.

Figure~\ref{fig:normalizedPrice160Method1} illustrates the discounted price reflecting this adjustment. In our configuration, with an average of 10 functions per core, we divide \(T_{private}\) by 1.025 before estimating the slowdown. In this figure, Litmus pricing estimates an average discount of 14.5\%, which falls 2.9\% short of the ideal discount of 17.4\%. While most benchmarks receive discounts lower than ideal, aes-py stands out with the largest error of 9.9\%, which is 6.9\% less than its ideal discount of 16.8\%.

\begin{figure}
\centering
% \includegraphics[width=1\columnwidth]{./fig/csImpactor}\\
\includegraphics[width=1\columnwidth]{./fig/csImpactor2}\\
\caption{\(T_{private}\) of functions over different co-running counts in the same core, normalized to when running alone}
% \vspace{-1em}
\label{fig:csImpactor}
\end{figure}

\begin{figure}
\centering
% \vspace{-1.2em}
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160Method1}\\
\caption{Prices derived from Litmus pricing (Method 1) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
% \vspace{-0.5em}
\label{fig:normalizedPrice160Method1}
\end{figure}

% In Figure~\ref{fig:normalizedPrice160Method1} we use the the same congestion and performance tables that we collected in the restricted environment. When checking the tables instead of using the original startup slowdown of tcore we use an adjusted slowdown by dividing the context switch impact factor. From figure~\ref{fig:normalizedPrice160Method1} we can see that the average Litums discount is 14.65\%, 3.01\% less than what they should receive compared to the ideal discount of 17.67\%. Most applications receive a smaller discount than the ideal price. The largest error is on aes-py with Litmus discount of 9.85\%, 6.87\% smaller than the ideal discount of 16.72\%. The smallest error is on dyn-py. It's Litmus discount is 22.45\%, only 0.47\% larger than the ideal discount of 21.97\%.

\textbf{Method 2, Updating Performance Tables:} Rather than reusing the performance/congestion tables designed for restrictive environments, arranging new tables for the sharing-enabled environments returns better accuracy. Although the notion of preparing separate tables for various sharing levels may seem challenging, we argue that only one or a few extra tables for heavily crowded systems would suffice, given that commercial systems are typically heavily crowded. Again, we emphasize that the impact of function co-placement stabilizes above a certain co-placement count, as shown in Figure~\ref{fig:csImpactor}.

For this test, we prepared new performance/congestion tables for the environment described above, where a testing function is assumed to co-locate and compete for a core with 9 other functions. Moreover, considering the scenario where a switched-out function has a low chance of being rescheduled to the same core, instead of assigning 10 functions to a specific core, we ran 50 functions across 5 dedicated cores; each can run on any of the 5 cores. We managed the congestion levels in shared resources using traffic generators on the other cores, as outlined in Section~\ref{sec:designDetails}.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPrice160}
% \vspace{-0.6em}
\end{figure}

% Figure~\ref{fig:normalizedPrice160} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{17.29\%}, which is only marginally smaller by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{17.67\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice160} shows the prices obtained from Litmus pricing with the new tables, which are normalized to those from commercial sources. Once more, as in Figure~\ref{fig:normalizedPrice26Rev}, the figure reveals marginal distinctions between the two price points, suggesting that Litmus pricing continues to offer a reasonable discount. Across all functions, the average discount provided by Litmus pricing stands at 17.2\%, merely 0.2\% less than the ideal discount of 17.4\%.


==> ASPLOS_2024_litmus/09_sensitivity.tex <==
\section{Sensitivity}
\label{sec:sensitivity}

While the aforementioned tests highlight Litmus's potential, we recognize the need for more compelling results. This section expands our analysis and examines Litmus pricing from various angles across diverse system environments.

% \textbf{Heavy Congestions:} We raise the congestion level significantly with 320 co-running applications to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. The Litmus pricing is still close to the ideal price, discounting the price by 20.00\%, which is only a 1.46\% difference from the ideal discount of 21.46\%. The highest Litmus discount is 26.01\% for dyn-py. It has an error of 2.83\% compared with the ideal discount.
\textbf{Heavy Congestion:} We significantly escalate the congestion level to verify Litmus pricing under conditions of substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} presents the outcomes of the same tests depicted in Figure~\ref{fig:normalizedPrice160} but with 320 co-running functions. Not only did we increase the function count, but we also specifically selected 8 memory-intensive functions, aes-py, compre-py, thum-py, bfs-py, auth-py, fib-go, geo-go, and profile-go, that produce the most L2 cache misses among the tested functions to create heavy congestion in shared resources deliberately. Even under such intensified congestion, Litmus pricing produces results remarkably close to the ideal price, discounting the price by 20.0\%, which deviates by merely 1.5\% from the ideal discount of 21.5\%. The highest discount by Litmus pricing is 26.0\% for dyn-py, a minor error of 2.8\% compared to the ideal discount.


% leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 320 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPriceCongested320}
% \vspace{-1em}
\end{figure}

\textbf{CPU Frequency:} Modern CPUs feature dynamic CPU frequency adjustments, which are controlled via software or hardware. A hardware technique like Intel Turbo Technology autonomously adjusts the CPU frequency based on the CPU's power and thermal budgets, allowing the CPU to operate at higher frequencies when conditions permit and lower frequencies under heavy load. Prior tests assumed that the frequencies were fixed and strictly managed by service providers who had knowledge of when and to what extent frequency adjustments were necessary. Also, we evaluated Litmus pricing under the other scenarios where CPU frequencies were not fixed, providing more dynamic perspectives.

% Figure~\ref{fig:normalizedPrice160unset} illustrates the prices from the Litmus pricing and the ideal price, which are normalized to commercial prices. We tested it under the configuration in Section 7.2 with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, the Litmus pricing's discount is lowered from 17.16\% to 16.84\%, while the ideal discount rate is decreased from 17.42\% to 17.31\%. Still, the discount rate difference from the ideal price is only 0.47\% without setting the CPU frequency. We observed that the CPU frequency changes rarely when the system runs with 160 functions. Overall, the varying frequency made a minor impact on performance as well as the pricing scheme. 
Figure~\ref{fig:normalizedPrice160unset} illustrates the prices derived from Litmus pricing alongside the ideal prices, both normalized to commercial prices. This evaluation was conducted under the configuration outlined in Section~\ref{sec:temporalCPUSharing} with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, we observe a slight decrease in Litmus pricing's discount, from 17.2\% to 16.8\%, while the ideal discount rate decreases from 17.4\% to 17.3\%. Still, even without fixed CPU frequencies, the difference in the discount rate from the ideal price is only 0.5\%. We noted that CPU frequency changes were infrequent when the system operated with 160 functions. Overall, the variation in frequency had a negligible impact on Litmus pricing.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160unset}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others with unfixed CPU frequencies, both normalized to commercial prices}
\label{fig:normalizedPrice160unset}
% \vspace{-1em}
\end{figure}

% All the above experiments are done on Intel Xeon Gold 5218(Cascade Lake). We also perform our scheme on another CPU architecture, Intel Xeon Silver 4314(Ice Lake-SP). 
\textbf{CPU Architecture:} Ensuring the validity of Litmus pricing across different architectures is crucial. Our Litmus tests rely on the performance counter that measures a stall count due to L2 cache misses (cycle\_activity.stalls\_L2\_miss)~\cite{perfMonEvents}, supported by Intel's CPUs. Unfortunately, other vendors like AMD do not yet offer the same performance counter~\cite{amdPMC}, restricting our tests to Intel CPUs. Alternatively, we conducted tests on another Intel CPU based on the Ice Lake architecture, Xeon Silver 4314, to broaden the scope of our analysis.

\begin{figure}[b]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun70kiwi}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 70 others on Xeon Silver 4314, both normalized to commercial prices}
\label{fig:normalizedPriceCorun70kiwi}
\end{figure}

% Because of the limitation of our memory size, we test Limtmus with 70 co-running applications. In this test, we use method 2 introduced in section~\ref{sec:temporalCPUSharing}. We first conduct the congestion and performance tables with 50 applications running in the first 5 cores. Then for the evaluation, we run 70 applications in the first 7 cores to let our testing application compete with 9 other applications for a core.  Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus discounting the tenant only pays 82.52\% commercial price. It's 0.696\% less than with the ideal discount.
Once again, this evaluation was conducted following the configuration outlined in Section~\ref{sec:temporalCPUSharing}, albeit with 70 co-running functions, limited by the main memory capacity of 128GB. Following Method 2, we constructed new congestion and performance tables with 50 functions running across 5 cores. Then, we ran 70 functions across 7 cores to match the competition count, averaging 10 functions per core. Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus pricing, the tenant only pays 82.5\% of the commercial prices, which is merely 0.7\% less than the ideal price.

% \textbf{Per-core Function Count:} When altering the co-located applications in each core the performance of the application can also be influenced. In this test, we put 240 applications in the first 16 cores. The testing application is competing with 14 other applications. We used the same congestion and performance tables from section~\ref{sec:temporalCPUSharing} method 2. Figure~\ref{fig:normalizedPriceCorun15} presents the results. The error of Litmus pricing is 1.23\% with The average discount of 16.69\%. The ideal discount is 17.92\%. The mean price of Litmus is larger than the ideal price because we are using the tables that are made based on 10 applications per-core. The context-switching overhead is larger. But, from figure~\ref{fig:csImpactor} we know that there is a diminishing impact of per-core application count. The error of the Litmus pricing is still under control when we increase the per-core application count.
\textbf{CPU Sharing Overhead:} The co-located function count determines the level of interference, impacting a function's performance differently. To assess Litmus pricing under various co-running function counts, we increased the function count to 240 from the configuration outlined in Section~\ref{sec:temporalCPUSharing}, making an average of 15 functions running on each core. However, we reused the performance and congestion tables generated in Section~\ref{sec:temporalCPUSharing}. Figure~\ref{fig:normalizedPriceCorun15} illustrates the results, where the Litmus pricing's error is 1.2\% with an average discount of 16.7\%, compared to the ideal of 17.9\%. Despite reusing the tables constructed for 10 co-running functions per core, the error remains negligible. This outcome aligns with Figure~\ref{fig:csImpactor}, which highlights the diminishing impact of temporal sharing when running more than 10 co-running functions. Given the perpetual overcrowding of commercial systems, any configuration gap between the environment where constructing the tables and where conducting tests is expected to remain minor and easily manageable.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun15}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 15 functions per core and reusing tables, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun15}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun160smt}
\end{figure}

\textbf{Simultaneous Multithreading (SMT):} SMT is a technique aimed at maximizing resource utilization by enabling multiple threads to execute concurrently on the same core, extending the shared resource domain across the entire processor. However, while SMT enhances resource utilization, it significantly complicates the measurement of interference impact. Moreover, SMT introduces additional side channels, thereby increasing the processor's vulnerability to security attacks. Due to these concerns, serverless platforms like Amazon Lambda disable SMT in their systems~\cite{schall2023warming,agache2020firecracker,schall2022lukewarm}. Nonetheless, we have conducted a study to assess the impact of SMT on our Litmus pricing methodology.

% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
% \caption{Prices computed via Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, normalized to the commercial prices}
% \vspace{-0.5em}
% \label{fig:normalizedPriceCorun160smt}
% \end{figure}

% To generate the performance/congestion tables, we executed 50 applications across 5 dedicated physical cores. In this way, the testing function is co-located with 9 other applications in the same virtual core and 19 other applications in the same physical core. Fiugre~\ref{fig:normalizedPriceCorun160smt} illustrates the results. The first thing we notice is that the normalized price is much smaller compared with the setups without SMT turned on. The average discount of Litmus is 45.42\% which is 1.9\% smaller than the average ideal discount of 47.32\%.
To construct the performance and congestion tables, we executed 50 applications across 5 physically separated cores, allowing an average of 10 functions to share two virtual cores. Figure~\ref{fig:normalizedPriceCorun160smt} illustrates the results,  presenting prices derived from Litmus pricing and ideal prices, both normalized to commercial prices without discounts. The normalized price experiences a significant drop compared to other configurations, highlighting the impact of heavy congestion within a physical core. The ideal price, which assumes no interference, stands at 47.3\% of the commercial price. Meanwhile, Litmus pricing offers a discount of 45.4\%, which is only 1.9\% less, confirming the effectiveness of Litmus pricing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Node JS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Nodejs Startup:}NodeJs is another well-adopted language in serverless platforms besides Python. It's one of the earliest languages to be supported by AWS Lambda ~\cite{serverless1}. From Section~\ref{sec:designDetails} we see that NodeJs has a long startup phase which makes it a great candidate when we need to pick a language startup phase for the Litmus test. 

%\begin{figure}[h]
%\centering
%\vspace{-0.5em}
%\includegraphics[width=1\columnwidth]{./fig/njReferenceStartupSlowdown}\\
%\vspace{-1em}
%\caption{The correlation between the normalized NodeJs's startup phase and the normalized reference applications.}
%\vspace{-0.5em}
%\label{fig:njReferenceStartupSlowdown}
%\end{figure}

%Figure~\ref{fig:njReferenceStartupSlowdown} shows the correlation between NodeJs startup phases and reference applications. After applying the Litmus test with NodeJs applications, with this figure, we can use the slowdown of the NodeJs startup phase to find the corresponding system congestion level and the discount rate for both private and shared resources. NodeJs has a longer startup phase compared with Python. It gives us more room when picking the most suitable portions of the startup phase. We can choose the language to be used for the Litmus test based on the density of the startup phase. 


==> ASPLOS_2024_litmus/10_related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Serverless:} Many works address the performance bottleneck of serverless execution~\cite{du2020catalyzer}~\cite{agarwal2021reinforcement}~\cite{roy2022icebreaker}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Schall et al.~\cite{schall2022lukewarm} record and reload the instructions to reduce the front-end stalls when reaccessing the same application. Jovan et al.~\cite{stojkovic2023specfaas} focus on the performance of an application chain. They break the execution flow and speculative execute the functions. However, we are focusing on the price which is one of the most important potions of the cloud ecosystem.

% For the cloud providers, accommodating more tenants in a machine is a key strategy, gaining higher profits by maximizing the utilization of their machines. However, the approach inevitably introduces interference between tenants, slowing down applications unpredictably. Thus, prior researchers solved this challenge by allowing the tenants more non-biased, predictable, quality services~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed a clustering-based cache partitioning to remove unfairness between tenants. Rohan et al.~\cite{roy2021satori} simultaneously control multiple architectural resources to aim for both fairness and throughput. However, offering fairness inevitably sacrifices resource utilization. Thus, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} solve the unfairness uniquely by adjusting their prices while leaving the unfairness at a certain degree. This paper follows this direction but explores a more practical solution in serverless computing. 

Cloud providers strive to maximize profits by accommodating more tenants on their machines, which inevitably introduces interference between tenants, leading to unpredictable application slowdowns. To address this challenge, prior researchers have focused on providing tenants with a more unbiased and predictable quality of service~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed clustering-based cache partitioning to mitigate unfairness between tenants. Rohan et al.~\cite{roy2021satori} aimed for both fairness and throughput by simultaneously controlling multiple architectural resources. However, achieving fairness comes at the cost of sacrificing resource utilization. In contrast, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} addressed the unfairness by adjusting their prices while accepting a certain degree of unfairness. Our study follows a similar direction but explores a more practical solution within the context of serverless computing.

% delete the following section: the approaches are against our scheme. 
% \textbf{Serverless Computing:} Many studies focus on reducing the latencies of serverless applications~\cite{cadden2020seuss,oakes2018sock,wang2019replayable,jia2021boki}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Ustiugov et al.~\cite{ustiugov2021benchmarking} record and prefetches the functions’ stable working set of guest memory pages to further reduce the function's startup time. Wei et al.~\cite{wei2023no} remote forking the serverless functions to reduce the cold start latency while limiting the resource usage. Schall et al. record and reload the instructions~\cite{schall2022lukewarm} or the BTB entries ~\cite{schall2023warming} to reduce the front-end stalls when reaccessing the same application. 
% \hl{Litmus is orthogonal to these approaches and can be adopted together.}

==> ASPLOS_2024_litmus/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Serverless computing is a key technology in present cloud computing, offering numerous advantages. One primary advantage is its effective cost-saving, as tenants only pay for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion. While tenants suffer slowdowns, they also have to pay more for the slowdowns. Unlike prior approaches that aim to maintain quality of service, this paper discounts the tenant's cost to compensate for the loss. Litmus pricing proposed in this work monitors the machine states and adjusts the tenants' costs. The congestion level can be frequently gauged before every function using the proposed Litmus test, an effectively lightweight testing approach. Our tests show that Litmus offers near-ideal prices with a 0.38\% difference, compared to the ideal price that discounts proportional to its slowdown. 
Serverless computing is a key technology in contemporary cloud computing, offering a range of benefits. One primary advantage is effective cost-saving, as tenants are billed only for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion, which not only results in slowdowns but also higher costs for tenants. Rather than aiming to maintain service quality, this paper suggests discounting tenants' costs to compensate for performance losses. Litmus pricing proposed in this work monitors machine states through Litmus tests and adjusts tenant costs accordingly. The Litmus test is a lightweight testing approach for serverless platforms, which assesses the machine's congestion level before starting a user's function. Our tests prove that Litmus pricing offers nearly ideal prices in heavily congested environments, with an average deviation of just 0.2\% from the ideal price that adjusts discounts in proportion to the slowdown experienced.


==> ASPLOS_2024_litmus/12_ack.tex <==
\section{Acknowledgment}
\label{ack}

We would like to thank our reviewers for their valuable feedback to improve this paper. This work was supported by NSF CAREER Award CCF-2146475.


==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/00_abstract.tex <==
\begin{abstract}

% Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While the providers can utilize their machines more efficiently, the tenants only need to pay for the resources they consume. However, a serverless system co-runs thousands of short-living functions concurrently to maximize resource utilization, bearing frequent state shifts. Meanwhile, when the system gets too congested, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants are also charged higher costs when experiencing slowdowns since all commercial serverless platforms determine the tenants' costs proportional to their execution times.
Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times.

% This paper argues that the cloud providers should compensate the tenants for their loss when the server is over-provisioned. However, estimating the tenant's loss is challenging when there is no pre-profiled information about the function. Prior studies showed assessing the tenant's loss introduces heavy overheads. Instead, this paper proposes a new pricing model, Litmus pricing, which offers discounts based on the machine's state while presuming the tenant's loss under the state. To monitor the machine state correctly, Litmus pricing frequently conducts Litmus tests, an effectively lightweight solution to measure system congestion. Our experiments show that Litmus pricing can detect the impact of system congestion and offer near-ideal prices, with only a 0.38\% price difference. 
This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2\% price difference on average, in a heavily congested system.

\end{abstract}


==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Serverless computing is growing fast, satisfying today's high demands for better programmability. It allows tenants to develop their programs as stateless functions in high-level languages such as Python, Go, and JavaScript without concerns with low-level resource management and task scheduling~\cite{serverless2,serverless1,schall2022lukewarm,schall2023warming,mohammad2020SerInWild}. This advantage attracts cloud users, helping them to deploy their programs quickly with minimal effort. Recent reports note that over 50-70\% of cloud users have adopted serverless computing for their tasks~\cite{serverless1}.

% Serverless computing claims a pay-as-you-go pricing model where users only pay for the resources used by their functions. This requires the service provider to monitor and estimate the fine-grained resource usage by each user accurately. However, today's high-performance systems maximize resource efficiency by accommodating multiple applications simultaneously and allowing the resources to be shared by them. Such a shared system raises two major challenges. First, tracking a user's resource usage is a challenging task. While being shared, the system tracks the total usage but not a single user's. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress. These inferences between the applications not only make the system hard to track resource usage, but the users may get charged unfairly due to the delayed execution time.
Serverless computing also benefits tenants financially. Unlike traditional cloud platforms that require tenants to purchase the hardware resources needed to deploy their servers regardless of actual usage~\cite{amazonEC2Pricing}, serverless computing claims a pay-as-you-go pricing model, where tenants only pay for the resources consumed during the execution of their functions, facilitating significant cost savings. Meanwhile, this pricing requires service providers to accurately monitor and estimate each user's fine-grained resource usage~\cite{microsoftAzurePricing,awsLambdaPricing,googleCloudFunctionPricing}. 

% However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared system raises two major challenges. First, tracking a tenant's resource usage is a challenging task. While being shared, the system can only monitor a tenant's use of specific resources. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference between the applications not only makes the system hard to track resource usage, but the tenants may get charged unfairly due to the extended execution time~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}. 
However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared serverless system raises two major challenges. First, tracking a tenant's resource usage becomes challenging, as the system can only monitor a tenant's use of exclusively dedicated resources while the system is shared. Second, and more importantly, co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference not only complicates tracking resource usage but also leads to tenants being charged unfairly due to delayed execution times~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}.

% A serverless platform should provide an isolated runtime environment to a user. Otherwise, we argue that the platform provider must compensate a tenant's loss as a discount when it is not achievable. Therefore, we define a charged fee as fair when it reflects the tenant's slowdowns due to the resource sharing. The following two methods can be used to estimate a fair price under a multi-tenant environment. 
A serverless platform should provide a user with an isolated runtime environment. Otherwise, we argue that the platform provider should compensate a tenant's loss as a discount when the isolation is not achievable. Thus, we define a charged fee as fair when it reflects the tenant's slowdowns caused by resource sharing. The following two methods can be used to offer a fair price in a multi-tenant environment.

% First, strict resource partitioning can divide shared resources into multiple partitions, each assigned to a user exclusively. The user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strictly partitioned resources are well known to cancel the opportunities to utilize the given resource efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delayed execution directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources when requesting them. 
First, strict resource partitioning can divide shared resources into multiple partitions, each assigned exclusively to a user. This means the user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strict partitioning is known to cancel opportunities to utilize resources efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delay directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources they need when requested. 

% Alternatively, a discount-based scheme estimates a user's price relative to its slowdown, discounting from the price when run without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources. Thus, the providers can maximize their hardware utilization and earn more money with given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns or interference they get from co-running tasks without overpaying for exclusive resources.
% The tenants also can get a discount reasonably proportional to the amount of their slowdown when their jobs suffer from interference rather than endeavoring to secure necessary resources exclusively.
Alternatively, a discount-based scheme estimates a user's price relative to the slowdown experienced, discounting from the price when running the task without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources, enabling providers to maximize hardware utilization and generate more revenue with the given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns they experience due to co-running tasks, preventing them from overpaying for lowered service quality.

% While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Even if the platform can measure its execution time, computing the slowdown still requires knowing its baseline, which can be gained when executing it alone. The cloud platform could not pre-profile users' applications for reasons such as mandated privacy when processing confidential information. Even if the platform has such information, the function could operate differently when receiving different inputs. That is to say, online profiling is necessary, which unfortunately requires expensive runtime sampling, as proposed in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. All co-running tasks must be stalled when estimating a task's baseline performance. Massive short-living serverless functions make such a sampling-based solution even more impractical. Frequently sampling the baseline performance of thousands of co-running functions is unrealistic. This motivates a new practical solution that can be adopted in commercial platforms. 
While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Although the platform can measure its execution time, determining the slowdown requires knowing its baseline performance, which can be obtained when it runs without interference. However, such profiling is often prohibited due to security concerns, particularly when the function processes confidential information. Additionally, the function may behave differently, with varying inputs each time it runs. That is to say, online profiling is necessary. Unfortunately, this requires expensive runtime sampling, as presented in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. When assessing baseline performance, all co-running tasks must be stalled. Hundreds to thousands of concurrent short-lived functions make this approach indeed impractical, as frequently sampling the baseline performance of such numerous functions is unrealistic. Thus, a new, practical solution that can be adopted in serverless platforms is needed.

%In either approach, a tenant or a service provider bears the problem's complexity alone. Resource partitioning demands the tenant to know the needed resources while losing opportunities to utilize the resources better. Discounting demands a service provider to estimate the task's slowdown with heavy sampling overheads. Accordingly, both approaches complicate the problem while sacrificing the machine's efficiency. Instead, we claim this problem becomes simpler when both entities participate and carry a portion of the responsibilities. 

% Litmus addresses this challenge by imposing the responsibility on both entities. With Litmus, the serverless platform measures the system congestion that may delay a function's execution when every tenant's function starts. The service provider needs to determine a discount rate for a corresponding congestion state. Meanwhile, the tenant needs to know about a possible slowdown and a corresponding discount. 

% We highlight that both partitioning and sampling complicate the problem while sacrificing the machine's efficiency and can hardly be employed in serverless computing. The approaches in serverless must be lightweight and frequent to deal with the fast-changing environment with thousands of concurrent functions. This paper proposes Litmus pricing that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening the system performance. 
We highlight that both partitioning-based and sampling-based approaches complicate the problem, either sacrificing the machine's efficiency or appearing impractical for serverless computing. Approaches in serverless computing must be lightweight, frequent, and sensitive enough to deal with quickly changing environments with numerous concurrent functions. This paper proposes Litmus pricing, a method that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening system performance. 

% \hl{Measuring the server's congestion status is challenging work. Here, Litmus relies on our key observation that, although not limited, function implementation in serverless computing largely relies on high-level programming languages such as Python and GoLang, which require a relatively long startup. This startup overhead has been considered one of the major challenges in serverless computing. However, Litmus utilizes this startup to measure the system's congestion state. Our analysis of Python and GoLang observed that the activities during the startups are almost identical, with plenty of memory operations, regardless of the functions. Thus, we claim that the startup performance can be an index of the system state.}

% \hl{The Litmus test is based on our insight that the serverless functions perform broadly identical operations, with plenty of memory operations, during their long startups, preparing the runtime environment for the functions. Leveraging this observation, the platform can assess the system's congestion level, which hints at the tenant's discount amount. Additionally, Litmus pricing exploits our second insight that the performance of two resources, private and shared, are affected differently by the congestion. In particular, its impact on private resources is minor and predictable, while many functions significantly rely on them, spending most of their execution time with them. }

% During the execution of every function, Litmus pricing conducts a Litmus test, which measures the level of system congestion with no extra overhead using the function's startup process. The Litmus test is based on the observation that serverless functions perform largely identical operations during their startup time. Those operations usually prepare the runtime and include a large amount of memory access to shared hardware resources. In addition, Litmus pricing splits the hardware resources into "private" and "shared" and proposes charging different ratios on each. This further improves the accuracy of the discount calculation.
During each function's execution, Litmus pricing conducts a Litmus test, which measures the level of system congestion without adding extra overhead, using the function's startup process. Litmus test is based on the observation that serverless functions perform largely identical operations during their startup, typically involving significant memory accesses. Additionally, Litmus pricing splits the hardware resources into "private" and "shared" categories, proposing different charging ratios for each. This approach further enhances the accuracy of the discount calculation.

% In our experiments, the Litmus pricing estimates a tenant's price to be nearly ideal, with a \hl{0.38\%} difference from the ideal price, which discounts tenants proportional to their slowdowns.
% This study investigates Litmus pricing across different environments, ranging from restricted to crowded settings. We verify that crowded environments pose additional challenges. Despite this, Litmus pricing accurately estimates a tenant's price, deviating by only 0.26\% from the ideal price, discounting tenants proportional to their slowdowns.
This study investigates Litmus pricing across diverse environments with varying levels of system congestion. We confirm that crowded environments pose complex challenges. Despite this, Litmus pricing accurately estimates a tenant's cost, deviating by only 0.2\% on average from the ideal price that discounts tenants proportional to slowdowns.



==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/02_background.tex <==
\section{Background}
\label{sec:background}

% \textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while the service providers handle back-end implementation~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers, which are later invoked upon associated events~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. The serverless platform guarantees security by executing the tenant's function in a sandbox such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.
\textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while leaving back-end implementation managed by service providers~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. These functions are later invoked upon associated events. The serverless platform ensures security by executing the tenant's function in a sandbox, such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.

% Each tenant's function is stateless and expected to be short~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using the short-lived functions, the tenant can easily scale by invoking many of the functions without provisioning needed resources for themselves, relying on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. Inherently, massive short-living serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. The tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and clients mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Later, under the pay-as-you-go pricing, the tenant is charged for the consumed resources, typically the product of time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
Each tenant's function is stateless and expected to be short-lived~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using these short-lived functions, tenants can easily scale by invoking many functions without provisioning the needed resources for themselves, relying instead on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. In serverless computing, numerous short-lived serverless workloads run together on a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. Tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and tenants mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% In the traditional cloud, tenants purchase hardware resources for the contracted term to support their applications, which are often expected to be large in a server form. Thus, tenants must pay for the agreed period regardless of actual use. Instead, serverless workloads are generally small and launched on-demand as short-living event handlers. This workload difference develops a unique pricing policy, pay-as-you-go pricing. The tenant is charged only for the consumed resources during the execution, typically the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
In traditional cloud computing, tenants purchase hardware resources for a contracted term to support their applications, which are typically large servers. Thus, tenants must pay for the agreed period regardless of actual usage. In contrast, serverless workloads are generally small and launched on-demand as short-lived event handlers. This difference leads to a unique pricing policy known as pay-as-you-go. Under this model, tenants are charged only for the resources consumed during execution, typically calculated as the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, where Python is utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Also, over 90\% of organizations choose Python and Node.js for their AWS services. Other popular language runtimes are Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer a high level of abstraction from machine codes with good programmability and portability, improving the programmer's productivity. As a result, they have been adopted widely by serverless users. However, such high-level languages typically rely on runtime interpretation, which results in a slow start of program execution with extra launching steps. For instance, in the case of Python, when an application is launched, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the codes are compiled and executed. Once the execution is complete, the Python program is terminated, and all assigned resources are released~\cite{pythonUsage}.
\textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python used in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Over 90\% of organizations choose Python and Node.js for their AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer significant abstraction from machine code with good programmability and portability, which in turn improves programmer productivity. Consequently, they are widely adopted by serverless users. However, high-level languages typically rely on runtime interpretation, leading to slower program startup due to extra launching steps. For example, when an application is launched in Python, the interpreter is first prepared. It then parses command-line arguments and imports necessary modules. Afterward, the codes are compiled and executed. Upon completion, the Python program terminates, and all allocated resources are released~\cite{pythonUsage}.

 
% list of pricing models? 
% Amazon? 
% Google?
% The price is calculated by duration time multiplies to the unit price plus the request charges. The duration time is from the time user's code begins executing until it returns or terminates. The unit price depends on the amount of memory the user allocate to their function. The request charges is based on how many times the function has been invoked minus the free requests~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% may need service agreement here, contention impact

%\textbf{Traditional cloud platforms:} In the context of traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage, data transfer, etc. The instance type is the combination of Virtual CPUs(VCPUs), RAM, storage and network performances. The time unit price will be higher with more powerful instance type. Typically, more powerful instance types have higher time unit prices. There are two main pricing options: On-Demand and Reserved Instances. On-demand instance let the customers pay for compute capacity by the hour or second based on the actual usage with no long-term commitments. Reserved Instances, on the other hand, require a commitment to a specific instance type for a contract term and offer cost savings compared to On-Demand pricing. Storage and data transfer for the VM instance can also impact the pricing. The more storage space a customer uses or the more data they transfer, the higher their costs will be. The traditional cloud platform can also be affected by the co-running applications~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} In traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage space, data bandwidth, etc. The instance type includes virtual CPUs, RAM, storage, and network performances. Typically, more powerful instance types charge higher prices. Also, two pricing options are commonly offered: on-demand and reserved instances. On-demand instances allow tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved instances require a commitment to a specific instance type for an agreed term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period. Storage space and data bandwidth for the VM instance also influence the price. Demanding more storage space or more data transfer raises the cost~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} 

% The price of traditional cloud platforms is determined by computing capabilities such as processor type, memory capacity, and network bandwidth. While more and better resources typically charge higher prices, two pricing options are commonly offered: on-demand and reserved instances. On-demand pricing allows tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved pricing requires a commitment to specific resources for an agreed-upon term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period~\cite{amazonEC2Pricing}. 

% There are several differences between traditional cloud platforms and serverless platform. 
% Firstly, the roles of customers in the execution environment differ between traditional and serverless platforms. In the traditional cloud, customers are responsible for configuring and maintaining virtual machines (VMs), setting up networking, and managing databases~\cite{amazonEC2Pricing}. And it's the customers's responsibility to detact and update the configurations to balance their expenses and performance. On the other hand, in serverless platforms, users only provide a single file to indicate their system and library requirement, while the service provider handles the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. This feature enables users to focus solely on their actual workload without the burden of managing the infrastructures. Additionally, the platform can automatically scale the resources for the users based on the current demand of the application to guarantee the customer satisfaction~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% There are apparent differences between traditional and serverless cloud platforms. First, tenants are responsible for managing hardware resources in traditional platforms. The tenants need to configure and maintain virtual machines, set up networking, and manage databases~\cite{amazonEC2Pricing}. Also, tenants should study the optimal configurations to balance their expenses and performance. Meanwhile, in serverless platforms, tenants only provide a single file to specify their system requirements while the cloud provider prepares the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. The platform provisions or scales the needed resources on demand. Consequently, the serverless platforms encourage tenants to focus solely on their front-end workloads without the burden of managing the low-level back-ends~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% Secondly, there are notable differences in compute power and memory size options between the two platforms. For traditional cloud, the granularity usually 1 VCPU and 1GB memory. But, for serverless platform, the smallest memory size is 128 MB~\cite{awsLambdaApiGateWay,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Thirdly, the characteristics of workloads on these platforms set them apart. Serverless applications are generally small and executed on-demand, resulting in very short workload durations~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can complete in less than one second. In contrast, traditional cloud applications tend to be larger and may require hours to complete. Additionally, the number of co-located applications on a single computing node is smaller in traditional cloud setups, making their execution environment less dynamic compared to serverless platforms.
% Lastly, the billing periods differ significantly between traditional cloud and serverless platforms. Traditional cloud users are charged for the allocated time period. Regardless of whether they are actively running tasks on the machine, they are still need to pay for the allocated time period. However, serverless customers are only billed for the actual execution time of their tasks on the platform.

% Second, the workloads are expected to be small in serverless computing. Serverless workloads are generally small and launched on-demand as short-living event handlers~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can be completed in less than one second, unlike traditional cloud applications that are often expected to be large in a server form. Inherently, massive serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. This workload difference develops a unique pricing policy in serverless computing, pay-as-you-go pricing. In the traditional cloud, the tenants purchase hardware resources for the contracted term. Regardless of actual use, they need to pay for the agreed period. However, the serverless platforms bill their tenants for the actual execution time of their tasks.


% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python being utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Furthermore, over 90\% of organizations leverage Python and Node.js alongside AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer numerous advantages for programmers, such as user-friendliness, portability, reduced error risks, and thriving ecosystems. As a result, they have garnered widespread acceptance within serverless platforms. High-level programming languages typically follow a fixed execution procedure. For instance, in Python, when an application is executed, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the code is compiled and executed. Once the execution is complete, the Python program is terminated, and all resources used by the program are released. Due to the consistency of the operating system and Python version, the beginning of the execution process remains the same each time~\cite{pythonUsage}.



% \textbf{Resource based discount vs. Slowdown based discount:} To fully utilize the available resources, service providers often run as many applications as they can in one computing node within the service agreement requirement. However, this may lead to resource congestion and cause slowdowns for users, which can be unfair, since the customers are paying more money for the worse experiences. The intuitionistic solution could be for the service provider to track the resource usage of each application and offer discounts to users who consume fewer resources. However, serverless applications are typically very small, and contention can affect different applications differently, making this approach less practical. A more suitable solution for serverless platforms could involve offering slowdown-based discounts. In this approach, the service provider dynamically updates unit prices based on the level of system congestion. When there is less contention, users normally stiffed with the experiences and pay the regular price. However, during periods of high congestion, when the system is under heavy load, users could receive discounted prices as compensation for potential slowdowns. This approach would align pricing with the actual performance experienced by users, ensuring a fair and responsive pricing model.


==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/03_methodology.tex <==
\section{Methodology}
\label{sec:method}

% \textbf{Hardware Infrastructure:} All the experiments are performed on a dual-socket server platform. Each socket has 16 simultaneous multithreading(SMT) cores. The CPU model is Intel Xeon Gold 5218(Cascade Lake). The maximum frequency of the machine is 3.9GHz. Each core has a 32KB L1 instruction cache, a 32KB L1 data cache and a 1MB L2 cache. The 32 virtual cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The computer node runs the latest Ubuntu server version(Ubuntu 22.04 LTS) with kernel version 5.15.0. For consistency in the results, the core frequency was set to 3.0GHz using the 'cpupower frequency-set' command. We use linux perf~\cite{perfWiki} to collect the performance counters for each experiment. To analyze the startup status, we use -I 1 option to obtain count deltas at one-millisecond intervals. By utilizing interpolation, we can know the performance counters of each execution period. 

% In this study, we test today's server systems with serverless functions. This section describes our test configuration. 
This section outlines our test setup for evaluating serverless functions in this study.

% % original version
% \textbf{Hardware Infrastructure:} All experiments are performed on a dual-socket server platform with two Intel Xeon Gold 5218 (Cascade Lake). The CPU offers 16 simultaneous multithreading (SMT) cores with 3.9 GHz maximum frequency. We pin the core frequency at 3.0GHz for our tests. Each core has 32KB L1 instruction/data caches and 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The machine runs the Ubuntu server OS (Ubuntu 22.04 LTS) with a kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to collect the performance counters, which are collected at every one-millisecond interval. 
\textbf{Hardware Infrastructure:} All experiments are conducted on a dual-socket server platform equipped with two Intel Xeon Gold 5218 processors based on the Cascade Lake architecture. Each CPU provides 16 cores that support simultaneous multithreading (SMT) with a maximum frequency of 3.9 GHz. Every core features 32KB of L1 instruction/data caches and a 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets collectively have access to 384GB of main memory. The server operates on Ubuntu Server OS, version 22.04 LTS, with kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to gather performance counters.

% The CPU frequency is a key performance/energy factor, significantly affecting a function's execution time and energy consumption. A CPU's frequency can be altered in software or hardware based on its power and thermal budget, configuring it for better energy efficiency or performance. However, varying frequencies cause the system performance/energy to be unsettled, making system management intractable. For this reason, commercial systems such as Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. In our tests, when the frequency is not fixed by software, Intel's Turbo technology alters the frequency occasionally but mainly employs 2.8GHz. We will discuss this further in the sensitivity section.
The CPU frequency is a critical factor influencing both performance and energy consumption, significantly affecting a function's execution time and energy usage. A CPU's frequency can be adjusted through software or hardware based on power and thermal budget, optimizing for either energy efficiency or performance. However, varying frequencies can cause instability in system performance and energy usage, complicating system management. For this reason, commercial systems like Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. If we do not fix the frequency through software, Intel's Turbo technology occasionally adjusts it, but it mostly remains at 2.8 GHz during our tests. We will provide more details on this in Section~\ref{sec:sensitivity}.

% \textbf{Stressing Programs:} We used two stressing programs to investigate how applications and the startup portion of the high level languages behave in a resource contention environment. FigureXXX illustrates the number of instructions, L3 accesses, and L3 misses that the stressing programs can generate in five seconds as the stressing levels increase. By combining different stress levels of these stress-testing programs, we can simulate various resource-congested environments. The XXX-stressor(lineXXX)  generates more L3 accesses with a high L3 hit rate. While XXX-stressor(lineXXX), in each stressing level, generates fewer L3 accesses but more L3 misses. With these two stressors and different stressing levels, we can simulate the system with varying contentions to the shared resources by creating various  L3 accesses and L3 misses. In figureXXX we can see that the L3 accesses generated from the L2-stressor (update name later) begin to decrease after reaching stressing level 20.  However, during this period, the L3 misses continue to increase. The reason behind this trend is that, after stressing level 20, the heightened L3 miss rate starts to impact the stressor's performance, leading to a decline in the committed instruction count. Consequently, the stressor generates fewer L3 accesses and more L3 misses. 

% \begin{table}[h]
%     \begin{center}
%     % \vspace{-1.0em}
%         \caption{Serverless Benchmarks \& Runtimes}
%         \label{tb:benchmarks}
%         % \vspace{-1.0em}
%         \begin{tabular}{|l l||l l|} \hline
%             Function & Abbr. & Function & Abbr. \\ \hline \hline
%             \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  & \multicolumn{2}{c|}{\textbf{Hotel Reservation~\cite{gan2019open}}} \\ \hline
%             Dyn HTML & dyn-py & Geo & geo-go* \\ \hline
%             Thumbnail & thum-py* & Profile & profile-go \\ \hline
%             Compression & compre-py & Rate & rate-go \\ \hline
%             Image Recogn & recogn-py* & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
%             Graph Rank & pager-py & Currency & cur-nj* \\ \hline
%             Graph Mst & mst-py & Payment & pay-nj \\ \hline
%             Graph Bfs & bfs-py* & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
%             DNA Visual & visual-py* & Authen & auth-py/nj/go \\ \hline
%             \multicolumn{2}{|c||}{\textbf{Function Bench~\cite{kim2019functionbench}}} & Fibonacci & fib-py/nj/go* \\ \hline
%             Chameleon & chame-py & AES & aes-py/nj/go \\ \hline
%             FloatOp & float-py* & & \\ \hline
%             % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
%         \end{tabular}
%     \end{center}
%     % \vspace{-1.5em}
% \end{table}

\begin{table}[h]
    \begin{center}
    % \vspace{-1.0em}
        \caption{Serverless Benchmarks \& Language Runtimes (py, nj, go)}
        \label{tb:benchmarks}
        % \vspace{-1.0em}
        \begin{tabular}{|l l||l l|} \hline
            Function & Abbr. & Function & Abbr. \\ \hline \hline
            \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  &  \multicolumn{2}{|c|}{\textbf{Function Bench~\cite{kim2019functionbench}}}\\ \hline
            Dyn HTML & dyn-py & Chameleon & chame-py \\ \hline
            Thumbnail & thum-py* & FloatOp & float-py \\ \hline
            Compression & compre-py & Gzip & gzip-py* \\ \hline
            Image Recogn & recogn-py & RandDisk & randDisk-py* \\ \hline
            Graph Rank & pager-py & SequenDisk & seqDisk-py \\ \hline
            Graph Mst & mst-py & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
            Graph Bfs & bfs-py* & Currency & cur-nj* \\ \hline
            DNA Visual & visual-py* & Payment & pay-nj \\ \hline
            \multicolumn{2}{|c||}{\textbf{Hotel Reservation~\cite{gan2019open}}} & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
            Geo & geo-go & Authen & auth-py*/nj/go \\ \hline
            Profile & profile-go* & Fibonacci & fib-py*/nj*/go* \\ \hline
            Rate & rate-go & AES & aes-py/nj*/go* \\ \hline
            % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
        \end{tabular}
    \end{center}
    % \vspace{-1.5em}
\end{table}

% revision version
% \textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we select 27 distinct serverless functions from different benchmark suites, including AWS' authentication serverless functions~\cite{awsLambdaApiGateWay}, Hotel Reservation from the DeathStarBench suite~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and SeBS serverless benchmark suite~\cite{copik2021sebs}. The three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating 3 separate test cases per function. Among them, we pick 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. The functions are implemented using three languages: Python, Nodejs, and Go. We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. 
\textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we selected 27 distinct serverless functions from various benchmark suites, including AWS authentication serverless functions~\cite{awsLambdaApiGateWay}, the Hotel Reservation from DeathStarBench~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and the SeBS serverless benchmark suite~\cite{copik2021sebs}. The functions are implemented using three languages: Python, Nodejs, and Go. Notably, the three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating three separate test cases per function. 
% This comprehensive language support ensures that our test coverage is thorough and representative of the diverse language preferences in the serverless computing community. 
We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. Additionally, we selected 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. 


%\hl{The benchmarks we choose include I/O-bound, memory-bound, and compute-bound functions. For an experiment, we put the testing function in core 0 to core 4. We also put 50 other functions in core 0-4 to let the application co-running with 10 other applications to observe the impact of context switching.}

% \hl{We select benchmarks with mixed performance characteristics: I/O, memory, and compute-bound. Also, to replicate the congested commercial systems, we located a testing function with 50 other functions and tied them to selected 5 cores, Core 0 to 4. During our evaluation, those functions run simultaneously and compete to secure any core among the five.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
\caption{(a) L2 misses and (b) L3 misses of traffic generators, both normalized with the average L2 and L3 misses of serverless applications listed in Table~\ref{tb:benchmarks}}
% \vspace{-0.5em}
\label{fig:stressing_specs}
\end{figure}

% \textbf{Traffic Generator:} We divide the CPU's shared resources into two distinct categories: resources before and after the L3 caches. To pressure each resource group individually, we developed two separate traffic generators aimed at generating traffic and congestion in these resources. The first traffic generator, CT-Gen, applies pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another traffic generator, MB-Gen, induces massive L3 misses that stress the resources after the L3 cache, mainly the off-chip memory bandwidth and L3 cache spaces.
\textbf{Traffic Generator:} We categorize the CPU's shared resources into two groups: those before the L3 caches and those after. To stress each group independently, we developed two separate traffic generators designed to generate traffic and congestion within these resources. The first generator, CT-Gen, exerts pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another generator, MB-Gen, induces massive L3 misses, which stress the resources beyond the L3 cache, primarily targeting off-chip memory bandwidth and L3 cache spaces.

% Both traffic generators are multi-threaded, governing the volume of traffic by adjusting the number of threads they spawn. Each thread spawned by the traffic generator is pinned on each core to prevent conflicts between threads; consequently, this setup allows us to vary the stress level across our 32-core processors, ranging from level 1 to 31. Figure~\ref{fig:stressing_specs} shows each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), for every thread count increment, CT-Gen makes massive L2 misses. The CT-Gen's L2 misses are ended with L3 hits, as shown in Figure~\ref{fig:stressing_specs}(b). Meanwhile, MB-Gen creates huge L2 and L3 misses, as implemented. Interestingly, its L2 misses are fewer than CT-Gen's because MB-Gen is slowed by its L3 misses, suffering from a self-created bandwidth bottleneck. 
Both traffic generators are multi-threaded and govern the amount of traffic by adjusting the number of threads they spawn. Each thread is pinned to a specific core to avoid conflicts between threads, allowing us to vary the stress level on our 32-core processors from level 1 to 31. Figure~\ref{fig:stressing_specs} illustrates each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), with each increase in thread count, CT-Gen generates substantial L2 cache misses. These L2 misses by CT-Gen are ended with L3 cache hits, as shown in Figure~\ref{fig:stressing_specs}(b). In contrast, MB-Gen produces significant L2 and L3 cache misses. Interestingly, MB-Gen's L2 misses are fewer than those of CT-Gen because MB-Gen is hindered by its L3 misses, suffering from a self-imposed performance bottleneck.



==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/04_motivation.tex <==
\section{The Need for Fair Pricing}
\label{sec:motivation}

% Offering fairness appears in different approaches in cloud computing when multiple tenants share hardware resources. One standard is SLA, which defines the level of services the cloud provider furnishes while a tenant sets their expectation. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving unfairness between tenants. Although serverless computing highlights the pay-as-you-go pricing model, such unfairness still exists.
Fairness in cloud computing, especially when multiple tenants share hardware resources, is addressed through various approaches. One standard method is the Service Level Agreement (SLA), which specifies the level of service the cloud provider must deliver and the tenants' expectations. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving fairness issues. Despite serverless computing's emphasis on a pay-as-you-go pricing model, unfairness among tenants still exists.

% Unfortunately, modern systems are designed to maximize hardware efficiency by co-running multiple applications; the function's execution time can be affected by co-scheduled applications with conflicts when using shared resources. Ironically, whenever the service provider squeezes their resources further for better profit by accommodating more functions into a single machine, each function's execution time increases, charging them a higher cost for the same workload. However, in serverless computing, tenants lack control and insights into how their software is executed and billed for the cost of convenience. 
Unfortunately, modern systems are designed to maximize hardware efficiency by running multiple applications concurrently. This results in conflicts over shared resources, affecting each function's execution time. Ironically, when service providers optimize for profit by packing more functions into a single machine, the execution time for each function increases, resulting in higher costs for the same workload. In serverless computing, tenants have no control or visibility over how their software is executed, leading to potential inefficiencies and higher costs for the sake of convenience.

% Genuine pay-as-you-go pricing can be achieved when there is no interference. However, that is not desired by the providers who expect to utilize their resources to maximize profits. In serverless, although each function runs virtually exclusively in a sandbox with private resources, it still shares a few resources with other co-running functions, such as shared caches and memory bandwidth. Resource partitioning, a traditional solution that eliminates interference, can promise exclusively dedicated resources to a tenant but cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 
In serverless computing, although each function runs exclusively in a virtual sandbox with private resources, it still shares certain resources like caches and memory bandwidth with other functions. Resource partitioning, a traditional solution that eliminates interference by dedicating resources exclusively to a tenant, cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 

\begin{figure}[h]
\centering
% \vspace{-0.7 em}
\includegraphics[width=1\columnwidth]{./fig/normalizedCPIRunWith26Rev}\\
% \vspace{-1 em}
\caption{Execution time of applications that run with 26 others, normalized to the execution time when running alone}
% \vspace{-0.4 em}
\label{fig:normalizedCPIRunWith26Rev}
\end{figure}

% Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed down when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. \hl{Whenever a function finishes, another function is randomly launched to maintain a total of 26 co-running functions.} The figure shows a function's performance drops by up to 35\%, and most functions are significantly influenced by the co-running functions. Compared to when an isolated environment is offered, the function performs 11.5\% slower on average, charging 11.5\% more to users. We highlight that the function runs only with 26 other functions, which is tiny compared to massively crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.
Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. Whenever a function finishes, a new randomly-selected function is launched to maintain a total of 26 co-running functions. The figure shows a function's performance can drop by up to 35\%, with most functions significantly impacted by the co-running functions. On average, functions perform 11.5\% slower in this shared environment compared to an isolated one, resulting in users being charged 11.5\% more. We highlight that this scenario involves only 26 co-running functions, which is tiny compared to heavily crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.

% Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} attempted to offer price discounts if it has a slowdown, compensating for the slowdowns. To provide the discount, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount reflecting the slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all the responsibilities of the contentions between co-running functions, guaranteeing all tenants an invariant price for their use. Any unexpected slowdowns that a tenant experiences are returned with a discount. However, sampling is an expensive operation, requiring all co-running processes to stall during the sampling. Moreover, accurate measurement requires frequent sampling when its system environment quickly alters, making the approach impossible in a fast-shifting environment like a serverless platform.   
Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} offers price discounts to compensate for slowdowns. To provide these discounts, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount based on the observed slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all responsibilities related to contentions from resource sharing, ensuring tenants pay a consistent price for their usage. Any unexpected slowdowns that a tenant experiences are compensated with a discount. However, sampling is an expensive operation that requires stalling all co-running processes during the sampling. Moreover, accurate measurement necessitates frequent sampling, especially in rapidly changing environments, making the approach impractical for dynamic environments like serverless platforms.


% A tenant needs a new pricing model based on more than just execution time. However, prior approaches have limitations, burdening cloud participants too heavily; it is unsuitable for \hl{thousands} of concurrent short-lived functions in serverless computing. This motivates us to propose a new solution, Litmus pricing, that discounts prices based on the system state but offers lightweight with no overheads.
Overall, tenants need a new pricing model that considers more than just execution time. Prior approaches have limitations, excessively burdening cloud participants and being unsuitable for the many short-lived functions typical in serverless computing. This motivates us to propose a new solution: Litmus pricing, which discounts prices based on the system congestion while remaining lightweight and imposing no additional overhead.


==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/05_design.tex <==
\section{Litmus Pricing}
\subsection{Overview}

% The estimated prices of serverless functions should reflect the congestion level of the system inside their machines. With the massive short-living functions, the serverless system's state can dramatically change in a short time. Accordingly, the system state can be congested at any moment and also resolved in a short time. However, such a temporary traffic jam may significantly impact the performance of short-living functions. Therefore, assessing the congestion must be lightweight, quick, and on time. However, a prior approach, POPPA\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling with considerable performance overheads, preventing them from wide adoption. Instead, we propose a new scheme, Litmus pricing, that quickly estimates system congestion at the start of every function and reflects the estimation into pricing the function. 
The estimated prices of serverless functions should reflect the system's congestion state. The presence of numerous small transient functions within the serverless system can rapidly alter its congestion state, causing sudden congestion or swift resolution. Nevertheless, such transient traffic jams can significantly impact the performance of short-lived functions. Thus, assessing the congestion must be lightweight, quick, and timely. However, a prior approach, POPPA~\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling, which incurs considerable performance costs, thereby limiting its widespread adoption. Alternatively, this study introduces Litmus pricing, which promptly gauges system congestion at the onset of each function and reflects the estimated congestion level into pricing the function.

% Like the prior approach~\cite{tiwari2013enabling,alex2013ScFairPrice}, Litmus pricing suggests that the service provider discounts when a tenant's functions are intervened, compensating for the performance loss. To determine the discount ratio, Litmus measures system congestion level, which can also help service providers evaluate remaining resources and make decisions on job scheduling. 
Like the prior approach, Litmus pricing suggests that service providers should offer discounts when a tenant's functions experience interference, thus compensating for the performance loss. Litmus pricing determines the discount rate based on the system's congestion level. Evaluating congestion also assists providers in estimating remaining resources and making informed decisions regarding job scheduling.

%Nevertheless, the Litmus pricing does not quantify each function's slowdown; the discount amount is determined only by the severity of the measured congestion. The impact of the congestion on distinct functions appears differently despite facing the same congestion level, and precisely estimating a function's performance loss is a complex problem. That's why the prior approach had to rely on expensive sampling. Instead, the Litmus pricing avoids the overheads and limits the service provider's responsibility to measure the current congestion. 
However, Litmus pricing does not quantify the slowdown of each individual function; the discount amount is solely determined by the severity of the measured congestion. Even though different functions face the same congestion level, their respective impacts can vary, making precise estimation of each function's performance loss a challenging task. This complexity necessitated the expensive sampling relied upon by the previous approach. Instead, Litmus pricing circumvents such overheads and lightens the service provider's burden solely to measure ongoing congestion levels.

% Litmus pricing embodies the varying value of shared resources across different system conditions by applying equal discounts to all functions under the same system condition, although the functions experience different slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that a function that is slowed more than others demands the over-crowded resources more while exacerbating the adverse over-crowded conditions. Litmus pricing does not provide additional compensation for their extra loss compared to others due to their heavy use of shared resources.
Litmus pricing captures the dynamic significance of shared resources under varying system conditions by offering uniform discounts to all functions under the same system congestion, regardless of their individual slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that functions experiencing larger slowdowns tend to demand more of the crowded resources, thereby exacerbating adverse overcrowded conditions. However, Litmus pricing does not offer additional compensation for the larger loss experienced by functions that use shared resources more heavily than others.

% As a result, Litmus inherently incentivizes users who use shared resources sparingly. When over-crowded, functions with minimal needs for shared resources still enjoy discounts but encounter slight slowdowns. This implies that users may take advantage of this policy by minimizing their use of shared resources, receiving substantial discounts despite enduring only minor slowdowns. Such a trade-off is considered acceptable because the user's shared resource usage reduces their contribution to congestion, thereby benefiting the overall system over the other users.
As a result, Litmus inherently incentivizes users who use shared resources sparingly. During periods of overcrowding, functions with minimal needs for shared resources still enjoy discounts but with only slight slowdowns. This implies that users may take advantage of this policy by minimizing their reliance on shared resources, receiving substantial discounts despite only experiencing minor slowdowns. This trade-off is considered acceptable because reduced shared resource usage by users helps mitigate congestion, thereby benefiting the overall system and other users.
% Lastly, the system refrains from scheduling a function if the congestion level exceeds a predetermined threshold, thus preventing resource thrashing.


\subsection{Pricing Model}
\label{pricing model}

% Developing Litmus pricing raises two challenges. First, Litmus needs a new pricing model to estimate a function's price. Second, Litmus needs a way to measure the system's congestion state. Due to the serverless's fast-shifting environment, assessing the congestion must be lightweight and frequent at the right time. Nevertheless, all present commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants must pay more with prolonged execution time when using over-crowded resources. Rather than simply imposing a price by multiplying the main memory usage and a function's total execution time, Litmus suggests the price as a sum of two distinct price components as follows.
Developing Litmus pricing raises two challenges. First, it needs a new model to estimate a function's price. Second, it needs a way to measure the system's congestion state. Due to the rapidly changing environment in serverless computing, assessing congestion must be lightweight and timely. Commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants end up paying more for prolonged execution time when using over-crowded resources. Rather than simply imposing the price by multiplying the main memory usage and a function's execution time, Litmus pricing determines the price as a sum of two distinct pricing components as follows.

\begin{equation} 
P = P_{private} + P_{shared}
\end{equation}

% In this equation, \(P\) denotes the total price tenants need to pay to execute their functions. Litmus pricing divides the tenant's price into two pricing components, each with a different resource type. \(P_{private}\) represents the price the tenant needs to pay for private resources, which are entirely assigned to a tenant. \(P_{shared}\) is the price the tenant needs to pay for the shared resources. Each price component is measured proportional to a user's time to occupy the corresponding resources. However, such occupied time can be extended when contention disturbs a process's execution in the shared resources. This delayed time increases a tenant's price unfairly. 
In this equation, \(P\) denotes the total price tenants must pay to execute their functions. Litmus pricing divides this cost into two pricing components, each associated with a different resource type. \(P_{private}\) is the cost for private resources, which are entirely assigned to a single tenant. \(P_{shared}\) is the cost for shared resources. Each pricing component is measured proportional to the time users occupy the respective resources. However, if contention disturbs a process's execution in the shared resources, the occupied time will be extended. This delay unfairly increases the tenant's cost. 


\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/slowdownRunwith26Rev}\\
\caption{\(T_{private}\) and \(T_{shared}\) of applications that run with 26 others, normalized to those when running alone}
\vspace{-0.5em}
\label{fig:slowdownRunwith26Rev}
\end{figure}

% Using Perf, we measure the delays due to the shared resources and split a function's execution time into two distinct slices: one slice, \(T_{private}\), which is time spent on private resources and another slice, \(T_{shared}\), which is time spent on shared resources. Figure~\ref{fig:normalizedTcore&Tuncore-runWith16} shows the impact of the contentions on each time slice, where we normalize \(T_{private}\) per instruction and \(T_{shared}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 207\% on average and 364\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions. 

% We observe that the system congestion influences the occupied time for each resource type differently. The time to hold private resources is slightly affected, with minor changes, even under heavy congestion. Meanwhile, the time due to shared resources is broadly affected, showing significant differences. Thus, we separately measure the two delays and charge their use with a different rule.
We observed that system congestion influences the occupied time for each resource type differently. The time to use private resources is only slightly affected, with minor changes, even under heavy congestion. In contrast, the time spent on shared resources is broadly affected, showing significant differences. Thus, we separately measure the delays for the two resource types and apply different charging rules for their use. 

% Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where we normalize \(T_{shared}\) per instruction and \(T_{private}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 181\% on average and 488\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions.
Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is calculated as the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where \(T_{shared}\) per instruction and \(T_{private}\) per instruction are normalized to the same tests when running alone. The figure shows that \(T_{shared}\) is significantly affected by system congestion compared to \(T_{private}\). On average, \(T_{shared}\) increases by 181\%, with a maximum increase of 488\%. Meanwhile, \(T_{private}\) increases by only 4\%, with minor variance between functions.

% This figure gives insights into two key factors. First, the congestion in the shared resources does not impact the performance of private resources. Accordingly, when the system gets congested, the degree of a function's dependence on the shared resources determines the function's performance. If the \(T_{shared}\) takes a minor portion of a function's execution, severe congestion still barely influences its overall execution. Second, hardware PMUs available in modern CPUs, and profiling tools such as Linux Perf are widely available and can be used to distinguish the usage of shared and private resources. Across the paper, we will take advantage of such tools to develop Litmus pricing.
This figure highlights two key factors. First, congestion in shared resources has a negligible impact on the performance of private resources. Accordingly, when the system gets congested, the extent of a function's reliance on shared resources determines its performance. If \(T_{shared}\) constitutes a minor portion of a function's execution, even severe congestion will have minimal impact on its overall execution. Second, hardware Performance Monitoring Units (PMUs) in modern CPUs and profiling tools like Linux Perf are widely available and can be utilized to differentiate between the use of shared and private resources. Throughout this paper, we will leverage these tools to develop Litmus pricing.

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/TpriTshardDistriRev}\\
% \caption{\(T_{private}\) and \(T_{shared}\) distribution when they run alone}
\caption{Execution time distribution of \(T_{private}\) and \(T_{shared}\)}
\vspace{-0.5em}
\label{fig:TpriTshardDistriRev}
\end{figure}

% Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) in a function's execution. The compute-intensive workloads (e.g., fib-py, float-py) have a substantial \(T_{private}\) portion that can reach 99.96\% of the execution time. However, the portion decreases when running memory-intensive workloads such as fib-nj. This distribution indicates how much other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase float-py's \(T_{shared}\), its total execution time, $T_{private}+T_{shared}$, will undergo minor change.
Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) during a function's execution. Compute-intensive workloads (e.g., fib-py, float-py) exhibit a substantial \(T_{private}\) portion, accounting for up to 99.96\% of the execution time. However, this portion decreases when running memory-intensive workloads such as fib-nj. This distribution reflects how other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase its \(T_{shared}\), the total execution time, $T_{private}+T_{shared}$, will undergo only a minor change.

% For each pricing component, we calculate the price by multiplying its charging rate with its time distribution. Thus we can further update the pricing equation.
After collecting the time slices spent on each resource, Litmus calculates each pricing component by multiplying two different charging rates with corresponding slices. Consequently, a new pricing equation emerges as follows:

\begin{equation} 
P = R_{private} * T_{private}  + R_{shared} * T_{shared}
\end{equation}

% \(T_{shared}\) is the cycles stalled due to L2 misses. It is measured from the perf counter, STALLS\_L2\_Misses. \(T_{private}\) is the total execution minus STALLS\_L2\_Misses. 
% Using Perf, Litmus collects\(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total cycles to complete the application minus \(T_{shared}\). 
% While Litmus returns the system's congestion state, the service provider still needs to determine reasonable prices charged for a service when having different congestion levels. 

% \(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. Again, the two charging rates are necessary since each component is affected differently, directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from the crowded execution environment. Thus, the charging rates should be measured as follows.
\(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. These two charging rates are necessary because each component is affected differently, either directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from a crowded execution environment. Thus, the charging rates should be measured as follows:

\begin{equation} 
R = R_{base} * \frac{T_{solo}}{T_{congestion}}
\end{equation}

% In this equation, \(R\) is the charging rate for executions on either private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free execution environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is the execution time when the function runs alone, and \(T_{congestion}\) is its execution time in the congested environment. Again, we should collect a separate \(T_{solo}\) and \(T_{congestion}\) for each pricing component. To measure \(T_{solo}\), \hl{the prior work}~\cite{alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. Litmus pricing avoids such a costly approach but presumes the function's \textit{solo} performance by examining reference workloads on the system.
In this equation, \(R\) represents the charging rate for executions on private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free runtime environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is its non-interfered execution time when the function runs alone, and \(T_{congestion}\) is its execution time in a congested environment. We need to collect separate \(T_{solo}\) and \(T_{congestion}\) values for each pricing component. To measure \(T_{solo}\), the prior study~\cite{tiwari2013enabling,alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. However, Litmus pricing avoids such a costly approach by presuming the function's solo performance through reference workloads on the system.

% Litmus pricing requires both providers and tenants to be involved in the price decision. The providers need to decide on reasonable rates for each resource use by analyzing the selected representative functions running on the system. To offer reasonable discounts, the providers must choose the functions analyzed carefully, collecting the functions representing the system. The tenants must also know the consequences when their tasks heavily rely on any of the shared resources. Unfortunately, their tasks may get delayed more than the provider's expectation while still receiving the discount rate up to the expectation. 
Litmus pricing requires both providers and tenants to be involved in the price decision process. Providers need to establish reasonable rates for each resource usage by analyzing selected representative functions. To offer fair discounts, providers must carefully choose the functions to be analyzed, ensuring the functions accurately represent the system condition. Tenants must also know the consequences when their tasks heavily rely on shared resources. Unfortunately, their tasks may get delayed more than the provider's expectations while still receiving the expected discount rate. 

% Here, the Litmus pricing reflects the varying value of the shared resources when the system's congestion level changes; the importance of shared resources becomes more valuable when congested. 



==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/06_design_details.tex <==
\section{Estimating prices with Litmus}
\label{sec:designDetails}

% The providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}, before using Litmus pricing. The numbers in both tables are the slowdowns of codes while testing the system congestion. Shortly, the congestion table is filled with the slowdowns of startup codes, and the performance table is filled with the slowdowns of reference benchmarks. Litmus pricing needs three steps to charge the final price with a discount. First, the providers assess the system's congestion at multiple levels and range them in a table. This step completes the congestion table. Second, the providers study the impact of congestion on tenants' functions and complete the performance table. Lastly, the service provider determines a tenant's price based on the two tables. 
Before using Litmus pricing, service providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}. The congestion table lists the slowdowns during the startup phases, whereas the performance table lists the slowdowns of reference functions. Litmus pricing needs three steps to determine the final price with a discount. First, providers assess system congestion at multiple levels and record the results in the congestion table. Second, providers analyze the impact of congestion on reference functions and fill out the performance table. Lastly, providers determine a tenant's price based on the data from both tables.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tables}\\
\caption{Congestion and performance tables: numbers in both tables indicate the slowdowns of startup codes and reference functions, collected with CT-Gen and MB-Gen}
\vspace{-0.7em}
\label{fig:litmust_tables}
\end{figure}

\textbf{Step 1, Defining Congestion Levels:} We manage the system's congestion levels using two traffic generators that create a range of congestion states by stressing shared resources differently. The traffic generator is multi-threaded, creating traffic in shared resources to incur congestion, with each thread running on a separate core. We rank the stress levels from 1 to 32 by changing the number of active threads running on distinct cores. Entries from top to bottom in the congestion table indicate increasing stress levels.

% \begin{figure}[h]
% \centering
% \vspace{-1.5em}
% \includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
% \vspace{-1em}
% \caption{stressing program's instruction, L3 accesses and L3 misses }
% \vspace{-0.5em}
% \label{fig:stressing_specs}
% \end{figure}

% \textbf{Step 2. Measuring System Congestion:} Measuring the current level of system congestion that may influence a function's performance is a crucial challenge. If we assume that the platform does not have pre-profiled information about a function's performance, the platform cannot figure out whether co-running functions influenced the function. Additionally, the serverless platform's fast-changing states with massive short-living functions make the assessment even more complicated, requiring quick and frequent examinations.

% Meanwhile, measuring the amount of a system's congestion and its impact on performance is a crucial challenge. This challenge particularly stands apparent when being demanded to quantify the impact of the congestion on a running application without pre-profiled information about the application. Moreover, the serverless platform's fast-changing system states with \hl{numerous} short-lived functions make the assessment even more complicated, requiring quick and frequent performance examinations.
Measuring the amount of system congestion and its impact on performance is a crucial challenge. This challenge becomes particularly pronounced when trying to quantify the impact of the congestion on a running application without pre-profiled information about the application. The fast-changing system states of a serverless platform, with numerous short-lived functions, further complicate the assessment, necessitating quick and frequent performance examinations.

% Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. The proposal is based on the observation that high-level languages, such as Python and Node.js, used in serverless computing have long startup times to accommodate their runtime environments. Since the inception of serverless computing, these startups have been recognized as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests leverage these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests further validated that all tested functions exhibited similar performance characteristics during their startups. 
Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. This method leverages our observation that high-level languages like Python and Node.js, commonly used in serverless computing, have lengthy startup phases to accommodate their runtime environments. Since the inception of serverless computing, these startup delays have been identified as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests exploit these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests have validated that tested functions exhibit similar performance characteristics during startup phases. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_all}\\
% \caption{IPC for serverless applications with different runtimes in the first 100 milliseconds of their execution}
% \vspace{-0.5em}
% \label{fig:startupIPC_all}
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped}\\
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-1}\\
\includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped_3}\\
% \caption{IPC for serverless applications grouped by language runtime in the first 100 milliseconds of their execution}
\caption{IPC of serverless applications based on languages (Go, Python, and NodeJS) during their startup phase}
% \vspace{-0.7em}
\label{fig:startupIPC_grouped}
\end{figure}

% Figure~\ref{fig:startupIPC_grouped} depicts the fluctuation in IPC (Instructions Per Cycle) of a function during the first milliseconds of its execution. The x-axis shows a time flow since the beginning; every tick indicates a millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language, and the throughput of each group is represented in separate figures. Although figures exhibit different patterns, functions in the same figure display notable similarities. The figures imply that functions written in the same language have nearly identical startups.
Figure~\ref{fig:startupIPC_grouped} depicts a function's fluctuation in IPC (Instructions Per Cycle) during its startup phases. The x-axis represents the time elapsed since the beginning, with each tick indicating one millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language runtime, and the IPC of each group is presented in separate figures. As shown in these figures, functions in the same figure show notable similarities. This implies that functions written in the same language have nearly identical startups.

% The startup of a runtime usually includes bursts of memory reads to load images and libraries, which can probe the traffic in the shared resources. By conducting a Litmus test before executing every tenant's codes, the providers can observe the system state for the function. Meanwhile, the providers also need to study how the startup codes perform in different system states. They complete the congestion tables by performing the Litmus tests with the startups written in three languages while varying the congestion levels. To this end, the information in the congestion table is looked up when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}. 
% estimating the system's state upon receiving a result of a function's Litmus test. 
The startup of a runtime typically includes bursts of memory reads to load images and libraries, which can be used to probe the traffic in shared resources. By conducting a Litmus test before executing a tenant's function, providers can assess the system state. Meanwhile, providers also need to study how startup phases perform under different system states. They complete the congestion tables by conducting the Litmus tests with startups written in three languages while varying congestion levels. This information from the congestion table is then referenced when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tests}\\
\caption{Progress of serverless applications on four cores with Litmus tests (dotted arrows) over time}
% \vspace{-0.5em}
\label{fig:Litmus_tests}
\end{figure}

% Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests. The Litmus tests examine the level of system congestion with every function startup. \hl{Many} concurrent functions in serverless offer frequent test opportunities. Function\#1 is a memory-intensive function that raises a congestion level. While active, Litmus tests measure the congestion level above 8. After Function\#1's completion, the next Litmus test detects a non-congested system with a congestion level below 3. However, with the start of another heavy function, function\#2, the Litmus tests measure the new congestion in the system.
Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests, which examine the level of system congestion during each function's startup. Many concurrent functions in serverless offer frequent opportunities for testing. Function \#1, which is memory-intensive, causes congestion levels to rise above 8 during its execution. A Litmus test in Core 3 detects this congestion. After Function \#1 is complete, a subsequent Litmus test indicates a non-congested system with a congestion level below 3. However, during another resource-intensive function, Function \#2, the Litmus test identifies new system congestion with a level above 9.  

% \textbf{Step 2. Measuring the Impact of Congestion:} Although discerning the system congestion through the Litmus test, estimating its impact on a user's application is another challenge. This work proposes a discount based on the pre-studied impacts on reference functions, assuming the user's functions are alike. For this, the service providers need to select reference functions that represent users' functions running on their systems. In this work, we select the workloads in \hl{Section 2} as our reference applications. 
\textbf{Step 2, Measuring the Impact of Congestion:} Discerning system congestion through the Litmus test solves only one of the two challenges; the other is determining its impact on a tenant's function. Different tenants' functions could experience varying degrees of slowdown under the same congestion level. To address this, we propose using pre-selected reference functions to analyze these impacts, thereby avoiding the cost of runtime profiling. For this, providers need to carefully select reference functions that represent tenants' functions operating on the systems, as these selections influence the overall accuracy of congestion measurement. Later, in Section~\ref{sec:evaluation}, our tests will show that pre-selected reference functions can effectively represent unknown user applications. For this study, the selected reference applications (* marked) are listed in  Table~\ref{tb:benchmarks}. 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/refSlowdownStressing14}\\
% \includegraphics[width=1\columnwidth]{./fig/slowdownStressing16}\\
\caption{\(T_{private}\), \(T_{shared}\), and \(T_{total}\) of serverless applications that run with MB-Gen at stress level 14, normalized to their execution time when they run alone}
% \vspace{-0.5em}
\label{fig:refSlowdownStressing14}
\end{figure}

% Once the reference functions are ready, the providers study the slowdowns of the reference functions while varying different congestion levels again. This study completes the performance table in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. Again, our two traffic generators create two separate sub-tables. All entries in this table are 1-to-1 mapped to entries in the congestion table. The providers estimate a general function's slowdown when having a certain congestion level using this 1-to-1 mapping.
Once the reference functions are ready, providers analyze their slowdowns under varying congestion levels. This analysis completes the performance table shown in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. With two traffic generators, providers can complete another set of two sub-tables for the performance table. All entries in this table are mapped 1-to-1 to entries in the congestion table. Providers can estimate a general function's slowdown at a given congestion level using this one-to-one mapping.

% Figure~\ref{fig:refSlowdownStressing14} shows the reference functions' slowdowns when stressing the system. The X-axis shows different functions, each consisting of three bars: the first two bars show the CPI during each time slice, \(T_{private}\) and \(T_{shared}\), and the last bar shows the CPI of an entire execution. The figure shows that the tested functions suffer from different amounts of slowdowns, although the tests maintain consistent stress levels. \hl{The last group} shows the gmean of all the slowdowns, which is used when providers estimate a function's slowdown later. 
Figure~\ref{fig:refSlowdownStressing14} shows an example of the reference functions' slowdowns when stressing the system. The X-axis shows tested functions, each depicted with three bars: the first two bars show \(T_{private}\) and \(T_{shared}\), while the last bar shows the total execution time, all normalized to their execution time when running alone without interference. The figure shows that the tested functions experience varying degrees of slowdown despite consistent stress levels maintained during the tests. The next-to-last group shows the gmean of all the slowdowns, which providers use to estimate a function's slowdown later.

% \hl{This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/referenceStartupSlowdownRev}\\
\caption{The correlation between the slowdown of Python's startup phase and the slowdown of reference applications. From left, (a) \(T_{private}\), (b) \(T_{shared}\), and (c) \(T_{total}\), normalized to the execution time when running alone}
\label{fig:referenceStartupSlowdownRev}
\end{figure}

% \textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while a range of congestion levels is continuous, the tables only contain a few slowdowns in discrete intervals. Thus, providers need a model that returns an estimated slowdown when receiving a congestion level as an input. In our tests, we employ a linear regression to achieve the model.
\textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while congestion levels vary continuously, the tables only contain slowdowns at discrete intervals. Therefore, providers need a model that estimates the slowdown for any given congestion level. In our tests, we employ linear regression to develop the model.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/interpolation}\\
\caption{Estimating a function's slowdown with logarithmic interpolation}
\label{fig:interpolation}
\end{figure}

% Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding references' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). We employed two traffic generators to extrapolate a more precise congestion level, yielding two sub-tables in both the congestion and the performance tables. Consequently, the figure presents two linear regression models, each associated with a different traffic generator. 
Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding reference applications' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). To extrapolate a precise congestion level, we created two sub-tables within both the congestion and performance tables using two distinct traffic generators. As a result, the figure depicts two linear regression lines (red and blue dotted lines), each associated with a different traffic generator.

% The provider needs to estimate the function's slowdown to uncover its price. However, the above two regression models return two vastly different slowdowns. Then, the providers need to determine which model is close to the current environment. We think the two models reflect two extreme congestions that the traffic generators create, one before the L3 and one after the L3. CT-Gen creates massive traffic from the core to the L3 cache, which filters the traffic, preventing the operations from consuming the memory bandwidth. MB-Gen also creates huge traffic but consumes the memory bandwidth and replaces L3 blocks. Since each traffic generator creates an extreme case, the machine state could be intermediate with congestion in the range between the two congestions created by CT-Gen and MB-Gen. However, Litmus pricing cannot answer this question with only the startup's slowdown. 

% To address this question, we note that the system's L3 misses are a critical indicator closely related to a function's performance. Functions suffer more when the system experiences more L3 misses, which stresses the cache space and off-chip memory bandwidth. Accordingly, Litmus test collects the system's L3 miss count as a supplementary index, which tells more about the crowdedness of shared resources.

These regression models return two different slowdowns. To estimate a function's slowdown, providers must determine which model reflects the current environment more accurately. The traffic generators create two extreme congestion scenarios: one before the L3 cache and one after. CT-Gen generates substantial traffic from the core to the L3 cache that filters the traffic and prevents operations from consuming memory bandwidth. Conversely, MB-Gen also generates massive traffic but consumes memory bandwidth and repeatedly evicts L3 cache blocks. Because each traffic generator represents a distinct extreme case, the actual machine state could fall somewhere between the two congestion levels created by CT-Gen and MB-Gen. However, Litmus pricing requires more than just the startup slowdown to identify the machine's state in these models. Thus, we have enabled Litmus tests to gather the system's L3 miss count as a supplementary metric that offers deeper insights into the crowdedness of shared resources.


% \hl{Figure 1} shows how to use the L3 cache misses with the performance sub-tables. The two traffic generators make the upper and lower boundary of the L3 miss rates. When performing a Litmus test, if the test's L3 miss rate is XXX, close to the L3 misses with CT-Gen, we can conclude that the congestion occurs before the L3 cache and select the expected slowdown of XXX. On the contrary, we choose XXX, in case the L3 miss rate is XXX, close to the L3 misses with MB-Gen. If the test's L3 miss rate is in-between, we interpolate the two slowdowns based on the L3 misses, assuming congestion in both resources. 
% Finally, we determine the Rprivate and Rshared based on the expected slowdown from its performance table. Calculating Rprivate and Rshared takes the same steps. The final discount price is computed using the equation with the computed rates. 

% Figure~\ref{fig:interpolation} shows how we employ the L3 misses when estimating the slowdown. The two traffic generators make the upper and lower boundary of the L3 misses. If a Litmus test reports the L3 miss count is 10, close to the L3 misses with CT-Gen, \textcircled{1}Litmus pricing estimates the discount (=expected slowdown) of the function to be near 1\%. This indicates that the congestion happens before the L3, as what CT-Gen creates. On the contrary, in case the L3 misses are 1000, close to the L3 misses with MB-Gen, \textcircled{2}Litmus pricing estimates the function's discount rate close to 6\%. Meanwhile, if the Litmus test reports the L3 misses as 100, we interpolate the two extreme discounts, 1 and 6, based on the L3 misses, assuming current congestion to stand in between the two extreme congestions. The congestion model in the figure shows how we interpolate with logarithmic interpolation. In this figure, \textcircled{3}applying the logarithmic interpolation to the L3 miss count returns the half-point between CT-Gen's 1\% and MB-Gen's 6\%, which is 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 
Figure~\ref{fig:interpolation} shows our approach to using L3 misses to estimate slowdowns. We created two figures illustrating separate regression models. The left figure (a) is derived from the startup slowdowns and L3 misses with logarithmic regression, indicating L3 misses at specific congestion levels. The right figure (b) is derived from the performance table with linear regression, displaying discounts at specific congestion levels. Each figure depicts two regression lines associated with different traffic generators.

The two traffic generators set the upper and lower boundaries for L3 misses. For instance, if a Litmus test reports 10 L3 misses, close to what CT-Gen generates: \textcircled{1}This suggests congestion occurs before reaching the L3 cache, similar to CT-Gen's scenario. Thus, Litmus pricing estimates the function's discount to be around 1\%. Conversely, if the Litmus test reports 1000 L3 misses, close to MB-Gen's results: \textcircled{2}Litmus pricing estimates the function's discount rate to be approximately 6\%, indicating congestion similar to MB-Gen, where memory bandwidth is heavily consumed and L3 cache blocks are frequently evicted. When the Litmus test reports 100 L3 misses, an interpolation between these extremes is applied: \textcircled{3}Using logarithmic interpolation, Litmus pricing estimates the function's discount rate to be midway between CT-Gen's 1\% and MB-Gen's 6\%, resulting in approximately 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 



==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/08_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \textbf{Litmus price \& error:}
% We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, and the other consists of selected reference applications to obtain the linear regression models for Litmus pricing. The discount models plug into the Litmus pricing used in our tests. For this experiment, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown.
We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, while the other consists of chosen reference applications to derive linear regression models for Litmus pricing. The discount models plug into the Litmus pricing employed in the tests. In this study, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown. 

% % original version
% We maintain the congestion state consistent across all tests, co-running each function with 26 other functions. Using Perf~\cite{perfWiki}, we collect the three key stats: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup, which implies the congestion level in these tests, as well as the discount rates that every function receives. We execute every function 100 times and collect the average of the function's \(T_{private}\) and \(T_{shared}\). Finally, we compute each function's \(P_{private}\), \(P_{shared}\), and \(P\), the total price, by summing \(P_{private}\) and \(P_{shared}\).  

\subsection{One Function Per Core}

% revision version
% We maintain consistent congestion states across all tests by co-running each function with 26 other functions. Using Perf, we collect the three key statistics: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup. These metrics hint at the congestion level during the tests as well as the discount rates that a function receives. Each function is executed 30 times, and the average of its \(T_{private}\) and \(T_{shared}\) is collected. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).
We maintain consistent congestion levels across all tests by co-running each function with 26 other functions. As outlined in Section~\ref{sec:motivation}, whenever a function finishes, another is randomly launched to keep a total of 26 co-running functions. Using Perf~\cite{perfWiki}, we collect three key statistics: \(T_{private}\), \(T_{shared}\), and the machine's L3 misses during the first 45 million instructions of the Python startup. Through these metrics, Litmus pricing estimates the level of system congestion and the discount rates a function receives. Each function is executed 30 times, and we average its \(T_{private}\) and \(T_{shared}\) values. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice26Rev}\\
% \caption{The total price for functions computed via Litmus pricing and ideal prices when co-running with 26 other functions normalized to the commercial price that offers no discount}
\caption{Prices computed via Litmus pricing and ideal prices when co-running with 26 other functions, normalized to the commercial price that offers no discount}
\label{fig:normalizedPrice26Rev}
\end{figure}

% In Figure~\ref{fig:normalizedPrice26}, we can see a minimal difference in the discount rate between the Litmus price and the Ideal price. The average Litmus discount rate stands at 11.5\%, which is only marginally larger by 0.6\% than the average Ideal discount rate of 10.9\%. Also, we can see that the difference between the Litmus price and Ideal price are different among the applications. Certain applications exhibit higher Litmus prices compared to the Ideal price, while conversely, some applications demonstrate smaller Litmus prices. 
 %Figure~\ref{fig:priceErrorRunwith26} shows further details, analyzing the errors in each pricing component. 

% Figure~\ref{fig:normalizedPrice26Rev} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{10.66\%}, which is only marginally larger by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{10.28\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice26Rev} illustrates estimated prices derived from Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices to offset delays in a congested execution environment. The figure shows minimal disparities between the two prices, implying that Litmus pricing offers a reasonable discount. The average discount from Litmus pricing across all functions is 10.7\%, which is only marginally higher by 0.4\% compared to the average slowdown experienced by functions, which stands at 10.3\%, as depicted by the ideal price.

% However, the discount rates per slowdown differ among functions. For instance, float-py's ideal discount rate is \hl{0.05\%}, but it enjoys a \hl{4.31\%} discount with the Litmus pricing. Meanwhile, pager-py's performance drops by \hl{15.63\%} while receiving a \hl{13.87\%} discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more easily affected than the reference when congested. In contrast, float-py runs mostly with private resources, receiving a minor impact from the execution environment. Figure~\ref{fig:priceErrorRunwith26Rev} shows further details, analyzing the differences in each pricing component.
However, the discounts per slowdown differ among functions. For instance, float-py's ideal discount rate is 0.05\%, but it benefits from a 4.3\% discount with Litmus pricing. Conversely, pager-py encounters a 15.6\% performance decline while receiving only a 13.9\% discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more susceptible to congestion than the references. In contrast, float-py predominantly utilizes private resources, resulting in minimal impact from the execution environment. Further insights into these variations in each pricing component are presented in Figure~\ref{fig:priceErrorRunwith26Rev}.


% From figure~\ref{fig:tcore\(T_{private}\)Distr}, we know that \(T_{private}\) dominates the execution time among all applications. The impact from \(T_{private}\) error has a bigger impact on the overall error. The slowdowns due to congestion in private resources are small. Theoretically, there should be no slowdowns when using private resources, but we observed that the congestion still influences it. The observed slowdown is 000, a small difference from an ideal slowdown. Meanwhile, the slowdowns in shared resources are significant. We observe that 

% % \[  Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}}\]

% \[Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{TotalIdealPrice}\]
% \[TotalIdealPrice = R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}\]

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/priceErrorRunwith26Rev}\\
\caption{Weighted errors in prices derived from Litmus pricing, which are compared to ideal prices}
% \vspace{-1em}
\label{fig:priceErrorRunwith26Rev}
\end{figure}

%%% We discuss error
% In figure~\ref{fig:priceErrorRunwith26} we can see that there are some applications receive positive errors and some receive negative errors.  A negative error indicates that our estimated slowdown for that application is higher than its actual slowdown, resulting in greater compensation than the observed performance losses. On the other hand, a positive error indicates that the compensation is smaller than its real slowdown. For most applications, the Litmus price is slightly higher than the Ideal price, with minimal differences. The highest price error is 0.0389 for auth-nj, while the lowest error is 0.007 for dyn-py. The geometric mean of the absolute error is 0.018. 
% Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors that each function experiences. The error rate is computed as the difference between the estimated and the ideal prices over the ideal price. The first two bars show the errors in \(P_{private}\) and \(P_{shared}\), which are weighted by their corresponding ratio in the execution time, considering their impacts, as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. The functions can have two different errors: positive and negative. A positive error indicates that the Litmus-estimated price is higher than its ideal price, implying that it receives smaller compensation than its performance losses. In other words, Litmus pricing estimates its slowdown to be less than its actual slowdown. A negative error implies the opposite; a function's compensation is higher than its slowdown. This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others. Meanwhile, the tenants need to acknowledge the consequences if their functions differ vastly from the reference workloads, heavily relying on shared memory.
Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors each function experiences. The error rate is computed by comparing the estimated prices with the ideal prices and dividing the difference by the ideal prices. The first two bars show errors in \(P_{private}\) and \(P_{shared}\), weighted by their corresponding ratios in execution time, reflecting their impacts as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. Functions may have two types of errors: positive and negative. A positive error means that the estimated price exceeds its ideal price, implying that the compensation received is less than the performance loss incurred. In other words, Litmus pricing underestimates the slowdown relative to the actual slowdown. Conversely, a negative error indicates the opposite; a function's compensation exceeds its slowdown. This discrepancy indicates Litmus pricing may offer varying advantages to different functions, favoring those with lesser slowdowns. Meanwhile, tenants must recognize the consequences if their functions differ vastly from the references, particularly those heavily reliant on shared resources.

% Delete the followings
% This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.

% The largest absolute error is \hl{0.0723} for rate-go, while the smallest absolute error is \hl{0.0039} for \hl{mst-py}. Overall, the Litmus pricing shows minor errors with an average of \hl{0.0231}. With further details, the Litmus pricing accurately estimates the slowdowns in \(P_{private}\) with \hl{0.0175} of an average weighted error rate. \(P_{private}\)'s highest weighted error rate is \hl{0.079}, yet minor, while the lowest rate is only \hl{0.0008}. The weighted error rate for the estimated \(P_{shared}\) is also small. The average error rate for \(P_{shared}\) is \hl{0.0068}, even lower than for \(P_{private}\). \(P_{shared}\)'s highest error rate is \hl{0.0404}.
% The largest absolute error is 0.072, which occurs with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, the Litmus pricing exhibits minor errors, averaging 0.023, \hl{with the estimated discount differing by 22.5\% over the ideal discount.} With more details, Litmus pricing accurately estimates slowdowns in \(P_{private}\), with an average weighted error rate of 0.018. \(P_{private}\)'s highest weighted error rate is 0.08, yet minor, while the lowest rate is only 0.0008. The weighted error rate for estimated \(P_{shared}\) is similarly small, averaging at 0.0068, even lower than for \(P_{private}\). The highest error rate for \(P_{shared}\) stands at 0.04.
The largest absolute error is 0.072, occurring with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, Litmus pricing exhibits minor errors, averaging 0.023. Thus, the estimated discount deviates by 22.5\% from the ideal discount. Note that Litmus pricing aims to match the average discount across all functions by applying a system-wide discount based on the system's congestion level rather than adjusting the discount for each function individually. Consequently, individual functions may experience either positive or negative errors. However, it is noteworthy that the average discount between Litmus and ideal pricing differs by just 0.4\%, as illustrated in Figure~\ref{fig:normalizedPrice26Rev}, satisfying its objectives.
% This policy may incentivize some functions while penalizing others based on shared resource usage. 
Specifically, Litmus pricing estimates slowdowns in \(P_{private}\) with an average weighted error rate of 0.018. The highest for \(P_{private}\) is 0.079, while the lowest is just 0.001. For \(P_{shared}\), the average weighted error rate is even lower, at 0.007. The highest for \(P_{shared}\) is 0.040.


% Litmus employs the average performance of applications to determine the discount rate applied universally. In this context, an application encounters a positive error when its speedup is less than the estimated average speedup across all applications. Also, the error rate depends on the difference between the actual speedup and the estimated average speedup, with larger differences resulting in more significant errors for the given application.
% As discussed in Figure~\ref{fig:TpriTshardDistri}, \(T_{private}\) dominates the execution time across all applications, implying that a small error in the estimated \(T_{private}\) largely influences the execution time. This explains why, for functions that demand little shared resources, such as float-py and chame-py, the error in P is almost identical to that in \(T_{private}\), and errors with \(T_{shared}\) can be overlooked. In contrast, for functions with a larger \(T_{shared}\) ratio, such as pager-py and mst-py, errors in \(T_{shared}\) meaningfully affect the total execution time. Note that the Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price.  

Litmus pricing estimates each pricing component separately with an individual discount rate. For functions that demand minimal shared resources, such as float-py, the errors in P are nearly identical to those in \(T_{private}\), and the errors in \(T_{shared}\) can be overlooked. As shown in Figure~\ref{fig:TpriTshardDistriRev}, \(T_{private}\) dominates the execution time across many applications. While even a small error in the estimated \(T_{private}\) influences the function's execution time, substantial errors in \(T_{shared}\) likely have limited impacts, except for functions that have a relatively meaningful \(T_{shared}\) ratio, such as pager-py and mst-py, whose errors in \(T_{shared}\) are observable in the total price. 

% We emphasize that Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price. We observe that functions have similar slowdowns in \(T_{private}\) with slight variation when congested. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, also estimating reliable total prices since \(T_{private}\) mostly dominates the execution time. The \(T_{shared}\) fluctuates more dynamically across functions with a relatively large error, but the error's impact is little, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}. 
We emphasize that Litmus pricing cannot avoid producing a certain degree of error since it relies on estimation using a few metrics. However, the figure proves that Litmus pricing effectively captures a congested environment and reflects that environment in the price. Under the same congestion level, \(T_{private}\) values of all functions are delayed similarly with a little variation. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, leading to reliable total price estimates since \(T_{private}\) generally dominates execution time. \(T_{shared}\) fluctuates more dynamically across functions and has a relatively larger error, but the impact of this error is minimal, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}.

\begin{figure}[h]
\centering
% \vspace{-5em}
 \includegraphics[width=1\columnwidth]{./fig/normTprivtTshared26Rev}\\
% \vspace{-5.5em}
\caption{\(T_{private}\) \& \(T_{shared}\) of applications when co-running with 26 others, normalized to those when they run alone. The top(black) and bottom(blue) lines are discount rates from Litmus pricing for \(T_{private}\) and \(T_{shared}\)}
% \vspace{-1em}
\label{fig:normTprivtTshared26Rev}
\end{figure}

% To further investigate the price error differences, in igure~\ref{fig:normTprivtTshared}, we explore the \(T_{private}\) speedups across various serverless applications.  
% Notably, the difference between the Litmus discount (L-Discount) and the average speedup is merely 0.006.  This minute difference explains why Litmus can attains such high accuracy. 
%Furthermore, when comparing with figure~\ref{fig:priceErrorRunwith26}, a correlation between the error rate and the speedup differences becomes apparent. 
%For instance, float-py, with the most substantial difference above the Litmus discount, also experiences the most significant negative error rate. 
%Conversely, aes-go, with the smallest speedup, experiences the highest positive error rate.
% % original version
% Figure~\ref{fig:normTprivtTshared} shows the execution time of the baseline normalized to the execution time of each run under congestion. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the functions spend only 3.67\% more time on private resources, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, resulting in precise estimation with a Litmus test. 

% Figure~\ref{fig:normTprivtTshared26Rev} shows the execution time of each function run under congestion normalized to the execution time of the baseline. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the interferences in private resources extend the function execution time only by 5.3\%, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, enabling precise estimation with a Litmus test.
Figure~\ref{fig:normTprivtTshared26Rev} shows the \(T_{private}\) and \(T_{shared}\) of each function, normalized to the same time components of the baseline. The gap between the bar and 1 represents the amount of slowdown that should be translated into ideal discounts. The top (black) and bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that interferences in private resources extend the function execution time by only 5.3\%, implying the performance of the private resources is marginally affected by congestion. Additionally, all functions exhibit similar \(T_{private}\) values with little dispersion, helping precise estimation with Litmus tests.

% Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors are still in an acceptable range since their impacts are small. Functions that have a considerable \(T_{shared}\) ratio become more sensitive to system congestion. Instead, a function, such as float-py, with negligible \(T_{shared}\) ratio gains huge benefits with high discounts while its performance remains firm. This shows that Litmus pricing reflects the dynamically changing values of shared resources when the congestion level alters and encourages functions to be developed to use more private resources. 
Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors remain within an acceptable range as their impacts are minor. Functions that have a considerable \(T_{shared}\) ratio are more sensitive to system congestion. Conversely, a function like float-py, which has a negligible \(T_{shared}\) ratio, gains huge benefits from high discounts while maintaining stable performance under congestion. This shows that Litmus pricing accurately reflects the dynamic values of shared resources when the congestion level changes and incentivizes functions to be developed to use less shared resources. 

% \textbf{Litmus pricing under high congestion:} We test our Litmus pricing under a heavily congested environment to verify its pricing of functions with large slowdowns. To create a crowded environment, we concurrently execute 60 instances of Fibonacci-go, which produces the most L2 misses among our tested functions. 
% We raise the congestion level significantly with 60 co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo} shows the results from the same tests of Figure 11. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.8\%, which is only a 1.7\% difference from the ideal discount of 27.1\% with 2.48\% of an average absolute error. In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.151 and 4.299, which are only 2.45\% and 7.83\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. 
% \textbf{Litmus pricing under high congestion:} We raise the congestion level significantly with \hl{500} co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo500} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.1\%, which is only a 1\% difference from the ideal discount of 27.1\% with 0.088\% of an average absolute error. Litmus pricing discounts slightly more than an actual slowdown, leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% % \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
% \caption{The normalized total price for the applications calculated by using Litmus pricing and ideal prices when co-running with 500 Fibonacci-go}
% \label{fig:normalizedPriceCongested320}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\columnwidth]{./fig/diffStartupPortion-2Rev}\\
%\caption{The slowdown of Python's startup with 25 and 15 million instructions (X-axis) and the slowdown of reference applications (Y-axis). From left, \(T_{private}\), \(T_{shared}\), and \(T_{total}\), normalized to those when running alone}
%\label{fig:diffStartupPortion}
%\end{figure}

% \textbf{Instructions in Startup:} Litmus tests react differently to congestion when performed with different numbers of instructions from the startup phase. For example, Python's startup involves about 45 million instructions. While we have conducted Litmus tests using all these instructions, Figure~\ref{fig:diffStartupPortion} shows the response of these tests when running with the first 15 and 25 million instructions from this set. The figure shows the startups' \(T_{private}\), \(T_{shared}\), and \(T_{total}\) with two traffic generators, as depicted in Figure~\ref{fig:referenceStartupSlowdownRev}. Tests with fewer instructions are more sensitive to cold cache misses but less to interference in the L3 cache. Therefore, as the instruction count in Litmus tests decreases, they become less susceptible to conflicts in shared resources, especially from traffic by MB-Gen. As a result, tests with 25 million instructions exhibit reduced slowdowns. This trend becomes more apparent when running the tests with 15 million instructions, depicting that slowdowns when co-running with MB-Gen become nearly identical to those with CT-Gen. 

%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%







% \textbf{Instructions in Startup:} Python's whole startup phase contains about 45 million instructions. We can further divide the startup phase into smaller pieces with 10 million instructions code chunks. And each code chunk would have its characteristics. They react differently in the same congested environment. In section XXX we use the whole Python's startup portion's slowdown to indexsing the serverless application's slowdown. But, since the co-relationship between these two slowdown in different congestion source are different, one startup \(T_{private}\) slowdown may indicate two application's slowdown. By carefully picking the code chunks we can mitigate the difference between the two normalized slowdowns of the guidance application that correlated to the same startup phase slowdown. 

% Figure~\ref{fig:diffStartupPortion} depicts the correlation between the performance changes in the reference applications and distinct segments of Python's startup phase. From the figure, we see that selecting the first 15 million instructions as our startup phase results in the normalized \(T_{uncore}PerInst\) of the guidance application aligning nearly into a singular trendline. However, there are substantial gaps in the case of \(T_{core}PerInst\) with this code segment. Thus, we should pick xxx-xxx as our startup phase representation code for the normalized \(T_{core}PerInst\). We think that this can be used to mitigate the differences. But, we should be careful to use the small code chunks for the following reasons: First, only measuring the small portion can be a problem. The results might be too dynamic. Second, since we only measure this small portion there might be a huge execution period that cannot be covered.

% Continue to work from here

\subsection{Temporal CPU Sharing}
\label{sec:temporalCPUSharing}

The previous evaluation assumes an isolated environment where a CPU is assigned exclusively to an active function during execution, disallowing temporal sharing between functions through context-switching. While this setup ensures strict performance isolation, it inherently limits resource utilization. Conversely, enhancing utilization by permitting temporal CPU sharing among functions complicates price estimation. We explore how Litmus pricing can be applied in a less restrictive environment that permits sharing, where functions can temporarily share the same CPU and are not bound exclusively to specific cores. 

In this section, we deploy a testing function to co-run with 160 other functions across 16 cores without exclusive core assignments, assuming an average of 10 functions share a core. The reduction in the number of cores tested was necessitated by our system's memory limitations, as certain functions require significant memory space.

% \textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, the subsequent function clears the displaced one's cached data. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, the slowdown with extra sharing financially benefits the provider; we thereby argue that the extent of sharing should be factored into Litmus pricing as another discount factor.
\textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, a subsequent function evicts the cached data of the displaced one. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, delayed execution due to extra sharing financially benefits the providers. Thus, we argue that the extent of temporal sharing should be incorporated into Litmus pricing as another discount factor.

Figure~\ref{fig:csImpactor} depicts the switching overheads as concurrently running functions increase. The figure demonstrates that the sharing overhead follows a logarithmic growth pattern and stabilizes at around 20 co-running functions. Furthermore, we discovered that the switching overheads predominantly affect \(T_{private}\). Consequently, Litmus pricing needs to calibrate \(T_{private}\) to account for the impacts of sharing before estimating the slowdown using the performance table.

Figure~\ref{fig:normalizedPrice160Method1} illustrates the discounted price reflecting this adjustment. In our configuration, with an average of 10 functions per core, we divide \(T_{private}\) by 1.025 before estimating the slowdown. In this figure, Litmus pricing estimates an average discount of 14.5\%, which falls 2.9\% short of the ideal discount of 17.4\%. While most benchmarks receive discounts lower than ideal, aes-py stands out with the largest error of 9.9\%, which is 6.9\% less than its ideal discount of 16.8\%.

\begin{figure}
\centering
% \includegraphics[width=1\columnwidth]{./fig/csImpactor}\\
\includegraphics[width=1\columnwidth]{./fig/csImpactor2}\\
\caption{\(T_{private}\) of functions over different co-running counts in the same core, normalized to when running alone}
% \vspace{-1em}
\label{fig:csImpactor}
\end{figure}

\begin{figure}
\centering
% \vspace{-1.2em}
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160Method1}\\
\caption{Prices derived from Litmus pricing (Method 1) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
% \vspace{-0.5em}
\label{fig:normalizedPrice160Method1}
\end{figure}

% In Figure~\ref{fig:normalizedPrice160Method1} we use the the same congestion and performance tables that we collected in the restricted environment. When checking the tables instead of using the original startup slowdown of tcore we use an adjusted slowdown by dividing the context switch impact factor. From figure~\ref{fig:normalizedPrice160Method1} we can see that the average Litums discount is 14.65\%, 3.01\% less than what they should receive compared to the ideal discount of 17.67\%. Most applications receive a smaller discount than the ideal price. The largest error is on aes-py with Litmus discount of 9.85\%, 6.87\% smaller than the ideal discount of 16.72\%. The smallest error is on dyn-py. It's Litmus discount is 22.45\%, only 0.47\% larger than the ideal discount of 21.97\%.

\textbf{Method 2, Updating Performance Tables:} Rather than reusing the performance/congestion tables designed for restrictive environments, arranging new tables for the sharing-enabled environments returns better accuracy. Although the notion of preparing separate tables for various sharing levels may seem challenging, we argue that only one or a few extra tables for heavily crowded systems would suffice, given that commercial systems are typically heavily crowded. Again, we emphasize that the impact of function co-placement stabilizes above a certain co-placement count, as shown in Figure~\ref{fig:csImpactor}.

For this test, we prepared new performance/congestion tables for the environment described above, where a testing function is assumed to co-locate and compete for a core with 9 other functions. Moreover, considering the scenario where a switched-out function has a low chance of being rescheduled to the same core, instead of assigning 10 functions to a specific core, we ran 50 functions across 5 dedicated cores; each can run on any of the 5 cores. We managed the congestion levels in shared resources using traffic generators on the other cores, as outlined in Section~\ref{sec:designDetails}.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPrice160}
% \vspace{-0.6em}
\end{figure}

% Figure~\ref{fig:normalizedPrice160} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{17.29\%}, which is only marginally smaller by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{17.67\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice160} shows the prices obtained from Litmus pricing with the new tables, which are normalized to those from commercial sources. Once more, as in Figure~\ref{fig:normalizedPrice26Rev}, the figure reveals marginal distinctions between the two price points, suggesting that Litmus pricing continues to offer a reasonable discount. Across all functions, the average discount provided by Litmus pricing stands at 17.2\%, merely 0.2\% less than the ideal discount of 17.4\%.


==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/09_sensitivity.tex <==
\section{Sensitivity}
\label{sec:sensitivity}

While the aforementioned tests highlight Litmus's potential, we recognize the need for more compelling results. This section expands our analysis and examines Litmus pricing from various angles across diverse system environments.

% \textbf{Heavy Congestions:} We raise the congestion level significantly with 320 co-running applications to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. The Litmus pricing is still close to the ideal price, discounting the price by 20.00\%, which is only a 1.46\% difference from the ideal discount of 21.46\%. The highest Litmus discount is 26.01\% for dyn-py. It has an error of 2.83\% compared with the ideal discount.
\textbf{Heavy Congestion:} We significantly escalate the congestion level to verify Litmus pricing under conditions of substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} presents the outcomes of the same tests depicted in Figure~\ref{fig:normalizedPrice160} but with 320 co-running functions. Not only did we increase the function count, but we also specifically selected 8 memory-intensive functions, aes-py, compre-py, thum-py, bfs-py, auth-py, fib-go, geo-go, and profile-go, that produce the most L2 cache misses among the tested functions to create heavy congestion in shared resources deliberately. Even under such intensified congestion, Litmus pricing produces results remarkably close to the ideal price, discounting the price by 20.0\%, which deviates by merely 1.5\% from the ideal discount of 21.5\%. The highest discount by Litmus pricing is 26.0\% for dyn-py, a minor error of 2.8\% compared to the ideal discount.


% leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 320 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPriceCongested320}
% \vspace{-1em}
\end{figure}

\textbf{CPU Frequency:} Modern CPUs feature dynamic CPU frequency adjustments, which are controlled via software or hardware. A hardware technique like Intel Turbo Technology autonomously adjusts the CPU frequency based on the CPU's power and thermal budgets, allowing the CPU to operate at higher frequencies when conditions permit and lower frequencies under heavy load. Prior tests assumed that the frequencies were fixed and strictly managed by service providers who had knowledge of when and to what extent frequency adjustments were necessary. Also, we evaluated Litmus pricing under the other scenarios where CPU frequencies were not fixed, providing more dynamic perspectives.

% Figure~\ref{fig:normalizedPrice160unset} illustrates the prices from the Litmus pricing and the ideal price, which are normalized to commercial prices. We tested it under the configuration in Section 7.2 with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, the Litmus pricing's discount is lowered from 17.16\% to 16.84\%, while the ideal discount rate is decreased from 17.42\% to 17.31\%. Still, the discount rate difference from the ideal price is only 0.47\% without setting the CPU frequency. We observed that the CPU frequency changes rarely when the system runs with 160 functions. Overall, the varying frequency made a minor impact on performance as well as the pricing scheme. 
Figure~\ref{fig:normalizedPrice160unset} illustrates the prices derived from Litmus pricing alongside the ideal prices, both normalized to commercial prices. This evaluation was conducted under the configuration outlined in Section~\ref{sec:temporalCPUSharing} with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, we observe a slight decrease in Litmus pricing's discount, from 17.2\% to 16.8\%, while the ideal discount rate decreases from 17.4\% to 17.3\%. Still, even without fixed CPU frequencies, the difference in the discount rate from the ideal price is only 0.5\%. We noted that CPU frequency changes were infrequent when the system operated with 160 functions. Overall, the variation in frequency had a negligible impact on Litmus pricing.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160unset}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others with unfixed CPU frequencies, both normalized to commercial prices}
\label{fig:normalizedPrice160unset}
% \vspace{-1em}
\end{figure}

% All the above experiments are done on Intel Xeon Gold 5218(Cascade Lake). We also perform our scheme on another CPU architecture, Intel Xeon Silver 4314(Ice Lake-SP). 
\textbf{CPU Architecture:} Ensuring the validity of Litmus pricing across different architectures is crucial. Our Litmus tests rely on the performance counter that measures a stall count due to L2 cache misses (cycle\_activity.stalls\_L2\_miss)~\cite{perfMonEvents}, supported by Intel's CPUs. Unfortunately, other vendors like AMD do not yet offer the same performance counter~\cite{amdPMC}, restricting our tests to Intel CPUs. Alternatively, we conducted tests on another Intel CPU based on the Ice Lake architecture, Xeon Silver 4314, to broaden the scope of our analysis.

\begin{figure}[b]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun70kiwi}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 70 others on Xeon Silver 4314, both normalized to commercial prices}
\label{fig:normalizedPriceCorun70kiwi}
\end{figure}

% Because of the limitation of our memory size, we test Limtmus with 70 co-running applications. In this test, we use method 2 introduced in section~\ref{sec:temporalCPUSharing}. We first conduct the congestion and performance tables with 50 applications running in the first 5 cores. Then for the evaluation, we run 70 applications in the first 7 cores to let our testing application compete with 9 other applications for a core.  Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus discounting the tenant only pays 82.52\% commercial price. It's 0.696\% less than with the ideal discount.
Once again, this evaluation was conducted following the configuration outlined in Section~\ref{sec:temporalCPUSharing}, albeit with 70 co-running functions, limited by the main memory capacity of 128GB. Following Method 2, we constructed new congestion and performance tables with 50 functions running across 5 cores. Then, we ran 70 functions across 7 cores to match the competition count, averaging 10 functions per core. Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus pricing, the tenant only pays 82.5\% of the commercial prices, which is merely 0.7\% less than the ideal price.

% \textbf{Per-core Function Count:} When altering the co-located applications in each core the performance of the application can also be influenced. In this test, we put 240 applications in the first 16 cores. The testing application is competing with 14 other applications. We used the same congestion and performance tables from section~\ref{sec:temporalCPUSharing} method 2. Figure~\ref{fig:normalizedPriceCorun15} presents the results. The error of Litmus pricing is 1.23\% with The average discount of 16.69\%. The ideal discount is 17.92\%. The mean price of Litmus is larger than the ideal price because we are using the tables that are made based on 10 applications per-core. The context-switching overhead is larger. But, from figure~\ref{fig:csImpactor} we know that there is a diminishing impact of per-core application count. The error of the Litmus pricing is still under control when we increase the per-core application count.
\textbf{CPU Sharing Overhead:} The co-located function count determines the level of interference, impacting a function's performance differently. To assess Litmus pricing under various co-running function counts, we increased the function count to 240 from the configuration outlined in Section~\ref{sec:temporalCPUSharing}, making an average of 15 functions running on each core. However, we reused the performance and congestion tables generated in Section~\ref{sec:temporalCPUSharing}. Figure~\ref{fig:normalizedPriceCorun15} illustrates the results, where the Litmus pricing's error is 1.2\% with an average discount of 16.7\%, compared to the ideal of 17.9\%. Despite reusing the tables constructed for 10 co-running functions per core, the error remains negligible. This outcome aligns with Figure~\ref{fig:csImpactor}, which highlights the diminishing impact of temporal sharing when running more than 10 co-running functions. Given the perpetual overcrowding of commercial systems, any configuration gap between the environment where constructing the tables and where conducting tests is expected to remain minor and easily manageable.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun15}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 15 functions per core and reusing tables, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun15}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun160smt}
\end{figure}

\textbf{Simultaneous Multithreading (SMT):} SMT is a technique aimed at maximizing resource utilization by enabling multiple threads to execute concurrently on the same core, extending the shared resource domain across the entire processor. However, while SMT enhances resource utilization, it significantly complicates the measurement of interference impact. Moreover, SMT introduces additional side channels, thereby increasing the processor's vulnerability to security attacks. Due to these concerns, serverless platforms like Amazon Lambda disable SMT in their systems~\cite{schall2023warming,agache2020firecracker,schall2022lukewarm}. Nonetheless, we have conducted a study to assess the impact of SMT on our Litmus pricing methodology.

% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
% \caption{Prices computed via Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, normalized to the commercial prices}
% \vspace{-0.5em}
% \label{fig:normalizedPriceCorun160smt}
% \end{figure}

% To generate the performance/congestion tables, we executed 50 applications across 5 dedicated physical cores. In this way, the testing function is co-located with 9 other applications in the same virtual core and 19 other applications in the same physical core. Fiugre~\ref{fig:normalizedPriceCorun160smt} illustrates the results. The first thing we notice is that the normalized price is much smaller compared with the setups without SMT turned on. The average discount of Litmus is 45.42\% which is 1.9\% smaller than the average ideal discount of 47.32\%.
To construct the performance and congestion tables, we executed 50 applications across 5 physically separated cores, allowing an average of 10 functions to share two virtual cores. Figure~\ref{fig:normalizedPriceCorun160smt} illustrates the results,  presenting prices derived from Litmus pricing and ideal prices, both normalized to commercial prices without discounts. The normalized price experiences a significant drop compared to other configurations, highlighting the impact of heavy congestion within a physical core. The ideal price, which assumes no interference, stands at 47.3\% of the commercial price. Meanwhile, Litmus pricing offers a discount of 45.4\%, which is only 1.9\% less, confirming the effectiveness of Litmus pricing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Node JS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Nodejs Startup:}NodeJs is another well-adopted language in serverless platforms besides Python. It's one of the earliest languages to be supported by AWS Lambda ~\cite{serverless1}. From Section~\ref{sec:designDetails} we see that NodeJs has a long startup phase which makes it a great candidate when we need to pick a language startup phase for the Litmus test. 

%\begin{figure}[h]
%\centering
%\vspace{-0.5em}
%\includegraphics[width=1\columnwidth]{./fig/njReferenceStartupSlowdown}\\
%\vspace{-1em}
%\caption{The correlation between the normalized NodeJs's startup phase and the normalized reference applications.}
%\vspace{-0.5em}
%\label{fig:njReferenceStartupSlowdown}
%\end{figure}

%Figure~\ref{fig:njReferenceStartupSlowdown} shows the correlation between NodeJs startup phases and reference applications. After applying the Litmus test with NodeJs applications, with this figure, we can use the slowdown of the NodeJs startup phase to find the corresponding system congestion level and the discount rate for both private and shared resources. NodeJs has a longer startup phase compared with Python. It gives us more room when picking the most suitable portions of the startup phase. We can choose the language to be used for the Litmus test based on the density of the startup phase. 


==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/10_related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Serverless:} Many works address the performance bottleneck of serverless execution~\cite{du2020catalyzer}~\cite{agarwal2021reinforcement}~\cite{roy2022icebreaker}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Schall et al.~\cite{schall2022lukewarm} record and reload the instructions to reduce the front-end stalls when reaccessing the same application. Jovan et al.~\cite{stojkovic2023specfaas} focus on the performance of an application chain. They break the execution flow and speculative execute the functions. However, we are focusing on the price which is one of the most important potions of the cloud ecosystem.

% For the cloud providers, accommodating more tenants in a machine is a key strategy, gaining higher profits by maximizing the utilization of their machines. However, the approach inevitably introduces interference between tenants, slowing down applications unpredictably. Thus, prior researchers solved this challenge by allowing the tenants more non-biased, predictable, quality services~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed a clustering-based cache partitioning to remove unfairness between tenants. Rohan et al.~\cite{roy2021satori} simultaneously control multiple architectural resources to aim for both fairness and throughput. However, offering fairness inevitably sacrifices resource utilization. Thus, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} solve the unfairness uniquely by adjusting their prices while leaving the unfairness at a certain degree. This paper follows this direction but explores a more practical solution in serverless computing. 

Cloud providers strive to maximize profits by accommodating more tenants on their machines, which inevitably introduces interference between tenants, leading to unpredictable application slowdowns. To address this challenge, prior researchers have focused on providing tenants with a more unbiased and predictable quality of service~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed clustering-based cache partitioning to mitigate unfairness between tenants. Rohan et al.~\cite{roy2021satori} aimed for both fairness and throughput by simultaneously controlling multiple architectural resources. However, achieving fairness comes at the cost of sacrificing resource utilization. In contrast, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} addressed the unfairness by adjusting their prices while accepting a certain degree of unfairness. Our study follows a similar direction but explores a more practical solution within the context of serverless computing.

% delete the following section: the approaches are against our scheme. 
% \textbf{Serverless Computing:} Many studies focus on reducing the latencies of serverless applications~\cite{cadden2020seuss,oakes2018sock,wang2019replayable,jia2021boki}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Ustiugov et al.~\cite{ustiugov2021benchmarking} record and prefetches the functions’ stable working set of guest memory pages to further reduce the function's startup time. Wei et al.~\cite{wei2023no} remote forking the serverless functions to reduce the cold start latency while limiting the resource usage. Schall et al. record and reload the instructions~\cite{schall2022lukewarm} or the BTB entries ~\cite{schall2023warming} to reduce the front-end stalls when reaccessing the same application. 
% \hl{Litmus is orthogonal to these approaches and can be adopted together.}

==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Serverless computing is a key technology in present cloud computing, offering numerous advantages. One primary advantage is its effective cost-saving, as tenants only pay for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion. While tenants suffer slowdowns, they also have to pay more for the slowdowns. Unlike prior approaches that aim to maintain quality of service, this paper discounts the tenant's cost to compensate for the loss. Litmus pricing proposed in this work monitors the machine states and adjusts the tenants' costs. The congestion level can be frequently gauged before every function using the proposed Litmus test, an effectively lightweight testing approach. Our tests show that Litmus offers near-ideal prices with a 0.38\% difference, compared to the ideal price that discounts proportional to its slowdown. 
Serverless computing is a key technology in contemporary cloud computing, offering a range of benefits. One primary advantage is effective cost-saving, as tenants are billed only for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion, which not only results in slowdowns but also higher costs for tenants. Rather than aiming to maintain service quality, this paper suggests discounting tenants' costs to compensate for performance losses. Litmus pricing proposed in this work monitors machine states through Litmus tests and adjusts tenant costs accordingly. The Litmus test is a lightweight testing approach for serverless platforms, which assesses the machine's congestion level before starting a user's function. Our tests prove that Litmus pricing offers nearly ideal prices in heavily congested environments, with an average deviation of just 0.2\% from the ideal price that adjusts discounts in proportion to the slowdown experienced.


==> cmhpyvftcvqmzsrycsqstdrkwqtxtknq/12_ack.tex <==
\section{Acknowledgment}
\label{ack}

We would like to thank our reviewers for their valuable feedback to improve this paper. This work was supported by NSF CAREER Award CCF-2146475.


==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/00_abstract.tex <==
\begin{abstract}

% Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While the providers can utilize their machines more efficiently, the tenants only need to pay for the resources they consume. However, a serverless system co-runs thousands of short-living functions concurrently to maximize resource utilization, bearing frequent state shifts. Meanwhile, when the system gets too congested, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants are also charged higher costs when experiencing slowdowns since all commercial serverless platforms determine the tenants' costs proportional to their execution times.
Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times.

% This paper argues that the cloud providers should compensate the tenants for their loss when the server is over-provisioned. However, estimating the tenant's loss is challenging when there is no pre-profiled information about the function. Prior studies showed assessing the tenant's loss introduces heavy overheads. Instead, this paper proposes a new pricing model, Litmus pricing, which offers discounts based on the machine's state while presuming the tenant's loss under the state. To monitor the machine state correctly, Litmus pricing frequently conducts Litmus tests, an effectively lightweight solution to measure system congestion. Our experiments show that Litmus pricing can detect the impact of system congestion and offer near-ideal prices, with only a 0.38\% price difference. 
This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2\% price difference on average, in a heavily congested system.

\end{abstract}


==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Serverless computing is growing fast, satisfying today's high demands for better programmability. It allows tenants to develop their programs as stateless functions in high-level languages such as Python, Go, and JavaScript without concerns with low-level resource management and task scheduling~\cite{serverless2,serverless1,schall2022lukewarm,schall2023warming,mohammad2020SerInWild}. This advantage attracts cloud users, helping them to deploy their programs quickly with minimal effort. Recent reports note that over 50-70\% of cloud users have adopted serverless computing for their tasks~\cite{serverless1}.

% Serverless computing claims a pay-as-you-go pricing model where users only pay for the resources used by their functions. This requires the service provider to monitor and estimate the fine-grained resource usage by each user accurately. However, today's high-performance systems maximize resource efficiency by accommodating multiple applications simultaneously and allowing the resources to be shared by them. Such a shared system raises two major challenges. First, tracking a user's resource usage is a challenging task. While being shared, the system tracks the total usage but not a single user's. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress. These inferences between the applications not only make the system hard to track resource usage, but the users may get charged unfairly due to the delayed execution time.
Serverless computing also benefits tenants financially. Unlike traditional cloud platforms that require tenants to purchase the hardware resources needed to deploy their servers regardless of actual usage~\cite{amazonEC2Pricing}, serverless computing claims a pay-as-you-go pricing model, where tenants only pay for the resources consumed during the execution of their functions, facilitating significant cost savings. Meanwhile, this pricing requires service providers to accurately monitor and estimate each user's fine-grained resource usage~\cite{microsoftAzurePricing,awsLambdaPricing,googleCloudFunctionPricing}. 

% However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared system raises two major challenges. First, tracking a tenant's resource usage is a challenging task. While being shared, the system can only monitor a tenant's use of specific resources. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference between the applications not only makes the system hard to track resource usage, but the tenants may get charged unfairly due to the extended execution time~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}. 
However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared serverless system raises two major challenges. First, tracking a tenant's resource usage becomes challenging, as the system can only monitor a tenant's use of exclusively dedicated resources while the system is shared. Second, and more importantly, co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference not only complicates tracking resource usage but also leads to tenants being charged unfairly due to delayed execution times~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}.

% A serverless platform should provide an isolated runtime environment to a user. Otherwise, we argue that the platform provider must compensate a tenant's loss as a discount when it is not achievable. Therefore, we define a charged fee as fair when it reflects the tenant's slowdowns due to the resource sharing. The following two methods can be used to estimate a fair price under a multi-tenant environment. 
A serverless platform should provide a user with an isolated runtime environment. Otherwise, we argue that the platform provider should compensate a tenant's loss as a discount when the isolation is not achievable. Thus, we define a charged fee as fair when it reflects the tenant's slowdowns caused by resource sharing. The following two methods can be used to offer a fair price in a multi-tenant environment.

% First, strict resource partitioning can divide shared resources into multiple partitions, each assigned to a user exclusively. The user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strictly partitioned resources are well known to cancel the opportunities to utilize the given resource efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delayed execution directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources when requesting them. 
First, strict resource partitioning can divide shared resources into multiple partitions, each assigned exclusively to a user. This means the user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strict partitioning is known to cancel opportunities to utilize resources efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delay directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources they need when requested. 

% Alternatively, a discount-based scheme estimates a user's price relative to its slowdown, discounting from the price when run without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources. Thus, the providers can maximize their hardware utilization and earn more money with given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns or interference they get from co-running tasks without overpaying for exclusive resources.
% The tenants also can get a discount reasonably proportional to the amount of their slowdown when their jobs suffer from interference rather than endeavoring to secure necessary resources exclusively.
Alternatively, a discount-based scheme estimates a user's price relative to the slowdown experienced, discounting from the price when running the task without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources, enabling providers to maximize hardware utilization and generate more revenue with the given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns they experience due to co-running tasks, preventing them from overpaying for lowered service quality.

% While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Even if the platform can measure its execution time, computing the slowdown still requires knowing its baseline, which can be gained when executing it alone. The cloud platform could not pre-profile users' applications for reasons such as mandated privacy when processing confidential information. Even if the platform has such information, the function could operate differently when receiving different inputs. That is to say, online profiling is necessary, which unfortunately requires expensive runtime sampling, as proposed in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. All co-running tasks must be stalled when estimating a task's baseline performance. Massive short-living serverless functions make such a sampling-based solution even more impractical. Frequently sampling the baseline performance of thousands of co-running functions is unrealistic. This motivates a new practical solution that can be adopted in commercial platforms. 
While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Although the platform can measure its execution time, determining the slowdown requires knowing its baseline performance, which can be obtained when it runs without interference. However, such profiling is often prohibited due to security concerns, particularly when the function processes confidential information. Additionally, the function may behave differently, with varying inputs each time it runs. That is to say, online profiling is necessary. Unfortunately, this requires expensive runtime sampling, as presented in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. When assessing baseline performance, all co-running tasks must be stalled. Hundreds to thousands of concurrent short-lived functions make this approach indeed impractical, as frequently sampling the baseline performance of such numerous functions is unrealistic. Thus, a new, practical solution that can be adopted in serverless platforms is needed.

%In either approach, a tenant or a service provider bears the problem's complexity alone. Resource partitioning demands the tenant to know the needed resources while losing opportunities to utilize the resources better. Discounting demands a service provider to estimate the task's slowdown with heavy sampling overheads. Accordingly, both approaches complicate the problem while sacrificing the machine's efficiency. Instead, we claim this problem becomes simpler when both entities participate and carry a portion of the responsibilities. 

% Litmus addresses this challenge by imposing the responsibility on both entities. With Litmus, the serverless platform measures the system congestion that may delay a function's execution when every tenant's function starts. The service provider needs to determine a discount rate for a corresponding congestion state. Meanwhile, the tenant needs to know about a possible slowdown and a corresponding discount. 

% We highlight that both partitioning and sampling complicate the problem while sacrificing the machine's efficiency and can hardly be employed in serverless computing. The approaches in serverless must be lightweight and frequent to deal with the fast-changing environment with thousands of concurrent functions. This paper proposes Litmus pricing that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening the system performance. 
We highlight that both partitioning-based and sampling-based approaches complicate the problem, either sacrificing the machine's efficiency or appearing impractical for serverless computing. Approaches in serverless computing must be lightweight, frequent, and sensitive enough to deal with quickly changing environments with numerous concurrent functions. This paper proposes Litmus pricing, a method that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening system performance. 

% \hl{Measuring the server's congestion status is challenging work. Here, Litmus relies on our key observation that, although not limited, function implementation in serverless computing largely relies on high-level programming languages such as Python and GoLang, which require a relatively long startup. This startup overhead has been considered one of the major challenges in serverless computing. However, Litmus utilizes this startup to measure the system's congestion state. Our analysis of Python and GoLang observed that the activities during the startups are almost identical, with plenty of memory operations, regardless of the functions. Thus, we claim that the startup performance can be an index of the system state.}

% \hl{The Litmus test is based on our insight that the serverless functions perform broadly identical operations, with plenty of memory operations, during their long startups, preparing the runtime environment for the functions. Leveraging this observation, the platform can assess the system's congestion level, which hints at the tenant's discount amount. Additionally, Litmus pricing exploits our second insight that the performance of two resources, private and shared, are affected differently by the congestion. In particular, its impact on private resources is minor and predictable, while many functions significantly rely on them, spending most of their execution time with them. }

% During the execution of every function, Litmus pricing conducts a Litmus test, which measures the level of system congestion with no extra overhead using the function's startup process. The Litmus test is based on the observation that serverless functions perform largely identical operations during their startup time. Those operations usually prepare the runtime and include a large amount of memory access to shared hardware resources. In addition, Litmus pricing splits the hardware resources into "private" and "shared" and proposes charging different ratios on each. This further improves the accuracy of the discount calculation.
During each function's execution, Litmus pricing conducts a Litmus test, which measures the level of system congestion without adding extra overhead, using the function's startup process. Litmus test is based on the observation that serverless functions perform largely identical operations during their startup, typically involving significant memory accesses. Additionally, Litmus pricing splits the hardware resources into "private" and "shared" categories, proposing different charging ratios for each. This approach further enhances the accuracy of the discount calculation.

% In our experiments, the Litmus pricing estimates a tenant's price to be nearly ideal, with a \hl{0.38\%} difference from the ideal price, which discounts tenants proportional to their slowdowns.
% This study investigates Litmus pricing across different environments, ranging from restricted to crowded settings. We verify that crowded environments pose additional challenges. Despite this, Litmus pricing accurately estimates a tenant's price, deviating by only 0.26\% from the ideal price, discounting tenants proportional to their slowdowns.
This study investigates Litmus pricing across diverse environments with varying levels of system congestion. We confirm that crowded environments pose complex challenges. Despite this, Litmus pricing accurately estimates a tenant's cost, deviating by only 0.2\% on average from the ideal price that discounts tenants proportional to slowdowns.



==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/02_background.tex <==
\section{Background}
\label{sec:background}

% \textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while the service providers handle back-end implementation~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers, which are later invoked upon associated events~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. The serverless platform guarantees security by executing the tenant's function in a sandbox such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.
\textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while leaving back-end implementation managed by service providers~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. These functions are later invoked upon associated events. The serverless platform ensures security by executing the tenant's function in a sandbox, such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.

% Each tenant's function is stateless and expected to be short~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using the short-lived functions, the tenant can easily scale by invoking many of the functions without provisioning needed resources for themselves, relying on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. Inherently, massive short-living serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. The tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and clients mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Later, under the pay-as-you-go pricing, the tenant is charged for the consumed resources, typically the product of time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
Each tenant's function is stateless and expected to be short-lived~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using these short-lived functions, tenants can easily scale by invoking many functions without provisioning the needed resources for themselves, relying instead on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. In serverless computing, numerous short-lived serverless workloads run together on a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. Tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and tenants mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% In the traditional cloud, tenants purchase hardware resources for the contracted term to support their applications, which are often expected to be large in a server form. Thus, tenants must pay for the agreed period regardless of actual use. Instead, serverless workloads are generally small and launched on-demand as short-living event handlers. This workload difference develops a unique pricing policy, pay-as-you-go pricing. The tenant is charged only for the consumed resources during the execution, typically the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
In traditional cloud computing, tenants purchase hardware resources for a contracted term to support their applications, which are typically large servers. Thus, tenants must pay for the agreed period regardless of actual usage. In contrast, serverless workloads are generally small and launched on-demand as short-lived event handlers. This difference leads to a unique pricing policy known as pay-as-you-go. Under this model, tenants are charged only for the resources consumed during execution, typically calculated as the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, where Python is utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Also, over 90\% of organizations choose Python and Node.js for their AWS services. Other popular language runtimes are Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer a high level of abstraction from machine codes with good programmability and portability, improving the programmer's productivity. As a result, they have been adopted widely by serverless users. However, such high-level languages typically rely on runtime interpretation, which results in a slow start of program execution with extra launching steps. For instance, in the case of Python, when an application is launched, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the codes are compiled and executed. Once the execution is complete, the Python program is terminated, and all assigned resources are released~\cite{pythonUsage}.
\textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python used in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Over 90\% of organizations choose Python and Node.js for their AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer significant abstraction from machine code with good programmability and portability, which in turn improves programmer productivity. Consequently, they are widely adopted by serverless users. However, high-level languages typically rely on runtime interpretation, leading to slower program startup due to extra launching steps. For example, when an application is launched in Python, the interpreter is first prepared. It then parses command-line arguments and imports necessary modules. Afterward, the codes are compiled and executed. Upon completion, the Python program terminates, and all allocated resources are released~\cite{pythonUsage}.

 
% list of pricing models? 
% Amazon? 
% Google?
% The price is calculated by duration time multiplies to the unit price plus the request charges. The duration time is from the time user's code begins executing until it returns or terminates. The unit price depends on the amount of memory the user allocate to their function. The request charges is based on how many times the function has been invoked minus the free requests~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% may need service agreement here, contention impact

%\textbf{Traditional cloud platforms:} In the context of traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage, data transfer, etc. The instance type is the combination of Virtual CPUs(VCPUs), RAM, storage and network performances. The time unit price will be higher with more powerful instance type. Typically, more powerful instance types have higher time unit prices. There are two main pricing options: On-Demand and Reserved Instances. On-demand instance let the customers pay for compute capacity by the hour or second based on the actual usage with no long-term commitments. Reserved Instances, on the other hand, require a commitment to a specific instance type for a contract term and offer cost savings compared to On-Demand pricing. Storage and data transfer for the VM instance can also impact the pricing. The more storage space a customer uses or the more data they transfer, the higher their costs will be. The traditional cloud platform can also be affected by the co-running applications~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} In traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage space, data bandwidth, etc. The instance type includes virtual CPUs, RAM, storage, and network performances. Typically, more powerful instance types charge higher prices. Also, two pricing options are commonly offered: on-demand and reserved instances. On-demand instances allow tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved instances require a commitment to a specific instance type for an agreed term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period. Storage space and data bandwidth for the VM instance also influence the price. Demanding more storage space or more data transfer raises the cost~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} 

% The price of traditional cloud platforms is determined by computing capabilities such as processor type, memory capacity, and network bandwidth. While more and better resources typically charge higher prices, two pricing options are commonly offered: on-demand and reserved instances. On-demand pricing allows tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved pricing requires a commitment to specific resources for an agreed-upon term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period~\cite{amazonEC2Pricing}. 

% There are several differences between traditional cloud platforms and serverless platform. 
% Firstly, the roles of customers in the execution environment differ between traditional and serverless platforms. In the traditional cloud, customers are responsible for configuring and maintaining virtual machines (VMs), setting up networking, and managing databases~\cite{amazonEC2Pricing}. And it's the customers's responsibility to detact and update the configurations to balance their expenses and performance. On the other hand, in serverless platforms, users only provide a single file to indicate their system and library requirement, while the service provider handles the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. This feature enables users to focus solely on their actual workload without the burden of managing the infrastructures. Additionally, the platform can automatically scale the resources for the users based on the current demand of the application to guarantee the customer satisfaction~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% There are apparent differences between traditional and serverless cloud platforms. First, tenants are responsible for managing hardware resources in traditional platforms. The tenants need to configure and maintain virtual machines, set up networking, and manage databases~\cite{amazonEC2Pricing}. Also, tenants should study the optimal configurations to balance their expenses and performance. Meanwhile, in serverless platforms, tenants only provide a single file to specify their system requirements while the cloud provider prepares the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. The platform provisions or scales the needed resources on demand. Consequently, the serverless platforms encourage tenants to focus solely on their front-end workloads without the burden of managing the low-level back-ends~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% Secondly, there are notable differences in compute power and memory size options between the two platforms. For traditional cloud, the granularity usually 1 VCPU and 1GB memory. But, for serverless platform, the smallest memory size is 128 MB~\cite{awsLambdaApiGateWay,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Thirdly, the characteristics of workloads on these platforms set them apart. Serverless applications are generally small and executed on-demand, resulting in very short workload durations~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can complete in less than one second. In contrast, traditional cloud applications tend to be larger and may require hours to complete. Additionally, the number of co-located applications on a single computing node is smaller in traditional cloud setups, making their execution environment less dynamic compared to serverless platforms.
% Lastly, the billing periods differ significantly between traditional cloud and serverless platforms. Traditional cloud users are charged for the allocated time period. Regardless of whether they are actively running tasks on the machine, they are still need to pay for the allocated time period. However, serverless customers are only billed for the actual execution time of their tasks on the platform.

% Second, the workloads are expected to be small in serverless computing. Serverless workloads are generally small and launched on-demand as short-living event handlers~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can be completed in less than one second, unlike traditional cloud applications that are often expected to be large in a server form. Inherently, massive serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. This workload difference develops a unique pricing policy in serverless computing, pay-as-you-go pricing. In the traditional cloud, the tenants purchase hardware resources for the contracted term. Regardless of actual use, they need to pay for the agreed period. However, the serverless platforms bill their tenants for the actual execution time of their tasks.


% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python being utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Furthermore, over 90\% of organizations leverage Python and Node.js alongside AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer numerous advantages for programmers, such as user-friendliness, portability, reduced error risks, and thriving ecosystems. As a result, they have garnered widespread acceptance within serverless platforms. High-level programming languages typically follow a fixed execution procedure. For instance, in Python, when an application is executed, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the code is compiled and executed. Once the execution is complete, the Python program is terminated, and all resources used by the program are released. Due to the consistency of the operating system and Python version, the beginning of the execution process remains the same each time~\cite{pythonUsage}.



% \textbf{Resource based discount vs. Slowdown based discount:} To fully utilize the available resources, service providers often run as many applications as they can in one computing node within the service agreement requirement. However, this may lead to resource congestion and cause slowdowns for users, which can be unfair, since the customers are paying more money for the worse experiences. The intuitionistic solution could be for the service provider to track the resource usage of each application and offer discounts to users who consume fewer resources. However, serverless applications are typically very small, and contention can affect different applications differently, making this approach less practical. A more suitable solution for serverless platforms could involve offering slowdown-based discounts. In this approach, the service provider dynamically updates unit prices based on the level of system congestion. When there is less contention, users normally stiffed with the experiences and pay the regular price. However, during periods of high congestion, when the system is under heavy load, users could receive discounted prices as compensation for potential slowdowns. This approach would align pricing with the actual performance experienced by users, ensuring a fair and responsive pricing model.


==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/03_methodology.tex <==
\section{Methodology}
\label{sec:method}

% \textbf{Hardware Infrastructure:} All the experiments are performed on a dual-socket server platform. Each socket has 16 simultaneous multithreading(SMT) cores. The CPU model is Intel Xeon Gold 5218(Cascade Lake). The maximum frequency of the machine is 3.9GHz. Each core has a 32KB L1 instruction cache, a 32KB L1 data cache and a 1MB L2 cache. The 32 virtual cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The computer node runs the latest Ubuntu server version(Ubuntu 22.04 LTS) with kernel version 5.15.0. For consistency in the results, the core frequency was set to 3.0GHz using the 'cpupower frequency-set' command. We use linux perf~\cite{perfWiki} to collect the performance counters for each experiment. To analyze the startup status, we use -I 1 option to obtain count deltas at one-millisecond intervals. By utilizing interpolation, we can know the performance counters of each execution period. 

% In this study, we test today's server systems with serverless functions. This section describes our test configuration. 
This section outlines our test setup for evaluating serverless functions in this study.

% % original version
% \textbf{Hardware Infrastructure:} All experiments are performed on a dual-socket server platform with two Intel Xeon Gold 5218 (Cascade Lake). The CPU offers 16 simultaneous multithreading (SMT) cores with 3.9 GHz maximum frequency. We pin the core frequency at 3.0GHz for our tests. Each core has 32KB L1 instruction/data caches and 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The machine runs the Ubuntu server OS (Ubuntu 22.04 LTS) with a kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to collect the performance counters, which are collected at every one-millisecond interval. 
\textbf{Hardware Infrastructure:} All experiments are conducted on a dual-socket server platform equipped with two Intel Xeon Gold 5218 processors based on the Cascade Lake architecture. Each CPU provides 16 cores that support simultaneous multithreading (SMT) with a maximum frequency of 3.9 GHz. Every core features 32KB of L1 instruction/data caches and a 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets collectively have access to 384GB of main memory. The server operates on Ubuntu Server OS, version 22.04 LTS, with kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to gather performance counters.

% The CPU frequency is a key performance/energy factor, significantly affecting a function's execution time and energy consumption. A CPU's frequency can be altered in software or hardware based on its power and thermal budget, configuring it for better energy efficiency or performance. However, varying frequencies cause the system performance/energy to be unsettled, making system management intractable. For this reason, commercial systems such as Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. In our tests, when the frequency is not fixed by software, Intel's Turbo technology alters the frequency occasionally but mainly employs 2.8GHz. We will discuss this further in the sensitivity section.
The CPU frequency is a critical factor influencing both performance and energy consumption, significantly affecting a function's execution time and energy usage. A CPU's frequency can be adjusted through software or hardware based on power and thermal budget, optimizing for either energy efficiency or performance. However, varying frequencies can cause instability in system performance and energy usage, complicating system management. For this reason, commercial systems like Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. If we do not fix the frequency through software, Intel's Turbo technology occasionally adjusts it, but it mostly remains at 2.8 GHz during our tests. We will provide more details on this in Section~\ref{sec:sensitivity}.

% \textbf{Stressing Programs:} We used two stressing programs to investigate how applications and the startup portion of the high level languages behave in a resource contention environment. FigureXXX illustrates the number of instructions, L3 accesses, and L3 misses that the stressing programs can generate in five seconds as the stressing levels increase. By combining different stress levels of these stress-testing programs, we can simulate various resource-congested environments. The XXX-stressor(lineXXX)  generates more L3 accesses with a high L3 hit rate. While XXX-stressor(lineXXX), in each stressing level, generates fewer L3 accesses but more L3 misses. With these two stressors and different stressing levels, we can simulate the system with varying contentions to the shared resources by creating various  L3 accesses and L3 misses. In figureXXX we can see that the L3 accesses generated from the L2-stressor (update name later) begin to decrease after reaching stressing level 20.  However, during this period, the L3 misses continue to increase. The reason behind this trend is that, after stressing level 20, the heightened L3 miss rate starts to impact the stressor's performance, leading to a decline in the committed instruction count. Consequently, the stressor generates fewer L3 accesses and more L3 misses. 

% \begin{table}[h]
%     \begin{center}
%     % \vspace{-1.0em}
%         \caption{Serverless Benchmarks \& Runtimes}
%         \label{tb:benchmarks}
%         % \vspace{-1.0em}
%         \begin{tabular}{|l l||l l|} \hline
%             Function & Abbr. & Function & Abbr. \\ \hline \hline
%             \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  & \multicolumn{2}{c|}{\textbf{Hotel Reservation~\cite{gan2019open}}} \\ \hline
%             Dyn HTML & dyn-py & Geo & geo-go* \\ \hline
%             Thumbnail & thum-py* & Profile & profile-go \\ \hline
%             Compression & compre-py & Rate & rate-go \\ \hline
%             Image Recogn & recogn-py* & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
%             Graph Rank & pager-py & Currency & cur-nj* \\ \hline
%             Graph Mst & mst-py & Payment & pay-nj \\ \hline
%             Graph Bfs & bfs-py* & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
%             DNA Visual & visual-py* & Authen & auth-py/nj/go \\ \hline
%             \multicolumn{2}{|c||}{\textbf{Function Bench~\cite{kim2019functionbench}}} & Fibonacci & fib-py/nj/go* \\ \hline
%             Chameleon & chame-py & AES & aes-py/nj/go \\ \hline
%             FloatOp & float-py* & & \\ \hline
%             % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
%         \end{tabular}
%     \end{center}
%     % \vspace{-1.5em}
% \end{table}

\begin{table}[h]
    \begin{center}
    % \vspace{-1.0em}
        \caption{Serverless Benchmarks \& Language Runtimes (py, nj, go)}
        \label{tb:benchmarks}
        % \vspace{-1.0em}
        \begin{tabular}{|l l||l l|} \hline
            Function & Abbr. & Function & Abbr. \\ \hline \hline
            \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  &  \multicolumn{2}{|c|}{\textbf{Function Bench~\cite{kim2019functionbench}}}\\ \hline
            Dyn HTML & dyn-py & Chameleon & chame-py \\ \hline
            Thumbnail & thum-py* & FloatOp & float-py \\ \hline
            Compression & compre-py & Gzip & gzip-py* \\ \hline
            Image Recogn & recogn-py & RandDisk & randDisk-py* \\ \hline
            Graph Rank & pager-py & SequenDisk & seqDisk-py \\ \hline
            Graph Mst & mst-py & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
            Graph Bfs & bfs-py* & Currency & cur-nj* \\ \hline
            DNA Visual & visual-py* & Payment & pay-nj \\ \hline
            \multicolumn{2}{|c||}{\textbf{Hotel Reservation~\cite{gan2019open}}} & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
            Geo & geo-go & Authen & auth-py*/nj/go \\ \hline
            Profile & profile-go* & Fibonacci & fib-py*/nj*/go* \\ \hline
            Rate & rate-go & AES & aes-py/nj*/go* \\ \hline
            % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
        \end{tabular}
    \end{center}
    % \vspace{-1.5em}
\end{table}

% revision version
% \textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we select 27 distinct serverless functions from different benchmark suites, including AWS' authentication serverless functions~\cite{awsLambdaApiGateWay}, Hotel Reservation from the DeathStarBench suite~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and SeBS serverless benchmark suite~\cite{copik2021sebs}. The three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating 3 separate test cases per function. Among them, we pick 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. The functions are implemented using three languages: Python, Nodejs, and Go. We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. 
\textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we selected 27 distinct serverless functions from various benchmark suites, including AWS authentication serverless functions~\cite{awsLambdaApiGateWay}, the Hotel Reservation from DeathStarBench~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and the SeBS serverless benchmark suite~\cite{copik2021sebs}. The functions are implemented using three languages: Python, Nodejs, and Go. Notably, the three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating three separate test cases per function. 
% This comprehensive language support ensures that our test coverage is thorough and representative of the diverse language preferences in the serverless computing community. 
We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. Additionally, we selected 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. 


%\hl{The benchmarks we choose include I/O-bound, memory-bound, and compute-bound functions. For an experiment, we put the testing function in core 0 to core 4. We also put 50 other functions in core 0-4 to let the application co-running with 10 other applications to observe the impact of context switching.}

% \hl{We select benchmarks with mixed performance characteristics: I/O, memory, and compute-bound. Also, to replicate the congested commercial systems, we located a testing function with 50 other functions and tied them to selected 5 cores, Core 0 to 4. During our evaluation, those functions run simultaneously and compete to secure any core among the five.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
\caption{(a) L2 misses and (b) L3 misses of traffic generators, both normalized with the average L2 and L3 misses of serverless applications listed in Table~\ref{tb:benchmarks}}
% \vspace{-0.5em}
\label{fig:stressing_specs}
\end{figure}

% \textbf{Traffic Generator:} We divide the CPU's shared resources into two distinct categories: resources before and after the L3 caches. To pressure each resource group individually, we developed two separate traffic generators aimed at generating traffic and congestion in these resources. The first traffic generator, CT-Gen, applies pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another traffic generator, MB-Gen, induces massive L3 misses that stress the resources after the L3 cache, mainly the off-chip memory bandwidth and L3 cache spaces.
\textbf{Traffic Generator:} We categorize the CPU's shared resources into two groups: those before the L3 caches and those after. To stress each group independently, we developed two separate traffic generators designed to generate traffic and congestion within these resources. The first generator, CT-Gen, exerts pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another generator, MB-Gen, induces massive L3 misses, which stress the resources beyond the L3 cache, primarily targeting off-chip memory bandwidth and L3 cache spaces.

% Both traffic generators are multi-threaded, governing the volume of traffic by adjusting the number of threads they spawn. Each thread spawned by the traffic generator is pinned on each core to prevent conflicts between threads; consequently, this setup allows us to vary the stress level across our 32-core processors, ranging from level 1 to 31. Figure~\ref{fig:stressing_specs} shows each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), for every thread count increment, CT-Gen makes massive L2 misses. The CT-Gen's L2 misses are ended with L3 hits, as shown in Figure~\ref{fig:stressing_specs}(b). Meanwhile, MB-Gen creates huge L2 and L3 misses, as implemented. Interestingly, its L2 misses are fewer than CT-Gen's because MB-Gen is slowed by its L3 misses, suffering from a self-created bandwidth bottleneck. 
Both traffic generators are multi-threaded and govern the amount of traffic by adjusting the number of threads they spawn. Each thread is pinned to a specific core to avoid conflicts between threads, allowing us to vary the stress level on our 32-core processors from level 1 to 31. Figure~\ref{fig:stressing_specs} illustrates each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), with each increase in thread count, CT-Gen generates substantial L2 cache misses. These L2 misses by CT-Gen are ended with L3 cache hits, as shown in Figure~\ref{fig:stressing_specs}(b). In contrast, MB-Gen produces significant L2 and L3 cache misses. Interestingly, MB-Gen's L2 misses are fewer than those of CT-Gen because MB-Gen is hindered by its L3 misses, suffering from a self-imposed performance bottleneck.



==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/04_motivation.tex <==
\section{The Need for Fair Pricing}
\label{sec:motivation}

% Offering fairness appears in different approaches in cloud computing when multiple tenants share hardware resources. One standard is SLA, which defines the level of services the cloud provider furnishes while a tenant sets their expectation. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving unfairness between tenants. Although serverless computing highlights the pay-as-you-go pricing model, such unfairness still exists.
Fairness in cloud computing, especially when multiple tenants share hardware resources, is addressed through various approaches. One standard method is the Service Level Agreement (SLA), which specifies the level of service the cloud provider must deliver and the tenants' expectations. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving fairness issues. Despite serverless computing's emphasis on a pay-as-you-go pricing model, unfairness among tenants still exists.

% Unfortunately, modern systems are designed to maximize hardware efficiency by co-running multiple applications; the function's execution time can be affected by co-scheduled applications with conflicts when using shared resources. Ironically, whenever the service provider squeezes their resources further for better profit by accommodating more functions into a single machine, each function's execution time increases, charging them a higher cost for the same workload. However, in serverless computing, tenants lack control and insights into how their software is executed and billed for the cost of convenience. 
Unfortunately, modern systems are designed to maximize hardware efficiency by running multiple applications concurrently. This results in conflicts over shared resources, affecting each function's execution time. Ironically, when service providers optimize for profit by packing more functions into a single machine, the execution time for each function increases, resulting in higher costs for the same workload. In serverless computing, tenants have no control or visibility over how their software is executed, leading to potential inefficiencies and higher costs for the sake of convenience.

% Genuine pay-as-you-go pricing can be achieved when there is no interference. However, that is not desired by the providers who expect to utilize their resources to maximize profits. In serverless, although each function runs virtually exclusively in a sandbox with private resources, it still shares a few resources with other co-running functions, such as shared caches and memory bandwidth. Resource partitioning, a traditional solution that eliminates interference, can promise exclusively dedicated resources to a tenant but cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 
In serverless computing, although each function runs exclusively in a virtual sandbox with private resources, it still shares certain resources like caches and memory bandwidth with other functions. Resource partitioning, a traditional solution that eliminates interference by dedicating resources exclusively to a tenant, cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 

\begin{figure}[h]
\centering
% \vspace{-0.7 em}
\includegraphics[width=1\columnwidth]{./fig/normalizedCPIRunWith26Rev}\\
% \vspace{-1 em}
\caption{Execution time of applications that run with 26 others, normalized to the execution time when running alone}
% \vspace{-0.4 em}
\label{fig:normalizedCPIRunWith26Rev}
\end{figure}

% Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed down when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. \hl{Whenever a function finishes, another function is randomly launched to maintain a total of 26 co-running functions.} The figure shows a function's performance drops by up to 35\%, and most functions are significantly influenced by the co-running functions. Compared to when an isolated environment is offered, the function performs 11.5\% slower on average, charging 11.5\% more to users. We highlight that the function runs only with 26 other functions, which is tiny compared to massively crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.
Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. Whenever a function finishes, a new randomly-selected function is launched to maintain a total of 26 co-running functions. The figure shows a function's performance can drop by up to 35\%, with most functions significantly impacted by the co-running functions. On average, functions perform 11.5\% slower in this shared environment compared to an isolated one, resulting in users being charged 11.5\% more. We highlight that this scenario involves only 26 co-running functions, which is tiny compared to heavily crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.

% Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} attempted to offer price discounts if it has a slowdown, compensating for the slowdowns. To provide the discount, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount reflecting the slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all the responsibilities of the contentions between co-running functions, guaranteeing all tenants an invariant price for their use. Any unexpected slowdowns that a tenant experiences are returned with a discount. However, sampling is an expensive operation, requiring all co-running processes to stall during the sampling. Moreover, accurate measurement requires frequent sampling when its system environment quickly alters, making the approach impossible in a fast-shifting environment like a serverless platform.   
Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} offers price discounts to compensate for slowdowns. To provide these discounts, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount based on the observed slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all responsibilities related to contentions from resource sharing, ensuring tenants pay a consistent price for their usage. Any unexpected slowdowns that a tenant experiences are compensated with a discount. However, sampling is an expensive operation that requires stalling all co-running processes during the sampling. Moreover, accurate measurement necessitates frequent sampling, especially in rapidly changing environments, making the approach impractical for dynamic environments like serverless platforms.


% A tenant needs a new pricing model based on more than just execution time. However, prior approaches have limitations, burdening cloud participants too heavily; it is unsuitable for \hl{thousands} of concurrent short-lived functions in serverless computing. This motivates us to propose a new solution, Litmus pricing, that discounts prices based on the system state but offers lightweight with no overheads.
Overall, tenants need a new pricing model that considers more than just execution time. Prior approaches have limitations, excessively burdening cloud participants and being unsuitable for the many short-lived functions typical in serverless computing. This motivates us to propose a new solution: Litmus pricing, which discounts prices based on the system congestion while remaining lightweight and imposing no additional overhead.


==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/05_design.tex <==
\section{Litmus Pricing}
\subsection{Overview}

% The estimated prices of serverless functions should reflect the congestion level of the system inside their machines. With the massive short-living functions, the serverless system's state can dramatically change in a short time. Accordingly, the system state can be congested at any moment and also resolved in a short time. However, such a temporary traffic jam may significantly impact the performance of short-living functions. Therefore, assessing the congestion must be lightweight, quick, and on time. However, a prior approach, POPPA\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling with considerable performance overheads, preventing them from wide adoption. Instead, we propose a new scheme, Litmus pricing, that quickly estimates system congestion at the start of every function and reflects the estimation into pricing the function. 
The estimated prices of serverless functions should reflect the system's congestion state. The presence of numerous small transient functions within the serverless system can rapidly alter its congestion state, causing sudden congestion or swift resolution. Nevertheless, such transient traffic jams can significantly impact the performance of short-lived functions. Thus, assessing the congestion must be lightweight, quick, and timely. However, a prior approach, POPPA~\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling, which incurs considerable performance costs, thereby limiting its widespread adoption. Alternatively, this study introduces Litmus pricing, which promptly gauges system congestion at the onset of each function and reflects the estimated congestion level into pricing the function.

% Like the prior approach~\cite{tiwari2013enabling,alex2013ScFairPrice}, Litmus pricing suggests that the service provider discounts when a tenant's functions are intervened, compensating for the performance loss. To determine the discount ratio, Litmus measures system congestion level, which can also help service providers evaluate remaining resources and make decisions on job scheduling. 
Like the prior approach, Litmus pricing suggests that service providers should offer discounts when a tenant's functions experience interference, thus compensating for the performance loss. Litmus pricing determines the discount rate based on the system's congestion level. Evaluating congestion also assists providers in estimating remaining resources and making informed decisions regarding job scheduling.

%Nevertheless, the Litmus pricing does not quantify each function's slowdown; the discount amount is determined only by the severity of the measured congestion. The impact of the congestion on distinct functions appears differently despite facing the same congestion level, and precisely estimating a function's performance loss is a complex problem. That's why the prior approach had to rely on expensive sampling. Instead, the Litmus pricing avoids the overheads and limits the service provider's responsibility to measure the current congestion. 
However, Litmus pricing does not quantify the slowdown of each individual function; the discount amount is solely determined by the severity of the measured congestion. Even though different functions face the same congestion level, their respective impacts can vary, making precise estimation of each function's performance loss a challenging task. This complexity necessitated the expensive sampling relied upon by the previous approach. Instead, Litmus pricing circumvents such overheads and lightens the service provider's burden solely to measure ongoing congestion levels.

% Litmus pricing embodies the varying value of shared resources across different system conditions by applying equal discounts to all functions under the same system condition, although the functions experience different slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that a function that is slowed more than others demands the over-crowded resources more while exacerbating the adverse over-crowded conditions. Litmus pricing does not provide additional compensation for their extra loss compared to others due to their heavy use of shared resources.
Litmus pricing captures the dynamic significance of shared resources under varying system conditions by offering uniform discounts to all functions under the same system congestion, regardless of their individual slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that functions experiencing larger slowdowns tend to demand more of the crowded resources, thereby exacerbating adverse overcrowded conditions. However, Litmus pricing does not offer additional compensation for the larger loss experienced by functions that use shared resources more heavily than others.

% As a result, Litmus inherently incentivizes users who use shared resources sparingly. When over-crowded, functions with minimal needs for shared resources still enjoy discounts but encounter slight slowdowns. This implies that users may take advantage of this policy by minimizing their use of shared resources, receiving substantial discounts despite enduring only minor slowdowns. Such a trade-off is considered acceptable because the user's shared resource usage reduces their contribution to congestion, thereby benefiting the overall system over the other users.
As a result, Litmus inherently incentivizes users who use shared resources sparingly. During periods of overcrowding, functions with minimal needs for shared resources still enjoy discounts but with only slight slowdowns. This implies that users may take advantage of this policy by minimizing their reliance on shared resources, receiving substantial discounts despite only experiencing minor slowdowns. This trade-off is considered acceptable because reduced shared resource usage by users helps mitigate congestion, thereby benefiting the overall system and other users.
% Lastly, the system refrains from scheduling a function if the congestion level exceeds a predetermined threshold, thus preventing resource thrashing.


\subsection{Pricing Model}
\label{pricing model}

% Developing Litmus pricing raises two challenges. First, Litmus needs a new pricing model to estimate a function's price. Second, Litmus needs a way to measure the system's congestion state. Due to the serverless's fast-shifting environment, assessing the congestion must be lightweight and frequent at the right time. Nevertheless, all present commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants must pay more with prolonged execution time when using over-crowded resources. Rather than simply imposing a price by multiplying the main memory usage and a function's total execution time, Litmus suggests the price as a sum of two distinct price components as follows.
Developing Litmus pricing raises two challenges. First, it needs a new model to estimate a function's price. Second, it needs a way to measure the system's congestion state. Due to the rapidly changing environment in serverless computing, assessing congestion must be lightweight and timely. Commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants end up paying more for prolonged execution time when using over-crowded resources. Rather than simply imposing the price by multiplying the main memory usage and a function's execution time, Litmus pricing determines the price as a sum of two distinct pricing components as follows.

\begin{equation} 
P = P_{private} + P_{shared}
\end{equation}

% In this equation, \(P\) denotes the total price tenants need to pay to execute their functions. Litmus pricing divides the tenant's price into two pricing components, each with a different resource type. \(P_{private}\) represents the price the tenant needs to pay for private resources, which are entirely assigned to a tenant. \(P_{shared}\) is the price the tenant needs to pay for the shared resources. Each price component is measured proportional to a user's time to occupy the corresponding resources. However, such occupied time can be extended when contention disturbs a process's execution in the shared resources. This delayed time increases a tenant's price unfairly. 
In this equation, \(P\) denotes the total price tenants must pay to execute their functions. Litmus pricing divides this cost into two pricing components, each associated with a different resource type. \(P_{private}\) is the cost for private resources, which are entirely assigned to a single tenant. \(P_{shared}\) is the cost for shared resources. Each pricing component is measured proportional to the time users occupy the respective resources. However, if contention disturbs a process's execution in the shared resources, the occupied time will be extended. This delay unfairly increases the tenant's cost. 


\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/slowdownRunwith26Rev}\\
\caption{\(T_{private}\) and \(T_{shared}\) of applications that run with 26 others, normalized to those when running alone}
\vspace{-0.5em}
\label{fig:slowdownRunwith26Rev}
\end{figure}

% Using Perf, we measure the delays due to the shared resources and split a function's execution time into two distinct slices: one slice, \(T_{private}\), which is time spent on private resources and another slice, \(T_{shared}\), which is time spent on shared resources. Figure~\ref{fig:normalizedTcore&Tuncore-runWith16} shows the impact of the contentions on each time slice, where we normalize \(T_{private}\) per instruction and \(T_{shared}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 207\% on average and 364\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions. 

% We observe that the system congestion influences the occupied time for each resource type differently. The time to hold private resources is slightly affected, with minor changes, even under heavy congestion. Meanwhile, the time due to shared resources is broadly affected, showing significant differences. Thus, we separately measure the two delays and charge their use with a different rule.
We observed that system congestion influences the occupied time for each resource type differently. The time to use private resources is only slightly affected, with minor changes, even under heavy congestion. In contrast, the time spent on shared resources is broadly affected, showing significant differences. Thus, we separately measure the delays for the two resource types and apply different charging rules for their use. 

% Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where we normalize \(T_{shared}\) per instruction and \(T_{private}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 181\% on average and 488\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions.
Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is calculated as the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where \(T_{shared}\) per instruction and \(T_{private}\) per instruction are normalized to the same tests when running alone. The figure shows that \(T_{shared}\) is significantly affected by system congestion compared to \(T_{private}\). On average, \(T_{shared}\) increases by 181\%, with a maximum increase of 488\%. Meanwhile, \(T_{private}\) increases by only 4\%, with minor variance between functions.

% This figure gives insights into two key factors. First, the congestion in the shared resources does not impact the performance of private resources. Accordingly, when the system gets congested, the degree of a function's dependence on the shared resources determines the function's performance. If the \(T_{shared}\) takes a minor portion of a function's execution, severe congestion still barely influences its overall execution. Second, hardware PMUs available in modern CPUs, and profiling tools such as Linux Perf are widely available and can be used to distinguish the usage of shared and private resources. Across the paper, we will take advantage of such tools to develop Litmus pricing.
This figure highlights two key factors. First, congestion in shared resources has a negligible impact on the performance of private resources. Accordingly, when the system gets congested, the extent of a function's reliance on shared resources determines its performance. If \(T_{shared}\) constitutes a minor portion of a function's execution, even severe congestion will have minimal impact on its overall execution. Second, hardware Performance Monitoring Units (PMUs) in modern CPUs and profiling tools like Linux Perf are widely available and can be utilized to differentiate between the use of shared and private resources. Throughout this paper, we will leverage these tools to develop Litmus pricing.

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/TpriTshardDistriRev}\\
% \caption{\(T_{private}\) and \(T_{shared}\) distribution when they run alone}
\caption{Execution time distribution of \(T_{private}\) and \(T_{shared}\)}
\vspace{-0.5em}
\label{fig:TpriTshardDistriRev}
\end{figure}

% Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) in a function's execution. The compute-intensive workloads (e.g., fib-py, float-py) have a substantial \(T_{private}\) portion that can reach 99.96\% of the execution time. However, the portion decreases when running memory-intensive workloads such as fib-nj. This distribution indicates how much other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase float-py's \(T_{shared}\), its total execution time, $T_{private}+T_{shared}$, will undergo minor change.
Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) during a function's execution. Compute-intensive workloads (e.g., fib-py, float-py) exhibit a substantial \(T_{private}\) portion, accounting for up to 99.96\% of the execution time. However, this portion decreases when running memory-intensive workloads such as fib-nj. This distribution reflects how other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase its \(T_{shared}\), the total execution time, $T_{private}+T_{shared}$, will undergo only a minor change.

% For each pricing component, we calculate the price by multiplying its charging rate with its time distribution. Thus we can further update the pricing equation.
After collecting the time slices spent on each resource, Litmus calculates each pricing component by multiplying two different charging rates with corresponding slices. Consequently, a new pricing equation emerges as follows:

\begin{equation} 
P = R_{private} * T_{private}  + R_{shared} * T_{shared}
\end{equation}

% \(T_{shared}\) is the cycles stalled due to L2 misses. It is measured from the perf counter, STALLS\_L2\_Misses. \(T_{private}\) is the total execution minus STALLS\_L2\_Misses. 
% Using Perf, Litmus collects\(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total cycles to complete the application minus \(T_{shared}\). 
% While Litmus returns the system's congestion state, the service provider still needs to determine reasonable prices charged for a service when having different congestion levels. 

% \(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. Again, the two charging rates are necessary since each component is affected differently, directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from the crowded execution environment. Thus, the charging rates should be measured as follows.
\(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. These two charging rates are necessary because each component is affected differently, either directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from a crowded execution environment. Thus, the charging rates should be measured as follows:

\begin{equation} 
R = R_{base} * \frac{T_{solo}}{T_{congestion}}
\end{equation}

% In this equation, \(R\) is the charging rate for executions on either private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free execution environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is the execution time when the function runs alone, and \(T_{congestion}\) is its execution time in the congested environment. Again, we should collect a separate \(T_{solo}\) and \(T_{congestion}\) for each pricing component. To measure \(T_{solo}\), \hl{the prior work}~\cite{alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. Litmus pricing avoids such a costly approach but presumes the function's \textit{solo} performance by examining reference workloads on the system.
In this equation, \(R\) represents the charging rate for executions on private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free runtime environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is its non-interfered execution time when the function runs alone, and \(T_{congestion}\) is its execution time in a congested environment. We need to collect separate \(T_{solo}\) and \(T_{congestion}\) values for each pricing component. To measure \(T_{solo}\), the prior study~\cite{tiwari2013enabling,alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. However, Litmus pricing avoids such a costly approach by presuming the function's solo performance through reference workloads on the system.

% Litmus pricing requires both providers and tenants to be involved in the price decision. The providers need to decide on reasonable rates for each resource use by analyzing the selected representative functions running on the system. To offer reasonable discounts, the providers must choose the functions analyzed carefully, collecting the functions representing the system. The tenants must also know the consequences when their tasks heavily rely on any of the shared resources. Unfortunately, their tasks may get delayed more than the provider's expectation while still receiving the discount rate up to the expectation. 
Litmus pricing requires both providers and tenants to be involved in the price decision process. Providers need to establish reasonable rates for each resource usage by analyzing selected representative functions. To offer fair discounts, providers must carefully choose the functions to be analyzed, ensuring the functions accurately represent the system condition. Tenants must also know the consequences when their tasks heavily rely on shared resources. Unfortunately, their tasks may get delayed more than the provider's expectations while still receiving the expected discount rate. 

% Here, the Litmus pricing reflects the varying value of the shared resources when the system's congestion level changes; the importance of shared resources becomes more valuable when congested. 



==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/06_design_details.tex <==
\section{Estimating prices with Litmus}
\label{sec:designDetails}

% The providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}, before using Litmus pricing. The numbers in both tables are the slowdowns of codes while testing the system congestion. Shortly, the congestion table is filled with the slowdowns of startup codes, and the performance table is filled with the slowdowns of reference benchmarks. Litmus pricing needs three steps to charge the final price with a discount. First, the providers assess the system's congestion at multiple levels and range them in a table. This step completes the congestion table. Second, the providers study the impact of congestion on tenants' functions and complete the performance table. Lastly, the service provider determines a tenant's price based on the two tables. 
Before using Litmus pricing, service providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}. The congestion table lists the slowdowns during the startup phases, whereas the performance table lists the slowdowns of reference functions. Litmus pricing needs three steps to determine the final price with a discount. First, providers assess system congestion at multiple levels and record the results in the congestion table. Second, providers analyze the impact of congestion on reference functions and fill out the performance table. Lastly, providers determine a tenant's price based on the data from both tables.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tables}\\
\caption{Congestion and performance tables: numbers in both tables indicate the slowdowns of startup codes and reference functions, collected with CT-Gen and MB-Gen}
\vspace{-0.7em}
\label{fig:litmust_tables}
\end{figure}

\textbf{Step 1, Defining Congestion Levels:} We manage the system's congestion levels using two traffic generators that create a range of congestion states by stressing shared resources differently. The traffic generator is multi-threaded, creating traffic in shared resources to incur congestion, with each thread running on a separate core. We rank the stress levels from 1 to 32 by changing the number of active threads running on distinct cores. Entries from top to bottom in the congestion table indicate increasing stress levels.

% \begin{figure}[h]
% \centering
% \vspace{-1.5em}
% \includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
% \vspace{-1em}
% \caption{stressing program's instruction, L3 accesses and L3 misses }
% \vspace{-0.5em}
% \label{fig:stressing_specs}
% \end{figure}

% \textbf{Step 2. Measuring System Congestion:} Measuring the current level of system congestion that may influence a function's performance is a crucial challenge. If we assume that the platform does not have pre-profiled information about a function's performance, the platform cannot figure out whether co-running functions influenced the function. Additionally, the serverless platform's fast-changing states with massive short-living functions make the assessment even more complicated, requiring quick and frequent examinations.

% Meanwhile, measuring the amount of a system's congestion and its impact on performance is a crucial challenge. This challenge particularly stands apparent when being demanded to quantify the impact of the congestion on a running application without pre-profiled information about the application. Moreover, the serverless platform's fast-changing system states with \hl{numerous} short-lived functions make the assessment even more complicated, requiring quick and frequent performance examinations.
Measuring the amount of system congestion and its impact on performance is a crucial challenge. This challenge becomes particularly pronounced when trying to quantify the impact of the congestion on a running application without pre-profiled information about the application. The fast-changing system states of a serverless platform, with numerous short-lived functions, further complicate the assessment, necessitating quick and frequent performance examinations.

% Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. The proposal is based on the observation that high-level languages, such as Python and Node.js, used in serverless computing have long startup times to accommodate their runtime environments. Since the inception of serverless computing, these startups have been recognized as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests leverage these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests further validated that all tested functions exhibited similar performance characteristics during their startups. 
Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. This method leverages our observation that high-level languages like Python and Node.js, commonly used in serverless computing, have lengthy startup phases to accommodate their runtime environments. Since the inception of serverless computing, these startup delays have been identified as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests exploit these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests have validated that tested functions exhibit similar performance characteristics during startup phases. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_all}\\
% \caption{IPC for serverless applications with different runtimes in the first 100 milliseconds of their execution}
% \vspace{-0.5em}
% \label{fig:startupIPC_all}
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped}\\
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-1}\\
\includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped_3}\\
% \caption{IPC for serverless applications grouped by language runtime in the first 100 milliseconds of their execution}
\caption{IPC of serverless applications based on languages (Go, Python, and NodeJS) during their startup phase}
% \vspace{-0.7em}
\label{fig:startupIPC_grouped}
\end{figure}

% Figure~\ref{fig:startupIPC_grouped} depicts the fluctuation in IPC (Instructions Per Cycle) of a function during the first milliseconds of its execution. The x-axis shows a time flow since the beginning; every tick indicates a millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language, and the throughput of each group is represented in separate figures. Although figures exhibit different patterns, functions in the same figure display notable similarities. The figures imply that functions written in the same language have nearly identical startups.
Figure~\ref{fig:startupIPC_grouped} depicts a function's fluctuation in IPC (Instructions Per Cycle) during its startup phases. The x-axis represents the time elapsed since the beginning, with each tick indicating one millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language runtime, and the IPC of each group is presented in separate figures. As shown in these figures, functions in the same figure show notable similarities. This implies that functions written in the same language have nearly identical startups.

% The startup of a runtime usually includes bursts of memory reads to load images and libraries, which can probe the traffic in the shared resources. By conducting a Litmus test before executing every tenant's codes, the providers can observe the system state for the function. Meanwhile, the providers also need to study how the startup codes perform in different system states. They complete the congestion tables by performing the Litmus tests with the startups written in three languages while varying the congestion levels. To this end, the information in the congestion table is looked up when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}. 
% estimating the system's state upon receiving a result of a function's Litmus test. 
The startup of a runtime typically includes bursts of memory reads to load images and libraries, which can be used to probe the traffic in shared resources. By conducting a Litmus test before executing a tenant's function, providers can assess the system state. Meanwhile, providers also need to study how startup phases perform under different system states. They complete the congestion tables by conducting the Litmus tests with startups written in three languages while varying congestion levels. This information from the congestion table is then referenced when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tests}\\
\caption{Progress of serverless applications on four cores with Litmus tests (dotted arrows) over time}
% \vspace{-0.5em}
\label{fig:Litmus_tests}
\end{figure}

% Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests. The Litmus tests examine the level of system congestion with every function startup. \hl{Many} concurrent functions in serverless offer frequent test opportunities. Function\#1 is a memory-intensive function that raises a congestion level. While active, Litmus tests measure the congestion level above 8. After Function\#1's completion, the next Litmus test detects a non-congested system with a congestion level below 3. However, with the start of another heavy function, function\#2, the Litmus tests measure the new congestion in the system.
Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests, which examine the level of system congestion during each function's startup. Many concurrent functions in serverless offer frequent opportunities for testing. Function \#1, which is memory-intensive, causes congestion levels to rise above 8 during its execution. A Litmus test in Core 3 detects this congestion. After Function \#1 is complete, a subsequent Litmus test indicates a non-congested system with a congestion level below 3. However, during another resource-intensive function, Function \#2, the Litmus test identifies new system congestion with a level above 9.  

% \textbf{Step 2. Measuring the Impact of Congestion:} Although discerning the system congestion through the Litmus test, estimating its impact on a user's application is another challenge. This work proposes a discount based on the pre-studied impacts on reference functions, assuming the user's functions are alike. For this, the service providers need to select reference functions that represent users' functions running on their systems. In this work, we select the workloads in \hl{Section 2} as our reference applications. 
\textbf{Step 2, Measuring the Impact of Congestion:} Discerning system congestion through the Litmus test solves only one of the two challenges; the other is determining its impact on a tenant's function. Different tenants' functions could experience varying degrees of slowdown under the same congestion level. To address this, we propose using pre-selected reference functions to analyze these impacts, thereby avoiding the cost of runtime profiling. For this, providers need to carefully select reference functions that represent tenants' functions operating on the systems, as these selections influence the overall accuracy of congestion measurement. Later, in Section~\ref{sec:evaluation}, our tests will show that pre-selected reference functions can effectively represent unknown user applications. For this study, the selected reference applications (* marked) are listed in  Table~\ref{tb:benchmarks}. 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/refSlowdownStressing14}\\
% \includegraphics[width=1\columnwidth]{./fig/slowdownStressing16}\\
\caption{\(T_{private}\), \(T_{shared}\), and \(T_{total}\) of serverless applications that run with MB-Gen at stress level 14, normalized to their execution time when they run alone}
% \vspace{-0.5em}
\label{fig:refSlowdownStressing14}
\end{figure}

% Once the reference functions are ready, the providers study the slowdowns of the reference functions while varying different congestion levels again. This study completes the performance table in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. Again, our two traffic generators create two separate sub-tables. All entries in this table are 1-to-1 mapped to entries in the congestion table. The providers estimate a general function's slowdown when having a certain congestion level using this 1-to-1 mapping.
Once the reference functions are ready, providers analyze their slowdowns under varying congestion levels. This analysis completes the performance table shown in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. With two traffic generators, providers can complete another set of two sub-tables for the performance table. All entries in this table are mapped 1-to-1 to entries in the congestion table. Providers can estimate a general function's slowdown at a given congestion level using this one-to-one mapping.

% Figure~\ref{fig:refSlowdownStressing14} shows the reference functions' slowdowns when stressing the system. The X-axis shows different functions, each consisting of three bars: the first two bars show the CPI during each time slice, \(T_{private}\) and \(T_{shared}\), and the last bar shows the CPI of an entire execution. The figure shows that the tested functions suffer from different amounts of slowdowns, although the tests maintain consistent stress levels. \hl{The last group} shows the gmean of all the slowdowns, which is used when providers estimate a function's slowdown later. 
Figure~\ref{fig:refSlowdownStressing14} shows an example of the reference functions' slowdowns when stressing the system. The X-axis shows tested functions, each depicted with three bars: the first two bars show \(T_{private}\) and \(T_{shared}\), while the last bar shows the total execution time, all normalized to their execution time when running alone without interference. The figure shows that the tested functions experience varying degrees of slowdown despite consistent stress levels maintained during the tests. The next-to-last group shows the gmean of all the slowdowns, which providers use to estimate a function's slowdown later.

% \hl{This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/referenceStartupSlowdownRev}\\
\caption{The correlation between the slowdown of Python's startup phase and the slowdown of reference applications. From left, (a) \(T_{private}\), (b) \(T_{shared}\), and (c) \(T_{total}\), normalized to the execution time when running alone}
\label{fig:referenceStartupSlowdownRev}
\end{figure}

% \textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while a range of congestion levels is continuous, the tables only contain a few slowdowns in discrete intervals. Thus, providers need a model that returns an estimated slowdown when receiving a congestion level as an input. In our tests, we employ a linear regression to achieve the model.
\textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while congestion levels vary continuously, the tables only contain slowdowns at discrete intervals. Therefore, providers need a model that estimates the slowdown for any given congestion level. In our tests, we employ linear regression to develop the model.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/interpolation}\\
\caption{Estimating a function's slowdown with logarithmic interpolation}
\label{fig:interpolation}
\end{figure}

% Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding references' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). We employed two traffic generators to extrapolate a more precise congestion level, yielding two sub-tables in both the congestion and the performance tables. Consequently, the figure presents two linear regression models, each associated with a different traffic generator. 
Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding reference applications' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). To extrapolate a precise congestion level, we created two sub-tables within both the congestion and performance tables using two distinct traffic generators. As a result, the figure depicts two linear regression lines (red and blue dotted lines), each associated with a different traffic generator.

% The provider needs to estimate the function's slowdown to uncover its price. However, the above two regression models return two vastly different slowdowns. Then, the providers need to determine which model is close to the current environment. We think the two models reflect two extreme congestions that the traffic generators create, one before the L3 and one after the L3. CT-Gen creates massive traffic from the core to the L3 cache, which filters the traffic, preventing the operations from consuming the memory bandwidth. MB-Gen also creates huge traffic but consumes the memory bandwidth and replaces L3 blocks. Since each traffic generator creates an extreme case, the machine state could be intermediate with congestion in the range between the two congestions created by CT-Gen and MB-Gen. However, Litmus pricing cannot answer this question with only the startup's slowdown. 

% To address this question, we note that the system's L3 misses are a critical indicator closely related to a function's performance. Functions suffer more when the system experiences more L3 misses, which stresses the cache space and off-chip memory bandwidth. Accordingly, Litmus test collects the system's L3 miss count as a supplementary index, which tells more about the crowdedness of shared resources.

These regression models return two different slowdowns. To estimate a function's slowdown, providers must determine which model reflects the current environment more accurately. The traffic generators create two extreme congestion scenarios: one before the L3 cache and one after. CT-Gen generates substantial traffic from the core to the L3 cache that filters the traffic and prevents operations from consuming memory bandwidth. Conversely, MB-Gen also generates massive traffic but consumes memory bandwidth and repeatedly evicts L3 cache blocks. Because each traffic generator represents a distinct extreme case, the actual machine state could fall somewhere between the two congestion levels created by CT-Gen and MB-Gen. However, Litmus pricing requires more than just the startup slowdown to identify the machine's state in these models. Thus, we have enabled Litmus tests to gather the system's L3 miss count as a supplementary metric that offers deeper insights into the crowdedness of shared resources.


% \hl{Figure 1} shows how to use the L3 cache misses with the performance sub-tables. The two traffic generators make the upper and lower boundary of the L3 miss rates. When performing a Litmus test, if the test's L3 miss rate is XXX, close to the L3 misses with CT-Gen, we can conclude that the congestion occurs before the L3 cache and select the expected slowdown of XXX. On the contrary, we choose XXX, in case the L3 miss rate is XXX, close to the L3 misses with MB-Gen. If the test's L3 miss rate is in-between, we interpolate the two slowdowns based on the L3 misses, assuming congestion in both resources. 
% Finally, we determine the Rprivate and Rshared based on the expected slowdown from its performance table. Calculating Rprivate and Rshared takes the same steps. The final discount price is computed using the equation with the computed rates. 

% Figure~\ref{fig:interpolation} shows how we employ the L3 misses when estimating the slowdown. The two traffic generators make the upper and lower boundary of the L3 misses. If a Litmus test reports the L3 miss count is 10, close to the L3 misses with CT-Gen, \textcircled{1}Litmus pricing estimates the discount (=expected slowdown) of the function to be near 1\%. This indicates that the congestion happens before the L3, as what CT-Gen creates. On the contrary, in case the L3 misses are 1000, close to the L3 misses with MB-Gen, \textcircled{2}Litmus pricing estimates the function's discount rate close to 6\%. Meanwhile, if the Litmus test reports the L3 misses as 100, we interpolate the two extreme discounts, 1 and 6, based on the L3 misses, assuming current congestion to stand in between the two extreme congestions. The congestion model in the figure shows how we interpolate with logarithmic interpolation. In this figure, \textcircled{3}applying the logarithmic interpolation to the L3 miss count returns the half-point between CT-Gen's 1\% and MB-Gen's 6\%, which is 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 
Figure~\ref{fig:interpolation} shows our approach to using L3 misses to estimate slowdowns. We created two figures illustrating separate regression models. The left figure (a) is derived from the startup slowdowns and L3 misses with logarithmic regression, indicating L3 misses at specific congestion levels. The right figure (b) is derived from the performance table with linear regression, displaying discounts at specific congestion levels. Each figure depicts two regression lines associated with different traffic generators.

The two traffic generators set the upper and lower boundaries for L3 misses. For instance, if a Litmus test reports 10 L3 misses, close to what CT-Gen generates: \textcircled{1}This suggests congestion occurs before reaching the L3 cache, similar to CT-Gen's scenario. Thus, Litmus pricing estimates the function's discount to be around 1\%. Conversely, if the Litmus test reports 1000 L3 misses, close to MB-Gen's results: \textcircled{2}Litmus pricing estimates the function's discount rate to be approximately 6\%, indicating congestion similar to MB-Gen, where memory bandwidth is heavily consumed and L3 cache blocks are frequently evicted. When the Litmus test reports 100 L3 misses, an interpolation between these extremes is applied: \textcircled{3}Using logarithmic interpolation, Litmus pricing estimates the function's discount rate to be midway between CT-Gen's 1\% and MB-Gen's 6\%, resulting in approximately 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 



==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/08_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \textbf{Litmus price \& error:}
% We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, and the other consists of selected reference applications to obtain the linear regression models for Litmus pricing. The discount models plug into the Litmus pricing used in our tests. For this experiment, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown.
We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, while the other consists of chosen reference applications to derive linear regression models for Litmus pricing. The discount models plug into the Litmus pricing employed in the tests. In this study, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown. 

% % original version
% We maintain the congestion state consistent across all tests, co-running each function with 26 other functions. Using Perf~\cite{perfWiki}, we collect the three key stats: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup, which implies the congestion level in these tests, as well as the discount rates that every function receives. We execute every function 100 times and collect the average of the function's \(T_{private}\) and \(T_{shared}\). Finally, we compute each function's \(P_{private}\), \(P_{shared}\), and \(P\), the total price, by summing \(P_{private}\) and \(P_{shared}\).  

\subsection{One Function Per Core}

% revision version
% We maintain consistent congestion states across all tests by co-running each function with 26 other functions. Using Perf, we collect the three key statistics: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup. These metrics hint at the congestion level during the tests as well as the discount rates that a function receives. Each function is executed 30 times, and the average of its \(T_{private}\) and \(T_{shared}\) is collected. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).
We maintain consistent congestion levels across all tests by co-running each function with 26 other functions. As outlined in Section~\ref{sec:motivation}, whenever a function finishes, another is randomly launched to keep a total of 26 co-running functions. Using Perf~\cite{perfWiki}, we collect three key statistics: \(T_{private}\), \(T_{shared}\), and the machine's L3 misses during the first 45 million instructions of the Python startup. Through these metrics, Litmus pricing estimates the level of system congestion and the discount rates a function receives. Each function is executed 30 times, and we average its \(T_{private}\) and \(T_{shared}\) values. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice26Rev}\\
% \caption{The total price for functions computed via Litmus pricing and ideal prices when co-running with 26 other functions normalized to the commercial price that offers no discount}
\caption{Prices computed via Litmus pricing and ideal prices when co-running with 26 other functions, normalized to the commercial price that offers no discount}
\label{fig:normalizedPrice26Rev}
\end{figure}

% In Figure~\ref{fig:normalizedPrice26}, we can see a minimal difference in the discount rate between the Litmus price and the Ideal price. The average Litmus discount rate stands at 11.5\%, which is only marginally larger by 0.6\% than the average Ideal discount rate of 10.9\%. Also, we can see that the difference between the Litmus price and Ideal price are different among the applications. Certain applications exhibit higher Litmus prices compared to the Ideal price, while conversely, some applications demonstrate smaller Litmus prices. 
 %Figure~\ref{fig:priceErrorRunwith26} shows further details, analyzing the errors in each pricing component. 

% Figure~\ref{fig:normalizedPrice26Rev} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{10.66\%}, which is only marginally larger by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{10.28\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice26Rev} illustrates estimated prices derived from Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices to offset delays in a congested execution environment. The figure shows minimal disparities between the two prices, implying that Litmus pricing offers a reasonable discount. The average discount from Litmus pricing across all functions is 10.7\%, which is only marginally higher by 0.4\% compared to the average slowdown experienced by functions, which stands at 10.3\%, as depicted by the ideal price.

% However, the discount rates per slowdown differ among functions. For instance, float-py's ideal discount rate is \hl{0.05\%}, but it enjoys a \hl{4.31\%} discount with the Litmus pricing. Meanwhile, pager-py's performance drops by \hl{15.63\%} while receiving a \hl{13.87\%} discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more easily affected than the reference when congested. In contrast, float-py runs mostly with private resources, receiving a minor impact from the execution environment. Figure~\ref{fig:priceErrorRunwith26Rev} shows further details, analyzing the differences in each pricing component.
However, the discounts per slowdown differ among functions. For instance, float-py's ideal discount rate is 0.05\%, but it benefits from a 4.3\% discount with Litmus pricing. Conversely, pager-py encounters a 15.6\% performance decline while receiving only a 13.9\% discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more susceptible to congestion than the references. In contrast, float-py predominantly utilizes private resources, resulting in minimal impact from the execution environment. Further insights into these variations in each pricing component are presented in Figure~\ref{fig:priceErrorRunwith26Rev}.


% From figure~\ref{fig:tcore\(T_{private}\)Distr}, we know that \(T_{private}\) dominates the execution time among all applications. The impact from \(T_{private}\) error has a bigger impact on the overall error. The slowdowns due to congestion in private resources are small. Theoretically, there should be no slowdowns when using private resources, but we observed that the congestion still influences it. The observed slowdown is 000, a small difference from an ideal slowdown. Meanwhile, the slowdowns in shared resources are significant. We observe that 

% % \[  Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}}\]

% \[Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{TotalIdealPrice}\]
% \[TotalIdealPrice = R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}\]

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/priceErrorRunwith26Rev}\\
\caption{Weighted errors in prices derived from Litmus pricing, which are compared to ideal prices}
% \vspace{-1em}
\label{fig:priceErrorRunwith26Rev}
\end{figure}

%%% We discuss error
% In figure~\ref{fig:priceErrorRunwith26} we can see that there are some applications receive positive errors and some receive negative errors.  A negative error indicates that our estimated slowdown for that application is higher than its actual slowdown, resulting in greater compensation than the observed performance losses. On the other hand, a positive error indicates that the compensation is smaller than its real slowdown. For most applications, the Litmus price is slightly higher than the Ideal price, with minimal differences. The highest price error is 0.0389 for auth-nj, while the lowest error is 0.007 for dyn-py. The geometric mean of the absolute error is 0.018. 
% Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors that each function experiences. The error rate is computed as the difference between the estimated and the ideal prices over the ideal price. The first two bars show the errors in \(P_{private}\) and \(P_{shared}\), which are weighted by their corresponding ratio in the execution time, considering their impacts, as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. The functions can have two different errors: positive and negative. A positive error indicates that the Litmus-estimated price is higher than its ideal price, implying that it receives smaller compensation than its performance losses. In other words, Litmus pricing estimates its slowdown to be less than its actual slowdown. A negative error implies the opposite; a function's compensation is higher than its slowdown. This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others. Meanwhile, the tenants need to acknowledge the consequences if their functions differ vastly from the reference workloads, heavily relying on shared memory.
Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors each function experiences. The error rate is computed by comparing the estimated prices with the ideal prices and dividing the difference by the ideal prices. The first two bars show errors in \(P_{private}\) and \(P_{shared}\), weighted by their corresponding ratios in execution time, reflecting their impacts as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. Functions may have two types of errors: positive and negative. A positive error means that the estimated price exceeds its ideal price, implying that the compensation received is less than the performance loss incurred. In other words, Litmus pricing underestimates the slowdown relative to the actual slowdown. Conversely, a negative error indicates the opposite; a function's compensation exceeds its slowdown. This discrepancy indicates Litmus pricing may offer varying advantages to different functions, favoring those with lesser slowdowns. Meanwhile, tenants must recognize the consequences if their functions differ vastly from the references, particularly those heavily reliant on shared resources.

% Delete the followings
% This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.

% The largest absolute error is \hl{0.0723} for rate-go, while the smallest absolute error is \hl{0.0039} for \hl{mst-py}. Overall, the Litmus pricing shows minor errors with an average of \hl{0.0231}. With further details, the Litmus pricing accurately estimates the slowdowns in \(P_{private}\) with \hl{0.0175} of an average weighted error rate. \(P_{private}\)'s highest weighted error rate is \hl{0.079}, yet minor, while the lowest rate is only \hl{0.0008}. The weighted error rate for the estimated \(P_{shared}\) is also small. The average error rate for \(P_{shared}\) is \hl{0.0068}, even lower than for \(P_{private}\). \(P_{shared}\)'s highest error rate is \hl{0.0404}.
% The largest absolute error is 0.072, which occurs with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, the Litmus pricing exhibits minor errors, averaging 0.023, \hl{with the estimated discount differing by 22.5\% over the ideal discount.} With more details, Litmus pricing accurately estimates slowdowns in \(P_{private}\), with an average weighted error rate of 0.018. \(P_{private}\)'s highest weighted error rate is 0.08, yet minor, while the lowest rate is only 0.0008. The weighted error rate for estimated \(P_{shared}\) is similarly small, averaging at 0.0068, even lower than for \(P_{private}\). The highest error rate for \(P_{shared}\) stands at 0.04.
The largest absolute error is 0.072, occurring with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, Litmus pricing exhibits minor errors, averaging 0.023. Thus, the estimated discount deviates by 22.5\% from the ideal discount. Note that Litmus pricing aims to match the average discount across all functions by applying a system-wide discount based on the system's congestion level rather than adjusting the discount for each function individually. Consequently, individual functions may experience either positive or negative errors. However, it is noteworthy that the average discount between Litmus and ideal pricing differs by just 0.4\%, as illustrated in Figure~\ref{fig:normalizedPrice26Rev}, satisfying its objectives.
% This policy may incentivize some functions while penalizing others based on shared resource usage. 
Specifically, Litmus pricing estimates slowdowns in \(P_{private}\) with an average weighted error rate of 0.018. The highest for \(P_{private}\) is 0.079, while the lowest is just 0.001. For \(P_{shared}\), the average weighted error rate is even lower, at 0.007. The highest for \(P_{shared}\) is 0.040.


% Litmus employs the average performance of applications to determine the discount rate applied universally. In this context, an application encounters a positive error when its speedup is less than the estimated average speedup across all applications. Also, the error rate depends on the difference between the actual speedup and the estimated average speedup, with larger differences resulting in more significant errors for the given application.
% As discussed in Figure~\ref{fig:TpriTshardDistri}, \(T_{private}\) dominates the execution time across all applications, implying that a small error in the estimated \(T_{private}\) largely influences the execution time. This explains why, for functions that demand little shared resources, such as float-py and chame-py, the error in P is almost identical to that in \(T_{private}\), and errors with \(T_{shared}\) can be overlooked. In contrast, for functions with a larger \(T_{shared}\) ratio, such as pager-py and mst-py, errors in \(T_{shared}\) meaningfully affect the total execution time. Note that the Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price.  

Litmus pricing estimates each pricing component separately with an individual discount rate. For functions that demand minimal shared resources, such as float-py, the errors in P are nearly identical to those in \(T_{private}\), and the errors in \(T_{shared}\) can be overlooked. As shown in Figure~\ref{fig:TpriTshardDistriRev}, \(T_{private}\) dominates the execution time across many applications. While even a small error in the estimated \(T_{private}\) influences the function's execution time, substantial errors in \(T_{shared}\) likely have limited impacts, except for functions that have a relatively meaningful \(T_{shared}\) ratio, such as pager-py and mst-py, whose errors in \(T_{shared}\) are observable in the total price. 

% We emphasize that Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price. We observe that functions have similar slowdowns in \(T_{private}\) with slight variation when congested. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, also estimating reliable total prices since \(T_{private}\) mostly dominates the execution time. The \(T_{shared}\) fluctuates more dynamically across functions with a relatively large error, but the error's impact is little, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}. 
We emphasize that Litmus pricing cannot avoid producing a certain degree of error since it relies on estimation using a few metrics. However, the figure proves that Litmus pricing effectively captures a congested environment and reflects that environment in the price. Under the same congestion level, \(T_{private}\) values of all functions are delayed similarly with a little variation. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, leading to reliable total price estimates since \(T_{private}\) generally dominates execution time. \(T_{shared}\) fluctuates more dynamically across functions and has a relatively larger error, but the impact of this error is minimal, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}.

\begin{figure}[h]
\centering
% \vspace{-5em}
 \includegraphics[width=1\columnwidth]{./fig/normTprivtTshared26Rev}\\
% \vspace{-5.5em}
\caption{\(T_{private}\) \& \(T_{shared}\) of applications when co-running with 26 others, normalized to those when they run alone. The top(black) and bottom(blue) lines are discount rates from Litmus pricing for \(T_{private}\) and \(T_{shared}\)}
% \vspace{-1em}
\label{fig:normTprivtTshared26Rev}
\end{figure}

% To further investigate the price error differences, in igure~\ref{fig:normTprivtTshared}, we explore the \(T_{private}\) speedups across various serverless applications.  
% Notably, the difference between the Litmus discount (L-Discount) and the average speedup is merely 0.006.  This minute difference explains why Litmus can attains such high accuracy. 
%Furthermore, when comparing with figure~\ref{fig:priceErrorRunwith26}, a correlation between the error rate and the speedup differences becomes apparent. 
%For instance, float-py, with the most substantial difference above the Litmus discount, also experiences the most significant negative error rate. 
%Conversely, aes-go, with the smallest speedup, experiences the highest positive error rate.
% % original version
% Figure~\ref{fig:normTprivtTshared} shows the execution time of the baseline normalized to the execution time of each run under congestion. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the functions spend only 3.67\% more time on private resources, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, resulting in precise estimation with a Litmus test. 

% Figure~\ref{fig:normTprivtTshared26Rev} shows the execution time of each function run under congestion normalized to the execution time of the baseline. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the interferences in private resources extend the function execution time only by 5.3\%, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, enabling precise estimation with a Litmus test.
Figure~\ref{fig:normTprivtTshared26Rev} shows the \(T_{private}\) and \(T_{shared}\) of each function, normalized to the same time components of the baseline. The gap between the bar and 1 represents the amount of slowdown that should be translated into ideal discounts. The top (black) and bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that interferences in private resources extend the function execution time by only 5.3\%, implying the performance of the private resources is marginally affected by congestion. Additionally, all functions exhibit similar \(T_{private}\) values with little dispersion, helping precise estimation with Litmus tests.

% Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors are still in an acceptable range since their impacts are small. Functions that have a considerable \(T_{shared}\) ratio become more sensitive to system congestion. Instead, a function, such as float-py, with negligible \(T_{shared}\) ratio gains huge benefits with high discounts while its performance remains firm. This shows that Litmus pricing reflects the dynamically changing values of shared resources when the congestion level alters and encourages functions to be developed to use more private resources. 
Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors remain within an acceptable range as their impacts are minor. Functions that have a considerable \(T_{shared}\) ratio are more sensitive to system congestion. Conversely, a function like float-py, which has a negligible \(T_{shared}\) ratio, gains huge benefits from high discounts while maintaining stable performance under congestion. This shows that Litmus pricing accurately reflects the dynamic values of shared resources when the congestion level changes and incentivizes functions to be developed to use less shared resources. 

% \textbf{Litmus pricing under high congestion:} We test our Litmus pricing under a heavily congested environment to verify its pricing of functions with large slowdowns. To create a crowded environment, we concurrently execute 60 instances of Fibonacci-go, which produces the most L2 misses among our tested functions. 
% We raise the congestion level significantly with 60 co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo} shows the results from the same tests of Figure 11. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.8\%, which is only a 1.7\% difference from the ideal discount of 27.1\% with 2.48\% of an average absolute error. In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.151 and 4.299, which are only 2.45\% and 7.83\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. 
% \textbf{Litmus pricing under high congestion:} We raise the congestion level significantly with \hl{500} co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo500} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.1\%, which is only a 1\% difference from the ideal discount of 27.1\% with 0.088\% of an average absolute error. Litmus pricing discounts slightly more than an actual slowdown, leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% % \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
% \caption{The normalized total price for the applications calculated by using Litmus pricing and ideal prices when co-running with 500 Fibonacci-go}
% \label{fig:normalizedPriceCongested320}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\columnwidth]{./fig/diffStartupPortion-2Rev}\\
%\caption{The slowdown of Python's startup with 25 and 15 million instructions (X-axis) and the slowdown of reference applications (Y-axis). From left, \(T_{private}\), \(T_{shared}\), and \(T_{total}\), normalized to those when running alone}
%\label{fig:diffStartupPortion}
%\end{figure}

% \textbf{Instructions in Startup:} Litmus tests react differently to congestion when performed with different numbers of instructions from the startup phase. For example, Python's startup involves about 45 million instructions. While we have conducted Litmus tests using all these instructions, Figure~\ref{fig:diffStartupPortion} shows the response of these tests when running with the first 15 and 25 million instructions from this set. The figure shows the startups' \(T_{private}\), \(T_{shared}\), and \(T_{total}\) with two traffic generators, as depicted in Figure~\ref{fig:referenceStartupSlowdownRev}. Tests with fewer instructions are more sensitive to cold cache misses but less to interference in the L3 cache. Therefore, as the instruction count in Litmus tests decreases, they become less susceptible to conflicts in shared resources, especially from traffic by MB-Gen. As a result, tests with 25 million instructions exhibit reduced slowdowns. This trend becomes more apparent when running the tests with 15 million instructions, depicting that slowdowns when co-running with MB-Gen become nearly identical to those with CT-Gen. 

%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%







% \textbf{Instructions in Startup:} Python's whole startup phase contains about 45 million instructions. We can further divide the startup phase into smaller pieces with 10 million instructions code chunks. And each code chunk would have its characteristics. They react differently in the same congested environment. In section XXX we use the whole Python's startup portion's slowdown to indexsing the serverless application's slowdown. But, since the co-relationship between these two slowdown in different congestion source are different, one startup \(T_{private}\) slowdown may indicate two application's slowdown. By carefully picking the code chunks we can mitigate the difference between the two normalized slowdowns of the guidance application that correlated to the same startup phase slowdown. 

% Figure~\ref{fig:diffStartupPortion} depicts the correlation between the performance changes in the reference applications and distinct segments of Python's startup phase. From the figure, we see that selecting the first 15 million instructions as our startup phase results in the normalized \(T_{uncore}PerInst\) of the guidance application aligning nearly into a singular trendline. However, there are substantial gaps in the case of \(T_{core}PerInst\) with this code segment. Thus, we should pick xxx-xxx as our startup phase representation code for the normalized \(T_{core}PerInst\). We think that this can be used to mitigate the differences. But, we should be careful to use the small code chunks for the following reasons: First, only measuring the small portion can be a problem. The results might be too dynamic. Second, since we only measure this small portion there might be a huge execution period that cannot be covered.

% Continue to work from here

\subsection{Temporal CPU Sharing}
\label{sec:temporalCPUSharing}

The previous evaluation assumes an isolated environment where a CPU is assigned exclusively to an active function during execution, disallowing temporal sharing between functions through context-switching. While this setup ensures strict performance isolation, it inherently limits resource utilization. Conversely, enhancing utilization by permitting temporal CPU sharing among functions complicates price estimation. We explore how Litmus pricing can be applied in a less restrictive environment that permits sharing, where functions can temporarily share the same CPU and are not bound exclusively to specific cores. 

In this section, we deploy a testing function to co-run with 160 other functions across 16 cores without exclusive core assignments, assuming an average of 10 functions share a core. The reduction in the number of cores tested was necessitated by our system's memory limitations, as certain functions require significant memory space.

% \textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, the subsequent function clears the displaced one's cached data. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, the slowdown with extra sharing financially benefits the provider; we thereby argue that the extent of sharing should be factored into Litmus pricing as another discount factor.
\textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, a subsequent function evicts the cached data of the displaced one. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, delayed execution due to extra sharing financially benefits the providers. Thus, we argue that the extent of temporal sharing should be incorporated into Litmus pricing as another discount factor.

Figure~\ref{fig:csImpactor} depicts the switching overheads as concurrently running functions increase. The figure demonstrates that the sharing overhead follows a logarithmic growth pattern and stabilizes at around 20 co-running functions. Furthermore, we discovered that the switching overheads predominantly affect \(T_{private}\). Consequently, Litmus pricing needs to calibrate \(T_{private}\) to account for the impacts of sharing before estimating the slowdown using the performance table.

Figure~\ref{fig:normalizedPrice160Method1} illustrates the discounted price reflecting this adjustment. In our configuration, with an average of 10 functions per core, we divide \(T_{private}\) by 1.025 before estimating the slowdown. In this figure, Litmus pricing estimates an average discount of 14.5\%, which falls 2.9\% short of the ideal discount of 17.4\%. While most benchmarks receive discounts lower than ideal, aes-py stands out with the largest error of 9.9\%, which is 6.9\% less than its ideal discount of 16.8\%.

\begin{figure}
\centering
% \includegraphics[width=1\columnwidth]{./fig/csImpactor}\\
\includegraphics[width=1\columnwidth]{./fig/csImpactor2}\\
\caption{\(T_{private}\) of functions over different co-running counts in the same core, normalized to when running alone}
% \vspace{-1em}
\label{fig:csImpactor}
\end{figure}

\begin{figure}
\centering
% \vspace{-1.2em}
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160Method1}\\
\caption{Prices derived from Litmus pricing (Method 1) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
% \vspace{-0.5em}
\label{fig:normalizedPrice160Method1}
\end{figure}

% In Figure~\ref{fig:normalizedPrice160Method1} we use the the same congestion and performance tables that we collected in the restricted environment. When checking the tables instead of using the original startup slowdown of tcore we use an adjusted slowdown by dividing the context switch impact factor. From figure~\ref{fig:normalizedPrice160Method1} we can see that the average Litums discount is 14.65\%, 3.01\% less than what they should receive compared to the ideal discount of 17.67\%. Most applications receive a smaller discount than the ideal price. The largest error is on aes-py with Litmus discount of 9.85\%, 6.87\% smaller than the ideal discount of 16.72\%. The smallest error is on dyn-py. It's Litmus discount is 22.45\%, only 0.47\% larger than the ideal discount of 21.97\%.

\textbf{Method 2, Updating Performance Tables:} Rather than reusing the performance/congestion tables designed for restrictive environments, arranging new tables for the sharing-enabled environments returns better accuracy. Although the notion of preparing separate tables for various sharing levels may seem challenging, we argue that only one or a few extra tables for heavily crowded systems would suffice, given that commercial systems are typically heavily crowded. Again, we emphasize that the impact of function co-placement stabilizes above a certain co-placement count, as shown in Figure~\ref{fig:csImpactor}.

For this test, we prepared new performance/congestion tables for the environment described above, where a testing function is assumed to co-locate and compete for a core with 9 other functions. Moreover, considering the scenario where a switched-out function has a low chance of being rescheduled to the same core, instead of assigning 10 functions to a specific core, we ran 50 functions across 5 dedicated cores; each can run on any of the 5 cores. We managed the congestion levels in shared resources using traffic generators on the other cores, as outlined in Section~\ref{sec:designDetails}.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPrice160}
% \vspace{-0.6em}
\end{figure}

% Figure~\ref{fig:normalizedPrice160} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{17.29\%}, which is only marginally smaller by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{17.67\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice160} shows the prices obtained from Litmus pricing with the new tables, which are normalized to those from commercial sources. Once more, as in Figure~\ref{fig:normalizedPrice26Rev}, the figure reveals marginal distinctions between the two price points, suggesting that Litmus pricing continues to offer a reasonable discount. Across all functions, the average discount provided by Litmus pricing stands at 17.2\%, merely 0.2\% less than the ideal discount of 17.4\%.


==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/09_sensitivity.tex <==
\section{Sensitivity}
\label{sec:sensitivity}

While the aforementioned tests highlight Litmus's potential, we recognize the need for more compelling results. This section expands our analysis and examines Litmus pricing from various angles across diverse system environments.

% \textbf{Heavy Congestions:} We raise the congestion level significantly with 320 co-running applications to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. The Litmus pricing is still close to the ideal price, discounting the price by 20.00\%, which is only a 1.46\% difference from the ideal discount of 21.46\%. The highest Litmus discount is 26.01\% for dyn-py. It has an error of 2.83\% compared with the ideal discount.
\textbf{Heavy Congestion:} We significantly escalate the congestion level to verify Litmus pricing under conditions of substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} presents the outcomes of the same tests depicted in Figure~\ref{fig:normalizedPrice160} but with 320 co-running functions. Not only did we increase the function count, but we also specifically selected 8 memory-intensive functions, aes-py, compre-py, thum-py, bfs-py, auth-py, fib-go, geo-go, and profile-go, that produce the most L2 cache misses among the tested functions to create heavy congestion in shared resources deliberately. Even under such intensified congestion, Litmus pricing produces results remarkably close to the ideal price, discounting the price by 20.0\%, which deviates by merely 1.5\% from the ideal discount of 21.5\%. The highest discount by Litmus pricing is 26.0\% for dyn-py, a minor error of 2.8\% compared to the ideal discount.


% leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 320 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPriceCongested320}
% \vspace{-1em}
\end{figure}

\textbf{CPU Frequency:} Modern CPUs feature dynamic CPU frequency adjustments, which are controlled via software or hardware. A hardware technique like Intel Turbo Technology autonomously adjusts the CPU frequency based on the CPU's power and thermal budgets, allowing the CPU to operate at higher frequencies when conditions permit and lower frequencies under heavy load. Prior tests assumed that the frequencies were fixed and strictly managed by service providers who had knowledge of when and to what extent frequency adjustments were necessary. Also, we evaluated Litmus pricing under the other scenarios where CPU frequencies were not fixed, providing more dynamic perspectives.

% Figure~\ref{fig:normalizedPrice160unset} illustrates the prices from the Litmus pricing and the ideal price, which are normalized to commercial prices. We tested it under the configuration in Section 7.2 with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, the Litmus pricing's discount is lowered from 17.16\% to 16.84\%, while the ideal discount rate is decreased from 17.42\% to 17.31\%. Still, the discount rate difference from the ideal price is only 0.47\% without setting the CPU frequency. We observed that the CPU frequency changes rarely when the system runs with 160 functions. Overall, the varying frequency made a minor impact on performance as well as the pricing scheme. 
Figure~\ref{fig:normalizedPrice160unset} illustrates the prices derived from Litmus pricing alongside the ideal prices, both normalized to commercial prices. This evaluation was conducted under the configuration outlined in Section~\ref{sec:temporalCPUSharing} with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, we observe a slight decrease in Litmus pricing's discount, from 17.2\% to 16.8\%, while the ideal discount rate decreases from 17.4\% to 17.3\%. Still, even without fixed CPU frequencies, the difference in the discount rate from the ideal price is only 0.5\%. We noted that CPU frequency changes were infrequent when the system operated with 160 functions. Overall, the variation in frequency had a negligible impact on Litmus pricing.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160unset}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others with unfixed CPU frequencies, both normalized to commercial prices}
\label{fig:normalizedPrice160unset}
% \vspace{-1em}
\end{figure}

% All the above experiments are done on Intel Xeon Gold 5218(Cascade Lake). We also perform our scheme on another CPU architecture, Intel Xeon Silver 4314(Ice Lake-SP). 
\textbf{CPU Architecture:} Ensuring the validity of Litmus pricing across different architectures is crucial. Our Litmus tests rely on the performance counter that measures a stall count due to L2 cache misses (cycle\_activity.stalls\_L2\_miss)~\cite{perfMonEvents}, supported by Intel's CPUs. Unfortunately, other vendors like AMD do not yet offer the same performance counter~\cite{amdPMC}, restricting our tests to Intel CPUs. Alternatively, we conducted tests on another Intel CPU based on the Ice Lake architecture, Xeon Silver 4314, to broaden the scope of our analysis.

\begin{figure}[b]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun70kiwi}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 70 others on Xeon Silver 4314, both normalized to commercial prices}
\label{fig:normalizedPriceCorun70kiwi}
\end{figure}

% Because of the limitation of our memory size, we test Limtmus with 70 co-running applications. In this test, we use method 2 introduced in section~\ref{sec:temporalCPUSharing}. We first conduct the congestion and performance tables with 50 applications running in the first 5 cores. Then for the evaluation, we run 70 applications in the first 7 cores to let our testing application compete with 9 other applications for a core.  Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus discounting the tenant only pays 82.52\% commercial price. It's 0.696\% less than with the ideal discount.
Once again, this evaluation was conducted following the configuration outlined in Section~\ref{sec:temporalCPUSharing}, albeit with 70 co-running functions, limited by the main memory capacity of 128GB. Following Method 2, we constructed new congestion and performance tables with 50 functions running across 5 cores. Then, we ran 70 functions across 7 cores to match the competition count, averaging 10 functions per core. Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus pricing, the tenant only pays 82.5\% of the commercial prices, which is merely 0.7\% less than the ideal price.

% \textbf{Per-core Function Count:} When altering the co-located applications in each core the performance of the application can also be influenced. In this test, we put 240 applications in the first 16 cores. The testing application is competing with 14 other applications. We used the same congestion and performance tables from section~\ref{sec:temporalCPUSharing} method 2. Figure~\ref{fig:normalizedPriceCorun15} presents the results. The error of Litmus pricing is 1.23\% with The average discount of 16.69\%. The ideal discount is 17.92\%. The mean price of Litmus is larger than the ideal price because we are using the tables that are made based on 10 applications per-core. The context-switching overhead is larger. But, from figure~\ref{fig:csImpactor} we know that there is a diminishing impact of per-core application count. The error of the Litmus pricing is still under control when we increase the per-core application count.
\textbf{CPU Sharing Overhead:} The co-located function count determines the level of interference, impacting a function's performance differently. To assess Litmus pricing under various co-running function counts, we increased the function count to 240 from the configuration outlined in Section~\ref{sec:temporalCPUSharing}, making an average of 15 functions running on each core. However, we reused the performance and congestion tables generated in Section~\ref{sec:temporalCPUSharing}. Figure~\ref{fig:normalizedPriceCorun15} illustrates the results, where the Litmus pricing's error is 1.2\% with an average discount of 16.7\%, compared to the ideal of 17.9\%. Despite reusing the tables constructed for 10 co-running functions per core, the error remains negligible. This outcome aligns with Figure~\ref{fig:csImpactor}, which highlights the diminishing impact of temporal sharing when running more than 10 co-running functions. Given the perpetual overcrowding of commercial systems, any configuration gap between the environment where constructing the tables and where conducting tests is expected to remain minor and easily manageable.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun15}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 15 functions per core and reusing tables, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun15}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun160smt}
\end{figure}

\textbf{Simultaneous Multithreading (SMT):} SMT is a technique aimed at maximizing resource utilization by enabling multiple threads to execute concurrently on the same core, extending the shared resource domain across the entire processor. However, while SMT enhances resource utilization, it significantly complicates the measurement of interference impact. Moreover, SMT introduces additional side channels, thereby increasing the processor's vulnerability to security attacks. Due to these concerns, serverless platforms like Amazon Lambda disable SMT in their systems~\cite{schall2023warming,agache2020firecracker,schall2022lukewarm}. Nonetheless, we have conducted a study to assess the impact of SMT on our Litmus pricing methodology.

% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
% \caption{Prices computed via Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, normalized to the commercial prices}
% \vspace{-0.5em}
% \label{fig:normalizedPriceCorun160smt}
% \end{figure}

% To generate the performance/congestion tables, we executed 50 applications across 5 dedicated physical cores. In this way, the testing function is co-located with 9 other applications in the same virtual core and 19 other applications in the same physical core. Fiugre~\ref{fig:normalizedPriceCorun160smt} illustrates the results. The first thing we notice is that the normalized price is much smaller compared with the setups without SMT turned on. The average discount of Litmus is 45.42\% which is 1.9\% smaller than the average ideal discount of 47.32\%.
To construct the performance and congestion tables, we executed 50 applications across 5 physically separated cores, allowing an average of 10 functions to share two virtual cores. Figure~\ref{fig:normalizedPriceCorun160smt} illustrates the results,  presenting prices derived from Litmus pricing and ideal prices, both normalized to commercial prices without discounts. The normalized price experiences a significant drop compared to other configurations, highlighting the impact of heavy congestion within a physical core. The ideal price, which assumes no interference, stands at 47.3\% of the commercial price. Meanwhile, Litmus pricing offers a discount of 45.4\%, which is only 1.9\% less, confirming the effectiveness of Litmus pricing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Node JS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Nodejs Startup:}NodeJs is another well-adopted language in serverless platforms besides Python. It's one of the earliest languages to be supported by AWS Lambda ~\cite{serverless1}. From Section~\ref{sec:designDetails} we see that NodeJs has a long startup phase which makes it a great candidate when we need to pick a language startup phase for the Litmus test. 

%\begin{figure}[h]
%\centering
%\vspace{-0.5em}
%\includegraphics[width=1\columnwidth]{./fig/njReferenceStartupSlowdown}\\
%\vspace{-1em}
%\caption{The correlation between the normalized NodeJs's startup phase and the normalized reference applications.}
%\vspace{-0.5em}
%\label{fig:njReferenceStartupSlowdown}
%\end{figure}

%Figure~\ref{fig:njReferenceStartupSlowdown} shows the correlation between NodeJs startup phases and reference applications. After applying the Litmus test with NodeJs applications, with this figure, we can use the slowdown of the NodeJs startup phase to find the corresponding system congestion level and the discount rate for both private and shared resources. NodeJs has a longer startup phase compared with Python. It gives us more room when picking the most suitable portions of the startup phase. We can choose the language to be used for the Litmus test based on the density of the startup phase. 


==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/10_related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Serverless:} Many works address the performance bottleneck of serverless execution~\cite{du2020catalyzer}~\cite{agarwal2021reinforcement}~\cite{roy2022icebreaker}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Schall et al.~\cite{schall2022lukewarm} record and reload the instructions to reduce the front-end stalls when reaccessing the same application. Jovan et al.~\cite{stojkovic2023specfaas} focus on the performance of an application chain. They break the execution flow and speculative execute the functions. However, we are focusing on the price which is one of the most important potions of the cloud ecosystem.

% For the cloud providers, accommodating more tenants in a machine is a key strategy, gaining higher profits by maximizing the utilization of their machines. However, the approach inevitably introduces interference between tenants, slowing down applications unpredictably. Thus, prior researchers solved this challenge by allowing the tenants more non-biased, predictable, quality services~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed a clustering-based cache partitioning to remove unfairness between tenants. Rohan et al.~\cite{roy2021satori} simultaneously control multiple architectural resources to aim for both fairness and throughput. However, offering fairness inevitably sacrifices resource utilization. Thus, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} solve the unfairness uniquely by adjusting their prices while leaving the unfairness at a certain degree. This paper follows this direction but explores a more practical solution in serverless computing. 

Cloud providers strive to maximize profits by accommodating more tenants on their machines, which inevitably introduces interference between tenants, leading to unpredictable application slowdowns. To address this challenge, prior researchers have focused on providing tenants with a more unbiased and predictable quality of service~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed clustering-based cache partitioning to mitigate unfairness between tenants. Rohan et al.~\cite{roy2021satori} aimed for both fairness and throughput by simultaneously controlling multiple architectural resources. However, achieving fairness comes at the cost of sacrificing resource utilization. In contrast, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} addressed the unfairness by adjusting their prices while accepting a certain degree of unfairness. Our study follows a similar direction but explores a more practical solution within the context of serverless computing.

% delete the following section: the approaches are against our scheme. 
% \textbf{Serverless Computing:} Many studies focus on reducing the latencies of serverless applications~\cite{cadden2020seuss,oakes2018sock,wang2019replayable,jia2021boki}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Ustiugov et al.~\cite{ustiugov2021benchmarking} record and prefetches the functions’ stable working set of guest memory pages to further reduce the function's startup time. Wei et al.~\cite{wei2023no} remote forking the serverless functions to reduce the cold start latency while limiting the resource usage. Schall et al. record and reload the instructions~\cite{schall2022lukewarm} or the BTB entries ~\cite{schall2023warming} to reduce the front-end stalls when reaccessing the same application. 
% \hl{Litmus is orthogonal to these approaches and can be adopted together.}

==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Serverless computing is a key technology in present cloud computing, offering numerous advantages. One primary advantage is its effective cost-saving, as tenants only pay for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion. While tenants suffer slowdowns, they also have to pay more for the slowdowns. Unlike prior approaches that aim to maintain quality of service, this paper discounts the tenant's cost to compensate for the loss. Litmus pricing proposed in this work monitors the machine states and adjusts the tenants' costs. The congestion level can be frequently gauged before every function using the proposed Litmus test, an effectively lightweight testing approach. Our tests show that Litmus offers near-ideal prices with a 0.38\% difference, compared to the ideal price that discounts proportional to its slowdown. 
Serverless computing is a key technology in contemporary cloud computing, offering a range of benefits. One primary advantage is effective cost-saving, as tenants are billed only for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion, which not only results in slowdowns but also higher costs for tenants. Rather than aiming to maintain service quality, this paper suggests discounting tenants' costs to compensate for performance losses. Litmus pricing proposed in this work monitors machine states through Litmus tests and adjusts tenant costs accordingly. The Litmus test is a lightweight testing approach for serverless platforms, which assesses the machine's congestion level before starting a user's function. Our tests prove that Litmus pricing offers nearly ideal prices in heavily congested environments, with an average deviation of just 0.2\% from the ideal price that adjusts discounts in proportion to the slowdown experienced.


==> ctcrcykcwxxfdgjzsjwjdnxngwntyqsg/12_ack.tex <==
\section{Acknowledgment}
\label{ack}

We would like to thank our reviewers for their valuable feedback to improve this paper. This work was supported by NSF CAREER Award CCF-2146475.


==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/00_abstract.tex <==
\begin{abstract}

% Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While the providers can utilize their machines more efficiently, the tenants only need to pay for the resources they consume. However, a serverless system co-runs thousands of short-living functions concurrently to maximize resource utilization, bearing frequent state shifts. Meanwhile, when the system gets too congested, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants are also charged higher costs when experiencing slowdowns since all commercial serverless platforms determine the tenants' costs proportional to their execution times.
Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times.

% This paper argues that the cloud providers should compensate the tenants for their loss when the server is over-provisioned. However, estimating the tenant's loss is challenging when there is no pre-profiled information about the function. Prior studies showed assessing the tenant's loss introduces heavy overheads. Instead, this paper proposes a new pricing model, Litmus pricing, which offers discounts based on the machine's state while presuming the tenant's loss under the state. To monitor the machine state correctly, Litmus pricing frequently conducts Litmus tests, an effectively lightweight solution to measure system congestion. Our experiments show that Litmus pricing can detect the impact of system congestion and offer near-ideal prices, with only a 0.38\% price difference. 
This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2\% price difference on average, in a heavily congested system.

\end{abstract}


==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Serverless computing is growing fast, satisfying today's high demands for better programmability. It allows tenants to develop their programs as stateless functions in high-level languages such as Python, Go, and JavaScript without concerns with low-level resource management and task scheduling~\cite{serverless2,serverless1,schall2022lukewarm,schall2023warming,mohammad2020SerInWild}. This advantage attracts cloud users, helping them to deploy their programs quickly with minimal effort. Recent reports note that over 50-70\% of cloud users have adopted serverless computing for their tasks~\cite{serverless1}.

% Serverless computing claims a pay-as-you-go pricing model where users only pay for the resources used by their functions. This requires the service provider to monitor and estimate the fine-grained resource usage by each user accurately. However, today's high-performance systems maximize resource efficiency by accommodating multiple applications simultaneously and allowing the resources to be shared by them. Such a shared system raises two major challenges. First, tracking a user's resource usage is a challenging task. While being shared, the system tracks the total usage but not a single user's. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress. These inferences between the applications not only make the system hard to track resource usage, but the users may get charged unfairly due to the delayed execution time.
Serverless computing also benefits tenants financially. Unlike traditional cloud platforms that require tenants to purchase the hardware resources needed to deploy their servers regardless of actual usage~\cite{amazonEC2Pricing}, serverless computing claims a pay-as-you-go pricing model, where tenants only pay for the resources consumed during the execution of their functions, facilitating significant cost savings. Meanwhile, this pricing requires service providers to accurately monitor and estimate each user's fine-grained resource usage~\cite{microsoftAzurePricing,awsLambdaPricing,googleCloudFunctionPricing}. 

% However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared system raises two major challenges. First, tracking a tenant's resource usage is a challenging task. While being shared, the system can only monitor a tenant's use of specific resources. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference between the applications not only makes the system hard to track resource usage, but the tenants may get charged unfairly due to the extended execution time~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}. 
However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared serverless system raises two major challenges. First, tracking a tenant's resource usage becomes challenging, as the system can only monitor a tenant's use of exclusively dedicated resources while the system is shared. Second, and more importantly, co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference not only complicates tracking resource usage but also leads to tenants being charged unfairly due to delayed execution times~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}.

% A serverless platform should provide an isolated runtime environment to a user. Otherwise, we argue that the platform provider must compensate a tenant's loss as a discount when it is not achievable. Therefore, we define a charged fee as fair when it reflects the tenant's slowdowns due to the resource sharing. The following two methods can be used to estimate a fair price under a multi-tenant environment. 
A serverless platform should provide a user with an isolated runtime environment. Otherwise, we argue that the platform provider should compensate a tenant's loss as a discount when the isolation is not achievable. Thus, we define a charged fee as fair when it reflects the tenant's slowdowns caused by resource sharing. The following two methods can be used to offer a fair price in a multi-tenant environment.

% First, strict resource partitioning can divide shared resources into multiple partitions, each assigned to a user exclusively. The user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strictly partitioned resources are well known to cancel the opportunities to utilize the given resource efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delayed execution directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources when requesting them. 
First, strict resource partitioning can divide shared resources into multiple partitions, each assigned exclusively to a user. This means the user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strict partitioning is known to cancel opportunities to utilize resources efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delay directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources they need when requested. 

% Alternatively, a discount-based scheme estimates a user's price relative to its slowdown, discounting from the price when run without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources. Thus, the providers can maximize their hardware utilization and earn more money with given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns or interference they get from co-running tasks without overpaying for exclusive resources.
% The tenants also can get a discount reasonably proportional to the amount of their slowdown when their jobs suffer from interference rather than endeavoring to secure necessary resources exclusively.
Alternatively, a discount-based scheme estimates a user's price relative to the slowdown experienced, discounting from the price when running the task without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources, enabling providers to maximize hardware utilization and generate more revenue with the given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns they experience due to co-running tasks, preventing them from overpaying for lowered service quality.

% While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Even if the platform can measure its execution time, computing the slowdown still requires knowing its baseline, which can be gained when executing it alone. The cloud platform could not pre-profile users' applications for reasons such as mandated privacy when processing confidential information. Even if the platform has such information, the function could operate differently when receiving different inputs. That is to say, online profiling is necessary, which unfortunately requires expensive runtime sampling, as proposed in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. All co-running tasks must be stalled when estimating a task's baseline performance. Massive short-living serverless functions make such a sampling-based solution even more impractical. Frequently sampling the baseline performance of thousands of co-running functions is unrealistic. This motivates a new practical solution that can be adopted in commercial platforms. 
While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Although the platform can measure its execution time, determining the slowdown requires knowing its baseline performance, which can be obtained when it runs without interference. However, such profiling is often prohibited due to security concerns, particularly when the function processes confidential information. Additionally, the function may behave differently, with varying inputs each time it runs. That is to say, online profiling is necessary. Unfortunately, this requires expensive runtime sampling, as presented in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. When assessing baseline performance, all co-running tasks must be stalled. Hundreds to thousands of concurrent short-lived functions make this approach indeed impractical, as frequently sampling the baseline performance of such numerous functions is unrealistic. Thus, a new, practical solution that can be adopted in serverless platforms is needed.

%In either approach, a tenant or a service provider bears the problem's complexity alone. Resource partitioning demands the tenant to know the needed resources while losing opportunities to utilize the resources better. Discounting demands a service provider to estimate the task's slowdown with heavy sampling overheads. Accordingly, both approaches complicate the problem while sacrificing the machine's efficiency. Instead, we claim this problem becomes simpler when both entities participate and carry a portion of the responsibilities. 

% Litmus addresses this challenge by imposing the responsibility on both entities. With Litmus, the serverless platform measures the system congestion that may delay a function's execution when every tenant's function starts. The service provider needs to determine a discount rate for a corresponding congestion state. Meanwhile, the tenant needs to know about a possible slowdown and a corresponding discount. 

% We highlight that both partitioning and sampling complicate the problem while sacrificing the machine's efficiency and can hardly be employed in serverless computing. The approaches in serverless must be lightweight and frequent to deal with the fast-changing environment with thousands of concurrent functions. This paper proposes Litmus pricing that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening the system performance. 
We highlight that both partitioning-based and sampling-based approaches complicate the problem, either sacrificing the machine's efficiency or appearing impractical for serverless computing. Approaches in serverless computing must be lightweight, frequent, and sensitive enough to deal with quickly changing environments with numerous concurrent functions. This paper proposes Litmus pricing, a method that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening system performance. 

% \hl{Measuring the server's congestion status is challenging work. Here, Litmus relies on our key observation that, although not limited, function implementation in serverless computing largely relies on high-level programming languages such as Python and GoLang, which require a relatively long startup. This startup overhead has been considered one of the major challenges in serverless computing. However, Litmus utilizes this startup to measure the system's congestion state. Our analysis of Python and GoLang observed that the activities during the startups are almost identical, with plenty of memory operations, regardless of the functions. Thus, we claim that the startup performance can be an index of the system state.}

% \hl{The Litmus test is based on our insight that the serverless functions perform broadly identical operations, with plenty of memory operations, during their long startups, preparing the runtime environment for the functions. Leveraging this observation, the platform can assess the system's congestion level, which hints at the tenant's discount amount. Additionally, Litmus pricing exploits our second insight that the performance of two resources, private and shared, are affected differently by the congestion. In particular, its impact on private resources is minor and predictable, while many functions significantly rely on them, spending most of their execution time with them. }

% During the execution of every function, Litmus pricing conducts a Litmus test, which measures the level of system congestion with no extra overhead using the function's startup process. The Litmus test is based on the observation that serverless functions perform largely identical operations during their startup time. Those operations usually prepare the runtime and include a large amount of memory access to shared hardware resources. In addition, Litmus pricing splits the hardware resources into "private" and "shared" and proposes charging different ratios on each. This further improves the accuracy of the discount calculation.
During each function's execution, Litmus pricing conducts a Litmus test, which measures the level of system congestion without adding extra overhead, using the function's startup process. Litmus test is based on the observation that serverless functions perform largely identical operations during their startup, typically involving significant memory accesses. Additionally, Litmus pricing splits the hardware resources into "private" and "shared" categories, proposing different charging ratios for each. This approach further enhances the accuracy of the discount calculation.

% In our experiments, the Litmus pricing estimates a tenant's price to be nearly ideal, with a \hl{0.38\%} difference from the ideal price, which discounts tenants proportional to their slowdowns.
% This study investigates Litmus pricing across different environments, ranging from restricted to crowded settings. We verify that crowded environments pose additional challenges. Despite this, Litmus pricing accurately estimates a tenant's price, deviating by only 0.26\% from the ideal price, discounting tenants proportional to their slowdowns.
This study investigates Litmus pricing across diverse environments with varying levels of system congestion. We confirm that crowded environments pose complex challenges. Despite this, Litmus pricing accurately estimates a tenant's cost, deviating by only 0.2\% on average from the ideal price that discounts tenants proportional to slowdowns.



==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/02_background.tex <==
\section{Background}
\label{sec:background}

% \textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while the service providers handle back-end implementation~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers, which are later invoked upon associated events~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. The serverless platform guarantees security by executing the tenant's function in a sandbox such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.
\textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while leaving back-end implementation managed by service providers~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. These functions are later invoked upon associated events. The serverless platform ensures security by executing the tenant's function in a sandbox, such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.

% Each tenant's function is stateless and expected to be short~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using the short-lived functions, the tenant can easily scale by invoking many of the functions without provisioning needed resources for themselves, relying on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. Inherently, massive short-living serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. The tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and clients mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Later, under the pay-as-you-go pricing, the tenant is charged for the consumed resources, typically the product of time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
Each tenant's function is stateless and expected to be short-lived~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using these short-lived functions, tenants can easily scale by invoking many functions without provisioning the needed resources for themselves, relying instead on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. In serverless computing, numerous short-lived serverless workloads run together on a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. Tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and tenants mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% In the traditional cloud, tenants purchase hardware resources for the contracted term to support their applications, which are often expected to be large in a server form. Thus, tenants must pay for the agreed period regardless of actual use. Instead, serverless workloads are generally small and launched on-demand as short-living event handlers. This workload difference develops a unique pricing policy, pay-as-you-go pricing. The tenant is charged only for the consumed resources during the execution, typically the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
In traditional cloud computing, tenants purchase hardware resources for a contracted term to support their applications, which are typically large servers. Thus, tenants must pay for the agreed period regardless of actual usage. In contrast, serverless workloads are generally small and launched on-demand as short-lived event handlers. This difference leads to a unique pricing policy known as pay-as-you-go. Under this model, tenants are charged only for the resources consumed during execution, typically calculated as the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, where Python is utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Also, over 90\% of organizations choose Python and Node.js for their AWS services. Other popular language runtimes are Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer a high level of abstraction from machine codes with good programmability and portability, improving the programmer's productivity. As a result, they have been adopted widely by serverless users. However, such high-level languages typically rely on runtime interpretation, which results in a slow start of program execution with extra launching steps. For instance, in the case of Python, when an application is launched, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the codes are compiled and executed. Once the execution is complete, the Python program is terminated, and all assigned resources are released~\cite{pythonUsage}.
\textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python used in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Over 90\% of organizations choose Python and Node.js for their AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer significant abstraction from machine code with good programmability and portability, which in turn improves programmer productivity. Consequently, they are widely adopted by serverless users. However, high-level languages typically rely on runtime interpretation, leading to slower program startup due to extra launching steps. For example, when an application is launched in Python, the interpreter is first prepared. It then parses command-line arguments and imports necessary modules. Afterward, the codes are compiled and executed. Upon completion, the Python program terminates, and all allocated resources are released~\cite{pythonUsage}.

 
% list of pricing models? 
% Amazon? 
% Google?
% The price is calculated by duration time multiplies to the unit price plus the request charges. The duration time is from the time user's code begins executing until it returns or terminates. The unit price depends on the amount of memory the user allocate to their function. The request charges is based on how many times the function has been invoked minus the free requests~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% may need service agreement here, contention impact

%\textbf{Traditional cloud platforms:} In the context of traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage, data transfer, etc. The instance type is the combination of Virtual CPUs(VCPUs), RAM, storage and network performances. The time unit price will be higher with more powerful instance type. Typically, more powerful instance types have higher time unit prices. There are two main pricing options: On-Demand and Reserved Instances. On-demand instance let the customers pay for compute capacity by the hour or second based on the actual usage with no long-term commitments. Reserved Instances, on the other hand, require a commitment to a specific instance type for a contract term and offer cost savings compared to On-Demand pricing. Storage and data transfer for the VM instance can also impact the pricing. The more storage space a customer uses or the more data they transfer, the higher their costs will be. The traditional cloud platform can also be affected by the co-running applications~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} In traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage space, data bandwidth, etc. The instance type includes virtual CPUs, RAM, storage, and network performances. Typically, more powerful instance types charge higher prices. Also, two pricing options are commonly offered: on-demand and reserved instances. On-demand instances allow tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved instances require a commitment to a specific instance type for an agreed term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period. Storage space and data bandwidth for the VM instance also influence the price. Demanding more storage space or more data transfer raises the cost~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} 

% The price of traditional cloud platforms is determined by computing capabilities such as processor type, memory capacity, and network bandwidth. While more and better resources typically charge higher prices, two pricing options are commonly offered: on-demand and reserved instances. On-demand pricing allows tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved pricing requires a commitment to specific resources for an agreed-upon term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period~\cite{amazonEC2Pricing}. 

% There are several differences between traditional cloud platforms and serverless platform. 
% Firstly, the roles of customers in the execution environment differ between traditional and serverless platforms. In the traditional cloud, customers are responsible for configuring and maintaining virtual machines (VMs), setting up networking, and managing databases~\cite{amazonEC2Pricing}. And it's the customers's responsibility to detact and update the configurations to balance their expenses and performance. On the other hand, in serverless platforms, users only provide a single file to indicate their system and library requirement, while the service provider handles the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. This feature enables users to focus solely on their actual workload without the burden of managing the infrastructures. Additionally, the platform can automatically scale the resources for the users based on the current demand of the application to guarantee the customer satisfaction~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% There are apparent differences between traditional and serverless cloud platforms. First, tenants are responsible for managing hardware resources in traditional platforms. The tenants need to configure and maintain virtual machines, set up networking, and manage databases~\cite{amazonEC2Pricing}. Also, tenants should study the optimal configurations to balance their expenses and performance. Meanwhile, in serverless platforms, tenants only provide a single file to specify their system requirements while the cloud provider prepares the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. The platform provisions or scales the needed resources on demand. Consequently, the serverless platforms encourage tenants to focus solely on their front-end workloads without the burden of managing the low-level back-ends~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% Secondly, there are notable differences in compute power and memory size options between the two platforms. For traditional cloud, the granularity usually 1 VCPU and 1GB memory. But, for serverless platform, the smallest memory size is 128 MB~\cite{awsLambdaApiGateWay,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Thirdly, the characteristics of workloads on these platforms set them apart. Serverless applications are generally small and executed on-demand, resulting in very short workload durations~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can complete in less than one second. In contrast, traditional cloud applications tend to be larger and may require hours to complete. Additionally, the number of co-located applications on a single computing node is smaller in traditional cloud setups, making their execution environment less dynamic compared to serverless platforms.
% Lastly, the billing periods differ significantly between traditional cloud and serverless platforms. Traditional cloud users are charged for the allocated time period. Regardless of whether they are actively running tasks on the machine, they are still need to pay for the allocated time period. However, serverless customers are only billed for the actual execution time of their tasks on the platform.

% Second, the workloads are expected to be small in serverless computing. Serverless workloads are generally small and launched on-demand as short-living event handlers~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can be completed in less than one second, unlike traditional cloud applications that are often expected to be large in a server form. Inherently, massive serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. This workload difference develops a unique pricing policy in serverless computing, pay-as-you-go pricing. In the traditional cloud, the tenants purchase hardware resources for the contracted term. Regardless of actual use, they need to pay for the agreed period. However, the serverless platforms bill their tenants for the actual execution time of their tasks.


% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python being utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Furthermore, over 90\% of organizations leverage Python and Node.js alongside AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer numerous advantages for programmers, such as user-friendliness, portability, reduced error risks, and thriving ecosystems. As a result, they have garnered widespread acceptance within serverless platforms. High-level programming languages typically follow a fixed execution procedure. For instance, in Python, when an application is executed, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the code is compiled and executed. Once the execution is complete, the Python program is terminated, and all resources used by the program are released. Due to the consistency of the operating system and Python version, the beginning of the execution process remains the same each time~\cite{pythonUsage}.



% \textbf{Resource based discount vs. Slowdown based discount:} To fully utilize the available resources, service providers often run as many applications as they can in one computing node within the service agreement requirement. However, this may lead to resource congestion and cause slowdowns for users, which can be unfair, since the customers are paying more money for the worse experiences. The intuitionistic solution could be for the service provider to track the resource usage of each application and offer discounts to users who consume fewer resources. However, serverless applications are typically very small, and contention can affect different applications differently, making this approach less practical. A more suitable solution for serverless platforms could involve offering slowdown-based discounts. In this approach, the service provider dynamically updates unit prices based on the level of system congestion. When there is less contention, users normally stiffed with the experiences and pay the regular price. However, during periods of high congestion, when the system is under heavy load, users could receive discounted prices as compensation for potential slowdowns. This approach would align pricing with the actual performance experienced by users, ensuring a fair and responsive pricing model.


==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/03_methodology.tex <==
\section{Methodology}
\label{sec:method}

% \textbf{Hardware Infrastructure:} All the experiments are performed on a dual-socket server platform. Each socket has 16 simultaneous multithreading(SMT) cores. The CPU model is Intel Xeon Gold 5218(Cascade Lake). The maximum frequency of the machine is 3.9GHz. Each core has a 32KB L1 instruction cache, a 32KB L1 data cache and a 1MB L2 cache. The 32 virtual cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The computer node runs the latest Ubuntu server version(Ubuntu 22.04 LTS) with kernel version 5.15.0. For consistency in the results, the core frequency was set to 3.0GHz using the 'cpupower frequency-set' command. We use linux perf~\cite{perfWiki} to collect the performance counters for each experiment. To analyze the startup status, we use -I 1 option to obtain count deltas at one-millisecond intervals. By utilizing interpolation, we can know the performance counters of each execution period. 

% In this study, we test today's server systems with serverless functions. This section describes our test configuration. 
This section outlines our test setup for evaluating serverless functions in this study.

% % original version
% \textbf{Hardware Infrastructure:} All experiments are performed on a dual-socket server platform with two Intel Xeon Gold 5218 (Cascade Lake). The CPU offers 16 simultaneous multithreading (SMT) cores with 3.9 GHz maximum frequency. We pin the core frequency at 3.0GHz for our tests. Each core has 32KB L1 instruction/data caches and 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The machine runs the Ubuntu server OS (Ubuntu 22.04 LTS) with a kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to collect the performance counters, which are collected at every one-millisecond interval. 
\textbf{Hardware Infrastructure:} All experiments are conducted on a dual-socket server platform equipped with two Intel Xeon Gold 5218 processors based on the Cascade Lake architecture. Each CPU provides 16 cores that support simultaneous multithreading (SMT) with a maximum frequency of 3.9 GHz. Every core features 32KB of L1 instruction/data caches and a 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets collectively have access to 384GB of main memory. The server operates on Ubuntu Server OS, version 22.04 LTS, with kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to gather performance counters.

% The CPU frequency is a key performance/energy factor, significantly affecting a function's execution time and energy consumption. A CPU's frequency can be altered in software or hardware based on its power and thermal budget, configuring it for better energy efficiency or performance. However, varying frequencies cause the system performance/energy to be unsettled, making system management intractable. For this reason, commercial systems such as Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. In our tests, when the frequency is not fixed by software, Intel's Turbo technology alters the frequency occasionally but mainly employs 2.8GHz. We will discuss this further in the sensitivity section.
The CPU frequency is a critical factor influencing both performance and energy consumption, significantly affecting a function's execution time and energy usage. A CPU's frequency can be adjusted through software or hardware based on power and thermal budget, optimizing for either energy efficiency or performance. However, varying frequencies can cause instability in system performance and energy usage, complicating system management. For this reason, commercial systems like Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. If we do not fix the frequency through software, Intel's Turbo technology occasionally adjusts it, but it mostly remains at 2.8 GHz during our tests. We will provide more details on this in Section~\ref{sec:sensitivity}.

% \textbf{Stressing Programs:} We used two stressing programs to investigate how applications and the startup portion of the high level languages behave in a resource contention environment. FigureXXX illustrates the number of instructions, L3 accesses, and L3 misses that the stressing programs can generate in five seconds as the stressing levels increase. By combining different stress levels of these stress-testing programs, we can simulate various resource-congested environments. The XXX-stressor(lineXXX)  generates more L3 accesses with a high L3 hit rate. While XXX-stressor(lineXXX), in each stressing level, generates fewer L3 accesses but more L3 misses. With these two stressors and different stressing levels, we can simulate the system with varying contentions to the shared resources by creating various  L3 accesses and L3 misses. In figureXXX we can see that the L3 accesses generated from the L2-stressor (update name later) begin to decrease after reaching stressing level 20.  However, during this period, the L3 misses continue to increase. The reason behind this trend is that, after stressing level 20, the heightened L3 miss rate starts to impact the stressor's performance, leading to a decline in the committed instruction count. Consequently, the stressor generates fewer L3 accesses and more L3 misses. 

% \begin{table}[h]
%     \begin{center}
%     % \vspace{-1.0em}
%         \caption{Serverless Benchmarks \& Runtimes}
%         \label{tb:benchmarks}
%         % \vspace{-1.0em}
%         \begin{tabular}{|l l||l l|} \hline
%             Function & Abbr. & Function & Abbr. \\ \hline \hline
%             \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  & \multicolumn{2}{c|}{\textbf{Hotel Reservation~\cite{gan2019open}}} \\ \hline
%             Dyn HTML & dyn-py & Geo & geo-go* \\ \hline
%             Thumbnail & thum-py* & Profile & profile-go \\ \hline
%             Compression & compre-py & Rate & rate-go \\ \hline
%             Image Recogn & recogn-py* & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
%             Graph Rank & pager-py & Currency & cur-nj* \\ \hline
%             Graph Mst & mst-py & Payment & pay-nj \\ \hline
%             Graph Bfs & bfs-py* & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
%             DNA Visual & visual-py* & Authen & auth-py/nj/go \\ \hline
%             \multicolumn{2}{|c||}{\textbf{Function Bench~\cite{kim2019functionbench}}} & Fibonacci & fib-py/nj/go* \\ \hline
%             Chameleon & chame-py & AES & aes-py/nj/go \\ \hline
%             FloatOp & float-py* & & \\ \hline
%             % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
%         \end{tabular}
%     \end{center}
%     % \vspace{-1.5em}
% \end{table}

\begin{table}[h]
    \begin{center}
    % \vspace{-1.0em}
        \caption{Serverless Benchmarks \& Language Runtimes (py, nj, go)}
        \label{tb:benchmarks}
        % \vspace{-1.0em}
        \begin{tabular}{|l l||l l|} \hline
            Function & Abbr. & Function & Abbr. \\ \hline \hline
            \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  &  \multicolumn{2}{|c|}{\textbf{Function Bench~\cite{kim2019functionbench}}}\\ \hline
            Dyn HTML & dyn-py & Chameleon & chame-py \\ \hline
            Thumbnail & thum-py* & FloatOp & float-py \\ \hline
            Compression & compre-py & Gzip & gzip-py* \\ \hline
            Image Recogn & recogn-py & RandDisk & randDisk-py* \\ \hline
            Graph Rank & pager-py & SequenDisk & seqDisk-py \\ \hline
            Graph Mst & mst-py & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
            Graph Bfs & bfs-py* & Currency & cur-nj* \\ \hline
            DNA Visual & visual-py* & Payment & pay-nj \\ \hline
            \multicolumn{2}{|c||}{\textbf{Hotel Reservation~\cite{gan2019open}}} & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
            Geo & geo-go & Authen & auth-py*/nj/go \\ \hline
            Profile & profile-go* & Fibonacci & fib-py*/nj*/go* \\ \hline
            Rate & rate-go & AES & aes-py/nj*/go* \\ \hline
            % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
        \end{tabular}
    \end{center}
    % \vspace{-1.5em}
\end{table}

% revision version
% \textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we select 27 distinct serverless functions from different benchmark suites, including AWS' authentication serverless functions~\cite{awsLambdaApiGateWay}, Hotel Reservation from the DeathStarBench suite~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and SeBS serverless benchmark suite~\cite{copik2021sebs}. The three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating 3 separate test cases per function. Among them, we pick 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. The functions are implemented using three languages: Python, Nodejs, and Go. We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. 
\textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we selected 27 distinct serverless functions from various benchmark suites, including AWS authentication serverless functions~\cite{awsLambdaApiGateWay}, the Hotel Reservation from DeathStarBench~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and the SeBS serverless benchmark suite~\cite{copik2021sebs}. The functions are implemented using three languages: Python, Nodejs, and Go. Notably, the three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating three separate test cases per function. 
% This comprehensive language support ensures that our test coverage is thorough and representative of the diverse language preferences in the serverless computing community. 
We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. Additionally, we selected 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. 


%\hl{The benchmarks we choose include I/O-bound, memory-bound, and compute-bound functions. For an experiment, we put the testing function in core 0 to core 4. We also put 50 other functions in core 0-4 to let the application co-running with 10 other applications to observe the impact of context switching.}

% \hl{We select benchmarks with mixed performance characteristics: I/O, memory, and compute-bound. Also, to replicate the congested commercial systems, we located a testing function with 50 other functions and tied them to selected 5 cores, Core 0 to 4. During our evaluation, those functions run simultaneously and compete to secure any core among the five.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
\caption{(a) L2 misses and (b) L3 misses of traffic generators, both normalized with the average L2 and L3 misses of serverless applications listed in Table~\ref{tb:benchmarks}}
% \vspace{-0.5em}
\label{fig:stressing_specs}
\end{figure}

% \textbf{Traffic Generator:} We divide the CPU's shared resources into two distinct categories: resources before and after the L3 caches. To pressure each resource group individually, we developed two separate traffic generators aimed at generating traffic and congestion in these resources. The first traffic generator, CT-Gen, applies pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another traffic generator, MB-Gen, induces massive L3 misses that stress the resources after the L3 cache, mainly the off-chip memory bandwidth and L3 cache spaces.
\textbf{Traffic Generator:} We categorize the CPU's shared resources into two groups: those before the L3 caches and those after. To stress each group independently, we developed two separate traffic generators designed to generate traffic and congestion within these resources. The first generator, CT-Gen, exerts pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another generator, MB-Gen, induces massive L3 misses, which stress the resources beyond the L3 cache, primarily targeting off-chip memory bandwidth and L3 cache spaces.

% Both traffic generators are multi-threaded, governing the volume of traffic by adjusting the number of threads they spawn. Each thread spawned by the traffic generator is pinned on each core to prevent conflicts between threads; consequently, this setup allows us to vary the stress level across our 32-core processors, ranging from level 1 to 31. Figure~\ref{fig:stressing_specs} shows each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), for every thread count increment, CT-Gen makes massive L2 misses. The CT-Gen's L2 misses are ended with L3 hits, as shown in Figure~\ref{fig:stressing_specs}(b). Meanwhile, MB-Gen creates huge L2 and L3 misses, as implemented. Interestingly, its L2 misses are fewer than CT-Gen's because MB-Gen is slowed by its L3 misses, suffering from a self-created bandwidth bottleneck. 
Both traffic generators are multi-threaded and govern the amount of traffic by adjusting the number of threads they spawn. Each thread is pinned to a specific core to avoid conflicts between threads, allowing us to vary the stress level on our 32-core processors from level 1 to 31. Figure~\ref{fig:stressing_specs} illustrates each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), with each increase in thread count, CT-Gen generates substantial L2 cache misses. These L2 misses by CT-Gen are ended with L3 cache hits, as shown in Figure~\ref{fig:stressing_specs}(b). In contrast, MB-Gen produces significant L2 and L3 cache misses. Interestingly, MB-Gen's L2 misses are fewer than those of CT-Gen because MB-Gen is hindered by its L3 misses, suffering from a self-imposed performance bottleneck.



==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/04_motivation.tex <==
\section{The Need for Fair Pricing}
\label{sec:motivation}

% Offering fairness appears in different approaches in cloud computing when multiple tenants share hardware resources. One standard is SLA, which defines the level of services the cloud provider furnishes while a tenant sets their expectation. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving unfairness between tenants. Although serverless computing highlights the pay-as-you-go pricing model, such unfairness still exists.
Fairness in cloud computing, especially when multiple tenants share hardware resources, is addressed through various approaches. One standard method is the Service Level Agreement (SLA), which specifies the level of service the cloud provider must deliver and the tenants' expectations. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving fairness issues. Despite serverless computing's emphasis on a pay-as-you-go pricing model, unfairness among tenants still exists.

% Unfortunately, modern systems are designed to maximize hardware efficiency by co-running multiple applications; the function's execution time can be affected by co-scheduled applications with conflicts when using shared resources. Ironically, whenever the service provider squeezes their resources further for better profit by accommodating more functions into a single machine, each function's execution time increases, charging them a higher cost for the same workload. However, in serverless computing, tenants lack control and insights into how their software is executed and billed for the cost of convenience. 
Unfortunately, modern systems are designed to maximize hardware efficiency by running multiple applications concurrently. This results in conflicts over shared resources, affecting each function's execution time. Ironically, when service providers optimize for profit by packing more functions into a single machine, the execution time for each function increases, resulting in higher costs for the same workload. In serverless computing, tenants have no control or visibility over how their software is executed, leading to potential inefficiencies and higher costs for the sake of convenience.

% Genuine pay-as-you-go pricing can be achieved when there is no interference. However, that is not desired by the providers who expect to utilize their resources to maximize profits. In serverless, although each function runs virtually exclusively in a sandbox with private resources, it still shares a few resources with other co-running functions, such as shared caches and memory bandwidth. Resource partitioning, a traditional solution that eliminates interference, can promise exclusively dedicated resources to a tenant but cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 
In serverless computing, although each function runs exclusively in a virtual sandbox with private resources, it still shares certain resources like caches and memory bandwidth with other functions. Resource partitioning, a traditional solution that eliminates interference by dedicating resources exclusively to a tenant, cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 

\begin{figure}[h]
\centering
% \vspace{-0.7 em}
\includegraphics[width=1\columnwidth]{./fig/normalizedCPIRunWith26Rev}\\
% \vspace{-1 em}
\caption{Execution time of applications that run with 26 others, normalized to the execution time when running alone}
% \vspace{-0.4 em}
\label{fig:normalizedCPIRunWith26Rev}
\end{figure}

% Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed down when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. \hl{Whenever a function finishes, another function is randomly launched to maintain a total of 26 co-running functions.} The figure shows a function's performance drops by up to 35\%, and most functions are significantly influenced by the co-running functions. Compared to when an isolated environment is offered, the function performs 11.5\% slower on average, charging 11.5\% more to users. We highlight that the function runs only with 26 other functions, which is tiny compared to massively crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.
Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. Whenever a function finishes, a new randomly-selected function is launched to maintain a total of 26 co-running functions. The figure shows a function's performance can drop by up to 35\%, with most functions significantly impacted by the co-running functions. On average, functions perform 11.5\% slower in this shared environment compared to an isolated one, resulting in users being charged 11.5\% more. We highlight that this scenario involves only 26 co-running functions, which is tiny compared to heavily crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.

% Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} attempted to offer price discounts if it has a slowdown, compensating for the slowdowns. To provide the discount, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount reflecting the slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all the responsibilities of the contentions between co-running functions, guaranteeing all tenants an invariant price for their use. Any unexpected slowdowns that a tenant experiences are returned with a discount. However, sampling is an expensive operation, requiring all co-running processes to stall during the sampling. Moreover, accurate measurement requires frequent sampling when its system environment quickly alters, making the approach impossible in a fast-shifting environment like a serverless platform.   
Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} offers price discounts to compensate for slowdowns. To provide these discounts, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount based on the observed slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all responsibilities related to contentions from resource sharing, ensuring tenants pay a consistent price for their usage. Any unexpected slowdowns that a tenant experiences are compensated with a discount. However, sampling is an expensive operation that requires stalling all co-running processes during the sampling. Moreover, accurate measurement necessitates frequent sampling, especially in rapidly changing environments, making the approach impractical for dynamic environments like serverless platforms.


% A tenant needs a new pricing model based on more than just execution time. However, prior approaches have limitations, burdening cloud participants too heavily; it is unsuitable for \hl{thousands} of concurrent short-lived functions in serverless computing. This motivates us to propose a new solution, Litmus pricing, that discounts prices based on the system state but offers lightweight with no overheads.
Overall, tenants need a new pricing model that considers more than just execution time. Prior approaches have limitations, excessively burdening cloud participants and being unsuitable for the many short-lived functions typical in serverless computing. This motivates us to propose a new solution: Litmus pricing, which discounts prices based on the system congestion while remaining lightweight and imposing no additional overhead.


==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/05_design.tex <==
\section{Litmus Pricing}
\subsection{Overview}

% The estimated prices of serverless functions should reflect the congestion level of the system inside their machines. With the massive short-living functions, the serverless system's state can dramatically change in a short time. Accordingly, the system state can be congested at any moment and also resolved in a short time. However, such a temporary traffic jam may significantly impact the performance of short-living functions. Therefore, assessing the congestion must be lightweight, quick, and on time. However, a prior approach, POPPA\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling with considerable performance overheads, preventing them from wide adoption. Instead, we propose a new scheme, Litmus pricing, that quickly estimates system congestion at the start of every function and reflects the estimation into pricing the function. 
The estimated prices of serverless functions should reflect the system's congestion state. The presence of numerous small transient functions within the serverless system can rapidly alter its congestion state, causing sudden congestion or swift resolution. Nevertheless, such transient traffic jams can significantly impact the performance of short-lived functions. Thus, assessing the congestion must be lightweight, quick, and timely. However, a prior approach, POPPA~\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling, which incurs considerable performance costs, thereby limiting its widespread adoption. Alternatively, this study introduces Litmus pricing, which promptly gauges system congestion at the onset of each function and reflects the estimated congestion level into pricing the function.

% Like the prior approach~\cite{tiwari2013enabling,alex2013ScFairPrice}, Litmus pricing suggests that the service provider discounts when a tenant's functions are intervened, compensating for the performance loss. To determine the discount ratio, Litmus measures system congestion level, which can also help service providers evaluate remaining resources and make decisions on job scheduling. 
Like the prior approach, Litmus pricing suggests that service providers should offer discounts when a tenant's functions experience interference, thus compensating for the performance loss. Litmus pricing determines the discount rate based on the system's congestion level. Evaluating congestion also assists providers in estimating remaining resources and making informed decisions regarding job scheduling.

%Nevertheless, the Litmus pricing does not quantify each function's slowdown; the discount amount is determined only by the severity of the measured congestion. The impact of the congestion on distinct functions appears differently despite facing the same congestion level, and precisely estimating a function's performance loss is a complex problem. That's why the prior approach had to rely on expensive sampling. Instead, the Litmus pricing avoids the overheads and limits the service provider's responsibility to measure the current congestion. 
However, Litmus pricing does not quantify the slowdown of each individual function; the discount amount is solely determined by the severity of the measured congestion. Even though different functions face the same congestion level, their respective impacts can vary, making precise estimation of each function's performance loss a challenging task. This complexity necessitated the expensive sampling relied upon by the previous approach. Instead, Litmus pricing circumvents such overheads and lightens the service provider's burden solely to measure ongoing congestion levels.

% Litmus pricing embodies the varying value of shared resources across different system conditions by applying equal discounts to all functions under the same system condition, although the functions experience different slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that a function that is slowed more than others demands the over-crowded resources more while exacerbating the adverse over-crowded conditions. Litmus pricing does not provide additional compensation for their extra loss compared to others due to their heavy use of shared resources.
Litmus pricing captures the dynamic significance of shared resources under varying system conditions by offering uniform discounts to all functions under the same system congestion, regardless of their individual slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that functions experiencing larger slowdowns tend to demand more of the crowded resources, thereby exacerbating adverse overcrowded conditions. However, Litmus pricing does not offer additional compensation for the larger loss experienced by functions that use shared resources more heavily than others.

% As a result, Litmus inherently incentivizes users who use shared resources sparingly. When over-crowded, functions with minimal needs for shared resources still enjoy discounts but encounter slight slowdowns. This implies that users may take advantage of this policy by minimizing their use of shared resources, receiving substantial discounts despite enduring only minor slowdowns. Such a trade-off is considered acceptable because the user's shared resource usage reduces their contribution to congestion, thereby benefiting the overall system over the other users.
As a result, Litmus inherently incentivizes users who use shared resources sparingly. During periods of overcrowding, functions with minimal needs for shared resources still enjoy discounts but with only slight slowdowns. This implies that users may take advantage of this policy by minimizing their reliance on shared resources, receiving substantial discounts despite only experiencing minor slowdowns. This trade-off is considered acceptable because reduced shared resource usage by users helps mitigate congestion, thereby benefiting the overall system and other users.
% Lastly, the system refrains from scheduling a function if the congestion level exceeds a predetermined threshold, thus preventing resource thrashing.


\subsection{Pricing Model}
\label{pricing model}

% Developing Litmus pricing raises two challenges. First, Litmus needs a new pricing model to estimate a function's price. Second, Litmus needs a way to measure the system's congestion state. Due to the serverless's fast-shifting environment, assessing the congestion must be lightweight and frequent at the right time. Nevertheless, all present commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants must pay more with prolonged execution time when using over-crowded resources. Rather than simply imposing a price by multiplying the main memory usage and a function's total execution time, Litmus suggests the price as a sum of two distinct price components as follows.
Developing Litmus pricing raises two challenges. First, it needs a new model to estimate a function's price. Second, it needs a way to measure the system's congestion state. Due to the rapidly changing environment in serverless computing, assessing congestion must be lightweight and timely. Commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants end up paying more for prolonged execution time when using over-crowded resources. Rather than simply imposing the price by multiplying the main memory usage and a function's execution time, Litmus pricing determines the price as a sum of two distinct pricing components as follows.

\begin{equation} 
P = P_{private} + P_{shared}
\end{equation}

% In this equation, \(P\) denotes the total price tenants need to pay to execute their functions. Litmus pricing divides the tenant's price into two pricing components, each with a different resource type. \(P_{private}\) represents the price the tenant needs to pay for private resources, which are entirely assigned to a tenant. \(P_{shared}\) is the price the tenant needs to pay for the shared resources. Each price component is measured proportional to a user's time to occupy the corresponding resources. However, such occupied time can be extended when contention disturbs a process's execution in the shared resources. This delayed time increases a tenant's price unfairly. 
In this equation, \(P\) denotes the total price tenants must pay to execute their functions. Litmus pricing divides this cost into two pricing components, each associated with a different resource type. \(P_{private}\) is the cost for private resources, which are entirely assigned to a single tenant. \(P_{shared}\) is the cost for shared resources. Each pricing component is measured proportional to the time users occupy the respective resources. However, if contention disturbs a process's execution in the shared resources, the occupied time will be extended. This delay unfairly increases the tenant's cost. 


\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/slowdownRunwith26Rev}\\
\caption{\(T_{private}\) and \(T_{shared}\) of applications that run with 26 others, normalized to those when running alone}
\vspace{-0.5em}
\label{fig:slowdownRunwith26Rev}
\end{figure}

% Using Perf, we measure the delays due to the shared resources and split a function's execution time into two distinct slices: one slice, \(T_{private}\), which is time spent on private resources and another slice, \(T_{shared}\), which is time spent on shared resources. Figure~\ref{fig:normalizedTcore&Tuncore-runWith16} shows the impact of the contentions on each time slice, where we normalize \(T_{private}\) per instruction and \(T_{shared}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 207\% on average and 364\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions. 

% We observe that the system congestion influences the occupied time for each resource type differently. The time to hold private resources is slightly affected, with minor changes, even under heavy congestion. Meanwhile, the time due to shared resources is broadly affected, showing significant differences. Thus, we separately measure the two delays and charge their use with a different rule.
We observed that system congestion influences the occupied time for each resource type differently. The time to use private resources is only slightly affected, with minor changes, even under heavy congestion. In contrast, the time spent on shared resources is broadly affected, showing significant differences. Thus, we separately measure the delays for the two resource types and apply different charging rules for their use. 

% Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where we normalize \(T_{shared}\) per instruction and \(T_{private}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 181\% on average and 488\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions.
Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is calculated as the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where \(T_{shared}\) per instruction and \(T_{private}\) per instruction are normalized to the same tests when running alone. The figure shows that \(T_{shared}\) is significantly affected by system congestion compared to \(T_{private}\). On average, \(T_{shared}\) increases by 181\%, with a maximum increase of 488\%. Meanwhile, \(T_{private}\) increases by only 4\%, with minor variance between functions.

% This figure gives insights into two key factors. First, the congestion in the shared resources does not impact the performance of private resources. Accordingly, when the system gets congested, the degree of a function's dependence on the shared resources determines the function's performance. If the \(T_{shared}\) takes a minor portion of a function's execution, severe congestion still barely influences its overall execution. Second, hardware PMUs available in modern CPUs, and profiling tools such as Linux Perf are widely available and can be used to distinguish the usage of shared and private resources. Across the paper, we will take advantage of such tools to develop Litmus pricing.
This figure highlights two key factors. First, congestion in shared resources has a negligible impact on the performance of private resources. Accordingly, when the system gets congested, the extent of a function's reliance on shared resources determines its performance. If \(T_{shared}\) constitutes a minor portion of a function's execution, even severe congestion will have minimal impact on its overall execution. Second, hardware Performance Monitoring Units (PMUs) in modern CPUs and profiling tools like Linux Perf are widely available and can be utilized to differentiate between the use of shared and private resources. Throughout this paper, we will leverage these tools to develop Litmus pricing.

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/TpriTshardDistriRev}\\
% \caption{\(T_{private}\) and \(T_{shared}\) distribution when they run alone}
\caption{Execution time distribution of \(T_{private}\) and \(T_{shared}\)}
\vspace{-0.5em}
\label{fig:TpriTshardDistriRev}
\end{figure}

% Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) in a function's execution. The compute-intensive workloads (e.g., fib-py, float-py) have a substantial \(T_{private}\) portion that can reach 99.96\% of the execution time. However, the portion decreases when running memory-intensive workloads such as fib-nj. This distribution indicates how much other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase float-py's \(T_{shared}\), its total execution time, $T_{private}+T_{shared}$, will undergo minor change.
Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) during a function's execution. Compute-intensive workloads (e.g., fib-py, float-py) exhibit a substantial \(T_{private}\) portion, accounting for up to 99.96\% of the execution time. However, this portion decreases when running memory-intensive workloads such as fib-nj. This distribution reflects how other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase its \(T_{shared}\), the total execution time, $T_{private}+T_{shared}$, will undergo only a minor change.

% For each pricing component, we calculate the price by multiplying its charging rate with its time distribution. Thus we can further update the pricing equation.
After collecting the time slices spent on each resource, Litmus calculates each pricing component by multiplying two different charging rates with corresponding slices. Consequently, a new pricing equation emerges as follows:

\begin{equation} 
P = R_{private} * T_{private}  + R_{shared} * T_{shared}
\end{equation}

% \(T_{shared}\) is the cycles stalled due to L2 misses. It is measured from the perf counter, STALLS\_L2\_Misses. \(T_{private}\) is the total execution minus STALLS\_L2\_Misses. 
% Using Perf, Litmus collects\(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total cycles to complete the application minus \(T_{shared}\). 
% While Litmus returns the system's congestion state, the service provider still needs to determine reasonable prices charged for a service when having different congestion levels. 

% \(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. Again, the two charging rates are necessary since each component is affected differently, directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from the crowded execution environment. Thus, the charging rates should be measured as follows.
\(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. These two charging rates are necessary because each component is affected differently, either directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from a crowded execution environment. Thus, the charging rates should be measured as follows:

\begin{equation} 
R = R_{base} * \frac{T_{solo}}{T_{congestion}}
\end{equation}

% In this equation, \(R\) is the charging rate for executions on either private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free execution environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is the execution time when the function runs alone, and \(T_{congestion}\) is its execution time in the congested environment. Again, we should collect a separate \(T_{solo}\) and \(T_{congestion}\) for each pricing component. To measure \(T_{solo}\), \hl{the prior work}~\cite{alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. Litmus pricing avoids such a costly approach but presumes the function's \textit{solo} performance by examining reference workloads on the system.
In this equation, \(R\) represents the charging rate for executions on private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free runtime environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is its non-interfered execution time when the function runs alone, and \(T_{congestion}\) is its execution time in a congested environment. We need to collect separate \(T_{solo}\) and \(T_{congestion}\) values for each pricing component. To measure \(T_{solo}\), the prior study~\cite{tiwari2013enabling,alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. However, Litmus pricing avoids such a costly approach by presuming the function's solo performance through reference workloads on the system.

% Litmus pricing requires both providers and tenants to be involved in the price decision. The providers need to decide on reasonable rates for each resource use by analyzing the selected representative functions running on the system. To offer reasonable discounts, the providers must choose the functions analyzed carefully, collecting the functions representing the system. The tenants must also know the consequences when their tasks heavily rely on any of the shared resources. Unfortunately, their tasks may get delayed more than the provider's expectation while still receiving the discount rate up to the expectation. 
Litmus pricing requires both providers and tenants to be involved in the price decision process. Providers need to establish reasonable rates for each resource usage by analyzing selected representative functions. To offer fair discounts, providers must carefully choose the functions to be analyzed, ensuring the functions accurately represent the system condition. Tenants must also know the consequences when their tasks heavily rely on shared resources. Unfortunately, their tasks may get delayed more than the provider's expectations while still receiving the expected discount rate. 

% Here, the Litmus pricing reflects the varying value of the shared resources when the system's congestion level changes; the importance of shared resources becomes more valuable when congested. 



==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/06_design_details.tex <==
\section{Estimating prices with Litmus}
\label{sec:designDetails}

% The providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}, before using Litmus pricing. The numbers in both tables are the slowdowns of codes while testing the system congestion. Shortly, the congestion table is filled with the slowdowns of startup codes, and the performance table is filled with the slowdowns of reference benchmarks. Litmus pricing needs three steps to charge the final price with a discount. First, the providers assess the system's congestion at multiple levels and range them in a table. This step completes the congestion table. Second, the providers study the impact of congestion on tenants' functions and complete the performance table. Lastly, the service provider determines a tenant's price based on the two tables. 
Before using Litmus pricing, service providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}. The congestion table lists the slowdowns during the startup phases, whereas the performance table lists the slowdowns of reference functions. Litmus pricing needs three steps to determine the final price with a discount. First, providers assess system congestion at multiple levels and record the results in the congestion table. Second, providers analyze the impact of congestion on reference functions and fill out the performance table. Lastly, providers determine a tenant's price based on the data from both tables.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tables}\\
\caption{Congestion and performance tables: numbers in both tables indicate the slowdowns of startup codes and reference functions, collected with CT-Gen and MB-Gen}
\vspace{-0.7em}
\label{fig:litmust_tables}
\end{figure}

\textbf{Step 1, Defining Congestion Levels:} We manage the system's congestion levels using two traffic generators that create a range of congestion states by stressing shared resources differently. The traffic generator is multi-threaded, creating traffic in shared resources to incur congestion, with each thread running on a separate core. We rank the stress levels from 1 to 32 by changing the number of active threads running on distinct cores. Entries from top to bottom in the congestion table indicate increasing stress levels.

% \begin{figure}[h]
% \centering
% \vspace{-1.5em}
% \includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
% \vspace{-1em}
% \caption{stressing program's instruction, L3 accesses and L3 misses }
% \vspace{-0.5em}
% \label{fig:stressing_specs}
% \end{figure}

% \textbf{Step 2. Measuring System Congestion:} Measuring the current level of system congestion that may influence a function's performance is a crucial challenge. If we assume that the platform does not have pre-profiled information about a function's performance, the platform cannot figure out whether co-running functions influenced the function. Additionally, the serverless platform's fast-changing states with massive short-living functions make the assessment even more complicated, requiring quick and frequent examinations.

% Meanwhile, measuring the amount of a system's congestion and its impact on performance is a crucial challenge. This challenge particularly stands apparent when being demanded to quantify the impact of the congestion on a running application without pre-profiled information about the application. Moreover, the serverless platform's fast-changing system states with \hl{numerous} short-lived functions make the assessment even more complicated, requiring quick and frequent performance examinations.
Measuring the amount of system congestion and its impact on performance is a crucial challenge. This challenge becomes particularly pronounced when trying to quantify the impact of the congestion on a running application without pre-profiled information about the application. The fast-changing system states of a serverless platform, with numerous short-lived functions, further complicate the assessment, necessitating quick and frequent performance examinations.

% Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. The proposal is based on the observation that high-level languages, such as Python and Node.js, used in serverless computing have long startup times to accommodate their runtime environments. Since the inception of serverless computing, these startups have been recognized as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests leverage these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests further validated that all tested functions exhibited similar performance characteristics during their startups. 
Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. This method leverages our observation that high-level languages like Python and Node.js, commonly used in serverless computing, have lengthy startup phases to accommodate their runtime environments. Since the inception of serverless computing, these startup delays have been identified as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests exploit these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests have validated that tested functions exhibit similar performance characteristics during startup phases. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_all}\\
% \caption{IPC for serverless applications with different runtimes in the first 100 milliseconds of their execution}
% \vspace{-0.5em}
% \label{fig:startupIPC_all}
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped}\\
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-1}\\
\includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped_3}\\
% \caption{IPC for serverless applications grouped by language runtime in the first 100 milliseconds of their execution}
\caption{IPC of serverless applications based on languages (Go, Python, and NodeJS) during their startup phase}
% \vspace{-0.7em}
\label{fig:startupIPC_grouped}
\end{figure}

% Figure~\ref{fig:startupIPC_grouped} depicts the fluctuation in IPC (Instructions Per Cycle) of a function during the first milliseconds of its execution. The x-axis shows a time flow since the beginning; every tick indicates a millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language, and the throughput of each group is represented in separate figures. Although figures exhibit different patterns, functions in the same figure display notable similarities. The figures imply that functions written in the same language have nearly identical startups.
Figure~\ref{fig:startupIPC_grouped} depicts a function's fluctuation in IPC (Instructions Per Cycle) during its startup phases. The x-axis represents the time elapsed since the beginning, with each tick indicating one millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language runtime, and the IPC of each group is presented in separate figures. As shown in these figures, functions in the same figure show notable similarities. This implies that functions written in the same language have nearly identical startups.

% The startup of a runtime usually includes bursts of memory reads to load images and libraries, which can probe the traffic in the shared resources. By conducting a Litmus test before executing every tenant's codes, the providers can observe the system state for the function. Meanwhile, the providers also need to study how the startup codes perform in different system states. They complete the congestion tables by performing the Litmus tests with the startups written in three languages while varying the congestion levels. To this end, the information in the congestion table is looked up when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}. 
% estimating the system's state upon receiving a result of a function's Litmus test. 
The startup of a runtime typically includes bursts of memory reads to load images and libraries, which can be used to probe the traffic in shared resources. By conducting a Litmus test before executing a tenant's function, providers can assess the system state. Meanwhile, providers also need to study how startup phases perform under different system states. They complete the congestion tables by conducting the Litmus tests with startups written in three languages while varying congestion levels. This information from the congestion table is then referenced when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tests}\\
\caption{Progress of serverless applications on four cores with Litmus tests (dotted arrows) over time}
% \vspace{-0.5em}
\label{fig:Litmus_tests}
\end{figure}

% Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests. The Litmus tests examine the level of system congestion with every function startup. \hl{Many} concurrent functions in serverless offer frequent test opportunities. Function\#1 is a memory-intensive function that raises a congestion level. While active, Litmus tests measure the congestion level above 8. After Function\#1's completion, the next Litmus test detects a non-congested system with a congestion level below 3. However, with the start of another heavy function, function\#2, the Litmus tests measure the new congestion in the system.
Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests, which examine the level of system congestion during each function's startup. Many concurrent functions in serverless offer frequent opportunities for testing. Function \#1, which is memory-intensive, causes congestion levels to rise above 8 during its execution. A Litmus test in Core 3 detects this congestion. After Function \#1 is complete, a subsequent Litmus test indicates a non-congested system with a congestion level below 3. However, during another resource-intensive function, Function \#2, the Litmus test identifies new system congestion with a level above 9.  

% \textbf{Step 2. Measuring the Impact of Congestion:} Although discerning the system congestion through the Litmus test, estimating its impact on a user's application is another challenge. This work proposes a discount based on the pre-studied impacts on reference functions, assuming the user's functions are alike. For this, the service providers need to select reference functions that represent users' functions running on their systems. In this work, we select the workloads in \hl{Section 2} as our reference applications. 
\textbf{Step 2, Measuring the Impact of Congestion:} Discerning system congestion through the Litmus test solves only one of the two challenges; the other is determining its impact on a tenant's function. Different tenants' functions could experience varying degrees of slowdown under the same congestion level. To address this, we propose using pre-selected reference functions to analyze these impacts, thereby avoiding the cost of runtime profiling. For this, providers need to carefully select reference functions that represent tenants' functions operating on the systems, as these selections influence the overall accuracy of congestion measurement. Later, in Section~\ref{sec:evaluation}, our tests will show that pre-selected reference functions can effectively represent unknown user applications. For this study, the selected reference applications (* marked) are listed in  Table~\ref{tb:benchmarks}. 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/refSlowdownStressing14}\\
% \includegraphics[width=1\columnwidth]{./fig/slowdownStressing16}\\
\caption{\(T_{private}\), \(T_{shared}\), and \(T_{total}\) of serverless applications that run with MB-Gen at stress level 14, normalized to their execution time when they run alone}
% \vspace{-0.5em}
\label{fig:refSlowdownStressing14}
\end{figure}

% Once the reference functions are ready, the providers study the slowdowns of the reference functions while varying different congestion levels again. This study completes the performance table in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. Again, our two traffic generators create two separate sub-tables. All entries in this table are 1-to-1 mapped to entries in the congestion table. The providers estimate a general function's slowdown when having a certain congestion level using this 1-to-1 mapping.
Once the reference functions are ready, providers analyze their slowdowns under varying congestion levels. This analysis completes the performance table shown in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. With two traffic generators, providers can complete another set of two sub-tables for the performance table. All entries in this table are mapped 1-to-1 to entries in the congestion table. Providers can estimate a general function's slowdown at a given congestion level using this one-to-one mapping.

% Figure~\ref{fig:refSlowdownStressing14} shows the reference functions' slowdowns when stressing the system. The X-axis shows different functions, each consisting of three bars: the first two bars show the CPI during each time slice, \(T_{private}\) and \(T_{shared}\), and the last bar shows the CPI of an entire execution. The figure shows that the tested functions suffer from different amounts of slowdowns, although the tests maintain consistent stress levels. \hl{The last group} shows the gmean of all the slowdowns, which is used when providers estimate a function's slowdown later. 
Figure~\ref{fig:refSlowdownStressing14} shows an example of the reference functions' slowdowns when stressing the system. The X-axis shows tested functions, each depicted with three bars: the first two bars show \(T_{private}\) and \(T_{shared}\), while the last bar shows the total execution time, all normalized to their execution time when running alone without interference. The figure shows that the tested functions experience varying degrees of slowdown despite consistent stress levels maintained during the tests. The next-to-last group shows the gmean of all the slowdowns, which providers use to estimate a function's slowdown later.

% \hl{This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/referenceStartupSlowdownRev}\\
\caption{The correlation between the slowdown of Python's startup phase and the slowdown of reference applications. From left, (a) \(T_{private}\), (b) \(T_{shared}\), and (c) \(T_{total}\), normalized to the execution time when running alone}
\label{fig:referenceStartupSlowdownRev}
\end{figure}

% \textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while a range of congestion levels is continuous, the tables only contain a few slowdowns in discrete intervals. Thus, providers need a model that returns an estimated slowdown when receiving a congestion level as an input. In our tests, we employ a linear regression to achieve the model.
\textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while congestion levels vary continuously, the tables only contain slowdowns at discrete intervals. Therefore, providers need a model that estimates the slowdown for any given congestion level. In our tests, we employ linear regression to develop the model.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/interpolation}\\
\caption{Estimating a function's slowdown with logarithmic interpolation}
\label{fig:interpolation}
\end{figure}

% Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding references' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). We employed two traffic generators to extrapolate a more precise congestion level, yielding two sub-tables in both the congestion and the performance tables. Consequently, the figure presents two linear regression models, each associated with a different traffic generator. 
Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding reference applications' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). To extrapolate a precise congestion level, we created two sub-tables within both the congestion and performance tables using two distinct traffic generators. As a result, the figure depicts two linear regression lines (red and blue dotted lines), each associated with a different traffic generator.

% The provider needs to estimate the function's slowdown to uncover its price. However, the above two regression models return two vastly different slowdowns. Then, the providers need to determine which model is close to the current environment. We think the two models reflect two extreme congestions that the traffic generators create, one before the L3 and one after the L3. CT-Gen creates massive traffic from the core to the L3 cache, which filters the traffic, preventing the operations from consuming the memory bandwidth. MB-Gen also creates huge traffic but consumes the memory bandwidth and replaces L3 blocks. Since each traffic generator creates an extreme case, the machine state could be intermediate with congestion in the range between the two congestions created by CT-Gen and MB-Gen. However, Litmus pricing cannot answer this question with only the startup's slowdown. 

% To address this question, we note that the system's L3 misses are a critical indicator closely related to a function's performance. Functions suffer more when the system experiences more L3 misses, which stresses the cache space and off-chip memory bandwidth. Accordingly, Litmus test collects the system's L3 miss count as a supplementary index, which tells more about the crowdedness of shared resources.

These regression models return two different slowdowns. To estimate a function's slowdown, providers must determine which model reflects the current environment more accurately. The traffic generators create two extreme congestion scenarios: one before the L3 cache and one after. CT-Gen generates substantial traffic from the core to the L3 cache that filters the traffic and prevents operations from consuming memory bandwidth. Conversely, MB-Gen also generates massive traffic but consumes memory bandwidth and repeatedly evicts L3 cache blocks. Because each traffic generator represents a distinct extreme case, the actual machine state could fall somewhere between the two congestion levels created by CT-Gen and MB-Gen. However, Litmus pricing requires more than just the startup slowdown to identify the machine's state in these models. Thus, we have enabled Litmus tests to gather the system's L3 miss count as a supplementary metric that offers deeper insights into the crowdedness of shared resources.


% \hl{Figure 1} shows how to use the L3 cache misses with the performance sub-tables. The two traffic generators make the upper and lower boundary of the L3 miss rates. When performing a Litmus test, if the test's L3 miss rate is XXX, close to the L3 misses with CT-Gen, we can conclude that the congestion occurs before the L3 cache and select the expected slowdown of XXX. On the contrary, we choose XXX, in case the L3 miss rate is XXX, close to the L3 misses with MB-Gen. If the test's L3 miss rate is in-between, we interpolate the two slowdowns based on the L3 misses, assuming congestion in both resources. 
% Finally, we determine the Rprivate and Rshared based on the expected slowdown from its performance table. Calculating Rprivate and Rshared takes the same steps. The final discount price is computed using the equation with the computed rates. 

% Figure~\ref{fig:interpolation} shows how we employ the L3 misses when estimating the slowdown. The two traffic generators make the upper and lower boundary of the L3 misses. If a Litmus test reports the L3 miss count is 10, close to the L3 misses with CT-Gen, \textcircled{1}Litmus pricing estimates the discount (=expected slowdown) of the function to be near 1\%. This indicates that the congestion happens before the L3, as what CT-Gen creates. On the contrary, in case the L3 misses are 1000, close to the L3 misses with MB-Gen, \textcircled{2}Litmus pricing estimates the function's discount rate close to 6\%. Meanwhile, if the Litmus test reports the L3 misses as 100, we interpolate the two extreme discounts, 1 and 6, based on the L3 misses, assuming current congestion to stand in between the two extreme congestions. The congestion model in the figure shows how we interpolate with logarithmic interpolation. In this figure, \textcircled{3}applying the logarithmic interpolation to the L3 miss count returns the half-point between CT-Gen's 1\% and MB-Gen's 6\%, which is 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 
Figure~\ref{fig:interpolation} shows our approach to using L3 misses to estimate slowdowns. We created two figures illustrating separate regression models. The left figure (a) is derived from the startup slowdowns and L3 misses with logarithmic regression, indicating L3 misses at specific congestion levels. The right figure (b) is derived from the performance table with linear regression, displaying discounts at specific congestion levels. Each figure depicts two regression lines associated with different traffic generators.

The two traffic generators set the upper and lower boundaries for L3 misses. For instance, if a Litmus test reports 10 L3 misses, close to what CT-Gen generates: \textcircled{1}This suggests congestion occurs before reaching the L3 cache, similar to CT-Gen's scenario. Thus, Litmus pricing estimates the function's discount to be around 1\%. Conversely, if the Litmus test reports 1000 L3 misses, close to MB-Gen's results: \textcircled{2}Litmus pricing estimates the function's discount rate to be approximately 6\%, indicating congestion similar to MB-Gen, where memory bandwidth is heavily consumed and L3 cache blocks are frequently evicted. When the Litmus test reports 100 L3 misses, an interpolation between these extremes is applied: \textcircled{3}Using logarithmic interpolation, Litmus pricing estimates the function's discount rate to be midway between CT-Gen's 1\% and MB-Gen's 6\%, resulting in approximately 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 



==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/08_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \textbf{Litmus price \& error:}
% We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, and the other consists of selected reference applications to obtain the linear regression models for Litmus pricing. The discount models plug into the Litmus pricing used in our tests. For this experiment, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown.
We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, while the other consists of chosen reference applications to derive linear regression models for Litmus pricing. The discount models plug into the Litmus pricing employed in the tests. In this study, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown. 

% % original version
% We maintain the congestion state consistent across all tests, co-running each function with 26 other functions. Using Perf~\cite{perfWiki}, we collect the three key stats: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup, which implies the congestion level in these tests, as well as the discount rates that every function receives. We execute every function 100 times and collect the average of the function's \(T_{private}\) and \(T_{shared}\). Finally, we compute each function's \(P_{private}\), \(P_{shared}\), and \(P\), the total price, by summing \(P_{private}\) and \(P_{shared}\).  

\subsection{One Function Per Core}

% revision version
% We maintain consistent congestion states across all tests by co-running each function with 26 other functions. Using Perf, we collect the three key statistics: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup. These metrics hint at the congestion level during the tests as well as the discount rates that a function receives. Each function is executed 30 times, and the average of its \(T_{private}\) and \(T_{shared}\) is collected. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).
We maintain consistent congestion levels across all tests by co-running each function with 26 other functions. As outlined in Section~\ref{sec:motivation}, whenever a function finishes, another is randomly launched to keep a total of 26 co-running functions. Using Perf~\cite{perfWiki}, we collect three key statistics: \(T_{private}\), \(T_{shared}\), and the machine's L3 misses during the first 45 million instructions of the Python startup. Through these metrics, Litmus pricing estimates the level of system congestion and the discount rates a function receives. Each function is executed 30 times, and we average its \(T_{private}\) and \(T_{shared}\) values. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice26Rev}\\
% \caption{The total price for functions computed via Litmus pricing and ideal prices when co-running with 26 other functions normalized to the commercial price that offers no discount}
\caption{Prices computed via Litmus pricing and ideal prices when co-running with 26 other functions, normalized to the commercial price that offers no discount}
\label{fig:normalizedPrice26Rev}
\end{figure}

% In Figure~\ref{fig:normalizedPrice26}, we can see a minimal difference in the discount rate between the Litmus price and the Ideal price. The average Litmus discount rate stands at 11.5\%, which is only marginally larger by 0.6\% than the average Ideal discount rate of 10.9\%. Also, we can see that the difference between the Litmus price and Ideal price are different among the applications. Certain applications exhibit higher Litmus prices compared to the Ideal price, while conversely, some applications demonstrate smaller Litmus prices. 
 %Figure~\ref{fig:priceErrorRunwith26} shows further details, analyzing the errors in each pricing component. 

% Figure~\ref{fig:normalizedPrice26Rev} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{10.66\%}, which is only marginally larger by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{10.28\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice26Rev} illustrates estimated prices derived from Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices to offset delays in a congested execution environment. The figure shows minimal disparities between the two prices, implying that Litmus pricing offers a reasonable discount. The average discount from Litmus pricing across all functions is 10.7\%, which is only marginally higher by 0.4\% compared to the average slowdown experienced by functions, which stands at 10.3\%, as depicted by the ideal price.

% However, the discount rates per slowdown differ among functions. For instance, float-py's ideal discount rate is \hl{0.05\%}, but it enjoys a \hl{4.31\%} discount with the Litmus pricing. Meanwhile, pager-py's performance drops by \hl{15.63\%} while receiving a \hl{13.87\%} discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more easily affected than the reference when congested. In contrast, float-py runs mostly with private resources, receiving a minor impact from the execution environment. Figure~\ref{fig:priceErrorRunwith26Rev} shows further details, analyzing the differences in each pricing component.
However, the discounts per slowdown differ among functions. For instance, float-py's ideal discount rate is 0.05\%, but it benefits from a 4.3\% discount with Litmus pricing. Conversely, pager-py encounters a 15.6\% performance decline while receiving only a 13.9\% discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more susceptible to congestion than the references. In contrast, float-py predominantly utilizes private resources, resulting in minimal impact from the execution environment. Further insights into these variations in each pricing component are presented in Figure~\ref{fig:priceErrorRunwith26Rev}.


% From figure~\ref{fig:tcore\(T_{private}\)Distr}, we know that \(T_{private}\) dominates the execution time among all applications. The impact from \(T_{private}\) error has a bigger impact on the overall error. The slowdowns due to congestion in private resources are small. Theoretically, there should be no slowdowns when using private resources, but we observed that the congestion still influences it. The observed slowdown is 000, a small difference from an ideal slowdown. Meanwhile, the slowdowns in shared resources are significant. We observe that 

% % \[  Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}}\]

% \[Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{TotalIdealPrice}\]
% \[TotalIdealPrice = R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}\]

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/priceErrorRunwith26Rev}\\
\caption{Weighted errors in prices derived from Litmus pricing, which are compared to ideal prices}
% \vspace{-1em}
\label{fig:priceErrorRunwith26Rev}
\end{figure}

%%% We discuss error
% In figure~\ref{fig:priceErrorRunwith26} we can see that there are some applications receive positive errors and some receive negative errors.  A negative error indicates that our estimated slowdown for that application is higher than its actual slowdown, resulting in greater compensation than the observed performance losses. On the other hand, a positive error indicates that the compensation is smaller than its real slowdown. For most applications, the Litmus price is slightly higher than the Ideal price, with minimal differences. The highest price error is 0.0389 for auth-nj, while the lowest error is 0.007 for dyn-py. The geometric mean of the absolute error is 0.018. 
% Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors that each function experiences. The error rate is computed as the difference between the estimated and the ideal prices over the ideal price. The first two bars show the errors in \(P_{private}\) and \(P_{shared}\), which are weighted by their corresponding ratio in the execution time, considering their impacts, as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. The functions can have two different errors: positive and negative. A positive error indicates that the Litmus-estimated price is higher than its ideal price, implying that it receives smaller compensation than its performance losses. In other words, Litmus pricing estimates its slowdown to be less than its actual slowdown. A negative error implies the opposite; a function's compensation is higher than its slowdown. This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others. Meanwhile, the tenants need to acknowledge the consequences if their functions differ vastly from the reference workloads, heavily relying on shared memory.
Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors each function experiences. The error rate is computed by comparing the estimated prices with the ideal prices and dividing the difference by the ideal prices. The first two bars show errors in \(P_{private}\) and \(P_{shared}\), weighted by their corresponding ratios in execution time, reflecting their impacts as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. Functions may have two types of errors: positive and negative. A positive error means that the estimated price exceeds its ideal price, implying that the compensation received is less than the performance loss incurred. In other words, Litmus pricing underestimates the slowdown relative to the actual slowdown. Conversely, a negative error indicates the opposite; a function's compensation exceeds its slowdown. This discrepancy indicates Litmus pricing may offer varying advantages to different functions, favoring those with lesser slowdowns. Meanwhile, tenants must recognize the consequences if their functions differ vastly from the references, particularly those heavily reliant on shared resources.

% Delete the followings
% This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.

% The largest absolute error is \hl{0.0723} for rate-go, while the smallest absolute error is \hl{0.0039} for \hl{mst-py}. Overall, the Litmus pricing shows minor errors with an average of \hl{0.0231}. With further details, the Litmus pricing accurately estimates the slowdowns in \(P_{private}\) with \hl{0.0175} of an average weighted error rate. \(P_{private}\)'s highest weighted error rate is \hl{0.079}, yet minor, while the lowest rate is only \hl{0.0008}. The weighted error rate for the estimated \(P_{shared}\) is also small. The average error rate for \(P_{shared}\) is \hl{0.0068}, even lower than for \(P_{private}\). \(P_{shared}\)'s highest error rate is \hl{0.0404}.
% The largest absolute error is 0.072, which occurs with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, the Litmus pricing exhibits minor errors, averaging 0.023, \hl{with the estimated discount differing by 22.5\% over the ideal discount.} With more details, Litmus pricing accurately estimates slowdowns in \(P_{private}\), with an average weighted error rate of 0.018. \(P_{private}\)'s highest weighted error rate is 0.08, yet minor, while the lowest rate is only 0.0008. The weighted error rate for estimated \(P_{shared}\) is similarly small, averaging at 0.0068, even lower than for \(P_{private}\). The highest error rate for \(P_{shared}\) stands at 0.04.
The largest absolute error is 0.072, occurring with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, Litmus pricing exhibits minor errors, averaging 0.023. Thus, the estimated discount deviates by 22.5\% from the ideal discount. Note that Litmus pricing aims to match the average discount across all functions by applying a system-wide discount based on the system's congestion level rather than adjusting the discount for each function individually. Consequently, individual functions may experience either positive or negative errors. However, it is noteworthy that the average discount between Litmus and ideal pricing differs by just 0.4\%, as illustrated in Figure~\ref{fig:normalizedPrice26Rev}, satisfying its objectives.
% This policy may incentivize some functions while penalizing others based on shared resource usage. 
Specifically, Litmus pricing estimates slowdowns in \(P_{private}\) with an average weighted error rate of 0.018. The highest for \(P_{private}\) is 0.079, while the lowest is just 0.001. For \(P_{shared}\), the average weighted error rate is even lower, at 0.007. The highest for \(P_{shared}\) is 0.040.


% Litmus employs the average performance of applications to determine the discount rate applied universally. In this context, an application encounters a positive error when its speedup is less than the estimated average speedup across all applications. Also, the error rate depends on the difference between the actual speedup and the estimated average speedup, with larger differences resulting in more significant errors for the given application.
% As discussed in Figure~\ref{fig:TpriTshardDistri}, \(T_{private}\) dominates the execution time across all applications, implying that a small error in the estimated \(T_{private}\) largely influences the execution time. This explains why, for functions that demand little shared resources, such as float-py and chame-py, the error in P is almost identical to that in \(T_{private}\), and errors with \(T_{shared}\) can be overlooked. In contrast, for functions with a larger \(T_{shared}\) ratio, such as pager-py and mst-py, errors in \(T_{shared}\) meaningfully affect the total execution time. Note that the Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price.  

Litmus pricing estimates each pricing component separately with an individual discount rate. For functions that demand minimal shared resources, such as float-py, the errors in P are nearly identical to those in \(T_{private}\), and the errors in \(T_{shared}\) can be overlooked. As shown in Figure~\ref{fig:TpriTshardDistriRev}, \(T_{private}\) dominates the execution time across many applications. While even a small error in the estimated \(T_{private}\) influences the function's execution time, substantial errors in \(T_{shared}\) likely have limited impacts, except for functions that have a relatively meaningful \(T_{shared}\) ratio, such as pager-py and mst-py, whose errors in \(T_{shared}\) are observable in the total price. 

% We emphasize that Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price. We observe that functions have similar slowdowns in \(T_{private}\) with slight variation when congested. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, also estimating reliable total prices since \(T_{private}\) mostly dominates the execution time. The \(T_{shared}\) fluctuates more dynamically across functions with a relatively large error, but the error's impact is little, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}. 
We emphasize that Litmus pricing cannot avoid producing a certain degree of error since it relies on estimation using a few metrics. However, the figure proves that Litmus pricing effectively captures a congested environment and reflects that environment in the price. Under the same congestion level, \(T_{private}\) values of all functions are delayed similarly with a little variation. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, leading to reliable total price estimates since \(T_{private}\) generally dominates execution time. \(T_{shared}\) fluctuates more dynamically across functions and has a relatively larger error, but the impact of this error is minimal, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}.

\begin{figure}[h]
\centering
% \vspace{-5em}
 \includegraphics[width=1\columnwidth]{./fig/normTprivtTshared26Rev}\\
% \vspace{-5.5em}
\caption{\(T_{private}\) \& \(T_{shared}\) of applications when co-running with 26 others, normalized to those when they run alone. The top(black) and bottom(blue) lines are discount rates from Litmus pricing for \(T_{private}\) and \(T_{shared}\)}
% \vspace{-1em}
\label{fig:normTprivtTshared26Rev}
\end{figure}

% To further investigate the price error differences, in igure~\ref{fig:normTprivtTshared}, we explore the \(T_{private}\) speedups across various serverless applications.  
% Notably, the difference between the Litmus discount (L-Discount) and the average speedup is merely 0.006.  This minute difference explains why Litmus can attains such high accuracy. 
%Furthermore, when comparing with figure~\ref{fig:priceErrorRunwith26}, a correlation between the error rate and the speedup differences becomes apparent. 
%For instance, float-py, with the most substantial difference above the Litmus discount, also experiences the most significant negative error rate. 
%Conversely, aes-go, with the smallest speedup, experiences the highest positive error rate.
% % original version
% Figure~\ref{fig:normTprivtTshared} shows the execution time of the baseline normalized to the execution time of each run under congestion. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the functions spend only 3.67\% more time on private resources, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, resulting in precise estimation with a Litmus test. 

% Figure~\ref{fig:normTprivtTshared26Rev} shows the execution time of each function run under congestion normalized to the execution time of the baseline. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the interferences in private resources extend the function execution time only by 5.3\%, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, enabling precise estimation with a Litmus test.
Figure~\ref{fig:normTprivtTshared26Rev} shows the \(T_{private}\) and \(T_{shared}\) of each function, normalized to the same time components of the baseline. The gap between the bar and 1 represents the amount of slowdown that should be translated into ideal discounts. The top (black) and bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that interferences in private resources extend the function execution time by only 5.3\%, implying the performance of the private resources is marginally affected by congestion. Additionally, all functions exhibit similar \(T_{private}\) values with little dispersion, helping precise estimation with Litmus tests.

% Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors are still in an acceptable range since their impacts are small. Functions that have a considerable \(T_{shared}\) ratio become more sensitive to system congestion. Instead, a function, such as float-py, with negligible \(T_{shared}\) ratio gains huge benefits with high discounts while its performance remains firm. This shows that Litmus pricing reflects the dynamically changing values of shared resources when the congestion level alters and encourages functions to be developed to use more private resources. 
Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors remain within an acceptable range as their impacts are minor. Functions that have a considerable \(T_{shared}\) ratio are more sensitive to system congestion. Conversely, a function like float-py, which has a negligible \(T_{shared}\) ratio, gains huge benefits from high discounts while maintaining stable performance under congestion. This shows that Litmus pricing accurately reflects the dynamic values of shared resources when the congestion level changes and incentivizes functions to be developed to use less shared resources. 

% \textbf{Litmus pricing under high congestion:} We test our Litmus pricing under a heavily congested environment to verify its pricing of functions with large slowdowns. To create a crowded environment, we concurrently execute 60 instances of Fibonacci-go, which produces the most L2 misses among our tested functions. 
% We raise the congestion level significantly with 60 co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo} shows the results from the same tests of Figure 11. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.8\%, which is only a 1.7\% difference from the ideal discount of 27.1\% with 2.48\% of an average absolute error. In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.151 and 4.299, which are only 2.45\% and 7.83\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. 
% \textbf{Litmus pricing under high congestion:} We raise the congestion level significantly with \hl{500} co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo500} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.1\%, which is only a 1\% difference from the ideal discount of 27.1\% with 0.088\% of an average absolute error. Litmus pricing discounts slightly more than an actual slowdown, leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% % \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
% \caption{The normalized total price for the applications calculated by using Litmus pricing and ideal prices when co-running with 500 Fibonacci-go}
% \label{fig:normalizedPriceCongested320}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\columnwidth]{./fig/diffStartupPortion-2Rev}\\
%\caption{The slowdown of Python's startup with 25 and 15 million instructions (X-axis) and the slowdown of reference applications (Y-axis). From left, \(T_{private}\), \(T_{shared}\), and \(T_{total}\), normalized to those when running alone}
%\label{fig:diffStartupPortion}
%\end{figure}

% \textbf{Instructions in Startup:} Litmus tests react differently to congestion when performed with different numbers of instructions from the startup phase. For example, Python's startup involves about 45 million instructions. While we have conducted Litmus tests using all these instructions, Figure~\ref{fig:diffStartupPortion} shows the response of these tests when running with the first 15 and 25 million instructions from this set. The figure shows the startups' \(T_{private}\), \(T_{shared}\), and \(T_{total}\) with two traffic generators, as depicted in Figure~\ref{fig:referenceStartupSlowdownRev}. Tests with fewer instructions are more sensitive to cold cache misses but less to interference in the L3 cache. Therefore, as the instruction count in Litmus tests decreases, they become less susceptible to conflicts in shared resources, especially from traffic by MB-Gen. As a result, tests with 25 million instructions exhibit reduced slowdowns. This trend becomes more apparent when running the tests with 15 million instructions, depicting that slowdowns when co-running with MB-Gen become nearly identical to those with CT-Gen. 

%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%







% \textbf{Instructions in Startup:} Python's whole startup phase contains about 45 million instructions. We can further divide the startup phase into smaller pieces with 10 million instructions code chunks. And each code chunk would have its characteristics. They react differently in the same congested environment. In section XXX we use the whole Python's startup portion's slowdown to indexsing the serverless application's slowdown. But, since the co-relationship between these two slowdown in different congestion source are different, one startup \(T_{private}\) slowdown may indicate two application's slowdown. By carefully picking the code chunks we can mitigate the difference between the two normalized slowdowns of the guidance application that correlated to the same startup phase slowdown. 

% Figure~\ref{fig:diffStartupPortion} depicts the correlation between the performance changes in the reference applications and distinct segments of Python's startup phase. From the figure, we see that selecting the first 15 million instructions as our startup phase results in the normalized \(T_{uncore}PerInst\) of the guidance application aligning nearly into a singular trendline. However, there are substantial gaps in the case of \(T_{core}PerInst\) with this code segment. Thus, we should pick xxx-xxx as our startup phase representation code for the normalized \(T_{core}PerInst\). We think that this can be used to mitigate the differences. But, we should be careful to use the small code chunks for the following reasons: First, only measuring the small portion can be a problem. The results might be too dynamic. Second, since we only measure this small portion there might be a huge execution period that cannot be covered.

% Continue to work from here

\subsection{Temporal CPU Sharing}
\label{sec:temporalCPUSharing}

The previous evaluation assumes an isolated environment where a CPU is assigned exclusively to an active function during execution, disallowing temporal sharing between functions through context-switching. While this setup ensures strict performance isolation, it inherently limits resource utilization. Conversely, enhancing utilization by permitting temporal CPU sharing among functions complicates price estimation. We explore how Litmus pricing can be applied in a less restrictive environment that permits sharing, where functions can temporarily share the same CPU and are not bound exclusively to specific cores. 

In this section, we deploy a testing function to co-run with 160 other functions across 16 cores without exclusive core assignments, assuming an average of 10 functions share a core. The reduction in the number of cores tested was necessitated by our system's memory limitations, as certain functions require significant memory space.

% \textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, the subsequent function clears the displaced one's cached data. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, the slowdown with extra sharing financially benefits the provider; we thereby argue that the extent of sharing should be factored into Litmus pricing as another discount factor.
\textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, a subsequent function evicts the cached data of the displaced one. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, delayed execution due to extra sharing financially benefits the providers. Thus, we argue that the extent of temporal sharing should be incorporated into Litmus pricing as another discount factor.

Figure~\ref{fig:csImpactor} depicts the switching overheads as concurrently running functions increase. The figure demonstrates that the sharing overhead follows a logarithmic growth pattern and stabilizes at around 20 co-running functions. Furthermore, we discovered that the switching overheads predominantly affect \(T_{private}\). Consequently, Litmus pricing needs to calibrate \(T_{private}\) to account for the impacts of sharing before estimating the slowdown using the performance table.

Figure~\ref{fig:normalizedPrice160Method1} illustrates the discounted price reflecting this adjustment. In our configuration, with an average of 10 functions per core, we divide \(T_{private}\) by 1.025 before estimating the slowdown. In this figure, Litmus pricing estimates an average discount of 14.5\%, which falls 2.9\% short of the ideal discount of 17.4\%. While most benchmarks receive discounts lower than ideal, aes-py stands out with the largest error of 9.9\%, which is 6.9\% less than its ideal discount of 16.8\%.

\begin{figure}
\centering
% \includegraphics[width=1\columnwidth]{./fig/csImpactor}\\
\includegraphics[width=1\columnwidth]{./fig/csImpactor2}\\
\caption{\(T_{private}\) of functions over different co-running counts in the same core, normalized to when running alone}
% \vspace{-1em}
\label{fig:csImpactor}
\end{figure}

\begin{figure}
\centering
% \vspace{-1.2em}
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160Method1}\\
\caption{Prices derived from Litmus pricing (Method 1) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
% \vspace{-0.5em}
\label{fig:normalizedPrice160Method1}
\end{figure}

% In Figure~\ref{fig:normalizedPrice160Method1} we use the the same congestion and performance tables that we collected in the restricted environment. When checking the tables instead of using the original startup slowdown of tcore we use an adjusted slowdown by dividing the context switch impact factor. From figure~\ref{fig:normalizedPrice160Method1} we can see that the average Litums discount is 14.65\%, 3.01\% less than what they should receive compared to the ideal discount of 17.67\%. Most applications receive a smaller discount than the ideal price. The largest error is on aes-py with Litmus discount of 9.85\%, 6.87\% smaller than the ideal discount of 16.72\%. The smallest error is on dyn-py. It's Litmus discount is 22.45\%, only 0.47\% larger than the ideal discount of 21.97\%.

\textbf{Method 2, Updating Performance Tables:} Rather than reusing the performance/congestion tables designed for restrictive environments, arranging new tables for the sharing-enabled environments returns better accuracy. Although the notion of preparing separate tables for various sharing levels may seem challenging, we argue that only one or a few extra tables for heavily crowded systems would suffice, given that commercial systems are typically heavily crowded. Again, we emphasize that the impact of function co-placement stabilizes above a certain co-placement count, as shown in Figure~\ref{fig:csImpactor}.

For this test, we prepared new performance/congestion tables for the environment described above, where a testing function is assumed to co-locate and compete for a core with 9 other functions. Moreover, considering the scenario where a switched-out function has a low chance of being rescheduled to the same core, instead of assigning 10 functions to a specific core, we ran 50 functions across 5 dedicated cores; each can run on any of the 5 cores. We managed the congestion levels in shared resources using traffic generators on the other cores, as outlined in Section~\ref{sec:designDetails}.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPrice160}
% \vspace{-0.6em}
\end{figure}

% Figure~\ref{fig:normalizedPrice160} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{17.29\%}, which is only marginally smaller by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{17.67\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice160} shows the prices obtained from Litmus pricing with the new tables, which are normalized to those from commercial sources. Once more, as in Figure~\ref{fig:normalizedPrice26Rev}, the figure reveals marginal distinctions between the two price points, suggesting that Litmus pricing continues to offer a reasonable discount. Across all functions, the average discount provided by Litmus pricing stands at 17.2\%, merely 0.2\% less than the ideal discount of 17.4\%.


==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/09_sensitivity.tex <==
\section{Sensitivity}
\label{sec:sensitivity}

While the aforementioned tests highlight Litmus's potential, we recognize the need for more compelling results. This section expands our analysis and examines Litmus pricing from various angles across diverse system environments.

% \textbf{Heavy Congestions:} We raise the congestion level significantly with 320 co-running applications to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. The Litmus pricing is still close to the ideal price, discounting the price by 20.00\%, which is only a 1.46\% difference from the ideal discount of 21.46\%. The highest Litmus discount is 26.01\% for dyn-py. It has an error of 2.83\% compared with the ideal discount.
\textbf{Heavy Congestion:} We significantly escalate the congestion level to verify Litmus pricing under conditions of substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} presents the outcomes of the same tests depicted in Figure~\ref{fig:normalizedPrice160} but with 320 co-running functions. Not only did we increase the function count, but we also specifically selected 8 memory-intensive functions, aes-py, compre-py, thum-py, bfs-py, auth-py, fib-go, geo-go, and profile-go, that produce the most L2 cache misses among the tested functions to create heavy congestion in shared resources deliberately. Even under such intensified congestion, Litmus pricing produces results remarkably close to the ideal price, discounting the price by 20.0\%, which deviates by merely 1.5\% from the ideal discount of 21.5\%. The highest discount by Litmus pricing is 26.0\% for dyn-py, a minor error of 2.8\% compared to the ideal discount.


% leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 320 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPriceCongested320}
% \vspace{-1em}
\end{figure}

\textbf{CPU Frequency:} Modern CPUs feature dynamic CPU frequency adjustments, which are controlled via software or hardware. A hardware technique like Intel Turbo Technology autonomously adjusts the CPU frequency based on the CPU's power and thermal budgets, allowing the CPU to operate at higher frequencies when conditions permit and lower frequencies under heavy load. Prior tests assumed that the frequencies were fixed and strictly managed by service providers who had knowledge of when and to what extent frequency adjustments were necessary. Also, we evaluated Litmus pricing under the other scenarios where CPU frequencies were not fixed, providing more dynamic perspectives.

% Figure~\ref{fig:normalizedPrice160unset} illustrates the prices from the Litmus pricing and the ideal price, which are normalized to commercial prices. We tested it under the configuration in Section 7.2 with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, the Litmus pricing's discount is lowered from 17.16\% to 16.84\%, while the ideal discount rate is decreased from 17.42\% to 17.31\%. Still, the discount rate difference from the ideal price is only 0.47\% without setting the CPU frequency. We observed that the CPU frequency changes rarely when the system runs with 160 functions. Overall, the varying frequency made a minor impact on performance as well as the pricing scheme. 
Figure~\ref{fig:normalizedPrice160unset} illustrates the prices derived from Litmus pricing alongside the ideal prices, both normalized to commercial prices. This evaluation was conducted under the configuration outlined in Section~\ref{sec:temporalCPUSharing} with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, we observe a slight decrease in Litmus pricing's discount, from 17.2\% to 16.8\%, while the ideal discount rate decreases from 17.4\% to 17.3\%. Still, even without fixed CPU frequencies, the difference in the discount rate from the ideal price is only 0.5\%. We noted that CPU frequency changes were infrequent when the system operated with 160 functions. Overall, the variation in frequency had a negligible impact on Litmus pricing.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160unset}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others with unfixed CPU frequencies, both normalized to commercial prices}
\label{fig:normalizedPrice160unset}
% \vspace{-1em}
\end{figure}

% All the above experiments are done on Intel Xeon Gold 5218(Cascade Lake). We also perform our scheme on another CPU architecture, Intel Xeon Silver 4314(Ice Lake-SP). 
\textbf{CPU Architecture:} Ensuring the validity of Litmus pricing across different architectures is crucial. Our Litmus tests rely on the performance counter that measures a stall count due to L2 cache misses (cycle\_activity.stalls\_L2\_miss)~\cite{perfMonEvents}, supported by Intel's CPUs. Unfortunately, other vendors like AMD do not yet offer the same performance counter~\cite{amdPMC}, restricting our tests to Intel CPUs. Alternatively, we conducted tests on another Intel CPU based on the Ice Lake architecture, Xeon Silver 4314, to broaden the scope of our analysis.

\begin{figure}[b]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun70kiwi}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 70 others on Xeon Silver 4314, both normalized to commercial prices}
\label{fig:normalizedPriceCorun70kiwi}
\end{figure}

% Because of the limitation of our memory size, we test Limtmus with 70 co-running applications. In this test, we use method 2 introduced in section~\ref{sec:temporalCPUSharing}. We first conduct the congestion and performance tables with 50 applications running in the first 5 cores. Then for the evaluation, we run 70 applications in the first 7 cores to let our testing application compete with 9 other applications for a core.  Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus discounting the tenant only pays 82.52\% commercial price. It's 0.696\% less than with the ideal discount.
Once again, this evaluation was conducted following the configuration outlined in Section~\ref{sec:temporalCPUSharing}, albeit with 70 co-running functions, limited by the main memory capacity of 128GB. Following Method 2, we constructed new congestion and performance tables with 50 functions running across 5 cores. Then, we ran 70 functions across 7 cores to match the competition count, averaging 10 functions per core. Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus pricing, the tenant only pays 82.5\% of the commercial prices, which is merely 0.7\% less than the ideal price.

% \textbf{Per-core Function Count:} When altering the co-located applications in each core the performance of the application can also be influenced. In this test, we put 240 applications in the first 16 cores. The testing application is competing with 14 other applications. We used the same congestion and performance tables from section~\ref{sec:temporalCPUSharing} method 2. Figure~\ref{fig:normalizedPriceCorun15} presents the results. The error of Litmus pricing is 1.23\% with The average discount of 16.69\%. The ideal discount is 17.92\%. The mean price of Litmus is larger than the ideal price because we are using the tables that are made based on 10 applications per-core. The context-switching overhead is larger. But, from figure~\ref{fig:csImpactor} we know that there is a diminishing impact of per-core application count. The error of the Litmus pricing is still under control when we increase the per-core application count.
\textbf{CPU Sharing Overhead:} The co-located function count determines the level of interference, impacting a function's performance differently. To assess Litmus pricing under various co-running function counts, we increased the function count to 240 from the configuration outlined in Section~\ref{sec:temporalCPUSharing}, making an average of 15 functions running on each core. However, we reused the performance and congestion tables generated in Section~\ref{sec:temporalCPUSharing}. Figure~\ref{fig:normalizedPriceCorun15} illustrates the results, where the Litmus pricing's error is 1.2\% with an average discount of 16.7\%, compared to the ideal of 17.9\%. Despite reusing the tables constructed for 10 co-running functions per core, the error remains negligible. This outcome aligns with Figure~\ref{fig:csImpactor}, which highlights the diminishing impact of temporal sharing when running more than 10 co-running functions. Given the perpetual overcrowding of commercial systems, any configuration gap between the environment where constructing the tables and where conducting tests is expected to remain minor and easily manageable.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun15}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 15 functions per core and reusing tables, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun15}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun160smt}
\end{figure}

\textbf{Simultaneous Multithreading (SMT):} SMT is a technique aimed at maximizing resource utilization by enabling multiple threads to execute concurrently on the same core, extending the shared resource domain across the entire processor. However, while SMT enhances resource utilization, it significantly complicates the measurement of interference impact. Moreover, SMT introduces additional side channels, thereby increasing the processor's vulnerability to security attacks. Due to these concerns, serverless platforms like Amazon Lambda disable SMT in their systems~\cite{schall2023warming,agache2020firecracker,schall2022lukewarm}. Nonetheless, we have conducted a study to assess the impact of SMT on our Litmus pricing methodology.

% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
% \caption{Prices computed via Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, normalized to the commercial prices}
% \vspace{-0.5em}
% \label{fig:normalizedPriceCorun160smt}
% \end{figure}

% To generate the performance/congestion tables, we executed 50 applications across 5 dedicated physical cores. In this way, the testing function is co-located with 9 other applications in the same virtual core and 19 other applications in the same physical core. Fiugre~\ref{fig:normalizedPriceCorun160smt} illustrates the results. The first thing we notice is that the normalized price is much smaller compared with the setups without SMT turned on. The average discount of Litmus is 45.42\% which is 1.9\% smaller than the average ideal discount of 47.32\%.
To construct the performance and congestion tables, we executed 50 applications across 5 physically separated cores, allowing an average of 10 functions to share two virtual cores. Figure~\ref{fig:normalizedPriceCorun160smt} illustrates the results,  presenting prices derived from Litmus pricing and ideal prices, both normalized to commercial prices without discounts. The normalized price experiences a significant drop compared to other configurations, highlighting the impact of heavy congestion within a physical core. The ideal price, which assumes no interference, stands at 47.3\% of the commercial price. Meanwhile, Litmus pricing offers a discount of 45.4\%, which is only 1.9\% less, confirming the effectiveness of Litmus pricing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Node JS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Nodejs Startup:}NodeJs is another well-adopted language in serverless platforms besides Python. It's one of the earliest languages to be supported by AWS Lambda ~\cite{serverless1}. From Section~\ref{sec:designDetails} we see that NodeJs has a long startup phase which makes it a great candidate when we need to pick a language startup phase for the Litmus test. 

%\begin{figure}[h]
%\centering
%\vspace{-0.5em}
%\includegraphics[width=1\columnwidth]{./fig/njReferenceStartupSlowdown}\\
%\vspace{-1em}
%\caption{The correlation between the normalized NodeJs's startup phase and the normalized reference applications.}
%\vspace{-0.5em}
%\label{fig:njReferenceStartupSlowdown}
%\end{figure}

%Figure~\ref{fig:njReferenceStartupSlowdown} shows the correlation between NodeJs startup phases and reference applications. After applying the Litmus test with NodeJs applications, with this figure, we can use the slowdown of the NodeJs startup phase to find the corresponding system congestion level and the discount rate for both private and shared resources. NodeJs has a longer startup phase compared with Python. It gives us more room when picking the most suitable portions of the startup phase. We can choose the language to be used for the Litmus test based on the density of the startup phase. 


==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/10_related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Serverless:} Many works address the performance bottleneck of serverless execution~\cite{du2020catalyzer}~\cite{agarwal2021reinforcement}~\cite{roy2022icebreaker}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Schall et al.~\cite{schall2022lukewarm} record and reload the instructions to reduce the front-end stalls when reaccessing the same application. Jovan et al.~\cite{stojkovic2023specfaas} focus on the performance of an application chain. They break the execution flow and speculative execute the functions. However, we are focusing on the price which is one of the most important potions of the cloud ecosystem.

% For the cloud providers, accommodating more tenants in a machine is a key strategy, gaining higher profits by maximizing the utilization of their machines. However, the approach inevitably introduces interference between tenants, slowing down applications unpredictably. Thus, prior researchers solved this challenge by allowing the tenants more non-biased, predictable, quality services~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed a clustering-based cache partitioning to remove unfairness between tenants. Rohan et al.~\cite{roy2021satori} simultaneously control multiple architectural resources to aim for both fairness and throughput. However, offering fairness inevitably sacrifices resource utilization. Thus, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} solve the unfairness uniquely by adjusting their prices while leaving the unfairness at a certain degree. This paper follows this direction but explores a more practical solution in serverless computing. 

Cloud providers strive to maximize profits by accommodating more tenants on their machines, which inevitably introduces interference between tenants, leading to unpredictable application slowdowns. To address this challenge, prior researchers have focused on providing tenants with a more unbiased and predictable quality of service~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed clustering-based cache partitioning to mitigate unfairness between tenants. Rohan et al.~\cite{roy2021satori} aimed for both fairness and throughput by simultaneously controlling multiple architectural resources. However, achieving fairness comes at the cost of sacrificing resource utilization. In contrast, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} addressed the unfairness by adjusting their prices while accepting a certain degree of unfairness. Our study follows a similar direction but explores a more practical solution within the context of serverless computing.

% delete the following section: the approaches are against our scheme. 
% \textbf{Serverless Computing:} Many studies focus on reducing the latencies of serverless applications~\cite{cadden2020seuss,oakes2018sock,wang2019replayable,jia2021boki}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Ustiugov et al.~\cite{ustiugov2021benchmarking} record and prefetches the functions’ stable working set of guest memory pages to further reduce the function's startup time. Wei et al.~\cite{wei2023no} remote forking the serverless functions to reduce the cold start latency while limiting the resource usage. Schall et al. record and reload the instructions~\cite{schall2022lukewarm} or the BTB entries ~\cite{schall2023warming} to reduce the front-end stalls when reaccessing the same application. 
% \hl{Litmus is orthogonal to these approaches and can be adopted together.}

==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Serverless computing is a key technology in present cloud computing, offering numerous advantages. One primary advantage is its effective cost-saving, as tenants only pay for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion. While tenants suffer slowdowns, they also have to pay more for the slowdowns. Unlike prior approaches that aim to maintain quality of service, this paper discounts the tenant's cost to compensate for the loss. Litmus pricing proposed in this work monitors the machine states and adjusts the tenants' costs. The congestion level can be frequently gauged before every function using the proposed Litmus test, an effectively lightweight testing approach. Our tests show that Litmus offers near-ideal prices with a 0.38\% difference, compared to the ideal price that discounts proportional to its slowdown. 
Serverless computing is a key technology in contemporary cloud computing, offering a range of benefits. One primary advantage is effective cost-saving, as tenants are billed only for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion, which not only results in slowdowns but also higher costs for tenants. Rather than aiming to maintain service quality, this paper suggests discounting tenants' costs to compensate for performance losses. Litmus pricing proposed in this work monitors machine states through Litmus tests and adjusts tenant costs accordingly. The Litmus test is a lightweight testing approach for serverless platforms, which assesses the machine's congestion level before starting a user's function. Our tests prove that Litmus pricing offers nearly ideal prices in heavily congested environments, with an average deviation of just 0.2\% from the ideal price that adjusts discounts in proportion to the slowdown experienced.


==> fsfnkbznrsyvxmvjvpkfpdvqsfzxykbs/12_ack.tex <==
\section{Acknowledgment}
\label{ack}

We would like to thank our reviewers for their valuable feedback to improve this paper. This work was supported by NSF CAREER Award CCF-2146475.


==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/00_abstract.tex <==
\begin{abstract}

% Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While the providers can utilize their machines more efficiently, the tenants only need to pay for the resources they consume. However, a serverless system co-runs thousands of short-living functions concurrently to maximize resource utilization, bearing frequent state shifts. Meanwhile, when the system gets too congested, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants are also charged higher costs when experiencing slowdowns since all commercial serverless platforms determine the tenants' costs proportional to their execution times.
Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times.

% This paper argues that the cloud providers should compensate the tenants for their loss when the server is over-provisioned. However, estimating the tenant's loss is challenging when there is no pre-profiled information about the function. Prior studies showed assessing the tenant's loss introduces heavy overheads. Instead, this paper proposes a new pricing model, Litmus pricing, which offers discounts based on the machine's state while presuming the tenant's loss under the state. To monitor the machine state correctly, Litmus pricing frequently conducts Litmus tests, an effectively lightweight solution to measure system congestion. Our experiments show that Litmus pricing can detect the impact of system congestion and offer near-ideal prices, with only a 0.38\% price difference. 
This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2\% price difference on average, in a heavily congested system.

\end{abstract}


==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Serverless computing is growing fast, satisfying today's high demands for better programmability. It allows tenants to develop their programs as stateless functions in high-level languages such as Python, Go, and JavaScript without concerns with low-level resource management and task scheduling~\cite{serverless2,serverless1,schall2022lukewarm,schall2023warming,mohammad2020SerInWild}. This advantage attracts cloud users, helping them to deploy their programs quickly with minimal effort. Recent reports note that over 50-70\% of cloud users have adopted serverless computing for their tasks~\cite{serverless1}.

% Serverless computing claims a pay-as-you-go pricing model where users only pay for the resources used by their functions. This requires the service provider to monitor and estimate the fine-grained resource usage by each user accurately. However, today's high-performance systems maximize resource efficiency by accommodating multiple applications simultaneously and allowing the resources to be shared by them. Such a shared system raises two major challenges. First, tracking a user's resource usage is a challenging task. While being shared, the system tracks the total usage but not a single user's. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress. These inferences between the applications not only make the system hard to track resource usage, but the users may get charged unfairly due to the delayed execution time.
Serverless computing also benefits tenants financially. Unlike traditional cloud platforms that require tenants to purchase the hardware resources needed to deploy their servers regardless of actual usage~\cite{amazonEC2Pricing}, serverless computing claims a pay-as-you-go pricing model, where tenants only pay for the resources consumed during the execution of their functions, facilitating significant cost savings. Meanwhile, this pricing requires service providers to accurately monitor and estimate each user's fine-grained resource usage~\cite{microsoftAzurePricing,awsLambdaPricing,googleCloudFunctionPricing}. 

% However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared system raises two major challenges. First, tracking a tenant's resource usage is a challenging task. While being shared, the system can only monitor a tenant's use of specific resources. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference between the applications not only makes the system hard to track resource usage, but the tenants may get charged unfairly due to the extended execution time~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}. 
However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared serverless system raises two major challenges. First, tracking a tenant's resource usage becomes challenging, as the system can only monitor a tenant's use of exclusively dedicated resources while the system is shared. Second, and more importantly, co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference not only complicates tracking resource usage but also leads to tenants being charged unfairly due to delayed execution times~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}.

% A serverless platform should provide an isolated runtime environment to a user. Otherwise, we argue that the platform provider must compensate a tenant's loss as a discount when it is not achievable. Therefore, we define a charged fee as fair when it reflects the tenant's slowdowns due to the resource sharing. The following two methods can be used to estimate a fair price under a multi-tenant environment. 
A serverless platform should provide a user with an isolated runtime environment. Otherwise, we argue that the platform provider should compensate a tenant's loss as a discount when the isolation is not achievable. Thus, we define a charged fee as fair when it reflects the tenant's slowdowns caused by resource sharing. The following two methods can be used to offer a fair price in a multi-tenant environment.

% First, strict resource partitioning can divide shared resources into multiple partitions, each assigned to a user exclusively. The user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strictly partitioned resources are well known to cancel the opportunities to utilize the given resource efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delayed execution directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources when requesting them. 
First, strict resource partitioning can divide shared resources into multiple partitions, each assigned exclusively to a user. This means the user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strict partitioning is known to cancel opportunities to utilize resources efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delay directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources they need when requested. 

% Alternatively, a discount-based scheme estimates a user's price relative to its slowdown, discounting from the price when run without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources. Thus, the providers can maximize their hardware utilization and earn more money with given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns or interference they get from co-running tasks without overpaying for exclusive resources.
% The tenants also can get a discount reasonably proportional to the amount of their slowdown when their jobs suffer from interference rather than endeavoring to secure necessary resources exclusively.
Alternatively, a discount-based scheme estimates a user's price relative to the slowdown experienced, discounting from the price when running the task without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources, enabling providers to maximize hardware utilization and generate more revenue with the given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns they experience due to co-running tasks, preventing them from overpaying for lowered service quality.

% While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Even if the platform can measure its execution time, computing the slowdown still requires knowing its baseline, which can be gained when executing it alone. The cloud platform could not pre-profile users' applications for reasons such as mandated privacy when processing confidential information. Even if the platform has such information, the function could operate differently when receiving different inputs. That is to say, online profiling is necessary, which unfortunately requires expensive runtime sampling, as proposed in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. All co-running tasks must be stalled when estimating a task's baseline performance. Massive short-living serverless functions make such a sampling-based solution even more impractical. Frequently sampling the baseline performance of thousands of co-running functions is unrealistic. This motivates a new practical solution that can be adopted in commercial platforms. 
While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Although the platform can measure its execution time, determining the slowdown requires knowing its baseline performance, which can be obtained when it runs without interference. However, such profiling is often prohibited due to security concerns, particularly when the function processes confidential information. Additionally, the function may behave differently, with varying inputs each time it runs. That is to say, online profiling is necessary. Unfortunately, this requires expensive runtime sampling, as presented in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. When assessing baseline performance, all co-running tasks must be stalled. Hundreds to thousands of concurrent short-lived functions make this approach indeed impractical, as frequently sampling the baseline performance of such numerous functions is unrealistic. Thus, a new, practical solution that can be adopted in serverless platforms is needed.

%In either approach, a tenant or a service provider bears the problem's complexity alone. Resource partitioning demands the tenant to know the needed resources while losing opportunities to utilize the resources better. Discounting demands a service provider to estimate the task's slowdown with heavy sampling overheads. Accordingly, both approaches complicate the problem while sacrificing the machine's efficiency. Instead, we claim this problem becomes simpler when both entities participate and carry a portion of the responsibilities. 

% Litmus addresses this challenge by imposing the responsibility on both entities. With Litmus, the serverless platform measures the system congestion that may delay a function's execution when every tenant's function starts. The service provider needs to determine a discount rate for a corresponding congestion state. Meanwhile, the tenant needs to know about a possible slowdown and a corresponding discount. 

% We highlight that both partitioning and sampling complicate the problem while sacrificing the machine's efficiency and can hardly be employed in serverless computing. The approaches in serverless must be lightweight and frequent to deal with the fast-changing environment with thousands of concurrent functions. This paper proposes Litmus pricing that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening the system performance. 
We highlight that both partitioning-based and sampling-based approaches complicate the problem, either sacrificing the machine's efficiency or appearing impractical for serverless computing. Approaches in serverless computing must be lightweight, frequent, and sensitive enough to deal with quickly changing environments with numerous concurrent functions. This paper proposes Litmus pricing, a method that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening system performance. 

% \hl{Measuring the server's congestion status is challenging work. Here, Litmus relies on our key observation that, although not limited, function implementation in serverless computing largely relies on high-level programming languages such as Python and GoLang, which require a relatively long startup. This startup overhead has been considered one of the major challenges in serverless computing. However, Litmus utilizes this startup to measure the system's congestion state. Our analysis of Python and GoLang observed that the activities during the startups are almost identical, with plenty of memory operations, regardless of the functions. Thus, we claim that the startup performance can be an index of the system state.}

% \hl{The Litmus test is based on our insight that the serverless functions perform broadly identical operations, with plenty of memory operations, during their long startups, preparing the runtime environment for the functions. Leveraging this observation, the platform can assess the system's congestion level, which hints at the tenant's discount amount. Additionally, Litmus pricing exploits our second insight that the performance of two resources, private and shared, are affected differently by the congestion. In particular, its impact on private resources is minor and predictable, while many functions significantly rely on them, spending most of their execution time with them. }

% During the execution of every function, Litmus pricing conducts a Litmus test, which measures the level of system congestion with no extra overhead using the function's startup process. The Litmus test is based on the observation that serverless functions perform largely identical operations during their startup time. Those operations usually prepare the runtime and include a large amount of memory access to shared hardware resources. In addition, Litmus pricing splits the hardware resources into "private" and "shared" and proposes charging different ratios on each. This further improves the accuracy of the discount calculation.
During each function's execution, Litmus pricing conducts a Litmus test, which measures the level of system congestion without adding extra overhead, using the function's startup process. Litmus test is based on the observation that serverless functions perform largely identical operations during their startup, typically involving significant memory accesses. Additionally, Litmus pricing splits the hardware resources into "private" and "shared" categories, proposing different charging ratios for each. This approach further enhances the accuracy of the discount calculation.

% In our experiments, the Litmus pricing estimates a tenant's price to be nearly ideal, with a \hl{0.38\%} difference from the ideal price, which discounts tenants proportional to their slowdowns.
% This study investigates Litmus pricing across different environments, ranging from restricted to crowded settings. We verify that crowded environments pose additional challenges. Despite this, Litmus pricing accurately estimates a tenant's price, deviating by only 0.26\% from the ideal price, discounting tenants proportional to their slowdowns.
This study investigates Litmus pricing across diverse environments with varying levels of system congestion. We confirm that crowded environments pose complex challenges. Despite this, Litmus pricing accurately estimates a tenant's cost, deviating by only 0.2\% on average from the ideal price that discounts tenants proportional to slowdowns.



==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/02_background.tex <==
\section{Background}
\label{sec:background}

% \textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while the service providers handle back-end implementation~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers, which are later invoked upon associated events~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. The serverless platform guarantees security by executing the tenant's function in a sandbox such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.
\textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while leaving back-end implementation managed by service providers~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. These functions are later invoked upon associated events. The serverless platform ensures security by executing the tenant's function in a sandbox, such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.

% Each tenant's function is stateless and expected to be short~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using the short-lived functions, the tenant can easily scale by invoking many of the functions without provisioning needed resources for themselves, relying on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. Inherently, massive short-living serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. The tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and clients mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Later, under the pay-as-you-go pricing, the tenant is charged for the consumed resources, typically the product of time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
Each tenant's function is stateless and expected to be short-lived~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using these short-lived functions, tenants can easily scale by invoking many functions without provisioning the needed resources for themselves, relying instead on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. In serverless computing, numerous short-lived serverless workloads run together on a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. Tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and tenants mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% In the traditional cloud, tenants purchase hardware resources for the contracted term to support their applications, which are often expected to be large in a server form. Thus, tenants must pay for the agreed period regardless of actual use. Instead, serverless workloads are generally small and launched on-demand as short-living event handlers. This workload difference develops a unique pricing policy, pay-as-you-go pricing. The tenant is charged only for the consumed resources during the execution, typically the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
In traditional cloud computing, tenants purchase hardware resources for a contracted term to support their applications, which are typically large servers. Thus, tenants must pay for the agreed period regardless of actual usage. In contrast, serverless workloads are generally small and launched on-demand as short-lived event handlers. This difference leads to a unique pricing policy known as pay-as-you-go. Under this model, tenants are charged only for the resources consumed during execution, typically calculated as the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, where Python is utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Also, over 90\% of organizations choose Python and Node.js for their AWS services. Other popular language runtimes are Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer a high level of abstraction from machine codes with good programmability and portability, improving the programmer's productivity. As a result, they have been adopted widely by serverless users. However, such high-level languages typically rely on runtime interpretation, which results in a slow start of program execution with extra launching steps. For instance, in the case of Python, when an application is launched, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the codes are compiled and executed. Once the execution is complete, the Python program is terminated, and all assigned resources are released~\cite{pythonUsage}.
\textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python used in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Over 90\% of organizations choose Python and Node.js for their AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer significant abstraction from machine code with good programmability and portability, which in turn improves programmer productivity. Consequently, they are widely adopted by serverless users. However, high-level languages typically rely on runtime interpretation, leading to slower program startup due to extra launching steps. For example, when an application is launched in Python, the interpreter is first prepared. It then parses command-line arguments and imports necessary modules. Afterward, the codes are compiled and executed. Upon completion, the Python program terminates, and all allocated resources are released~\cite{pythonUsage}.

 
% list of pricing models? 
% Amazon? 
% Google?
% The price is calculated by duration time multiplies to the unit price plus the request charges. The duration time is from the time user's code begins executing until it returns or terminates. The unit price depends on the amount of memory the user allocate to their function. The request charges is based on how many times the function has been invoked minus the free requests~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% may need service agreement here, contention impact

%\textbf{Traditional cloud platforms:} In the context of traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage, data transfer, etc. The instance type is the combination of Virtual CPUs(VCPUs), RAM, storage and network performances. The time unit price will be higher with more powerful instance type. Typically, more powerful instance types have higher time unit prices. There are two main pricing options: On-Demand and Reserved Instances. On-demand instance let the customers pay for compute capacity by the hour or second based on the actual usage with no long-term commitments. Reserved Instances, on the other hand, require a commitment to a specific instance type for a contract term and offer cost savings compared to On-Demand pricing. Storage and data transfer for the VM instance can also impact the pricing. The more storage space a customer uses or the more data they transfer, the higher their costs will be. The traditional cloud platform can also be affected by the co-running applications~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} In traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage space, data bandwidth, etc. The instance type includes virtual CPUs, RAM, storage, and network performances. Typically, more powerful instance types charge higher prices. Also, two pricing options are commonly offered: on-demand and reserved instances. On-demand instances allow tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved instances require a commitment to a specific instance type for an agreed term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period. Storage space and data bandwidth for the VM instance also influence the price. Demanding more storage space or more data transfer raises the cost~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} 

% The price of traditional cloud platforms is determined by computing capabilities such as processor type, memory capacity, and network bandwidth. While more and better resources typically charge higher prices, two pricing options are commonly offered: on-demand and reserved instances. On-demand pricing allows tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved pricing requires a commitment to specific resources for an agreed-upon term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period~\cite{amazonEC2Pricing}. 

% There are several differences between traditional cloud platforms and serverless platform. 
% Firstly, the roles of customers in the execution environment differ between traditional and serverless platforms. In the traditional cloud, customers are responsible for configuring and maintaining virtual machines (VMs), setting up networking, and managing databases~\cite{amazonEC2Pricing}. And it's the customers's responsibility to detact and update the configurations to balance their expenses and performance. On the other hand, in serverless platforms, users only provide a single file to indicate their system and library requirement, while the service provider handles the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. This feature enables users to focus solely on their actual workload without the burden of managing the infrastructures. Additionally, the platform can automatically scale the resources for the users based on the current demand of the application to guarantee the customer satisfaction~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% There are apparent differences between traditional and serverless cloud platforms. First, tenants are responsible for managing hardware resources in traditional platforms. The tenants need to configure and maintain virtual machines, set up networking, and manage databases~\cite{amazonEC2Pricing}. Also, tenants should study the optimal configurations to balance their expenses and performance. Meanwhile, in serverless platforms, tenants only provide a single file to specify their system requirements while the cloud provider prepares the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. The platform provisions or scales the needed resources on demand. Consequently, the serverless platforms encourage tenants to focus solely on their front-end workloads without the burden of managing the low-level back-ends~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% Secondly, there are notable differences in compute power and memory size options between the two platforms. For traditional cloud, the granularity usually 1 VCPU and 1GB memory. But, for serverless platform, the smallest memory size is 128 MB~\cite{awsLambdaApiGateWay,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Thirdly, the characteristics of workloads on these platforms set them apart. Serverless applications are generally small and executed on-demand, resulting in very short workload durations~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can complete in less than one second. In contrast, traditional cloud applications tend to be larger and may require hours to complete. Additionally, the number of co-located applications on a single computing node is smaller in traditional cloud setups, making their execution environment less dynamic compared to serverless platforms.
% Lastly, the billing periods differ significantly between traditional cloud and serverless platforms. Traditional cloud users are charged for the allocated time period. Regardless of whether they are actively running tasks on the machine, they are still need to pay for the allocated time period. However, serverless customers are only billed for the actual execution time of their tasks on the platform.

% Second, the workloads are expected to be small in serverless computing. Serverless workloads are generally small and launched on-demand as short-living event handlers~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can be completed in less than one second, unlike traditional cloud applications that are often expected to be large in a server form. Inherently, massive serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. This workload difference develops a unique pricing policy in serverless computing, pay-as-you-go pricing. In the traditional cloud, the tenants purchase hardware resources for the contracted term. Regardless of actual use, they need to pay for the agreed period. However, the serverless platforms bill their tenants for the actual execution time of their tasks.


% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python being utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Furthermore, over 90\% of organizations leverage Python and Node.js alongside AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer numerous advantages for programmers, such as user-friendliness, portability, reduced error risks, and thriving ecosystems. As a result, they have garnered widespread acceptance within serverless platforms. High-level programming languages typically follow a fixed execution procedure. For instance, in Python, when an application is executed, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the code is compiled and executed. Once the execution is complete, the Python program is terminated, and all resources used by the program are released. Due to the consistency of the operating system and Python version, the beginning of the execution process remains the same each time~\cite{pythonUsage}.



% \textbf{Resource based discount vs. Slowdown based discount:} To fully utilize the available resources, service providers often run as many applications as they can in one computing node within the service agreement requirement. However, this may lead to resource congestion and cause slowdowns for users, which can be unfair, since the customers are paying more money for the worse experiences. The intuitionistic solution could be for the service provider to track the resource usage of each application and offer discounts to users who consume fewer resources. However, serverless applications are typically very small, and contention can affect different applications differently, making this approach less practical. A more suitable solution for serverless platforms could involve offering slowdown-based discounts. In this approach, the service provider dynamically updates unit prices based on the level of system congestion. When there is less contention, users normally stiffed with the experiences and pay the regular price. However, during periods of high congestion, when the system is under heavy load, users could receive discounted prices as compensation for potential slowdowns. This approach would align pricing with the actual performance experienced by users, ensuring a fair and responsive pricing model.


==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/03_methodology.tex <==
\section{Methodology}
\label{sec:method}

% \textbf{Hardware Infrastructure:} All the experiments are performed on a dual-socket server platform. Each socket has 16 simultaneous multithreading(SMT) cores. The CPU model is Intel Xeon Gold 5218(Cascade Lake). The maximum frequency of the machine is 3.9GHz. Each core has a 32KB L1 instruction cache, a 32KB L1 data cache and a 1MB L2 cache. The 32 virtual cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The computer node runs the latest Ubuntu server version(Ubuntu 22.04 LTS) with kernel version 5.15.0. For consistency in the results, the core frequency was set to 3.0GHz using the 'cpupower frequency-set' command. We use linux perf~\cite{perfWiki} to collect the performance counters for each experiment. To analyze the startup status, we use -I 1 option to obtain count deltas at one-millisecond intervals. By utilizing interpolation, we can know the performance counters of each execution period. 

% In this study, we test today's server systems with serverless functions. This section describes our test configuration. 
This section outlines our test setup for evaluating serverless functions in this study.

% % original version
% \textbf{Hardware Infrastructure:} All experiments are performed on a dual-socket server platform with two Intel Xeon Gold 5218 (Cascade Lake). The CPU offers 16 simultaneous multithreading (SMT) cores with 3.9 GHz maximum frequency. We pin the core frequency at 3.0GHz for our tests. Each core has 32KB L1 instruction/data caches and 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The machine runs the Ubuntu server OS (Ubuntu 22.04 LTS) with a kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to collect the performance counters, which are collected at every one-millisecond interval. 
\textbf{Hardware Infrastructure:} All experiments are conducted on a dual-socket server platform equipped with two Intel Xeon Gold 5218 processors based on the Cascade Lake architecture. Each CPU provides 16 cores that support simultaneous multithreading (SMT) with a maximum frequency of 3.9 GHz. Every core features 32KB of L1 instruction/data caches and a 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets collectively have access to 384GB of main memory. The server operates on Ubuntu Server OS, version 22.04 LTS, with kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to gather performance counters.

% The CPU frequency is a key performance/energy factor, significantly affecting a function's execution time and energy consumption. A CPU's frequency can be altered in software or hardware based on its power and thermal budget, configuring it for better energy efficiency or performance. However, varying frequencies cause the system performance/energy to be unsettled, making system management intractable. For this reason, commercial systems such as Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. In our tests, when the frequency is not fixed by software, Intel's Turbo technology alters the frequency occasionally but mainly employs 2.8GHz. We will discuss this further in the sensitivity section.
The CPU frequency is a critical factor influencing both performance and energy consumption, significantly affecting a function's execution time and energy usage. A CPU's frequency can be adjusted through software or hardware based on power and thermal budget, optimizing for either energy efficiency or performance. However, varying frequencies can cause instability in system performance and energy usage, complicating system management. For this reason, commercial systems like Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. If we do not fix the frequency through software, Intel's Turbo technology occasionally adjusts it, but it mostly remains at 2.8 GHz during our tests. We will provide more details on this in Section~\ref{sec:sensitivity}.

% \textbf{Stressing Programs:} We used two stressing programs to investigate how applications and the startup portion of the high level languages behave in a resource contention environment. FigureXXX illustrates the number of instructions, L3 accesses, and L3 misses that the stressing programs can generate in five seconds as the stressing levels increase. By combining different stress levels of these stress-testing programs, we can simulate various resource-congested environments. The XXX-stressor(lineXXX)  generates more L3 accesses with a high L3 hit rate. While XXX-stressor(lineXXX), in each stressing level, generates fewer L3 accesses but more L3 misses. With these two stressors and different stressing levels, we can simulate the system with varying contentions to the shared resources by creating various  L3 accesses and L3 misses. In figureXXX we can see that the L3 accesses generated from the L2-stressor (update name later) begin to decrease after reaching stressing level 20.  However, during this period, the L3 misses continue to increase. The reason behind this trend is that, after stressing level 20, the heightened L3 miss rate starts to impact the stressor's performance, leading to a decline in the committed instruction count. Consequently, the stressor generates fewer L3 accesses and more L3 misses. 

% \begin{table}[h]
%     \begin{center}
%     % \vspace{-1.0em}
%         \caption{Serverless Benchmarks \& Runtimes}
%         \label{tb:benchmarks}
%         % \vspace{-1.0em}
%         \begin{tabular}{|l l||l l|} \hline
%             Function & Abbr. & Function & Abbr. \\ \hline \hline
%             \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  & \multicolumn{2}{c|}{\textbf{Hotel Reservation~\cite{gan2019open}}} \\ \hline
%             Dyn HTML & dyn-py & Geo & geo-go* \\ \hline
%             Thumbnail & thum-py* & Profile & profile-go \\ \hline
%             Compression & compre-py & Rate & rate-go \\ \hline
%             Image Recogn & recogn-py* & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
%             Graph Rank & pager-py & Currency & cur-nj* \\ \hline
%             Graph Mst & mst-py & Payment & pay-nj \\ \hline
%             Graph Bfs & bfs-py* & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
%             DNA Visual & visual-py* & Authen & auth-py/nj/go \\ \hline
%             \multicolumn{2}{|c||}{\textbf{Function Bench~\cite{kim2019functionbench}}} & Fibonacci & fib-py/nj/go* \\ \hline
%             Chameleon & chame-py & AES & aes-py/nj/go \\ \hline
%             FloatOp & float-py* & & \\ \hline
%             % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
%         \end{tabular}
%     \end{center}
%     % \vspace{-1.5em}
% \end{table}

\begin{table}[h]
    \begin{center}
    % \vspace{-1.0em}
        \caption{Serverless Benchmarks \& Language Runtimes (py, nj, go)}
        \label{tb:benchmarks}
        % \vspace{-1.0em}
        \begin{tabular}{|l l||l l|} \hline
            Function & Abbr. & Function & Abbr. \\ \hline \hline
            \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  &  \multicolumn{2}{|c|}{\textbf{Function Bench~\cite{kim2019functionbench}}}\\ \hline
            Dyn HTML & dyn-py & Chameleon & chame-py \\ \hline
            Thumbnail & thum-py* & FloatOp & float-py \\ \hline
            Compression & compre-py & Gzip & gzip-py* \\ \hline
            Image Recogn & recogn-py & RandDisk & randDisk-py* \\ \hline
            Graph Rank & pager-py & SequenDisk & seqDisk-py \\ \hline
            Graph Mst & mst-py & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
            Graph Bfs & bfs-py* & Currency & cur-nj* \\ \hline
            DNA Visual & visual-py* & Payment & pay-nj \\ \hline
            \multicolumn{2}{|c||}{\textbf{Hotel Reservation~\cite{gan2019open}}} & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
            Geo & geo-go & Authen & auth-py*/nj/go \\ \hline
            Profile & profile-go* & Fibonacci & fib-py*/nj*/go* \\ \hline
            Rate & rate-go & AES & aes-py/nj*/go* \\ \hline
            % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
        \end{tabular}
    \end{center}
    % \vspace{-1.5em}
\end{table}

% revision version
% \textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we select 27 distinct serverless functions from different benchmark suites, including AWS' authentication serverless functions~\cite{awsLambdaApiGateWay}, Hotel Reservation from the DeathStarBench suite~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and SeBS serverless benchmark suite~\cite{copik2021sebs}. The three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating 3 separate test cases per function. Among them, we pick 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. The functions are implemented using three languages: Python, Nodejs, and Go. We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. 
\textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we selected 27 distinct serverless functions from various benchmark suites, including AWS authentication serverless functions~\cite{awsLambdaApiGateWay}, the Hotel Reservation from DeathStarBench~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and the SeBS serverless benchmark suite~\cite{copik2021sebs}. The functions are implemented using three languages: Python, Nodejs, and Go. Notably, the three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating three separate test cases per function. 
% This comprehensive language support ensures that our test coverage is thorough and representative of the diverse language preferences in the serverless computing community. 
We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. Additionally, we selected 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. 


%\hl{The benchmarks we choose include I/O-bound, memory-bound, and compute-bound functions. For an experiment, we put the testing function in core 0 to core 4. We also put 50 other functions in core 0-4 to let the application co-running with 10 other applications to observe the impact of context switching.}

% \hl{We select benchmarks with mixed performance characteristics: I/O, memory, and compute-bound. Also, to replicate the congested commercial systems, we located a testing function with 50 other functions and tied them to selected 5 cores, Core 0 to 4. During our evaluation, those functions run simultaneously and compete to secure any core among the five.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
\caption{(a) L2 misses and (b) L3 misses of traffic generators, both normalized with the average L2 and L3 misses of serverless applications listed in Table~\ref{tb:benchmarks}}
% \vspace{-0.5em}
\label{fig:stressing_specs}
\end{figure}

% \textbf{Traffic Generator:} We divide the CPU's shared resources into two distinct categories: resources before and after the L3 caches. To pressure each resource group individually, we developed two separate traffic generators aimed at generating traffic and congestion in these resources. The first traffic generator, CT-Gen, applies pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another traffic generator, MB-Gen, induces massive L3 misses that stress the resources after the L3 cache, mainly the off-chip memory bandwidth and L3 cache spaces.
\textbf{Traffic Generator:} We categorize the CPU's shared resources into two groups: those before the L3 caches and those after. To stress each group independently, we developed two separate traffic generators designed to generate traffic and congestion within these resources. The first generator, CT-Gen, exerts pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another generator, MB-Gen, induces massive L3 misses, which stress the resources beyond the L3 cache, primarily targeting off-chip memory bandwidth and L3 cache spaces.

% Both traffic generators are multi-threaded, governing the volume of traffic by adjusting the number of threads they spawn. Each thread spawned by the traffic generator is pinned on each core to prevent conflicts between threads; consequently, this setup allows us to vary the stress level across our 32-core processors, ranging from level 1 to 31. Figure~\ref{fig:stressing_specs} shows each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), for every thread count increment, CT-Gen makes massive L2 misses. The CT-Gen's L2 misses are ended with L3 hits, as shown in Figure~\ref{fig:stressing_specs}(b). Meanwhile, MB-Gen creates huge L2 and L3 misses, as implemented. Interestingly, its L2 misses are fewer than CT-Gen's because MB-Gen is slowed by its L3 misses, suffering from a self-created bandwidth bottleneck. 
Both traffic generators are multi-threaded and govern the amount of traffic by adjusting the number of threads they spawn. Each thread is pinned to a specific core to avoid conflicts between threads, allowing us to vary the stress level on our 32-core processors from level 1 to 31. Figure~\ref{fig:stressing_specs} illustrates each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), with each increase in thread count, CT-Gen generates substantial L2 cache misses. These L2 misses by CT-Gen are ended with L3 cache hits, as shown in Figure~\ref{fig:stressing_specs}(b). In contrast, MB-Gen produces significant L2 and L3 cache misses. Interestingly, MB-Gen's L2 misses are fewer than those of CT-Gen because MB-Gen is hindered by its L3 misses, suffering from a self-imposed performance bottleneck.



==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/04_motivation.tex <==
\section{The Need for Fair Pricing}
\label{sec:motivation}

% Offering fairness appears in different approaches in cloud computing when multiple tenants share hardware resources. One standard is SLA, which defines the level of services the cloud provider furnishes while a tenant sets their expectation. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving unfairness between tenants. Although serverless computing highlights the pay-as-you-go pricing model, such unfairness still exists.
Fairness in cloud computing, especially when multiple tenants share hardware resources, is addressed through various approaches. One standard method is the Service Level Agreement (SLA), which specifies the level of service the cloud provider must deliver and the tenants' expectations. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving fairness issues. Despite serverless computing's emphasis on a pay-as-you-go pricing model, unfairness among tenants still exists.

% Unfortunately, modern systems are designed to maximize hardware efficiency by co-running multiple applications; the function's execution time can be affected by co-scheduled applications with conflicts when using shared resources. Ironically, whenever the service provider squeezes their resources further for better profit by accommodating more functions into a single machine, each function's execution time increases, charging them a higher cost for the same workload. However, in serverless computing, tenants lack control and insights into how their software is executed and billed for the cost of convenience. 
Unfortunately, modern systems are designed to maximize hardware efficiency by running multiple applications concurrently. This results in conflicts over shared resources, affecting each function's execution time. Ironically, when service providers optimize for profit by packing more functions into a single machine, the execution time for each function increases, resulting in higher costs for the same workload. In serverless computing, tenants have no control or visibility over how their software is executed, leading to potential inefficiencies and higher costs for the sake of convenience.

% Genuine pay-as-you-go pricing can be achieved when there is no interference. However, that is not desired by the providers who expect to utilize their resources to maximize profits. In serverless, although each function runs virtually exclusively in a sandbox with private resources, it still shares a few resources with other co-running functions, such as shared caches and memory bandwidth. Resource partitioning, a traditional solution that eliminates interference, can promise exclusively dedicated resources to a tenant but cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 
In serverless computing, although each function runs exclusively in a virtual sandbox with private resources, it still shares certain resources like caches and memory bandwidth with other functions. Resource partitioning, a traditional solution that eliminates interference by dedicating resources exclusively to a tenant, cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 

\begin{figure}[h]
\centering
% \vspace{-0.7 em}
\includegraphics[width=1\columnwidth]{./fig/normalizedCPIRunWith26Rev}\\
% \vspace{-1 em}
\caption{Execution time of applications that run with 26 others, normalized to the execution time when running alone}
% \vspace{-0.4 em}
\label{fig:normalizedCPIRunWith26Rev}
\end{figure}

% Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed down when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. \hl{Whenever a function finishes, another function is randomly launched to maintain a total of 26 co-running functions.} The figure shows a function's performance drops by up to 35\%, and most functions are significantly influenced by the co-running functions. Compared to when an isolated environment is offered, the function performs 11.5\% slower on average, charging 11.5\% more to users. We highlight that the function runs only with 26 other functions, which is tiny compared to massively crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.
Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. Whenever a function finishes, a new randomly-selected function is launched to maintain a total of 26 co-running functions. The figure shows a function's performance can drop by up to 35\%, with most functions significantly impacted by the co-running functions. On average, functions perform 11.5\% slower in this shared environment compared to an isolated one, resulting in users being charged 11.5\% more. We highlight that this scenario involves only 26 co-running functions, which is tiny compared to heavily crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.

% Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} attempted to offer price discounts if it has a slowdown, compensating for the slowdowns. To provide the discount, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount reflecting the slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all the responsibilities of the contentions between co-running functions, guaranteeing all tenants an invariant price for their use. Any unexpected slowdowns that a tenant experiences are returned with a discount. However, sampling is an expensive operation, requiring all co-running processes to stall during the sampling. Moreover, accurate measurement requires frequent sampling when its system environment quickly alters, making the approach impossible in a fast-shifting environment like a serverless platform.   
Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} offers price discounts to compensate for slowdowns. To provide these discounts, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount based on the observed slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all responsibilities related to contentions from resource sharing, ensuring tenants pay a consistent price for their usage. Any unexpected slowdowns that a tenant experiences are compensated with a discount. However, sampling is an expensive operation that requires stalling all co-running processes during the sampling. Moreover, accurate measurement necessitates frequent sampling, especially in rapidly changing environments, making the approach impractical for dynamic environments like serverless platforms.


% A tenant needs a new pricing model based on more than just execution time. However, prior approaches have limitations, burdening cloud participants too heavily; it is unsuitable for \hl{thousands} of concurrent short-lived functions in serverless computing. This motivates us to propose a new solution, Litmus pricing, that discounts prices based on the system state but offers lightweight with no overheads.
Overall, tenants need a new pricing model that considers more than just execution time. Prior approaches have limitations, excessively burdening cloud participants and being unsuitable for the many short-lived functions typical in serverless computing. This motivates us to propose a new solution: Litmus pricing, which discounts prices based on the system congestion while remaining lightweight and imposing no additional overhead.


==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/05_design.tex <==
\section{Litmus Pricing}
\subsection{Overview}

% The estimated prices of serverless functions should reflect the congestion level of the system inside their machines. With the massive short-living functions, the serverless system's state can dramatically change in a short time. Accordingly, the system state can be congested at any moment and also resolved in a short time. However, such a temporary traffic jam may significantly impact the performance of short-living functions. Therefore, assessing the congestion must be lightweight, quick, and on time. However, a prior approach, POPPA\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling with considerable performance overheads, preventing them from wide adoption. Instead, we propose a new scheme, Litmus pricing, that quickly estimates system congestion at the start of every function and reflects the estimation into pricing the function. 
The estimated prices of serverless functions should reflect the system's congestion state. The presence of numerous small transient functions within the serverless system can rapidly alter its congestion state, causing sudden congestion or swift resolution. Nevertheless, such transient traffic jams can significantly impact the performance of short-lived functions. Thus, assessing the congestion must be lightweight, quick, and timely. However, a prior approach, POPPA~\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling, which incurs considerable performance costs, thereby limiting its widespread adoption. Alternatively, this study introduces Litmus pricing, which promptly gauges system congestion at the onset of each function and reflects the estimated congestion level into pricing the function.

% Like the prior approach~\cite{tiwari2013enabling,alex2013ScFairPrice}, Litmus pricing suggests that the service provider discounts when a tenant's functions are intervened, compensating for the performance loss. To determine the discount ratio, Litmus measures system congestion level, which can also help service providers evaluate remaining resources and make decisions on job scheduling. 
Like the prior approach, Litmus pricing suggests that service providers should offer discounts when a tenant's functions experience interference, thus compensating for the performance loss. Litmus pricing determines the discount rate based on the system's congestion level. Evaluating congestion also assists providers in estimating remaining resources and making informed decisions regarding job scheduling.

%Nevertheless, the Litmus pricing does not quantify each function's slowdown; the discount amount is determined only by the severity of the measured congestion. The impact of the congestion on distinct functions appears differently despite facing the same congestion level, and precisely estimating a function's performance loss is a complex problem. That's why the prior approach had to rely on expensive sampling. Instead, the Litmus pricing avoids the overheads and limits the service provider's responsibility to measure the current congestion. 
However, Litmus pricing does not quantify the slowdown of each individual function; the discount amount is solely determined by the severity of the measured congestion. Even though different functions face the same congestion level, their respective impacts can vary, making precise estimation of each function's performance loss a challenging task. This complexity necessitated the expensive sampling relied upon by the previous approach. Instead, Litmus pricing circumvents such overheads and lightens the service provider's burden solely to measure ongoing congestion levels.

% Litmus pricing embodies the varying value of shared resources across different system conditions by applying equal discounts to all functions under the same system condition, although the functions experience different slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that a function that is slowed more than others demands the over-crowded resources more while exacerbating the adverse over-crowded conditions. Litmus pricing does not provide additional compensation for their extra loss compared to others due to their heavy use of shared resources.
Litmus pricing captures the dynamic significance of shared resources under varying system conditions by offering uniform discounts to all functions under the same system congestion, regardless of their individual slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that functions experiencing larger slowdowns tend to demand more of the crowded resources, thereby exacerbating adverse overcrowded conditions. However, Litmus pricing does not offer additional compensation for the larger loss experienced by functions that use shared resources more heavily than others.

% As a result, Litmus inherently incentivizes users who use shared resources sparingly. When over-crowded, functions with minimal needs for shared resources still enjoy discounts but encounter slight slowdowns. This implies that users may take advantage of this policy by minimizing their use of shared resources, receiving substantial discounts despite enduring only minor slowdowns. Such a trade-off is considered acceptable because the user's shared resource usage reduces their contribution to congestion, thereby benefiting the overall system over the other users.
As a result, Litmus inherently incentivizes users who use shared resources sparingly. During periods of overcrowding, functions with minimal needs for shared resources still enjoy discounts but with only slight slowdowns. This implies that users may take advantage of this policy by minimizing their reliance on shared resources, receiving substantial discounts despite only experiencing minor slowdowns. This trade-off is considered acceptable because reduced shared resource usage by users helps mitigate congestion, thereby benefiting the overall system and other users.
% Lastly, the system refrains from scheduling a function if the congestion level exceeds a predetermined threshold, thus preventing resource thrashing.


\subsection{Pricing Model}
\label{pricing model}

% Developing Litmus pricing raises two challenges. First, Litmus needs a new pricing model to estimate a function's price. Second, Litmus needs a way to measure the system's congestion state. Due to the serverless's fast-shifting environment, assessing the congestion must be lightweight and frequent at the right time. Nevertheless, all present commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants must pay more with prolonged execution time when using over-crowded resources. Rather than simply imposing a price by multiplying the main memory usage and a function's total execution time, Litmus suggests the price as a sum of two distinct price components as follows.
Developing Litmus pricing raises two challenges. First, it needs a new model to estimate a function's price. Second, it needs a way to measure the system's congestion state. Due to the rapidly changing environment in serverless computing, assessing congestion must be lightweight and timely. Commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants end up paying more for prolonged execution time when using over-crowded resources. Rather than simply imposing the price by multiplying the main memory usage and a function's execution time, Litmus pricing determines the price as a sum of two distinct pricing components as follows.

\begin{equation} 
P = P_{private} + P_{shared}
\end{equation}

% In this equation, \(P\) denotes the total price tenants need to pay to execute their functions. Litmus pricing divides the tenant's price into two pricing components, each with a different resource type. \(P_{private}\) represents the price the tenant needs to pay for private resources, which are entirely assigned to a tenant. \(P_{shared}\) is the price the tenant needs to pay for the shared resources. Each price component is measured proportional to a user's time to occupy the corresponding resources. However, such occupied time can be extended when contention disturbs a process's execution in the shared resources. This delayed time increases a tenant's price unfairly. 
In this equation, \(P\) denotes the total price tenants must pay to execute their functions. Litmus pricing divides this cost into two pricing components, each associated with a different resource type. \(P_{private}\) is the cost for private resources, which are entirely assigned to a single tenant. \(P_{shared}\) is the cost for shared resources. Each pricing component is measured proportional to the time users occupy the respective resources. However, if contention disturbs a process's execution in the shared resources, the occupied time will be extended. This delay unfairly increases the tenant's cost. 


\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/slowdownRunwith26Rev}\\
\caption{\(T_{private}\) and \(T_{shared}\) of applications that run with 26 others, normalized to those when running alone}
\vspace{-0.5em}
\label{fig:slowdownRunwith26Rev}
\end{figure}

% Using Perf, we measure the delays due to the shared resources and split a function's execution time into two distinct slices: one slice, \(T_{private}\), which is time spent on private resources and another slice, \(T_{shared}\), which is time spent on shared resources. Figure~\ref{fig:normalizedTcore&Tuncore-runWith16} shows the impact of the contentions on each time slice, where we normalize \(T_{private}\) per instruction and \(T_{shared}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 207\% on average and 364\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions. 

% We observe that the system congestion influences the occupied time for each resource type differently. The time to hold private resources is slightly affected, with minor changes, even under heavy congestion. Meanwhile, the time due to shared resources is broadly affected, showing significant differences. Thus, we separately measure the two delays and charge their use with a different rule.
We observed that system congestion influences the occupied time for each resource type differently. The time to use private resources is only slightly affected, with minor changes, even under heavy congestion. In contrast, the time spent on shared resources is broadly affected, showing significant differences. Thus, we separately measure the delays for the two resource types and apply different charging rules for their use. 

% Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where we normalize \(T_{shared}\) per instruction and \(T_{private}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 181\% on average and 488\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions.
Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is calculated as the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where \(T_{shared}\) per instruction and \(T_{private}\) per instruction are normalized to the same tests when running alone. The figure shows that \(T_{shared}\) is significantly affected by system congestion compared to \(T_{private}\). On average, \(T_{shared}\) increases by 181\%, with a maximum increase of 488\%. Meanwhile, \(T_{private}\) increases by only 4\%, with minor variance between functions.

% This figure gives insights into two key factors. First, the congestion in the shared resources does not impact the performance of private resources. Accordingly, when the system gets congested, the degree of a function's dependence on the shared resources determines the function's performance. If the \(T_{shared}\) takes a minor portion of a function's execution, severe congestion still barely influences its overall execution. Second, hardware PMUs available in modern CPUs, and profiling tools such as Linux Perf are widely available and can be used to distinguish the usage of shared and private resources. Across the paper, we will take advantage of such tools to develop Litmus pricing.
This figure highlights two key factors. First, congestion in shared resources has a negligible impact on the performance of private resources. Accordingly, when the system gets congested, the extent of a function's reliance on shared resources determines its performance. If \(T_{shared}\) constitutes a minor portion of a function's execution, even severe congestion will have minimal impact on its overall execution. Second, hardware Performance Monitoring Units (PMUs) in modern CPUs and profiling tools like Linux Perf are widely available and can be utilized to differentiate between the use of shared and private resources. Throughout this paper, we will leverage these tools to develop Litmus pricing.

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/TpriTshardDistriRev}\\
% \caption{\(T_{private}\) and \(T_{shared}\) distribution when they run alone}
\caption{Execution time distribution of \(T_{private}\) and \(T_{shared}\)}
\vspace{-0.5em}
\label{fig:TpriTshardDistriRev}
\end{figure}

% Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) in a function's execution. The compute-intensive workloads (e.g., fib-py, float-py) have a substantial \(T_{private}\) portion that can reach 99.96\% of the execution time. However, the portion decreases when running memory-intensive workloads such as fib-nj. This distribution indicates how much other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase float-py's \(T_{shared}\), its total execution time, $T_{private}+T_{shared}$, will undergo minor change.
Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) during a function's execution. Compute-intensive workloads (e.g., fib-py, float-py) exhibit a substantial \(T_{private}\) portion, accounting for up to 99.96\% of the execution time. However, this portion decreases when running memory-intensive workloads such as fib-nj. This distribution reflects how other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase its \(T_{shared}\), the total execution time, $T_{private}+T_{shared}$, will undergo only a minor change.

% For each pricing component, we calculate the price by multiplying its charging rate with its time distribution. Thus we can further update the pricing equation.
After collecting the time slices spent on each resource, Litmus calculates each pricing component by multiplying two different charging rates with corresponding slices. Consequently, a new pricing equation emerges as follows:

\begin{equation} 
P = R_{private} * T_{private}  + R_{shared} * T_{shared}
\end{equation}

% \(T_{shared}\) is the cycles stalled due to L2 misses. It is measured from the perf counter, STALLS\_L2\_Misses. \(T_{private}\) is the total execution minus STALLS\_L2\_Misses. 
% Using Perf, Litmus collects\(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total cycles to complete the application minus \(T_{shared}\). 
% While Litmus returns the system's congestion state, the service provider still needs to determine reasonable prices charged for a service when having different congestion levels. 

% \(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. Again, the two charging rates are necessary since each component is affected differently, directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from the crowded execution environment. Thus, the charging rates should be measured as follows.
\(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. These two charging rates are necessary because each component is affected differently, either directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from a crowded execution environment. Thus, the charging rates should be measured as follows:

\begin{equation} 
R = R_{base} * \frac{T_{solo}}{T_{congestion}}
\end{equation}

% In this equation, \(R\) is the charging rate for executions on either private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free execution environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is the execution time when the function runs alone, and \(T_{congestion}\) is its execution time in the congested environment. Again, we should collect a separate \(T_{solo}\) and \(T_{congestion}\) for each pricing component. To measure \(T_{solo}\), \hl{the prior work}~\cite{alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. Litmus pricing avoids such a costly approach but presumes the function's \textit{solo} performance by examining reference workloads on the system.
In this equation, \(R\) represents the charging rate for executions on private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free runtime environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is its non-interfered execution time when the function runs alone, and \(T_{congestion}\) is its execution time in a congested environment. We need to collect separate \(T_{solo}\) and \(T_{congestion}\) values for each pricing component. To measure \(T_{solo}\), the prior study~\cite{tiwari2013enabling,alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. However, Litmus pricing avoids such a costly approach by presuming the function's solo performance through reference workloads on the system.

% Litmus pricing requires both providers and tenants to be involved in the price decision. The providers need to decide on reasonable rates for each resource use by analyzing the selected representative functions running on the system. To offer reasonable discounts, the providers must choose the functions analyzed carefully, collecting the functions representing the system. The tenants must also know the consequences when their tasks heavily rely on any of the shared resources. Unfortunately, their tasks may get delayed more than the provider's expectation while still receiving the discount rate up to the expectation. 
Litmus pricing requires both providers and tenants to be involved in the price decision process. Providers need to establish reasonable rates for each resource usage by analyzing selected representative functions. To offer fair discounts, providers must carefully choose the functions to be analyzed, ensuring the functions accurately represent the system condition. Tenants must also know the consequences when their tasks heavily rely on shared resources. Unfortunately, their tasks may get delayed more than the provider's expectations while still receiving the expected discount rate. 

% Here, the Litmus pricing reflects the varying value of the shared resources when the system's congestion level changes; the importance of shared resources becomes more valuable when congested. 



==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/06_design_details.tex <==
\section{Estimating prices with Litmus}
\label{sec:designDetails}

% The providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}, before using Litmus pricing. The numbers in both tables are the slowdowns of codes while testing the system congestion. Shortly, the congestion table is filled with the slowdowns of startup codes, and the performance table is filled with the slowdowns of reference benchmarks. Litmus pricing needs three steps to charge the final price with a discount. First, the providers assess the system's congestion at multiple levels and range them in a table. This step completes the congestion table. Second, the providers study the impact of congestion on tenants' functions and complete the performance table. Lastly, the service provider determines a tenant's price based on the two tables. 
Before using Litmus pricing, service providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}. The congestion table lists the slowdowns during the startup phases, whereas the performance table lists the slowdowns of reference functions. Litmus pricing needs three steps to determine the final price with a discount. First, providers assess system congestion at multiple levels and record the results in the congestion table. Second, providers analyze the impact of congestion on reference functions and fill out the performance table. Lastly, providers determine a tenant's price based on the data from both tables.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tables}\\
\caption{Congestion and performance tables: numbers in both tables indicate the slowdowns of startup codes and reference functions, collected with CT-Gen and MB-Gen}
\vspace{-0.7em}
\label{fig:litmust_tables}
\end{figure}

\textbf{Step 1, Defining Congestion Levels:} We manage the system's congestion levels using two traffic generators that create a range of congestion states by stressing shared resources differently. The traffic generator is multi-threaded, creating traffic in shared resources to incur congestion, with each thread running on a separate core. We rank the stress levels from 1 to 32 by changing the number of active threads running on distinct cores. Entries from top to bottom in the congestion table indicate increasing stress levels.

% \begin{figure}[h]
% \centering
% \vspace{-1.5em}
% \includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
% \vspace{-1em}
% \caption{stressing program's instruction, L3 accesses and L3 misses }
% \vspace{-0.5em}
% \label{fig:stressing_specs}
% \end{figure}

% \textbf{Step 2. Measuring System Congestion:} Measuring the current level of system congestion that may influence a function's performance is a crucial challenge. If we assume that the platform does not have pre-profiled information about a function's performance, the platform cannot figure out whether co-running functions influenced the function. Additionally, the serverless platform's fast-changing states with massive short-living functions make the assessment even more complicated, requiring quick and frequent examinations.

% Meanwhile, measuring the amount of a system's congestion and its impact on performance is a crucial challenge. This challenge particularly stands apparent when being demanded to quantify the impact of the congestion on a running application without pre-profiled information about the application. Moreover, the serverless platform's fast-changing system states with \hl{numerous} short-lived functions make the assessment even more complicated, requiring quick and frequent performance examinations.
Measuring the amount of system congestion and its impact on performance is a crucial challenge. This challenge becomes particularly pronounced when trying to quantify the impact of the congestion on a running application without pre-profiled information about the application. The fast-changing system states of a serverless platform, with numerous short-lived functions, further complicate the assessment, necessitating quick and frequent performance examinations.

% Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. The proposal is based on the observation that high-level languages, such as Python and Node.js, used in serverless computing have long startup times to accommodate their runtime environments. Since the inception of serverless computing, these startups have been recognized as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests leverage these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests further validated that all tested functions exhibited similar performance characteristics during their startups. 
Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. This method leverages our observation that high-level languages like Python and Node.js, commonly used in serverless computing, have lengthy startup phases to accommodate their runtime environments. Since the inception of serverless computing, these startup delays have been identified as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests exploit these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests have validated that tested functions exhibit similar performance characteristics during startup phases. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_all}\\
% \caption{IPC for serverless applications with different runtimes in the first 100 milliseconds of their execution}
% \vspace{-0.5em}
% \label{fig:startupIPC_all}
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped}\\
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-1}\\
\includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped_3}\\
% \caption{IPC for serverless applications grouped by language runtime in the first 100 milliseconds of their execution}
\caption{IPC of serverless applications based on languages (Go, Python, and NodeJS) during their startup phase}
% \vspace{-0.7em}
\label{fig:startupIPC_grouped}
\end{figure}

% Figure~\ref{fig:startupIPC_grouped} depicts the fluctuation in IPC (Instructions Per Cycle) of a function during the first milliseconds of its execution. The x-axis shows a time flow since the beginning; every tick indicates a millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language, and the throughput of each group is represented in separate figures. Although figures exhibit different patterns, functions in the same figure display notable similarities. The figures imply that functions written in the same language have nearly identical startups.
Figure~\ref{fig:startupIPC_grouped} depicts a function's fluctuation in IPC (Instructions Per Cycle) during its startup phases. The x-axis represents the time elapsed since the beginning, with each tick indicating one millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language runtime, and the IPC of each group is presented in separate figures. As shown in these figures, functions in the same figure show notable similarities. This implies that functions written in the same language have nearly identical startups.

% The startup of a runtime usually includes bursts of memory reads to load images and libraries, which can probe the traffic in the shared resources. By conducting a Litmus test before executing every tenant's codes, the providers can observe the system state for the function. Meanwhile, the providers also need to study how the startup codes perform in different system states. They complete the congestion tables by performing the Litmus tests with the startups written in three languages while varying the congestion levels. To this end, the information in the congestion table is looked up when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}. 
% estimating the system's state upon receiving a result of a function's Litmus test. 
The startup of a runtime typically includes bursts of memory reads to load images and libraries, which can be used to probe the traffic in shared resources. By conducting a Litmus test before executing a tenant's function, providers can assess the system state. Meanwhile, providers also need to study how startup phases perform under different system states. They complete the congestion tables by conducting the Litmus tests with startups written in three languages while varying congestion levels. This information from the congestion table is then referenced when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tests}\\
\caption{Progress of serverless applications on four cores with Litmus tests (dotted arrows) over time}
% \vspace{-0.5em}
\label{fig:Litmus_tests}
\end{figure}

% Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests. The Litmus tests examine the level of system congestion with every function startup. \hl{Many} concurrent functions in serverless offer frequent test opportunities. Function\#1 is a memory-intensive function that raises a congestion level. While active, Litmus tests measure the congestion level above 8. After Function\#1's completion, the next Litmus test detects a non-congested system with a congestion level below 3. However, with the start of another heavy function, function\#2, the Litmus tests measure the new congestion in the system.
Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests, which examine the level of system congestion during each function's startup. Many concurrent functions in serverless offer frequent opportunities for testing. Function \#1, which is memory-intensive, causes congestion levels to rise above 8 during its execution. A Litmus test in Core 3 detects this congestion. After Function \#1 is complete, a subsequent Litmus test indicates a non-congested system with a congestion level below 3. However, during another resource-intensive function, Function \#2, the Litmus test identifies new system congestion with a level above 9.  

% \textbf{Step 2. Measuring the Impact of Congestion:} Although discerning the system congestion through the Litmus test, estimating its impact on a user's application is another challenge. This work proposes a discount based on the pre-studied impacts on reference functions, assuming the user's functions are alike. For this, the service providers need to select reference functions that represent users' functions running on their systems. In this work, we select the workloads in \hl{Section 2} as our reference applications. 
\textbf{Step 2, Measuring the Impact of Congestion:} Discerning system congestion through the Litmus test solves only one of the two challenges; the other is determining its impact on a tenant's function. Different tenants' functions could experience varying degrees of slowdown under the same congestion level. To address this, we propose using pre-selected reference functions to analyze these impacts, thereby avoiding the cost of runtime profiling. For this, providers need to carefully select reference functions that represent tenants' functions operating on the systems, as these selections influence the overall accuracy of congestion measurement. Later, in Section~\ref{sec:evaluation}, our tests will show that pre-selected reference functions can effectively represent unknown user applications. For this study, the selected reference applications (* marked) are listed in  Table~\ref{tb:benchmarks}. 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/refSlowdownStressing14}\\
% \includegraphics[width=1\columnwidth]{./fig/slowdownStressing16}\\
\caption{\(T_{private}\), \(T_{shared}\), and \(T_{total}\) of serverless applications that run with MB-Gen at stress level 14, normalized to their execution time when they run alone}
% \vspace{-0.5em}
\label{fig:refSlowdownStressing14}
\end{figure}

% Once the reference functions are ready, the providers study the slowdowns of the reference functions while varying different congestion levels again. This study completes the performance table in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. Again, our two traffic generators create two separate sub-tables. All entries in this table are 1-to-1 mapped to entries in the congestion table. The providers estimate a general function's slowdown when having a certain congestion level using this 1-to-1 mapping.
Once the reference functions are ready, providers analyze their slowdowns under varying congestion levels. This analysis completes the performance table shown in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. With two traffic generators, providers can complete another set of two sub-tables for the performance table. All entries in this table are mapped 1-to-1 to entries in the congestion table. Providers can estimate a general function's slowdown at a given congestion level using this one-to-one mapping.

% Figure~\ref{fig:refSlowdownStressing14} shows the reference functions' slowdowns when stressing the system. The X-axis shows different functions, each consisting of three bars: the first two bars show the CPI during each time slice, \(T_{private}\) and \(T_{shared}\), and the last bar shows the CPI of an entire execution. The figure shows that the tested functions suffer from different amounts of slowdowns, although the tests maintain consistent stress levels. \hl{The last group} shows the gmean of all the slowdowns, which is used when providers estimate a function's slowdown later. 
Figure~\ref{fig:refSlowdownStressing14} shows an example of the reference functions' slowdowns when stressing the system. The X-axis shows tested functions, each depicted with three bars: the first two bars show \(T_{private}\) and \(T_{shared}\), while the last bar shows the total execution time, all normalized to their execution time when running alone without interference. The figure shows that the tested functions experience varying degrees of slowdown despite consistent stress levels maintained during the tests. The next-to-last group shows the gmean of all the slowdowns, which providers use to estimate a function's slowdown later.

% \hl{This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/referenceStartupSlowdownRev}\\
\caption{The correlation between the slowdown of Python's startup phase and the slowdown of reference applications. From left, (a) \(T_{private}\), (b) \(T_{shared}\), and (c) \(T_{total}\), normalized to the execution time when running alone}
\label{fig:referenceStartupSlowdownRev}
\end{figure}

% \textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while a range of congestion levels is continuous, the tables only contain a few slowdowns in discrete intervals. Thus, providers need a model that returns an estimated slowdown when receiving a congestion level as an input. In our tests, we employ a linear regression to achieve the model.
\textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while congestion levels vary continuously, the tables only contain slowdowns at discrete intervals. Therefore, providers need a model that estimates the slowdown for any given congestion level. In our tests, we employ linear regression to develop the model.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/interpolation}\\
\caption{Estimating a function's slowdown with logarithmic interpolation}
\label{fig:interpolation}
\end{figure}

% Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding references' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). We employed two traffic generators to extrapolate a more precise congestion level, yielding two sub-tables in both the congestion and the performance tables. Consequently, the figure presents two linear regression models, each associated with a different traffic generator. 
Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding reference applications' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). To extrapolate a precise congestion level, we created two sub-tables within both the congestion and performance tables using two distinct traffic generators. As a result, the figure depicts two linear regression lines (red and blue dotted lines), each associated with a different traffic generator.

% The provider needs to estimate the function's slowdown to uncover its price. However, the above two regression models return two vastly different slowdowns. Then, the providers need to determine which model is close to the current environment. We think the two models reflect two extreme congestions that the traffic generators create, one before the L3 and one after the L3. CT-Gen creates massive traffic from the core to the L3 cache, which filters the traffic, preventing the operations from consuming the memory bandwidth. MB-Gen also creates huge traffic but consumes the memory bandwidth and replaces L3 blocks. Since each traffic generator creates an extreme case, the machine state could be intermediate with congestion in the range between the two congestions created by CT-Gen and MB-Gen. However, Litmus pricing cannot answer this question with only the startup's slowdown. 

% To address this question, we note that the system's L3 misses are a critical indicator closely related to a function's performance. Functions suffer more when the system experiences more L3 misses, which stresses the cache space and off-chip memory bandwidth. Accordingly, Litmus test collects the system's L3 miss count as a supplementary index, which tells more about the crowdedness of shared resources.

These regression models return two different slowdowns. To estimate a function's slowdown, providers must determine which model reflects the current environment more accurately. The traffic generators create two extreme congestion scenarios: one before the L3 cache and one after. CT-Gen generates substantial traffic from the core to the L3 cache that filters the traffic and prevents operations from consuming memory bandwidth. Conversely, MB-Gen also generates massive traffic but consumes memory bandwidth and repeatedly evicts L3 cache blocks. Because each traffic generator represents a distinct extreme case, the actual machine state could fall somewhere between the two congestion levels created by CT-Gen and MB-Gen. However, Litmus pricing requires more than just the startup slowdown to identify the machine's state in these models. Thus, we have enabled Litmus tests to gather the system's L3 miss count as a supplementary metric that offers deeper insights into the crowdedness of shared resources.


% \hl{Figure 1} shows how to use the L3 cache misses with the performance sub-tables. The two traffic generators make the upper and lower boundary of the L3 miss rates. When performing a Litmus test, if the test's L3 miss rate is XXX, close to the L3 misses with CT-Gen, we can conclude that the congestion occurs before the L3 cache and select the expected slowdown of XXX. On the contrary, we choose XXX, in case the L3 miss rate is XXX, close to the L3 misses with MB-Gen. If the test's L3 miss rate is in-between, we interpolate the two slowdowns based on the L3 misses, assuming congestion in both resources. 
% Finally, we determine the Rprivate and Rshared based on the expected slowdown from its performance table. Calculating Rprivate and Rshared takes the same steps. The final discount price is computed using the equation with the computed rates. 

% Figure~\ref{fig:interpolation} shows how we employ the L3 misses when estimating the slowdown. The two traffic generators make the upper and lower boundary of the L3 misses. If a Litmus test reports the L3 miss count is 10, close to the L3 misses with CT-Gen, \textcircled{1}Litmus pricing estimates the discount (=expected slowdown) of the function to be near 1\%. This indicates that the congestion happens before the L3, as what CT-Gen creates. On the contrary, in case the L3 misses are 1000, close to the L3 misses with MB-Gen, \textcircled{2}Litmus pricing estimates the function's discount rate close to 6\%. Meanwhile, if the Litmus test reports the L3 misses as 100, we interpolate the two extreme discounts, 1 and 6, based on the L3 misses, assuming current congestion to stand in between the two extreme congestions. The congestion model in the figure shows how we interpolate with logarithmic interpolation. In this figure, \textcircled{3}applying the logarithmic interpolation to the L3 miss count returns the half-point between CT-Gen's 1\% and MB-Gen's 6\%, which is 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 
Figure~\ref{fig:interpolation} shows our approach to using L3 misses to estimate slowdowns. We created two figures illustrating separate regression models. The left figure (a) is derived from the startup slowdowns and L3 misses with logarithmic regression, indicating L3 misses at specific congestion levels. The right figure (b) is derived from the performance table with linear regression, displaying discounts at specific congestion levels. Each figure depicts two regression lines associated with different traffic generators.

The two traffic generators set the upper and lower boundaries for L3 misses. For instance, if a Litmus test reports 10 L3 misses, close to what CT-Gen generates: \textcircled{1}This suggests congestion occurs before reaching the L3 cache, similar to CT-Gen's scenario. Thus, Litmus pricing estimates the function's discount to be around 1\%. Conversely, if the Litmus test reports 1000 L3 misses, close to MB-Gen's results: \textcircled{2}Litmus pricing estimates the function's discount rate to be approximately 6\%, indicating congestion similar to MB-Gen, where memory bandwidth is heavily consumed and L3 cache blocks are frequently evicted. When the Litmus test reports 100 L3 misses, an interpolation between these extremes is applied: \textcircled{3}Using logarithmic interpolation, Litmus pricing estimates the function's discount rate to be midway between CT-Gen's 1\% and MB-Gen's 6\%, resulting in approximately 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 



==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/08_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \textbf{Litmus price \& error:}
% We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, and the other consists of selected reference applications to obtain the linear regression models for Litmus pricing. The discount models plug into the Litmus pricing used in our tests. For this experiment, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown.
We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, while the other consists of chosen reference applications to derive linear regression models for Litmus pricing. The discount models plug into the Litmus pricing employed in the tests. In this study, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown. 

% % original version
% We maintain the congestion state consistent across all tests, co-running each function with 26 other functions. Using Perf~\cite{perfWiki}, we collect the three key stats: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup, which implies the congestion level in these tests, as well as the discount rates that every function receives. We execute every function 100 times and collect the average of the function's \(T_{private}\) and \(T_{shared}\). Finally, we compute each function's \(P_{private}\), \(P_{shared}\), and \(P\), the total price, by summing \(P_{private}\) and \(P_{shared}\).  

\subsection{One Function Per Core}

% revision version
% We maintain consistent congestion states across all tests by co-running each function with 26 other functions. Using Perf, we collect the three key statistics: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup. These metrics hint at the congestion level during the tests as well as the discount rates that a function receives. Each function is executed 30 times, and the average of its \(T_{private}\) and \(T_{shared}\) is collected. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).
We maintain consistent congestion levels across all tests by co-running each function with 26 other functions. As outlined in Section~\ref{sec:motivation}, whenever a function finishes, another is randomly launched to keep a total of 26 co-running functions. Using Perf~\cite{perfWiki}, we collect three key statistics: \(T_{private}\), \(T_{shared}\), and the machine's L3 misses during the first 45 million instructions of the Python startup. Through these metrics, Litmus pricing estimates the level of system congestion and the discount rates a function receives. Each function is executed 30 times, and we average its \(T_{private}\) and \(T_{shared}\) values. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice26Rev}\\
% \caption{The total price for functions computed via Litmus pricing and ideal prices when co-running with 26 other functions normalized to the commercial price that offers no discount}
\caption{Prices computed via Litmus pricing and ideal prices when co-running with 26 other functions, normalized to the commercial price that offers no discount}
\label{fig:normalizedPrice26Rev}
\end{figure}

% In Figure~\ref{fig:normalizedPrice26}, we can see a minimal difference in the discount rate between the Litmus price and the Ideal price. The average Litmus discount rate stands at 11.5\%, which is only marginally larger by 0.6\% than the average Ideal discount rate of 10.9\%. Also, we can see that the difference between the Litmus price and Ideal price are different among the applications. Certain applications exhibit higher Litmus prices compared to the Ideal price, while conversely, some applications demonstrate smaller Litmus prices. 
 %Figure~\ref{fig:priceErrorRunwith26} shows further details, analyzing the errors in each pricing component. 

% Figure~\ref{fig:normalizedPrice26Rev} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{10.66\%}, which is only marginally larger by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{10.28\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice26Rev} illustrates estimated prices derived from Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices to offset delays in a congested execution environment. The figure shows minimal disparities between the two prices, implying that Litmus pricing offers a reasonable discount. The average discount from Litmus pricing across all functions is 10.7\%, which is only marginally higher by 0.4\% compared to the average slowdown experienced by functions, which stands at 10.3\%, as depicted by the ideal price.

% However, the discount rates per slowdown differ among functions. For instance, float-py's ideal discount rate is \hl{0.05\%}, but it enjoys a \hl{4.31\%} discount with the Litmus pricing. Meanwhile, pager-py's performance drops by \hl{15.63\%} while receiving a \hl{13.87\%} discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more easily affected than the reference when congested. In contrast, float-py runs mostly with private resources, receiving a minor impact from the execution environment. Figure~\ref{fig:priceErrorRunwith26Rev} shows further details, analyzing the differences in each pricing component.
However, the discounts per slowdown differ among functions. For instance, float-py's ideal discount rate is 0.05\%, but it benefits from a 4.3\% discount with Litmus pricing. Conversely, pager-py encounters a 15.6\% performance decline while receiving only a 13.9\% discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more susceptible to congestion than the references. In contrast, float-py predominantly utilizes private resources, resulting in minimal impact from the execution environment. Further insights into these variations in each pricing component are presented in Figure~\ref{fig:priceErrorRunwith26Rev}.


% From figure~\ref{fig:tcore\(T_{private}\)Distr}, we know that \(T_{private}\) dominates the execution time among all applications. The impact from \(T_{private}\) error has a bigger impact on the overall error. The slowdowns due to congestion in private resources are small. Theoretically, there should be no slowdowns when using private resources, but we observed that the congestion still influences it. The observed slowdown is 000, a small difference from an ideal slowdown. Meanwhile, the slowdowns in shared resources are significant. We observe that 

% % \[  Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}}\]

% \[Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{TotalIdealPrice}\]
% \[TotalIdealPrice = R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}\]

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/priceErrorRunwith26Rev}\\
\caption{Weighted errors in prices derived from Litmus pricing, which are compared to ideal prices}
% \vspace{-1em}
\label{fig:priceErrorRunwith26Rev}
\end{figure}

%%% We discuss error
% In figure~\ref{fig:priceErrorRunwith26} we can see that there are some applications receive positive errors and some receive negative errors.  A negative error indicates that our estimated slowdown for that application is higher than its actual slowdown, resulting in greater compensation than the observed performance losses. On the other hand, a positive error indicates that the compensation is smaller than its real slowdown. For most applications, the Litmus price is slightly higher than the Ideal price, with minimal differences. The highest price error is 0.0389 for auth-nj, while the lowest error is 0.007 for dyn-py. The geometric mean of the absolute error is 0.018. 
% Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors that each function experiences. The error rate is computed as the difference between the estimated and the ideal prices over the ideal price. The first two bars show the errors in \(P_{private}\) and \(P_{shared}\), which are weighted by their corresponding ratio in the execution time, considering their impacts, as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. The functions can have two different errors: positive and negative. A positive error indicates that the Litmus-estimated price is higher than its ideal price, implying that it receives smaller compensation than its performance losses. In other words, Litmus pricing estimates its slowdown to be less than its actual slowdown. A negative error implies the opposite; a function's compensation is higher than its slowdown. This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others. Meanwhile, the tenants need to acknowledge the consequences if their functions differ vastly from the reference workloads, heavily relying on shared memory.
Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors each function experiences. The error rate is computed by comparing the estimated prices with the ideal prices and dividing the difference by the ideal prices. The first two bars show errors in \(P_{private}\) and \(P_{shared}\), weighted by their corresponding ratios in execution time, reflecting their impacts as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. Functions may have two types of errors: positive and negative. A positive error means that the estimated price exceeds its ideal price, implying that the compensation received is less than the performance loss incurred. In other words, Litmus pricing underestimates the slowdown relative to the actual slowdown. Conversely, a negative error indicates the opposite; a function's compensation exceeds its slowdown. This discrepancy indicates Litmus pricing may offer varying advantages to different functions, favoring those with lesser slowdowns. Meanwhile, tenants must recognize the consequences if their functions differ vastly from the references, particularly those heavily reliant on shared resources.

% Delete the followings
% This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.

% The largest absolute error is \hl{0.0723} for rate-go, while the smallest absolute error is \hl{0.0039} for \hl{mst-py}. Overall, the Litmus pricing shows minor errors with an average of \hl{0.0231}. With further details, the Litmus pricing accurately estimates the slowdowns in \(P_{private}\) with \hl{0.0175} of an average weighted error rate. \(P_{private}\)'s highest weighted error rate is \hl{0.079}, yet minor, while the lowest rate is only \hl{0.0008}. The weighted error rate for the estimated \(P_{shared}\) is also small. The average error rate for \(P_{shared}\) is \hl{0.0068}, even lower than for \(P_{private}\). \(P_{shared}\)'s highest error rate is \hl{0.0404}.
% The largest absolute error is 0.072, which occurs with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, the Litmus pricing exhibits minor errors, averaging 0.023, \hl{with the estimated discount differing by 22.5\% over the ideal discount.} With more details, Litmus pricing accurately estimates slowdowns in \(P_{private}\), with an average weighted error rate of 0.018. \(P_{private}\)'s highest weighted error rate is 0.08, yet minor, while the lowest rate is only 0.0008. The weighted error rate for estimated \(P_{shared}\) is similarly small, averaging at 0.0068, even lower than for \(P_{private}\). The highest error rate for \(P_{shared}\) stands at 0.04.
The largest absolute error is 0.072, occurring with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, Litmus pricing exhibits minor errors, averaging 0.023. Thus, the estimated discount deviates by 22.5\% from the ideal discount. Note that Litmus pricing aims to match the average discount across all functions by applying a system-wide discount based on the system's congestion level rather than adjusting the discount for each function individually. Consequently, individual functions may experience either positive or negative errors. However, it is noteworthy that the average discount between Litmus and ideal pricing differs by just 0.4\%, as illustrated in Figure~\ref{fig:normalizedPrice26Rev}, satisfying its objectives.
% This policy may incentivize some functions while penalizing others based on shared resource usage. 
Specifically, Litmus pricing estimates slowdowns in \(P_{private}\) with an average weighted error rate of 0.018. The highest for \(P_{private}\) is 0.079, while the lowest is just 0.001. For \(P_{shared}\), the average weighted error rate is even lower, at 0.007. The highest for \(P_{shared}\) is 0.040.


% Litmus employs the average performance of applications to determine the discount rate applied universally. In this context, an application encounters a positive error when its speedup is less than the estimated average speedup across all applications. Also, the error rate depends on the difference between the actual speedup and the estimated average speedup, with larger differences resulting in more significant errors for the given application.
% As discussed in Figure~\ref{fig:TpriTshardDistri}, \(T_{private}\) dominates the execution time across all applications, implying that a small error in the estimated \(T_{private}\) largely influences the execution time. This explains why, for functions that demand little shared resources, such as float-py and chame-py, the error in P is almost identical to that in \(T_{private}\), and errors with \(T_{shared}\) can be overlooked. In contrast, for functions with a larger \(T_{shared}\) ratio, such as pager-py and mst-py, errors in \(T_{shared}\) meaningfully affect the total execution time. Note that the Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price.  

Litmus pricing estimates each pricing component separately with an individual discount rate. For functions that demand minimal shared resources, such as float-py, the errors in P are nearly identical to those in \(T_{private}\), and the errors in \(T_{shared}\) can be overlooked. As shown in Figure~\ref{fig:TpriTshardDistriRev}, \(T_{private}\) dominates the execution time across many applications. While even a small error in the estimated \(T_{private}\) influences the function's execution time, substantial errors in \(T_{shared}\) likely have limited impacts, except for functions that have a relatively meaningful \(T_{shared}\) ratio, such as pager-py and mst-py, whose errors in \(T_{shared}\) are observable in the total price. 

% We emphasize that Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price. We observe that functions have similar slowdowns in \(T_{private}\) with slight variation when congested. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, also estimating reliable total prices since \(T_{private}\) mostly dominates the execution time. The \(T_{shared}\) fluctuates more dynamically across functions with a relatively large error, but the error's impact is little, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}. 
We emphasize that Litmus pricing cannot avoid producing a certain degree of error since it relies on estimation using a few metrics. However, the figure proves that Litmus pricing effectively captures a congested environment and reflects that environment in the price. Under the same congestion level, \(T_{private}\) values of all functions are delayed similarly with a little variation. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, leading to reliable total price estimates since \(T_{private}\) generally dominates execution time. \(T_{shared}\) fluctuates more dynamically across functions and has a relatively larger error, but the impact of this error is minimal, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}.

\begin{figure}[h]
\centering
% \vspace{-5em}
 \includegraphics[width=1\columnwidth]{./fig/normTprivtTshared26Rev}\\
% \vspace{-5.5em}
\caption{\(T_{private}\) \& \(T_{shared}\) of applications when co-running with 26 others, normalized to those when they run alone. The top(black) and bottom(blue) lines are discount rates from Litmus pricing for \(T_{private}\) and \(T_{shared}\)}
% \vspace{-1em}
\label{fig:normTprivtTshared26Rev}
\end{figure}

% To further investigate the price error differences, in igure~\ref{fig:normTprivtTshared}, we explore the \(T_{private}\) speedups across various serverless applications.  
% Notably, the difference between the Litmus discount (L-Discount) and the average speedup is merely 0.006.  This minute difference explains why Litmus can attains such high accuracy. 
%Furthermore, when comparing with figure~\ref{fig:priceErrorRunwith26}, a correlation between the error rate and the speedup differences becomes apparent. 
%For instance, float-py, with the most substantial difference above the Litmus discount, also experiences the most significant negative error rate. 
%Conversely, aes-go, with the smallest speedup, experiences the highest positive error rate.
% % original version
% Figure~\ref{fig:normTprivtTshared} shows the execution time of the baseline normalized to the execution time of each run under congestion. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the functions spend only 3.67\% more time on private resources, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, resulting in precise estimation with a Litmus test. 

% Figure~\ref{fig:normTprivtTshared26Rev} shows the execution time of each function run under congestion normalized to the execution time of the baseline. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the interferences in private resources extend the function execution time only by 5.3\%, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, enabling precise estimation with a Litmus test.
Figure~\ref{fig:normTprivtTshared26Rev} shows the \(T_{private}\) and \(T_{shared}\) of each function, normalized to the same time components of the baseline. The gap between the bar and 1 represents the amount of slowdown that should be translated into ideal discounts. The top (black) and bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that interferences in private resources extend the function execution time by only 5.3\%, implying the performance of the private resources is marginally affected by congestion. Additionally, all functions exhibit similar \(T_{private}\) values with little dispersion, helping precise estimation with Litmus tests.

% Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors are still in an acceptable range since their impacts are small. Functions that have a considerable \(T_{shared}\) ratio become more sensitive to system congestion. Instead, a function, such as float-py, with negligible \(T_{shared}\) ratio gains huge benefits with high discounts while its performance remains firm. This shows that Litmus pricing reflects the dynamically changing values of shared resources when the congestion level alters and encourages functions to be developed to use more private resources. 
Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors remain within an acceptable range as their impacts are minor. Functions that have a considerable \(T_{shared}\) ratio are more sensitive to system congestion. Conversely, a function like float-py, which has a negligible \(T_{shared}\) ratio, gains huge benefits from high discounts while maintaining stable performance under congestion. This shows that Litmus pricing accurately reflects the dynamic values of shared resources when the congestion level changes and incentivizes functions to be developed to use less shared resources. 

% \textbf{Litmus pricing under high congestion:} We test our Litmus pricing under a heavily congested environment to verify its pricing of functions with large slowdowns. To create a crowded environment, we concurrently execute 60 instances of Fibonacci-go, which produces the most L2 misses among our tested functions. 
% We raise the congestion level significantly with 60 co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo} shows the results from the same tests of Figure 11. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.8\%, which is only a 1.7\% difference from the ideal discount of 27.1\% with 2.48\% of an average absolute error. In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.151 and 4.299, which are only 2.45\% and 7.83\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. 
% \textbf{Litmus pricing under high congestion:} We raise the congestion level significantly with \hl{500} co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo500} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.1\%, which is only a 1\% difference from the ideal discount of 27.1\% with 0.088\% of an average absolute error. Litmus pricing discounts slightly more than an actual slowdown, leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% % \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
% \caption{The normalized total price for the applications calculated by using Litmus pricing and ideal prices when co-running with 500 Fibonacci-go}
% \label{fig:normalizedPriceCongested320}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\columnwidth]{./fig/diffStartupPortion-2Rev}\\
%\caption{The slowdown of Python's startup with 25 and 15 million instructions (X-axis) and the slowdown of reference applications (Y-axis). From left, \(T_{private}\), \(T_{shared}\), and \(T_{total}\), normalized to those when running alone}
%\label{fig:diffStartupPortion}
%\end{figure}

% \textbf{Instructions in Startup:} Litmus tests react differently to congestion when performed with different numbers of instructions from the startup phase. For example, Python's startup involves about 45 million instructions. While we have conducted Litmus tests using all these instructions, Figure~\ref{fig:diffStartupPortion} shows the response of these tests when running with the first 15 and 25 million instructions from this set. The figure shows the startups' \(T_{private}\), \(T_{shared}\), and \(T_{total}\) with two traffic generators, as depicted in Figure~\ref{fig:referenceStartupSlowdownRev}. Tests with fewer instructions are more sensitive to cold cache misses but less to interference in the L3 cache. Therefore, as the instruction count in Litmus tests decreases, they become less susceptible to conflicts in shared resources, especially from traffic by MB-Gen. As a result, tests with 25 million instructions exhibit reduced slowdowns. This trend becomes more apparent when running the tests with 15 million instructions, depicting that slowdowns when co-running with MB-Gen become nearly identical to those with CT-Gen. 

%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%







% \textbf{Instructions in Startup:} Python's whole startup phase contains about 45 million instructions. We can further divide the startup phase into smaller pieces with 10 million instructions code chunks. And each code chunk would have its characteristics. They react differently in the same congested environment. In section XXX we use the whole Python's startup portion's slowdown to indexsing the serverless application's slowdown. But, since the co-relationship between these two slowdown in different congestion source are different, one startup \(T_{private}\) slowdown may indicate two application's slowdown. By carefully picking the code chunks we can mitigate the difference between the two normalized slowdowns of the guidance application that correlated to the same startup phase slowdown. 

% Figure~\ref{fig:diffStartupPortion} depicts the correlation between the performance changes in the reference applications and distinct segments of Python's startup phase. From the figure, we see that selecting the first 15 million instructions as our startup phase results in the normalized \(T_{uncore}PerInst\) of the guidance application aligning nearly into a singular trendline. However, there are substantial gaps in the case of \(T_{core}PerInst\) with this code segment. Thus, we should pick xxx-xxx as our startup phase representation code for the normalized \(T_{core}PerInst\). We think that this can be used to mitigate the differences. But, we should be careful to use the small code chunks for the following reasons: First, only measuring the small portion can be a problem. The results might be too dynamic. Second, since we only measure this small portion there might be a huge execution period that cannot be covered.

% Continue to work from here

\subsection{Temporal CPU Sharing}
\label{sec:temporalCPUSharing}

The previous evaluation assumes an isolated environment where a CPU is assigned exclusively to an active function during execution, disallowing temporal sharing between functions through context-switching. While this setup ensures strict performance isolation, it inherently limits resource utilization. Conversely, enhancing utilization by permitting temporal CPU sharing among functions complicates price estimation. We explore how Litmus pricing can be applied in a less restrictive environment that permits sharing, where functions can temporarily share the same CPU and are not bound exclusively to specific cores. 

In this section, we deploy a testing function to co-run with 160 other functions across 16 cores without exclusive core assignments, assuming an average of 10 functions share a core. The reduction in the number of cores tested was necessitated by our system's memory limitations, as certain functions require significant memory space.

% \textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, the subsequent function clears the displaced one's cached data. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, the slowdown with extra sharing financially benefits the provider; we thereby argue that the extent of sharing should be factored into Litmus pricing as another discount factor.
\textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, a subsequent function evicts the cached data of the displaced one. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, delayed execution due to extra sharing financially benefits the providers. Thus, we argue that the extent of temporal sharing should be incorporated into Litmus pricing as another discount factor.

Figure~\ref{fig:csImpactor} depicts the switching overheads as concurrently running functions increase. The figure demonstrates that the sharing overhead follows a logarithmic growth pattern and stabilizes at around 20 co-running functions. Furthermore, we discovered that the switching overheads predominantly affect \(T_{private}\). Consequently, Litmus pricing needs to calibrate \(T_{private}\) to account for the impacts of sharing before estimating the slowdown using the performance table.

Figure~\ref{fig:normalizedPrice160Method1} illustrates the discounted price reflecting this adjustment. In our configuration, with an average of 10 functions per core, we divide \(T_{private}\) by 1.025 before estimating the slowdown. In this figure, Litmus pricing estimates an average discount of 14.5\%, which falls 2.9\% short of the ideal discount of 17.4\%. While most benchmarks receive discounts lower than ideal, aes-py stands out with the largest error of 9.9\%, which is 6.9\% less than its ideal discount of 16.8\%.

\begin{figure}
\centering
% \includegraphics[width=1\columnwidth]{./fig/csImpactor}\\
\includegraphics[width=1\columnwidth]{./fig/csImpactor2}\\
\caption{\(T_{private}\) of functions over different co-running counts in the same core, normalized to when running alone}
% \vspace{-1em}
\label{fig:csImpactor}
\end{figure}

\begin{figure}
\centering
% \vspace{-1.2em}
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160Method1}\\
\caption{Prices derived from Litmus pricing (Method 1) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
% \vspace{-0.5em}
\label{fig:normalizedPrice160Method1}
\end{figure}

% In Figure~\ref{fig:normalizedPrice160Method1} we use the the same congestion and performance tables that we collected in the restricted environment. When checking the tables instead of using the original startup slowdown of tcore we use an adjusted slowdown by dividing the context switch impact factor. From figure~\ref{fig:normalizedPrice160Method1} we can see that the average Litums discount is 14.65\%, 3.01\% less than what they should receive compared to the ideal discount of 17.67\%. Most applications receive a smaller discount than the ideal price. The largest error is on aes-py with Litmus discount of 9.85\%, 6.87\% smaller than the ideal discount of 16.72\%. The smallest error is on dyn-py. It's Litmus discount is 22.45\%, only 0.47\% larger than the ideal discount of 21.97\%.

\textbf{Method 2, Updating Performance Tables:} Rather than reusing the performance/congestion tables designed for restrictive environments, arranging new tables for the sharing-enabled environments returns better accuracy. Although the notion of preparing separate tables for various sharing levels may seem challenging, we argue that only one or a few extra tables for heavily crowded systems would suffice, given that commercial systems are typically heavily crowded. Again, we emphasize that the impact of function co-placement stabilizes above a certain co-placement count, as shown in Figure~\ref{fig:csImpactor}.

For this test, we prepared new performance/congestion tables for the environment described above, where a testing function is assumed to co-locate and compete for a core with 9 other functions. Moreover, considering the scenario where a switched-out function has a low chance of being rescheduled to the same core, instead of assigning 10 functions to a specific core, we ran 50 functions across 5 dedicated cores; each can run on any of the 5 cores. We managed the congestion levels in shared resources using traffic generators on the other cores, as outlined in Section~\ref{sec:designDetails}.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPrice160}
% \vspace{-0.6em}
\end{figure}

% Figure~\ref{fig:normalizedPrice160} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{17.29\%}, which is only marginally smaller by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{17.67\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice160} shows the prices obtained from Litmus pricing with the new tables, which are normalized to those from commercial sources. Once more, as in Figure~\ref{fig:normalizedPrice26Rev}, the figure reveals marginal distinctions between the two price points, suggesting that Litmus pricing continues to offer a reasonable discount. Across all functions, the average discount provided by Litmus pricing stands at 17.2\%, merely 0.2\% less than the ideal discount of 17.4\%.


==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/09_sensitivity.tex <==
\section{Sensitivity}
\label{sec:sensitivity}

While the aforementioned tests highlight Litmus's potential, we recognize the need for more compelling results. This section expands our analysis and examines Litmus pricing from various angles across diverse system environments.

% \textbf{Heavy Congestions:} We raise the congestion level significantly with 320 co-running applications to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. The Litmus pricing is still close to the ideal price, discounting the price by 20.00\%, which is only a 1.46\% difference from the ideal discount of 21.46\%. The highest Litmus discount is 26.01\% for dyn-py. It has an error of 2.83\% compared with the ideal discount.
\textbf{Heavy Congestion:} We significantly escalate the congestion level to verify Litmus pricing under conditions of substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} presents the outcomes of the same tests depicted in Figure~\ref{fig:normalizedPrice160} but with 320 co-running functions. Not only did we increase the function count, but we also specifically selected 8 memory-intensive functions, aes-py, compre-py, thum-py, bfs-py, auth-py, fib-go, geo-go, and profile-go, that produce the most L2 cache misses among the tested functions to create heavy congestion in shared resources deliberately. Even under such intensified congestion, Litmus pricing produces results remarkably close to the ideal price, discounting the price by 20.0\%, which deviates by merely 1.5\% from the ideal discount of 21.5\%. The highest discount by Litmus pricing is 26.0\% for dyn-py, a minor error of 2.8\% compared to the ideal discount.


% leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 320 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPriceCongested320}
% \vspace{-1em}
\end{figure}

\textbf{CPU Frequency:} Modern CPUs feature dynamic CPU frequency adjustments, which are controlled via software or hardware. A hardware technique like Intel Turbo Technology autonomously adjusts the CPU frequency based on the CPU's power and thermal budgets, allowing the CPU to operate at higher frequencies when conditions permit and lower frequencies under heavy load. Prior tests assumed that the frequencies were fixed and strictly managed by service providers who had knowledge of when and to what extent frequency adjustments were necessary. Also, we evaluated Litmus pricing under the other scenarios where CPU frequencies were not fixed, providing more dynamic perspectives.

% Figure~\ref{fig:normalizedPrice160unset} illustrates the prices from the Litmus pricing and the ideal price, which are normalized to commercial prices. We tested it under the configuration in Section 7.2 with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, the Litmus pricing's discount is lowered from 17.16\% to 16.84\%, while the ideal discount rate is decreased from 17.42\% to 17.31\%. Still, the discount rate difference from the ideal price is only 0.47\% without setting the CPU frequency. We observed that the CPU frequency changes rarely when the system runs with 160 functions. Overall, the varying frequency made a minor impact on performance as well as the pricing scheme. 
Figure~\ref{fig:normalizedPrice160unset} illustrates the prices derived from Litmus pricing alongside the ideal prices, both normalized to commercial prices. This evaluation was conducted under the configuration outlined in Section~\ref{sec:temporalCPUSharing} with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, we observe a slight decrease in Litmus pricing's discount, from 17.2\% to 16.8\%, while the ideal discount rate decreases from 17.4\% to 17.3\%. Still, even without fixed CPU frequencies, the difference in the discount rate from the ideal price is only 0.5\%. We noted that CPU frequency changes were infrequent when the system operated with 160 functions. Overall, the variation in frequency had a negligible impact on Litmus pricing.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160unset}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others with unfixed CPU frequencies, both normalized to commercial prices}
\label{fig:normalizedPrice160unset}
% \vspace{-1em}
\end{figure}

% All the above experiments are done on Intel Xeon Gold 5218(Cascade Lake). We also perform our scheme on another CPU architecture, Intel Xeon Silver 4314(Ice Lake-SP). 
\textbf{CPU Architecture:} Ensuring the validity of Litmus pricing across different architectures is crucial. Our Litmus tests rely on the performance counter that measures a stall count due to L2 cache misses (cycle\_activity.stalls\_L2\_miss)~\cite{perfMonEvents}, supported by Intel's CPUs. Unfortunately, other vendors like AMD do not yet offer the same performance counter~\cite{amdPMC}, restricting our tests to Intel CPUs. Alternatively, we conducted tests on another Intel CPU based on the Ice Lake architecture, Xeon Silver 4314, to broaden the scope of our analysis.

\begin{figure}[b]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun70kiwi}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 70 others on Xeon Silver 4314, both normalized to commercial prices}
\label{fig:normalizedPriceCorun70kiwi}
\end{figure}

% Because of the limitation of our memory size, we test Limtmus with 70 co-running applications. In this test, we use method 2 introduced in section~\ref{sec:temporalCPUSharing}. We first conduct the congestion and performance tables with 50 applications running in the first 5 cores. Then for the evaluation, we run 70 applications in the first 7 cores to let our testing application compete with 9 other applications for a core.  Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus discounting the tenant only pays 82.52\% commercial price. It's 0.696\% less than with the ideal discount.
Once again, this evaluation was conducted following the configuration outlined in Section~\ref{sec:temporalCPUSharing}, albeit with 70 co-running functions, limited by the main memory capacity of 128GB. Following Method 2, we constructed new congestion and performance tables with 50 functions running across 5 cores. Then, we ran 70 functions across 7 cores to match the competition count, averaging 10 functions per core. Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus pricing, the tenant only pays 82.5\% of the commercial prices, which is merely 0.7\% less than the ideal price.

% \textbf{Per-core Function Count:} When altering the co-located applications in each core the performance of the application can also be influenced. In this test, we put 240 applications in the first 16 cores. The testing application is competing with 14 other applications. We used the same congestion and performance tables from section~\ref{sec:temporalCPUSharing} method 2. Figure~\ref{fig:normalizedPriceCorun15} presents the results. The error of Litmus pricing is 1.23\% with The average discount of 16.69\%. The ideal discount is 17.92\%. The mean price of Litmus is larger than the ideal price because we are using the tables that are made based on 10 applications per-core. The context-switching overhead is larger. But, from figure~\ref{fig:csImpactor} we know that there is a diminishing impact of per-core application count. The error of the Litmus pricing is still under control when we increase the per-core application count.
\textbf{CPU Sharing Overhead:} The co-located function count determines the level of interference, impacting a function's performance differently. To assess Litmus pricing under various co-running function counts, we increased the function count to 240 from the configuration outlined in Section~\ref{sec:temporalCPUSharing}, making an average of 15 functions running on each core. However, we reused the performance and congestion tables generated in Section~\ref{sec:temporalCPUSharing}. Figure~\ref{fig:normalizedPriceCorun15} illustrates the results, where the Litmus pricing's error is 1.2\% with an average discount of 16.7\%, compared to the ideal of 17.9\%. Despite reusing the tables constructed for 10 co-running functions per core, the error remains negligible. This outcome aligns with Figure~\ref{fig:csImpactor}, which highlights the diminishing impact of temporal sharing when running more than 10 co-running functions. Given the perpetual overcrowding of commercial systems, any configuration gap between the environment where constructing the tables and where conducting tests is expected to remain minor and easily manageable.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun15}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 15 functions per core and reusing tables, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun15}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun160smt}
\end{figure}

\textbf{Simultaneous Multithreading (SMT):} SMT is a technique aimed at maximizing resource utilization by enabling multiple threads to execute concurrently on the same core, extending the shared resource domain across the entire processor. However, while SMT enhances resource utilization, it significantly complicates the measurement of interference impact. Moreover, SMT introduces additional side channels, thereby increasing the processor's vulnerability to security attacks. Due to these concerns, serverless platforms like Amazon Lambda disable SMT in their systems~\cite{schall2023warming,agache2020firecracker,schall2022lukewarm}. Nonetheless, we have conducted a study to assess the impact of SMT on our Litmus pricing methodology.

% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
% \caption{Prices computed via Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, normalized to the commercial prices}
% \vspace{-0.5em}
% \label{fig:normalizedPriceCorun160smt}
% \end{figure}

% To generate the performance/congestion tables, we executed 50 applications across 5 dedicated physical cores. In this way, the testing function is co-located with 9 other applications in the same virtual core and 19 other applications in the same physical core. Fiugre~\ref{fig:normalizedPriceCorun160smt} illustrates the results. The first thing we notice is that the normalized price is much smaller compared with the setups without SMT turned on. The average discount of Litmus is 45.42\% which is 1.9\% smaller than the average ideal discount of 47.32\%.
To construct the performance and congestion tables, we executed 50 applications across 5 physically separated cores, allowing an average of 10 functions to share two virtual cores. Figure~\ref{fig:normalizedPriceCorun160smt} illustrates the results,  presenting prices derived from Litmus pricing and ideal prices, both normalized to commercial prices without discounts. The normalized price experiences a significant drop compared to other configurations, highlighting the impact of heavy congestion within a physical core. The ideal price, which assumes no interference, stands at 47.3\% of the commercial price. Meanwhile, Litmus pricing offers a discount of 45.4\%, which is only 1.9\% less, confirming the effectiveness of Litmus pricing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Node JS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Nodejs Startup:}NodeJs is another well-adopted language in serverless platforms besides Python. It's one of the earliest languages to be supported by AWS Lambda ~\cite{serverless1}. From Section~\ref{sec:designDetails} we see that NodeJs has a long startup phase which makes it a great candidate when we need to pick a language startup phase for the Litmus test. 

%\begin{figure}[h]
%\centering
%\vspace{-0.5em}
%\includegraphics[width=1\columnwidth]{./fig/njReferenceStartupSlowdown}\\
%\vspace{-1em}
%\caption{The correlation between the normalized NodeJs's startup phase and the normalized reference applications.}
%\vspace{-0.5em}
%\label{fig:njReferenceStartupSlowdown}
%\end{figure}

%Figure~\ref{fig:njReferenceStartupSlowdown} shows the correlation between NodeJs startup phases and reference applications. After applying the Litmus test with NodeJs applications, with this figure, we can use the slowdown of the NodeJs startup phase to find the corresponding system congestion level and the discount rate for both private and shared resources. NodeJs has a longer startup phase compared with Python. It gives us more room when picking the most suitable portions of the startup phase. We can choose the language to be used for the Litmus test based on the density of the startup phase. 


==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/10_related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Serverless:} Many works address the performance bottleneck of serverless execution~\cite{du2020catalyzer}~\cite{agarwal2021reinforcement}~\cite{roy2022icebreaker}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Schall et al.~\cite{schall2022lukewarm} record and reload the instructions to reduce the front-end stalls when reaccessing the same application. Jovan et al.~\cite{stojkovic2023specfaas} focus on the performance of an application chain. They break the execution flow and speculative execute the functions. However, we are focusing on the price which is one of the most important potions of the cloud ecosystem.

% For the cloud providers, accommodating more tenants in a machine is a key strategy, gaining higher profits by maximizing the utilization of their machines. However, the approach inevitably introduces interference between tenants, slowing down applications unpredictably. Thus, prior researchers solved this challenge by allowing the tenants more non-biased, predictable, quality services~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed a clustering-based cache partitioning to remove unfairness between tenants. Rohan et al.~\cite{roy2021satori} simultaneously control multiple architectural resources to aim for both fairness and throughput. However, offering fairness inevitably sacrifices resource utilization. Thus, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} solve the unfairness uniquely by adjusting their prices while leaving the unfairness at a certain degree. This paper follows this direction but explores a more practical solution in serverless computing. 

Cloud providers strive to maximize profits by accommodating more tenants on their machines, which inevitably introduces interference between tenants, leading to unpredictable application slowdowns. To address this challenge, prior researchers have focused on providing tenants with a more unbiased and predictable quality of service~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed clustering-based cache partitioning to mitigate unfairness between tenants. Rohan et al.~\cite{roy2021satori} aimed for both fairness and throughput by simultaneously controlling multiple architectural resources. However, achieving fairness comes at the cost of sacrificing resource utilization. In contrast, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} addressed the unfairness by adjusting their prices while accepting a certain degree of unfairness. Our study follows a similar direction but explores a more practical solution within the context of serverless computing.

% delete the following section: the approaches are against our scheme. 
% \textbf{Serverless Computing:} Many studies focus on reducing the latencies of serverless applications~\cite{cadden2020seuss,oakes2018sock,wang2019replayable,jia2021boki}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Ustiugov et al.~\cite{ustiugov2021benchmarking} record and prefetches the functions’ stable working set of guest memory pages to further reduce the function's startup time. Wei et al.~\cite{wei2023no} remote forking the serverless functions to reduce the cold start latency while limiting the resource usage. Schall et al. record and reload the instructions~\cite{schall2022lukewarm} or the BTB entries ~\cite{schall2023warming} to reduce the front-end stalls when reaccessing the same application. 
% \hl{Litmus is orthogonal to these approaches and can be adopted together.}

==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Serverless computing is a key technology in present cloud computing, offering numerous advantages. One primary advantage is its effective cost-saving, as tenants only pay for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion. While tenants suffer slowdowns, they also have to pay more for the slowdowns. Unlike prior approaches that aim to maintain quality of service, this paper discounts the tenant's cost to compensate for the loss. Litmus pricing proposed in this work monitors the machine states and adjusts the tenants' costs. The congestion level can be frequently gauged before every function using the proposed Litmus test, an effectively lightweight testing approach. Our tests show that Litmus offers near-ideal prices with a 0.38\% difference, compared to the ideal price that discounts proportional to its slowdown. 
Serverless computing is a key technology in contemporary cloud computing, offering a range of benefits. One primary advantage is effective cost-saving, as tenants are billed only for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion, which not only results in slowdowns but also higher costs for tenants. Rather than aiming to maintain service quality, this paper suggests discounting tenants' costs to compensate for performance losses. Litmus pricing proposed in this work monitors machine states through Litmus tests and adjusts tenant costs accordingly. The Litmus test is a lightweight testing approach for serverless platforms, which assesses the machine's congestion level before starting a user's function. Our tests prove that Litmus pricing offers nearly ideal prices in heavily congested environments, with an average deviation of just 0.2\% from the ideal price that adjusts discounts in proportion to the slowdown experienced.


==> ktntkvbtdcvxdrhfnzxnvhhqdfcjxtnr/12_ack.tex <==
\section{Acknowledgment}
\label{ack}

We would like to thank our reviewers for their valuable feedback to improve this paper. This work was supported by NSF CAREER Award CCF-2146475.


==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/00_abstract.tex <==
\begin{abstract}

% Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While the providers can utilize their machines more efficiently, the tenants only need to pay for the resources they consume. However, a serverless system co-runs thousands of short-living functions concurrently to maximize resource utilization, bearing frequent state shifts. Meanwhile, when the system gets too congested, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants are also charged higher costs when experiencing slowdowns since all commercial serverless platforms determine the tenants' costs proportional to their execution times.
Serverless computing has emerged as a market-dominant paradigm in modern cloud computing, benefiting both cloud providers and tenants. While service providers can optimize their machine utilization, tenants only need to pay for the resources they use. To maximize resource utilization, these serverless systems co-run numerous short-lived functions, bearing frequent system condition shifts. When the system gets overcrowded, a tenant's function may suffer from disturbing slowdowns. Ironically, tenants also incur higher costs during these slowdowns, as commercial serverless platforms determine costs proportional to their execution times.

% This paper argues that the cloud providers should compensate the tenants for their loss when the server is over-provisioned. However, estimating the tenant's loss is challenging when there is no pre-profiled information about the function. Prior studies showed assessing the tenant's loss introduces heavy overheads. Instead, this paper proposes a new pricing model, Litmus pricing, which offers discounts based on the machine's state while presuming the tenant's loss under the state. To monitor the machine state correctly, Litmus pricing frequently conducts Litmus tests, an effectively lightweight solution to measure system congestion. Our experiments show that Litmus pricing can detect the impact of system congestion and offer near-ideal prices, with only a 0.38\% price difference. 
This paper argues that cloud providers should compensate tenants for losses incurred when the server is over-provisioned. However, estimating tenants' losses is challenging without pre-profiled information about their functions. Prior studies have indicated that assessing tenant losses leads to heavy overheads. As a solution, this paper introduces a new pricing model that offers discounts based on the machine's state while presuming the tenant's loss under that state. To monitor the machine state accurately, Litmus pricing frequently conducts Litmus tests, an effective and lightweight solution for measuring system congestion. Our experiments show that Litmus pricing can accurately gauge the impact of system congestion and offer nearly ideal prices, with only a 0.2\% price difference on average, in a heavily congested system.

\end{abstract}


==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Serverless computing is growing fast, satisfying today's high demands for better programmability. It allows tenants to develop their programs as stateless functions in high-level languages such as Python, Go, and JavaScript without concerns with low-level resource management and task scheduling~\cite{serverless2,serverless1,schall2022lukewarm,schall2023warming,mohammad2020SerInWild}. This advantage attracts cloud users, helping them to deploy their programs quickly with minimal effort. Recent reports note that over 50-70\% of cloud users have adopted serverless computing for their tasks~\cite{serverless1}.

% Serverless computing claims a pay-as-you-go pricing model where users only pay for the resources used by their functions. This requires the service provider to monitor and estimate the fine-grained resource usage by each user accurately. However, today's high-performance systems maximize resource efficiency by accommodating multiple applications simultaneously and allowing the resources to be shared by them. Such a shared system raises two major challenges. First, tracking a user's resource usage is a challenging task. While being shared, the system tracks the total usage but not a single user's. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress. These inferences between the applications not only make the system hard to track resource usage, but the users may get charged unfairly due to the delayed execution time.
Serverless computing also benefits tenants financially. Unlike traditional cloud platforms that require tenants to purchase the hardware resources needed to deploy their servers regardless of actual usage~\cite{amazonEC2Pricing}, serverless computing claims a pay-as-you-go pricing model, where tenants only pay for the resources consumed during the execution of their functions, facilitating significant cost savings. Meanwhile, this pricing requires service providers to accurately monitor and estimate each user's fine-grained resource usage~\cite{microsoftAzurePricing,awsLambdaPricing,googleCloudFunctionPricing}. 

% However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared system raises two major challenges. First, tracking a tenant's resource usage is a challenging task. While being shared, the system can only monitor a tenant's use of specific resources. Second, more importantly, the co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference between the applications not only makes the system hard to track resource usage, but the tenants may get charged unfairly due to the extended execution time~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}. 
However, today's high-performance systems maximize resource efficiency by executing multiple applications simultaneously and allowing resources to be shared~\cite{zhao2021understanding}. Such a shared serverless system raises two major challenges. First, tracking a tenant's resource usage becomes challenging, as the system can only monitor a tenant's use of exclusively dedicated resources while the system is shared. Second, and more importantly, co-running applications compete to grab more resources, affecting each other's progress~\cite{jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown,zhao2021understanding}. This interference not only complicates tracking resource usage but also leads to tenants being charged unfairly due to delayed execution times~\cite{alex2013ScFairPrice,goltzsche2019acctee,jin2015hardware,tiwari2013enabling}.

% A serverless platform should provide an isolated runtime environment to a user. Otherwise, we argue that the platform provider must compensate a tenant's loss as a discount when it is not achievable. Therefore, we define a charged fee as fair when it reflects the tenant's slowdowns due to the resource sharing. The following two methods can be used to estimate a fair price under a multi-tenant environment. 
A serverless platform should provide a user with an isolated runtime environment. Otherwise, we argue that the platform provider should compensate a tenant's loss as a discount when the isolation is not achievable. Thus, we define a charged fee as fair when it reflects the tenant's slowdowns caused by resource sharing. The following two methods can be used to offer a fair price in a multi-tenant environment.

% First, strict resource partitioning can divide shared resources into multiple partitions, each assigned to a user exclusively. The user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strictly partitioned resources are well known to cancel the opportunities to utilize the given resource efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delayed execution directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources when requesting them. 
First, strict resource partitioning can divide shared resources into multiple partitions, each assigned exclusively to a user. This means the user only pays for the allocated resources and is free from others' interference~\cite{kim2004Partition,vicent2017AppClustering,roy2021satori,park2019copart}. However, strict partitioning is known to cancel opportunities to utilize resources efficiently~\cite{marangoz2021designing,wang2016simultaneous,el2018kpart,wang2008adaptive}. Also, a tenant's application may suffer unacceptable slowdowns when insufficient resources are allocated~\cite{roy2021satori,park2019copart}. Such a delay directly appears as an increased price. Consequently, resource partitioning inherently requires users to deduce the optimal amount of resources they need when requested. 

% Alternatively, a discount-based scheme estimates a user's price relative to its slowdown, discounting from the price when run without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources. Thus, the providers can maximize their hardware utilization and earn more money with given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns or interference they get from co-running tasks without overpaying for exclusive resources.
% The tenants also can get a discount reasonably proportional to the amount of their slowdown when their jobs suffer from interference rather than endeavoring to secure necessary resources exclusively.
Alternatively, a discount-based scheme estimates a user's price relative to the slowdown experienced, discounting from the price when running the task without interference, i.e., running the task alone on the machine~\cite{alex2013ScFairPrice,tiwari2013enabling}. Ideally, this scheme benefits both cloud providers and tenants compared to partitioning. Unlike partitioning, it allows tenants to share resources, enabling providers to maximize hardware utilization and generate more revenue with the given machines. Meanwhile, users get reasonable discounts proportional to the slowdowns they experience due to co-running tasks, preventing them from overpaying for lowered service quality.

% While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Even if the platform can measure its execution time, computing the slowdown still requires knowing its baseline, which can be gained when executing it alone. The cloud platform could not pre-profile users' applications for reasons such as mandated privacy when processing confidential information. Even if the platform has such information, the function could operate differently when receiving different inputs. That is to say, online profiling is necessary, which unfortunately requires expensive runtime sampling, as proposed in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. All co-running tasks must be stalled when estimating a task's baseline performance. Massive short-living serverless functions make such a sampling-based solution even more impractical. Frequently sampling the baseline performance of thousands of co-running functions is unrealistic. This motivates a new practical solution that can be adopted in commercial platforms. 
While the alternative scheme looks superior, it poses a new challenge: measuring a function's slowdown. Although the platform can measure its execution time, determining the slowdown requires knowing its baseline performance, which can be obtained when it runs without interference. However, such profiling is often prohibited due to security concerns, particularly when the function processes confidential information. Additionally, the function may behave differently, with varying inputs each time it runs. That is to say, online profiling is necessary. Unfortunately, this requires expensive runtime sampling, as presented in POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling}. When assessing baseline performance, all co-running tasks must be stalled. Hundreds to thousands of concurrent short-lived functions make this approach indeed impractical, as frequently sampling the baseline performance of such numerous functions is unrealistic. Thus, a new, practical solution that can be adopted in serverless platforms is needed.

%In either approach, a tenant or a service provider bears the problem's complexity alone. Resource partitioning demands the tenant to know the needed resources while losing opportunities to utilize the resources better. Discounting demands a service provider to estimate the task's slowdown with heavy sampling overheads. Accordingly, both approaches complicate the problem while sacrificing the machine's efficiency. Instead, we claim this problem becomes simpler when both entities participate and carry a portion of the responsibilities. 

% Litmus addresses this challenge by imposing the responsibility on both entities. With Litmus, the serverless platform measures the system congestion that may delay a function's execution when every tenant's function starts. The service provider needs to determine a discount rate for a corresponding congestion state. Meanwhile, the tenant needs to know about a possible slowdown and a corresponding discount. 

% We highlight that both partitioning and sampling complicate the problem while sacrificing the machine's efficiency and can hardly be employed in serverless computing. The approaches in serverless must be lightweight and frequent to deal with the fast-changing environment with thousands of concurrent functions. This paper proposes Litmus pricing that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening the system performance. 
We highlight that both partitioning-based and sampling-based approaches complicate the problem, either sacrificing the machine's efficiency or appearing impractical for serverless computing. Approaches in serverless computing must be lightweight, frequent, and sensitive enough to deal with quickly changing environments with numerous concurrent functions. This paper proposes Litmus pricing, a method that efficiently estimates a tenant's price with a discount proportional to the level of system congestion without burdening system performance. 

% \hl{Measuring the server's congestion status is challenging work. Here, Litmus relies on our key observation that, although not limited, function implementation in serverless computing largely relies on high-level programming languages such as Python and GoLang, which require a relatively long startup. This startup overhead has been considered one of the major challenges in serverless computing. However, Litmus utilizes this startup to measure the system's congestion state. Our analysis of Python and GoLang observed that the activities during the startups are almost identical, with plenty of memory operations, regardless of the functions. Thus, we claim that the startup performance can be an index of the system state.}

% \hl{The Litmus test is based on our insight that the serverless functions perform broadly identical operations, with plenty of memory operations, during their long startups, preparing the runtime environment for the functions. Leveraging this observation, the platform can assess the system's congestion level, which hints at the tenant's discount amount. Additionally, Litmus pricing exploits our second insight that the performance of two resources, private and shared, are affected differently by the congestion. In particular, its impact on private resources is minor and predictable, while many functions significantly rely on them, spending most of their execution time with them. }

% During the execution of every function, Litmus pricing conducts a Litmus test, which measures the level of system congestion with no extra overhead using the function's startup process. The Litmus test is based on the observation that serverless functions perform largely identical operations during their startup time. Those operations usually prepare the runtime and include a large amount of memory access to shared hardware resources. In addition, Litmus pricing splits the hardware resources into "private" and "shared" and proposes charging different ratios on each. This further improves the accuracy of the discount calculation.
During each function's execution, Litmus pricing conducts a Litmus test, which measures the level of system congestion without adding extra overhead, using the function's startup process. Litmus test is based on the observation that serverless functions perform largely identical operations during their startup, typically involving significant memory accesses. Additionally, Litmus pricing splits the hardware resources into "private" and "shared" categories, proposing different charging ratios for each. This approach further enhances the accuracy of the discount calculation.

% In our experiments, the Litmus pricing estimates a tenant's price to be nearly ideal, with a \hl{0.38\%} difference from the ideal price, which discounts tenants proportional to their slowdowns.
% This study investigates Litmus pricing across different environments, ranging from restricted to crowded settings. We verify that crowded environments pose additional challenges. Despite this, Litmus pricing accurately estimates a tenant's price, deviating by only 0.26\% from the ideal price, discounting tenants proportional to their slowdowns.
This study investigates Litmus pricing across diverse environments with varying levels of system congestion. We confirm that crowded environments pose complex challenges. Despite this, Litmus pricing accurately estimates a tenant's cost, deviating by only 0.2\% on average from the ideal price that discounts tenants proportional to slowdowns.



==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/02_background.tex <==
\section{Background}
\label{sec:background}

% \textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while the service providers handle back-end implementation~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers, which are later invoked upon associated events~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. The serverless platform guarantees security by executing the tenant's function in a sandbox such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.
\textbf{Serverless Computing:} Serverless computing is a new cloud execution model that allows cloud tenants to focus on developing front-end applications while leaving back-end implementation managed by service providers~\cite{serverless1, schall2022lukewarm}. This model benefits tenants by easing their burdens to secure and maintain the hardware resources and allowing them to write their code (functions) in high-level languages (e.g., Python or Node-js) as event handlers~\cite{serverless1,mohammad2020SerInWild,schleier2021serverless}. These functions are later invoked upon associated events. The serverless platform ensures security by executing the tenant's function in a sandbox, such as a container or a virtual machine~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing,zhang2021faster}.

% Each tenant's function is stateless and expected to be short~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using the short-lived functions, the tenant can easily scale by invoking many of the functions without provisioning needed resources for themselves, relying on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. Inherently, massive short-living serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. The tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and clients mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Later, under the pay-as-you-go pricing, the tenant is charged for the consumed resources, typically the product of time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
Each tenant's function is stateless and expected to be short-lived~\cite{serverless1,serverless2,eismann2020review,mohammad2020SerInWild,jia2021nightcore}. Using these short-lived functions, tenants can easily scale by invoking many functions without provisioning the needed resources for themselves, relying instead on the serverless platform~\cite{ska20ISCABabelFish,mohammad2020SerInWild}. In serverless computing, numerous short-lived serverless workloads run together on a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. Tenants need to trust the service provider to provision enough necessary resources, expecting the quality of service defined in the service level agreements (SLA) that the provider and tenants mutually agreed upon~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% In the traditional cloud, tenants purchase hardware resources for the contracted term to support their applications, which are often expected to be large in a server form. Thus, tenants must pay for the agreed period regardless of actual use. Instead, serverless workloads are generally small and launched on-demand as short-living event handlers. This workload difference develops a unique pricing policy, pay-as-you-go pricing. The tenant is charged only for the consumed resources during the execution, typically the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.
In traditional cloud computing, tenants purchase hardware resources for a contracted term to support their applications, which are typically large servers. Thus, tenants must pay for the agreed period regardless of actual usage. In contrast, serverless workloads are generally small and launched on-demand as short-lived event handlers. This difference leads to a unique pricing policy known as pay-as-you-go. Under this model, tenants are charged only for the resources consumed during execution, typically calculated as the product of execution time and assigned memory capacity~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}.

% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, where Python is utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Also, over 90\% of organizations choose Python and Node.js for their AWS services. Other popular language runtimes are Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer a high level of abstraction from machine codes with good programmability and portability, improving the programmer's productivity. As a result, they have been adopted widely by serverless users. However, such high-level languages typically rely on runtime interpretation, which results in a slow start of program execution with extra launching steps. For instance, in the case of Python, when an application is launched, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the codes are compiled and executed. Once the execution is complete, the Python program is terminated, and all assigned resources are released~\cite{pythonUsage}.
\textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python used in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Over 90\% of organizations choose Python and Node.js for their AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer significant abstraction from machine code with good programmability and portability, which in turn improves programmer productivity. Consequently, they are widely adopted by serverless users. However, high-level languages typically rely on runtime interpretation, leading to slower program startup due to extra launching steps. For example, when an application is launched in Python, the interpreter is first prepared. It then parses command-line arguments and imports necessary modules. Afterward, the codes are compiled and executed. Upon completion, the Python program terminates, and all allocated resources are released~\cite{pythonUsage}.

 
% list of pricing models? 
% Amazon? 
% Google?
% The price is calculated by duration time multiplies to the unit price plus the request charges. The duration time is from the time user's code begins executing until it returns or terminates. The unit price depends on the amount of memory the user allocate to their function. The request charges is based on how many times the function has been invoked minus the free requests~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. 
% may need service agreement here, contention impact

%\textbf{Traditional cloud platforms:} In the context of traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage, data transfer, etc. The instance type is the combination of Virtual CPUs(VCPUs), RAM, storage and network performances. The time unit price will be higher with more powerful instance type. Typically, more powerful instance types have higher time unit prices. There are two main pricing options: On-Demand and Reserved Instances. On-demand instance let the customers pay for compute capacity by the hour or second based on the actual usage with no long-term commitments. Reserved Instances, on the other hand, require a commitment to a specific instance type for a contract term and offer cost savings compared to On-Demand pricing. Storage and data transfer for the VM instance can also impact the pricing. The more storage space a customer uses or the more data they transfer, the higher their costs will be. The traditional cloud platform can also be affected by the co-running applications~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} In traditional cloud platforms, the price can be influenced by various factors such as instance type, pricing options, storage space, data bandwidth, etc. The instance type includes virtual CPUs, RAM, storage, and network performances. Typically, more powerful instance types charge higher prices. Also, two pricing options are commonly offered: on-demand and reserved instances. On-demand instances allow tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved instances require a commitment to a specific instance type for an agreed term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period. Storage space and data bandwidth for the VM instance also influence the price. Demanding more storage space or more data transfer raises the cost~\cite{amazonEC2Pricing}. 
% \textbf{Traditional cloud platforms:} 

% The price of traditional cloud platforms is determined by computing capabilities such as processor type, memory capacity, and network bandwidth. While more and better resources typically charge higher prices, two pricing options are commonly offered: on-demand and reserved instances. On-demand pricing allows tenants to pay for computing capacity for short-term use without any long-term commitments. Instead, reserved pricing requires a commitment to specific resources for an agreed-upon term, accommodating cost-saving for a tenant who needs the instance consistently for a lengthy period~\cite{amazonEC2Pricing}. 

% There are several differences between traditional cloud platforms and serverless platform. 
% Firstly, the roles of customers in the execution environment differ between traditional and serverless platforms. In the traditional cloud, customers are responsible for configuring and maintaining virtual machines (VMs), setting up networking, and managing databases~\cite{amazonEC2Pricing}. And it's the customers's responsibility to detact and update the configurations to balance their expenses and performance. On the other hand, in serverless platforms, users only provide a single file to indicate their system and library requirement, while the service provider handles the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. This feature enables users to focus solely on their actual workload without the burden of managing the infrastructures. Additionally, the platform can automatically scale the resources for the users based on the current demand of the application to guarantee the customer satisfaction~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% There are apparent differences between traditional and serverless cloud platforms. First, tenants are responsible for managing hardware resources in traditional platforms. The tenants need to configure and maintain virtual machines, set up networking, and manage databases~\cite{amazonEC2Pricing}. Also, tenants should study the optimal configurations to balance their expenses and performance. Meanwhile, in serverless platforms, tenants only provide a single file to specify their system requirements while the cloud provider prepares the execution environment~\cite{awsLambdaPricing,googleCloudFunctionPricing,microsoftAzurePricing}. The platform provisions or scales the needed resources on demand. Consequently, the serverless platforms encourage tenants to focus solely on their front-end workloads without the burden of managing the low-level back-ends~\cite{ska20ISCABabelFish,mohammad2020SerInWild}.

% Secondly, there are notable differences in compute power and memory size options between the two platforms. For traditional cloud, the granularity usually 1 VCPU and 1GB memory. But, for serverless platform, the smallest memory size is 128 MB~\cite{awsLambdaApiGateWay,googleCloudFunctionPricing,microsoftAzurePricing}. 
% Thirdly, the characteristics of workloads on these platforms set them apart. Serverless applications are generally small and executed on-demand, resulting in very short workload durations~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can complete in less than one second. In contrast, traditional cloud applications tend to be larger and may require hours to complete. Additionally, the number of co-located applications on a single computing node is smaller in traditional cloud setups, making their execution environment less dynamic compared to serverless platforms.
% Lastly, the billing periods differ significantly between traditional cloud and serverless platforms. Traditional cloud users are charged for the allocated time period. Regardless of whether they are actively running tasks on the machine, they are still need to pay for the allocated time period. However, serverless customers are only billed for the actual execution time of their tasks on the platform.

% Second, the workloads are expected to be small in serverless computing. Serverless workloads are generally small and launched on-demand as short-living event handlers~\cite{eismann2020review,mohammad2020SerInWild}. For instance, 50\% of serverless functions can be completed in less than one second, unlike traditional cloud applications that are often expected to be large in a server form. Inherently, massive serverless workloads run together in a single machine, making the execution environment more dynamic than the traditional cloud~\cite{ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}. This workload difference develops a unique pricing policy in serverless computing, pay-as-you-go pricing. In the traditional cloud, the tenants purchase hardware resources for the contracted term. Regardless of actual use, they need to pay for the agreed period. However, the serverless platforms bill their tenants for the actual execution time of their tasks.


% \textbf{Language runtime:} Python and Node.js stand out as the most popular runtimes in AWS Lambda, with Python being utilized in 58\% of all Lambda functions and Node.js in 31\%~\cite{serverless3}. Furthermore, over 90\% of organizations leverage Python and Node.js alongside AWS services. Other popular runtimes include Java, Go, .NET, and Ruby~\cite{serverless1,serverless2}. These high-level languages offer numerous advantages for programmers, such as user-friendliness, portability, reduced error risks, and thriving ecosystems. As a result, they have garnered widespread acceptance within serverless platforms. High-level programming languages typically follow a fixed execution procedure. For instance, in Python, when an application is executed, the Python Interpreter is first initialized. It then proceeds to parse the command-line arguments and import the necessary modules. After that, the code is compiled and executed. Once the execution is complete, the Python program is terminated, and all resources used by the program are released. Due to the consistency of the operating system and Python version, the beginning of the execution process remains the same each time~\cite{pythonUsage}.



% \textbf{Resource based discount vs. Slowdown based discount:} To fully utilize the available resources, service providers often run as many applications as they can in one computing node within the service agreement requirement. However, this may lead to resource congestion and cause slowdowns for users, which can be unfair, since the customers are paying more money for the worse experiences. The intuitionistic solution could be for the service provider to track the resource usage of each application and offer discounts to users who consume fewer resources. However, serverless applications are typically very small, and contention can affect different applications differently, making this approach less practical. A more suitable solution for serverless platforms could involve offering slowdown-based discounts. In this approach, the service provider dynamically updates unit prices based on the level of system congestion. When there is less contention, users normally stiffed with the experiences and pay the regular price. However, during periods of high congestion, when the system is under heavy load, users could receive discounted prices as compensation for potential slowdowns. This approach would align pricing with the actual performance experienced by users, ensuring a fair and responsive pricing model.


==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/03_methodology.tex <==
\section{Methodology}
\label{sec:method}

% \textbf{Hardware Infrastructure:} All the experiments are performed on a dual-socket server platform. Each socket has 16 simultaneous multithreading(SMT) cores. The CPU model is Intel Xeon Gold 5218(Cascade Lake). The maximum frequency of the machine is 3.9GHz. Each core has a 32KB L1 instruction cache, a 32KB L1 data cache and a 1MB L2 cache. The 32 virtual cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The computer node runs the latest Ubuntu server version(Ubuntu 22.04 LTS) with kernel version 5.15.0. For consistency in the results, the core frequency was set to 3.0GHz using the 'cpupower frequency-set' command. We use linux perf~\cite{perfWiki} to collect the performance counters for each experiment. To analyze the startup status, we use -I 1 option to obtain count deltas at one-millisecond intervals. By utilizing interpolation, we can know the performance counters of each execution period. 

% In this study, we test today's server systems with serverless functions. This section describes our test configuration. 
This section outlines our test setup for evaluating serverless functions in this study.

% % original version
% \textbf{Hardware Infrastructure:} All experiments are performed on a dual-socket server platform with two Intel Xeon Gold 5218 (Cascade Lake). The CPU offers 16 simultaneous multithreading (SMT) cores with 3.9 GHz maximum frequency. We pin the core frequency at 3.0GHz for our tests. Each core has 32KB L1 instruction/data caches and 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets share a 384GB main memory. The machine runs the Ubuntu server OS (Ubuntu 22.04 LTS) with a kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to collect the performance counters, which are collected at every one-millisecond interval. 
\textbf{Hardware Infrastructure:} All experiments are conducted on a dual-socket server platform equipped with two Intel Xeon Gold 5218 processors based on the Cascade Lake architecture. Each CPU provides 16 cores that support simultaneous multithreading (SMT) with a maximum frequency of 3.9 GHz. Every core features 32KB of L1 instruction/data caches and a 1MB L2 cache. All cores in each socket share a 22MB L3 cache. The two sockets collectively have access to 384GB of main memory. The server operates on Ubuntu Server OS, version 22.04 LTS, with kernel version 5.15.0. We use Linux Perf~\cite{perfWiki} to gather performance counters.

% The CPU frequency is a key performance/energy factor, significantly affecting a function's execution time and energy consumption. A CPU's frequency can be altered in software or hardware based on its power and thermal budget, configuring it for better energy efficiency or performance. However, varying frequencies cause the system performance/energy to be unsettled, making system management intractable. For this reason, commercial systems such as Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. In our tests, when the frequency is not fixed by software, Intel's Turbo technology alters the frequency occasionally but mainly employs 2.8GHz. We will discuss this further in the sensitivity section.
The CPU frequency is a critical factor influencing both performance and energy consumption, significantly affecting a function's execution time and energy usage. A CPU's frequency can be adjusted through software or hardware based on power and thermal budget, optimizing for either energy efficiency or performance. However, varying frequencies can cause instability in system performance and energy usage, complicating system management. For this reason, commercial systems like Google Cloud offer only one fixed frequency for their vCPUs~\cite{googleCloudFunctionPricing}. Accordingly, we set our CPUs' frequency at 2.8GHz. If we do not fix the frequency through software, Intel's Turbo technology occasionally adjusts it, but it mostly remains at 2.8 GHz during our tests. We will provide more details on this in Section~\ref{sec:sensitivity}.

% \textbf{Stressing Programs:} We used two stressing programs to investigate how applications and the startup portion of the high level languages behave in a resource contention environment. FigureXXX illustrates the number of instructions, L3 accesses, and L3 misses that the stressing programs can generate in five seconds as the stressing levels increase. By combining different stress levels of these stress-testing programs, we can simulate various resource-congested environments. The XXX-stressor(lineXXX)  generates more L3 accesses with a high L3 hit rate. While XXX-stressor(lineXXX), in each stressing level, generates fewer L3 accesses but more L3 misses. With these two stressors and different stressing levels, we can simulate the system with varying contentions to the shared resources by creating various  L3 accesses and L3 misses. In figureXXX we can see that the L3 accesses generated from the L2-stressor (update name later) begin to decrease after reaching stressing level 20.  However, during this period, the L3 misses continue to increase. The reason behind this trend is that, after stressing level 20, the heightened L3 miss rate starts to impact the stressor's performance, leading to a decline in the committed instruction count. Consequently, the stressor generates fewer L3 accesses and more L3 misses. 

% \begin{table}[h]
%     \begin{center}
%     % \vspace{-1.0em}
%         \caption{Serverless Benchmarks \& Runtimes}
%         \label{tb:benchmarks}
%         % \vspace{-1.0em}
%         \begin{tabular}{|l l||l l|} \hline
%             Function & Abbr. & Function & Abbr. \\ \hline \hline
%             \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  & \multicolumn{2}{c|}{\textbf{Hotel Reservation~\cite{gan2019open}}} \\ \hline
%             Dyn HTML & dyn-py & Geo & geo-go* \\ \hline
%             Thumbnail & thum-py* & Profile & profile-go \\ \hline
%             Compression & compre-py & Rate & rate-go \\ \hline
%             Image Recogn & recogn-py* & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
%             Graph Rank & pager-py & Currency & cur-nj* \\ \hline
%             Graph Mst & mst-py & Payment & pay-nj \\ \hline
%             Graph Bfs & bfs-py* & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
%             DNA Visual & visual-py* & Authen & auth-py/nj/go \\ \hline
%             \multicolumn{2}{|c||}{\textbf{Function Bench~\cite{kim2019functionbench}}} & Fibonacci & fib-py/nj/go* \\ \hline
%             Chameleon & chame-py & AES & aes-py/nj/go \\ \hline
%             FloatOp & float-py* & & \\ \hline
%             % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
%         \end{tabular}
%     \end{center}
%     % \vspace{-1.5em}
% \end{table}

\begin{table}[h]
    \begin{center}
    % \vspace{-1.0em}
        \caption{Serverless Benchmarks \& Language Runtimes (py, nj, go)}
        \label{tb:benchmarks}
        % \vspace{-1.0em}
        \begin{tabular}{|l l||l l|} \hline
            Function & Abbr. & Function & Abbr. \\ \hline \hline
            \multicolumn{2}{|c||}{\textbf{SeBs~\cite{copik2021sebs}}}  &  \multicolumn{2}{|c|}{\textbf{Function Bench~\cite{kim2019functionbench}}}\\ \hline
            Dyn HTML & dyn-py & Chameleon & chame-py \\ \hline
            Thumbnail & thum-py* & FloatOp & float-py \\ \hline
            Compression & compre-py & Gzip & gzip-py* \\ \hline
            Image Recogn & recogn-py & RandDisk & randDisk-py* \\ \hline
            Graph Rank & pager-py & SequenDisk & seqDisk-py \\ \hline
            Graph Mst & mst-py & \multicolumn{2}{c|}{\textbf{Online Boutique~\cite{googleMicroserviceDemo}}} \\ \hline
            Graph Bfs & bfs-py* & Currency & cur-nj* \\ \hline
            DNA Visual & visual-py* & Payment & pay-nj \\ \hline
            \multicolumn{2}{|c||}{\textbf{Hotel Reservation~\cite{gan2019open}}} & \multicolumn{2}{c|}{\textbf{Other~\cite{awsLambdaApiGateWay,copik2021sebs}}}  \\ \hline
            Geo & geo-go & Authen & auth-py*/nj/go \\ \hline
            Profile & profile-go* & Fibonacci & fib-py*/nj*/go* \\ \hline
            Rate & rate-go & AES & aes-py/nj*/go* \\ \hline
            % Float Operation & float-py & Hello World & hello-nj/go \\ \hline
        \end{tabular}
    \end{center}
    % \vspace{-1.5em}
\end{table}

% revision version
% \textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we select 27 distinct serverless functions from different benchmark suites, including AWS' authentication serverless functions~\cite{awsLambdaApiGateWay}, Hotel Reservation from the DeathStarBench suite~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and SeBS serverless benchmark suite~\cite{copik2021sebs}. The three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating 3 separate test cases per function. Among them, we pick 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. The functions are implemented using three languages: Python, Nodejs, and Go. We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. 
\textbf{Workload:} As listed in Table~\ref{tb:benchmarks}, we selected 27 distinct serverless functions from various benchmark suites, including AWS authentication serverless functions~\cite{awsLambdaApiGateWay}, the Hotel Reservation from DeathStarBench~\cite{gan2019open}, Google's Online Boutique application~\cite{googleMicroserviceDemo}, FunctionBench~\cite{kim2019functionbench}, and the SeBS serverless benchmark suite~\cite{copik2021sebs}. The functions are implemented using three languages: Python, Nodejs, and Go. Notably, the three functions, Authen, Fibonacci, and AES, are implemented in all three languages, creating three separate test cases per function. 
% This comprehensive language support ensures that our test coverage is thorough and representative of the diverse language preferences in the serverless computing community. 
We installed Python 3.10.6, Nodejs v12.22.9, and Go 1.19.2 to support them. Additionally, we selected 13 benchmarks (* marked) in Table~\ref{tb:benchmarks} as our reference applications, which are explained later. 


%\hl{The benchmarks we choose include I/O-bound, memory-bound, and compute-bound functions. For an experiment, we put the testing function in core 0 to core 4. We also put 50 other functions in core 0-4 to let the application co-running with 10 other applications to observe the impact of context switching.}

% \hl{We select benchmarks with mixed performance characteristics: I/O, memory, and compute-bound. Also, to replicate the congested commercial systems, we located a testing function with 50 other functions and tied them to selected 5 cores, Core 0 to 4. During our evaluation, those functions run simultaneously and compete to secure any core among the five.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
\caption{(a) L2 misses and (b) L3 misses of traffic generators, both normalized with the average L2 and L3 misses of serverless applications listed in Table~\ref{tb:benchmarks}}
% \vspace{-0.5em}
\label{fig:stressing_specs}
\end{figure}

% \textbf{Traffic Generator:} We divide the CPU's shared resources into two distinct categories: resources before and after the L3 caches. To pressure each resource group individually, we developed two separate traffic generators aimed at generating traffic and congestion in these resources. The first traffic generator, CT-Gen, applies pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another traffic generator, MB-Gen, induces massive L3 misses that stress the resources after the L3 cache, mainly the off-chip memory bandwidth and L3 cache spaces.
\textbf{Traffic Generator:} We categorize the CPU's shared resources into two groups: those before the L3 caches and those after. To stress each group independently, we developed two separate traffic generators designed to generate traffic and congestion within these resources. The first generator, CT-Gen, exerts pressure from the core up to the L3 cache by creating substantial memory accesses that mostly miss the L2 cache but hit the L3 cache. Another generator, MB-Gen, induces massive L3 misses, which stress the resources beyond the L3 cache, primarily targeting off-chip memory bandwidth and L3 cache spaces.

% Both traffic generators are multi-threaded, governing the volume of traffic by adjusting the number of threads they spawn. Each thread spawned by the traffic generator is pinned on each core to prevent conflicts between threads; consequently, this setup allows us to vary the stress level across our 32-core processors, ranging from level 1 to 31. Figure~\ref{fig:stressing_specs} shows each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), for every thread count increment, CT-Gen makes massive L2 misses. The CT-Gen's L2 misses are ended with L3 hits, as shown in Figure~\ref{fig:stressing_specs}(b). Meanwhile, MB-Gen creates huge L2 and L3 misses, as implemented. Interestingly, its L2 misses are fewer than CT-Gen's because MB-Gen is slowed by its L3 misses, suffering from a self-created bandwidth bottleneck. 
Both traffic generators are multi-threaded and govern the amount of traffic by adjusting the number of threads they spawn. Each thread is pinned to a specific core to avoid conflicts between threads, allowing us to vary the stress level on our 32-core processors from level 1 to 31. Figure~\ref{fig:stressing_specs} illustrates each generator's characteristics. In Figure~\ref{fig:stressing_specs}(a), with each increase in thread count, CT-Gen generates substantial L2 cache misses. These L2 misses by CT-Gen are ended with L3 cache hits, as shown in Figure~\ref{fig:stressing_specs}(b). In contrast, MB-Gen produces significant L2 and L3 cache misses. Interestingly, MB-Gen's L2 misses are fewer than those of CT-Gen because MB-Gen is hindered by its L3 misses, suffering from a self-imposed performance bottleneck.



==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/04_motivation.tex <==
\section{The Need for Fair Pricing}
\label{sec:motivation}

% Offering fairness appears in different approaches in cloud computing when multiple tenants share hardware resources. One standard is SLA, which defines the level of services the cloud provider furnishes while a tenant sets their expectation. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving unfairness between tenants. Although serverless computing highlights the pay-as-you-go pricing model, such unfairness still exists.
Fairness in cloud computing, especially when multiple tenants share hardware resources, is addressed through various approaches. One standard method is the Service Level Agreement (SLA), which specifies the level of service the cloud provider must deliver and the tenants' expectations. However, the SLA outlines the minimum quality of service the providers should deliver rather than solving fairness issues. Despite serverless computing's emphasis on a pay-as-you-go pricing model, unfairness among tenants still exists.

% Unfortunately, modern systems are designed to maximize hardware efficiency by co-running multiple applications; the function's execution time can be affected by co-scheduled applications with conflicts when using shared resources. Ironically, whenever the service provider squeezes their resources further for better profit by accommodating more functions into a single machine, each function's execution time increases, charging them a higher cost for the same workload. However, in serverless computing, tenants lack control and insights into how their software is executed and billed for the cost of convenience. 
Unfortunately, modern systems are designed to maximize hardware efficiency by running multiple applications concurrently. This results in conflicts over shared resources, affecting each function's execution time. Ironically, when service providers optimize for profit by packing more functions into a single machine, the execution time for each function increases, resulting in higher costs for the same workload. In serverless computing, tenants have no control or visibility over how their software is executed, leading to potential inefficiencies and higher costs for the sake of convenience.

% Genuine pay-as-you-go pricing can be achieved when there is no interference. However, that is not desired by the providers who expect to utilize their resources to maximize profits. In serverless, although each function runs virtually exclusively in a sandbox with private resources, it still shares a few resources with other co-running functions, such as shared caches and memory bandwidth. Resource partitioning, a traditional solution that eliminates interference, can promise exclusively dedicated resources to a tenant but cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 
In serverless computing, although each function runs exclusively in a virtual sandbox with private resources, it still shares certain resources like caches and memory bandwidth with other functions. Resource partitioning, a traditional solution that eliminates interference by dedicating resources exclusively to a tenant, cannot avoid inefficient resource utilization. It is also against the serverless philosophy, demanding the tenants govern their hardware resources. 

\begin{figure}[h]
\centering
% \vspace{-0.7 em}
\includegraphics[width=1\columnwidth]{./fig/normalizedCPIRunWith26Rev}\\
% \vspace{-1 em}
\caption{Execution time of applications that run with 26 others, normalized to the execution time when running alone}
% \vspace{-0.4 em}
\label{fig:normalizedCPIRunWith26Rev}
\end{figure}

% Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed down when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. \hl{Whenever a function finishes, another function is randomly launched to maintain a total of 26 co-running functions.} The figure shows a function's performance drops by up to 35\%, and most functions are significantly influenced by the co-running functions. Compared to when an isolated environment is offered, the function performs 11.5\% slower on average, charging 11.5\% more to users. We highlight that the function runs only with 26 other functions, which is tiny compared to massively crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.
Figure~\ref{fig:normalizedCPIRunWith26Rev} shows how much a function can be slowed when co-running with 26 other workloads. The workloads are randomly selected from the benchmarks listed in Table~\ref{tb:benchmarks}. Whenever a function finishes, a new randomly-selected function is launched to maintain a total of 26 co-running functions. The figure shows a function's performance can drop by up to 35\%, with most functions significantly impacted by the co-running functions. On average, functions perform 11.5\% slower in this shared environment compared to an isolated one, resulting in users being charged 11.5\% more. We highlight that this scenario involves only 26 co-running functions, which is tiny compared to heavily crowded commercial serverless platforms that run hundreds to thousands of functions simultaneously~\cite {ustiugov2021benchmarking,schall2022lukewarm,tariq2020sequoia}.

% Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} attempted to offer price discounts if it has a slowdown, compensating for the slowdowns. To provide the discount, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount reflecting the slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all the responsibilities of the contentions between co-running functions, guaranteeing all tenants an invariant price for their use. Any unexpected slowdowns that a tenant experiences are returned with a discount. However, sampling is an expensive operation, requiring all co-running processes to stall during the sampling. Moreover, accurate measurement requires frequent sampling when its system environment quickly alters, making the approach impossible in a fast-shifting environment like a serverless platform.   
Instead of guaranteeing invariant performance, POPPA~\cite{alex2013ScFairPrice,tiwari2013enabling} offers price discounts to compensate for slowdowns. To provide these discounts, POPPA measures a task's slowdown due to interference through sampling and determines the discount amount based on the observed slowdowns. Unlike partitioning, this scheme requires the service provider to carry out all responsibilities related to contentions from resource sharing, ensuring tenants pay a consistent price for their usage. Any unexpected slowdowns that a tenant experiences are compensated with a discount. However, sampling is an expensive operation that requires stalling all co-running processes during the sampling. Moreover, accurate measurement necessitates frequent sampling, especially in rapidly changing environments, making the approach impractical for dynamic environments like serverless platforms.


% A tenant needs a new pricing model based on more than just execution time. However, prior approaches have limitations, burdening cloud participants too heavily; it is unsuitable for \hl{thousands} of concurrent short-lived functions in serverless computing. This motivates us to propose a new solution, Litmus pricing, that discounts prices based on the system state but offers lightweight with no overheads.
Overall, tenants need a new pricing model that considers more than just execution time. Prior approaches have limitations, excessively burdening cloud participants and being unsuitable for the many short-lived functions typical in serverless computing. This motivates us to propose a new solution: Litmus pricing, which discounts prices based on the system congestion while remaining lightweight and imposing no additional overhead.


==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/05_design.tex <==
\section{Litmus Pricing}
\subsection{Overview}

% The estimated prices of serverless functions should reflect the congestion level of the system inside their machines. With the massive short-living functions, the serverless system's state can dramatically change in a short time. Accordingly, the system state can be congested at any moment and also resolved in a short time. However, such a temporary traffic jam may significantly impact the performance of short-living functions. Therefore, assessing the congestion must be lightweight, quick, and on time. However, a prior approach, POPPA\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling with considerable performance overheads, preventing them from wide adoption. Instead, we propose a new scheme, Litmus pricing, that quickly estimates system congestion at the start of every function and reflects the estimation into pricing the function. 
The estimated prices of serverless functions should reflect the system's congestion state. The presence of numerous small transient functions within the serverless system can rapidly alter its congestion state, causing sudden congestion or swift resolution. Nevertheless, such transient traffic jams can significantly impact the performance of short-lived functions. Thus, assessing the congestion must be lightweight, quick, and timely. However, a prior approach, POPPA~\cite{tiwari2013enabling,alex2013ScFairPrice}, relies on sampling, which incurs considerable performance costs, thereby limiting its widespread adoption. Alternatively, this study introduces Litmus pricing, which promptly gauges system congestion at the onset of each function and reflects the estimated congestion level into pricing the function.

% Like the prior approach~\cite{tiwari2013enabling,alex2013ScFairPrice}, Litmus pricing suggests that the service provider discounts when a tenant's functions are intervened, compensating for the performance loss. To determine the discount ratio, Litmus measures system congestion level, which can also help service providers evaluate remaining resources and make decisions on job scheduling. 
Like the prior approach, Litmus pricing suggests that service providers should offer discounts when a tenant's functions experience interference, thus compensating for the performance loss. Litmus pricing determines the discount rate based on the system's congestion level. Evaluating congestion also assists providers in estimating remaining resources and making informed decisions regarding job scheduling.

%Nevertheless, the Litmus pricing does not quantify each function's slowdown; the discount amount is determined only by the severity of the measured congestion. The impact of the congestion on distinct functions appears differently despite facing the same congestion level, and precisely estimating a function's performance loss is a complex problem. That's why the prior approach had to rely on expensive sampling. Instead, the Litmus pricing avoids the overheads and limits the service provider's responsibility to measure the current congestion. 
However, Litmus pricing does not quantify the slowdown of each individual function; the discount amount is solely determined by the severity of the measured congestion. Even though different functions face the same congestion level, their respective impacts can vary, making precise estimation of each function's performance loss a challenging task. This complexity necessitated the expensive sampling relied upon by the previous approach. Instead, Litmus pricing circumvents such overheads and lightens the service provider's burden solely to measure ongoing congestion levels.

% Litmus pricing embodies the varying value of shared resources across different system conditions by applying equal discounts to all functions under the same system condition, although the functions experience different slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that a function that is slowed more than others demands the over-crowded resources more while exacerbating the adverse over-crowded conditions. Litmus pricing does not provide additional compensation for their extra loss compared to others due to their heavy use of shared resources.
Litmus pricing captures the dynamic significance of shared resources under varying system conditions by offering uniform discounts to all functions under the same system congestion, regardless of their individual slowdowns. Embedded within this policy is the distribution of pricing responsibility to both parties. During periods of system congestion, shared resources become more valuable and meaningfully influence a function's performance. We observed that functions experiencing larger slowdowns tend to demand more of the crowded resources, thereby exacerbating adverse overcrowded conditions. However, Litmus pricing does not offer additional compensation for the larger loss experienced by functions that use shared resources more heavily than others.

% As a result, Litmus inherently incentivizes users who use shared resources sparingly. When over-crowded, functions with minimal needs for shared resources still enjoy discounts but encounter slight slowdowns. This implies that users may take advantage of this policy by minimizing their use of shared resources, receiving substantial discounts despite enduring only minor slowdowns. Such a trade-off is considered acceptable because the user's shared resource usage reduces their contribution to congestion, thereby benefiting the overall system over the other users.
As a result, Litmus inherently incentivizes users who use shared resources sparingly. During periods of overcrowding, functions with minimal needs for shared resources still enjoy discounts but with only slight slowdowns. This implies that users may take advantage of this policy by minimizing their reliance on shared resources, receiving substantial discounts despite only experiencing minor slowdowns. This trade-off is considered acceptable because reduced shared resource usage by users helps mitigate congestion, thereby benefiting the overall system and other users.
% Lastly, the system refrains from scheduling a function if the congestion level exceeds a predetermined threshold, thus preventing resource thrashing.


\subsection{Pricing Model}
\label{pricing model}

% Developing Litmus pricing raises two challenges. First, Litmus needs a new pricing model to estimate a function's price. Second, Litmus needs a way to measure the system's congestion state. Due to the serverless's fast-shifting environment, assessing the congestion must be lightweight and frequent at the right time. Nevertheless, all present commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants must pay more with prolonged execution time when using over-crowded resources. Rather than simply imposing a price by multiplying the main memory usage and a function's total execution time, Litmus suggests the price as a sum of two distinct price components as follows.
Developing Litmus pricing raises two challenges. First, it needs a new model to estimate a function's price. Second, it needs a way to measure the system's congestion state. Due to the rapidly changing environment in serverless computing, assessing congestion must be lightweight and timely. Commercial serverless platforms employ a uniform pricing model regardless of resource congestion dynamics. Consequently, tenants end up paying more for prolonged execution time when using over-crowded resources. Rather than simply imposing the price by multiplying the main memory usage and a function's execution time, Litmus pricing determines the price as a sum of two distinct pricing components as follows.

\begin{equation} 
P = P_{private} + P_{shared}
\end{equation}

% In this equation, \(P\) denotes the total price tenants need to pay to execute their functions. Litmus pricing divides the tenant's price into two pricing components, each with a different resource type. \(P_{private}\) represents the price the tenant needs to pay for private resources, which are entirely assigned to a tenant. \(P_{shared}\) is the price the tenant needs to pay for the shared resources. Each price component is measured proportional to a user's time to occupy the corresponding resources. However, such occupied time can be extended when contention disturbs a process's execution in the shared resources. This delayed time increases a tenant's price unfairly. 
In this equation, \(P\) denotes the total price tenants must pay to execute their functions. Litmus pricing divides this cost into two pricing components, each associated with a different resource type. \(P_{private}\) is the cost for private resources, which are entirely assigned to a single tenant. \(P_{shared}\) is the cost for shared resources. Each pricing component is measured proportional to the time users occupy the respective resources. However, if contention disturbs a process's execution in the shared resources, the occupied time will be extended. This delay unfairly increases the tenant's cost. 


\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/slowdownRunwith26Rev}\\
\caption{\(T_{private}\) and \(T_{shared}\) of applications that run with 26 others, normalized to those when running alone}
\vspace{-0.5em}
\label{fig:slowdownRunwith26Rev}
\end{figure}

% Using Perf, we measure the delays due to the shared resources and split a function's execution time into two distinct slices: one slice, \(T_{private}\), which is time spent on private resources and another slice, \(T_{shared}\), which is time spent on shared resources. Figure~\ref{fig:normalizedTcore&Tuncore-runWith16} shows the impact of the contentions on each time slice, where we normalize \(T_{private}\) per instruction and \(T_{shared}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 207\% on average and 364\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions. 

% We observe that the system congestion influences the occupied time for each resource type differently. The time to hold private resources is slightly affected, with minor changes, even under heavy congestion. Meanwhile, the time due to shared resources is broadly affected, showing significant differences. Thus, we separately measure the two delays and charge their use with a different rule.
We observed that system congestion influences the occupied time for each resource type differently. The time to use private resources is only slightly affected, with minor changes, even under heavy congestion. In contrast, the time spent on shared resources is broadly affected, showing significant differences. Thus, we separately measure the delays for the two resource types and apply different charging rules for their use. 

% Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where we normalize \(T_{shared}\) per instruction and \(T_{private}\) per instruction to the same tests when running alone. The figure shows that \(T_{shared}\) is affected significantly if the system gets congested, compared to \(T_{private}\). A function's \(T_{shared}\) increases by 181\% on average and 488\% at worst. Meanwhile, \(T_{private}\) only increases by 4\% with minor variance between functions.
Using Perf~\cite{perfWiki}, we split a function's execution time into two slices: \(T_{private}\), the time spent on private resources, and \(T_{shared}\), the time spent on shared resources. Litmus pricing collects \(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is calculated as the total execution cycles to complete the application minus \(T_{shared}\). Figure~\ref{fig:slowdownRunwith26Rev} shows the impact of the contentions on each time slice, where \(T_{shared}\) per instruction and \(T_{private}\) per instruction are normalized to the same tests when running alone. The figure shows that \(T_{shared}\) is significantly affected by system congestion compared to \(T_{private}\). On average, \(T_{shared}\) increases by 181\%, with a maximum increase of 488\%. Meanwhile, \(T_{private}\) increases by only 4\%, with minor variance between functions.

% This figure gives insights into two key factors. First, the congestion in the shared resources does not impact the performance of private resources. Accordingly, when the system gets congested, the degree of a function's dependence on the shared resources determines the function's performance. If the \(T_{shared}\) takes a minor portion of a function's execution, severe congestion still barely influences its overall execution. Second, hardware PMUs available in modern CPUs, and profiling tools such as Linux Perf are widely available and can be used to distinguish the usage of shared and private resources. Across the paper, we will take advantage of such tools to develop Litmus pricing.
This figure highlights two key factors. First, congestion in shared resources has a negligible impact on the performance of private resources. Accordingly, when the system gets congested, the extent of a function's reliance on shared resources determines its performance. If \(T_{shared}\) constitutes a minor portion of a function's execution, even severe congestion will have minimal impact on its overall execution. Second, hardware Performance Monitoring Units (PMUs) in modern CPUs and profiling tools like Linux Perf are widely available and can be utilized to differentiate between the use of shared and private resources. Throughout this paper, we will leverage these tools to develop Litmus pricing.

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/TpriTshardDistriRev}\\
% \caption{\(T_{private}\) and \(T_{shared}\) distribution when they run alone}
\caption{Execution time distribution of \(T_{private}\) and \(T_{shared}\)}
\vspace{-0.5em}
\label{fig:TpriTshardDistriRev}
\end{figure}

% Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) in a function's execution. The compute-intensive workloads (e.g., fib-py, float-py) have a substantial \(T_{private}\) portion that can reach 99.96\% of the execution time. However, the portion decreases when running memory-intensive workloads such as fib-nj. This distribution indicates how much other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase float-py's \(T_{shared}\), its total execution time, $T_{private}+T_{shared}$, will undergo minor change.
Figure~\ref{fig:TpriTshardDistriRev} shows the distribution of \(T_{private}\) and \(T_{shared}\) during a function's execution. Compute-intensive workloads (e.g., fib-py, float-py) exhibit a substantial \(T_{private}\) portion, accounting for up to 99.96\% of the execution time. However, this portion decreases when running memory-intensive workloads such as fib-nj. This distribution reflects how other co-running functions can influence its execution. For example, although running float-py in a crowded system may increase its \(T_{shared}\), the total execution time, $T_{private}+T_{shared}$, will undergo only a minor change.

% For each pricing component, we calculate the price by multiplying its charging rate with its time distribution. Thus we can further update the pricing equation.
After collecting the time slices spent on each resource, Litmus calculates each pricing component by multiplying two different charging rates with corresponding slices. Consequently, a new pricing equation emerges as follows:

\begin{equation} 
P = R_{private} * T_{private}  + R_{shared} * T_{shared}
\end{equation}

% \(T_{shared}\) is the cycles stalled due to L2 misses. It is measured from the perf counter, STALLS\_L2\_Misses. \(T_{private}\) is the total execution minus STALLS\_L2\_Misses. 
% Using Perf, Litmus collects\(T_{shared}\) by reading the cycles stalled due to L2 cache misses. \(T_{private}\) is the total cycles to complete the application minus \(T_{shared}\). 
% While Litmus returns the system's congestion state, the service provider still needs to determine reasonable prices charged for a service when having different congestion levels. 

% \(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. Again, the two charging rates are necessary since each component is affected differently, directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from the crowded execution environment. Thus, the charging rates should be measured as follows.
\(R_{private}\) and \(R_{shared}\) are the charging rates for private and shared resources, determined by the congestion level. These two charging rates are necessary because each component is affected differently, either directly or indirectly. The charging rate determines the actual discount amount, reflecting the degradation of applications' performance caused by interference from a crowded execution environment. Thus, the charging rates should be measured as follows:

\begin{equation} 
R = R_{base} * \frac{T_{solo}}{T_{congestion}}
\end{equation}

% In this equation, \(R\) is the charging rate for executions on either private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free execution environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is the execution time when the function runs alone, and \(T_{congestion}\) is its execution time in the congested environment. Again, we should collect a separate \(T_{solo}\) and \(T_{congestion}\) for each pricing component. To measure \(T_{solo}\), \hl{the prior work}~\cite{alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. Litmus pricing avoids such a costly approach but presumes the function's \textit{solo} performance by examining reference workloads on the system.
In this equation, \(R\) represents the charging rate for executions on private or shared resources. \(R_{base}\) is the base charging rate when the function runs in a congestion-free runtime environment; our tests select 1 for \(R_{base}\). \(T_{solo}\) is its non-interfered execution time when the function runs alone, and \(T_{congestion}\) is its execution time in a congested environment. We need to collect separate \(T_{solo}\) and \(T_{congestion}\) values for each pricing component. To measure \(T_{solo}\), the prior study~\cite{tiwari2013enabling,alex2013ScFairPrice} employs an expensive approach that suspends all co-running applications whenever sampling an application's non-interfered performance. However, Litmus pricing avoids such a costly approach by presuming the function's solo performance through reference workloads on the system.

% Litmus pricing requires both providers and tenants to be involved in the price decision. The providers need to decide on reasonable rates for each resource use by analyzing the selected representative functions running on the system. To offer reasonable discounts, the providers must choose the functions analyzed carefully, collecting the functions representing the system. The tenants must also know the consequences when their tasks heavily rely on any of the shared resources. Unfortunately, their tasks may get delayed more than the provider's expectation while still receiving the discount rate up to the expectation. 
Litmus pricing requires both providers and tenants to be involved in the price decision process. Providers need to establish reasonable rates for each resource usage by analyzing selected representative functions. To offer fair discounts, providers must carefully choose the functions to be analyzed, ensuring the functions accurately represent the system condition. Tenants must also know the consequences when their tasks heavily rely on shared resources. Unfortunately, their tasks may get delayed more than the provider's expectations while still receiving the expected discount rate. 

% Here, the Litmus pricing reflects the varying value of the shared resources when the system's congestion level changes; the importance of shared resources becomes more valuable when congested. 



==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/06_design_details.tex <==
\section{Estimating prices with Litmus}
\label{sec:designDetails}

% The providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}, before using Litmus pricing. The numbers in both tables are the slowdowns of codes while testing the system congestion. Shortly, the congestion table is filled with the slowdowns of startup codes, and the performance table is filled with the slowdowns of reference benchmarks. Litmus pricing needs three steps to charge the final price with a discount. First, the providers assess the system's congestion at multiple levels and range them in a table. This step completes the congestion table. Second, the providers study the impact of congestion on tenants' functions and complete the performance table. Lastly, the service provider determines a tenant's price based on the two tables. 
Before using Litmus pricing, service providers need to complete the congestion and performance tables, shown in Figure~\ref{fig:litmust_tables}. The congestion table lists the slowdowns during the startup phases, whereas the performance table lists the slowdowns of reference functions. Litmus pricing needs three steps to determine the final price with a discount. First, providers assess system congestion at multiple levels and record the results in the congestion table. Second, providers analyze the impact of congestion on reference functions and fill out the performance table. Lastly, providers determine a tenant's price based on the data from both tables.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tables}\\
\caption{Congestion and performance tables: numbers in both tables indicate the slowdowns of startup codes and reference functions, collected with CT-Gen and MB-Gen}
\vspace{-0.7em}
\label{fig:litmust_tables}
\end{figure}

\textbf{Step 1, Defining Congestion Levels:} We manage the system's congestion levels using two traffic generators that create a range of congestion states by stressing shared resources differently. The traffic generator is multi-threaded, creating traffic in shared resources to incur congestion, with each thread running on a separate core. We rank the stress levels from 1 to 32 by changing the number of active threads running on distinct cores. Entries from top to bottom in the congestion table indicate increasing stress levels.

% \begin{figure}[h]
% \centering
% \vspace{-1.5em}
% \includegraphics[width=1\columnwidth]{./fig/stressing_specs}\\
% \vspace{-1em}
% \caption{stressing program's instruction, L3 accesses and L3 misses }
% \vspace{-0.5em}
% \label{fig:stressing_specs}
% \end{figure}

% \textbf{Step 2. Measuring System Congestion:} Measuring the current level of system congestion that may influence a function's performance is a crucial challenge. If we assume that the platform does not have pre-profiled information about a function's performance, the platform cannot figure out whether co-running functions influenced the function. Additionally, the serverless platform's fast-changing states with massive short-living functions make the assessment even more complicated, requiring quick and frequent examinations.

% Meanwhile, measuring the amount of a system's congestion and its impact on performance is a crucial challenge. This challenge particularly stands apparent when being demanded to quantify the impact of the congestion on a running application without pre-profiled information about the application. Moreover, the serverless platform's fast-changing system states with \hl{numerous} short-lived functions make the assessment even more complicated, requiring quick and frequent performance examinations.
Measuring the amount of system congestion and its impact on performance is a crucial challenge. This challenge becomes particularly pronounced when trying to quantify the impact of the congestion on a running application without pre-profiled information about the application. The fast-changing system states of a serverless platform, with numerous short-lived functions, further complicate the assessment, necessitating quick and frequent performance examinations.

% Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. The proposal is based on the observation that high-level languages, such as Python and Node.js, used in serverless computing have long startup times to accommodate their runtime environments. Since the inception of serverless computing, these startups have been recognized as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests leverage these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests further validated that all tested functions exhibited similar performance characteristics during their startups. 
Litmus pricing includes a novel method, named a \textit{Litmus test}, that examines the system's state quickly without imposing additional overheads. This method leverages our observation that high-level languages like Python and Node.js, commonly used in serverless computing, have lengthy startup phases to accommodate their runtime environments. Since the inception of serverless computing, these startup delays have been identified as a major source of latency issues~\cite{ismail2018quantitative}. Litmus tests exploit these startups to read the system's state, utilizing their fixed routines with consistent operations. Our tests have validated that tested functions exhibit similar performance characteristics during startup phases. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_all}\\
% \caption{IPC for serverless applications with different runtimes in the first 100 milliseconds of their execution}
% \vspace{-0.5em}
% \label{fig:startupIPC_all}
% \end{figure}

\begin{figure}[h]
\centering
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped}\\
% \includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped-1}\\
\includegraphics[width=1\columnwidth]{./fig/startupIPC_grouped_3}\\
% \caption{IPC for serverless applications grouped by language runtime in the first 100 milliseconds of their execution}
\caption{IPC of serverless applications based on languages (Go, Python, and NodeJS) during their startup phase}
% \vspace{-0.7em}
\label{fig:startupIPC_grouped}
\end{figure}

% Figure~\ref{fig:startupIPC_grouped} depicts the fluctuation in IPC (Instructions Per Cycle) of a function during the first milliseconds of its execution. The x-axis shows a time flow since the beginning; every tick indicates a millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language, and the throughput of each group is represented in separate figures. Although figures exhibit different patterns, functions in the same figure display notable similarities. The figures imply that functions written in the same language have nearly identical startups.
Figure~\ref{fig:startupIPC_grouped} depicts a function's fluctuation in IPC (Instructions Per Cycle) during its startup phases. The x-axis represents the time elapsed since the beginning, with each tick indicating one millisecond. The y-axis shows the function's IPC measured for a millisecond at corresponding time intervals. We picked functions with different languages and characteristics from those listed in Table~\ref{tb:benchmarks}. These functions were categorized into three groups based on language runtime, and the IPC of each group is presented in separate figures. As shown in these figures, functions in the same figure show notable similarities. This implies that functions written in the same language have nearly identical startups.

% The startup of a runtime usually includes bursts of memory reads to load images and libraries, which can probe the traffic in the shared resources. By conducting a Litmus test before executing every tenant's codes, the providers can observe the system state for the function. Meanwhile, the providers also need to study how the startup codes perform in different system states. They complete the congestion tables by performing the Litmus tests with the startups written in three languages while varying the congestion levels. To this end, the information in the congestion table is looked up when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}. 
% estimating the system's state upon receiving a result of a function's Litmus test. 
The startup of a runtime typically includes bursts of memory reads to load images and libraries, which can be used to probe the traffic in shared resources. By conducting a Litmus test before executing a tenant's function, providers can assess the system state. Meanwhile, providers also need to study how startup phases perform under different system states. They complete the congestion tables by conducting the Litmus tests with startups written in three languages while varying congestion levels. This information from the congestion table is then referenced when constructing the congestion model in Figure~\ref{fig:referenceStartupSlowdownRev}.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/Litmus_tests}\\
\caption{Progress of serverless applications on four cores with Litmus tests (dotted arrows) over time}
% \vspace{-0.5em}
\label{fig:Litmus_tests}
\end{figure}

% Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests. The Litmus tests examine the level of system congestion with every function startup. \hl{Many} concurrent functions in serverless offer frequent test opportunities. Function\#1 is a memory-intensive function that raises a congestion level. While active, Litmus tests measure the congestion level above 8. After Function\#1's completion, the next Litmus test detects a non-congested system with a congestion level below 3. However, with the start of another heavy function, function\#2, the Litmus tests measure the new congestion in the system.
Figure~\ref{fig:Litmus_tests} shows the progress of serverless functions with Litmus tests, which examine the level of system congestion during each function's startup. Many concurrent functions in serverless offer frequent opportunities for testing. Function \#1, which is memory-intensive, causes congestion levels to rise above 8 during its execution. A Litmus test in Core 3 detects this congestion. After Function \#1 is complete, a subsequent Litmus test indicates a non-congested system with a congestion level below 3. However, during another resource-intensive function, Function \#2, the Litmus test identifies new system congestion with a level above 9.  

% \textbf{Step 2. Measuring the Impact of Congestion:} Although discerning the system congestion through the Litmus test, estimating its impact on a user's application is another challenge. This work proposes a discount based on the pre-studied impacts on reference functions, assuming the user's functions are alike. For this, the service providers need to select reference functions that represent users' functions running on their systems. In this work, we select the workloads in \hl{Section 2} as our reference applications. 
\textbf{Step 2, Measuring the Impact of Congestion:} Discerning system congestion through the Litmus test solves only one of the two challenges; the other is determining its impact on a tenant's function. Different tenants' functions could experience varying degrees of slowdown under the same congestion level. To address this, we propose using pre-selected reference functions to analyze these impacts, thereby avoiding the cost of runtime profiling. For this, providers need to carefully select reference functions that represent tenants' functions operating on the systems, as these selections influence the overall accuracy of congestion measurement. Later, in Section~\ref{sec:evaluation}, our tests will show that pre-selected reference functions can effectively represent unknown user applications. For this study, the selected reference applications (* marked) are listed in  Table~\ref{tb:benchmarks}. 

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/refSlowdownStressing14}\\
% \includegraphics[width=1\columnwidth]{./fig/slowdownStressing16}\\
\caption{\(T_{private}\), \(T_{shared}\), and \(T_{total}\) of serverless applications that run with MB-Gen at stress level 14, normalized to their execution time when they run alone}
% \vspace{-0.5em}
\label{fig:refSlowdownStressing14}
\end{figure}

% Once the reference functions are ready, the providers study the slowdowns of the reference functions while varying different congestion levels again. This study completes the performance table in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. Again, our two traffic generators create two separate sub-tables. All entries in this table are 1-to-1 mapped to entries in the congestion table. The providers estimate a general function's slowdown when having a certain congestion level using this 1-to-1 mapping.
Once the reference functions are ready, providers analyze their slowdowns under varying congestion levels. This analysis completes the performance table shown in Figure~\ref{fig:litmust_tables}. Each entry in the table holds the geometric average of all reference functions' slowdowns at the corresponding stress level. With two traffic generators, providers can complete another set of two sub-tables for the performance table. All entries in this table are mapped 1-to-1 to entries in the congestion table. Providers can estimate a general function's slowdown at a given congestion level using this one-to-one mapping.

% Figure~\ref{fig:refSlowdownStressing14} shows the reference functions' slowdowns when stressing the system. The X-axis shows different functions, each consisting of three bars: the first two bars show the CPI during each time slice, \(T_{private}\) and \(T_{shared}\), and the last bar shows the CPI of an entire execution. The figure shows that the tested functions suffer from different amounts of slowdowns, although the tests maintain consistent stress levels. \hl{The last group} shows the gmean of all the slowdowns, which is used when providers estimate a function's slowdown later. 
Figure~\ref{fig:refSlowdownStressing14} shows an example of the reference functions' slowdowns when stressing the system. The X-axis shows tested functions, each depicted with three bars: the first two bars show \(T_{private}\) and \(T_{shared}\), while the last bar shows the total execution time, all normalized to their execution time when running alone without interference. The figure shows that the tested functions experience varying degrees of slowdown despite consistent stress levels maintained during the tests. The next-to-last group shows the gmean of all the slowdowns, which providers use to estimate a function's slowdown later.

% \hl{This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.}

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/referenceStartupSlowdownRev}\\
\caption{The correlation between the slowdown of Python's startup phase and the slowdown of reference applications. From left, (a) \(T_{private}\), (b) \(T_{shared}\), and (c) \(T_{total}\), normalized to the execution time when running alone}
\label{fig:referenceStartupSlowdownRev}
\end{figure}

% \textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while a range of congestion levels is continuous, the tables only contain a few slowdowns in discrete intervals. Thus, providers need a model that returns an estimated slowdown when receiving a congestion level as an input. In our tests, we employ a linear regression to achieve the model.
\textbf{Step 3, Determining Discount Rates:} Providers can determine a function's price through the Litmus test once the congestion and performance tables are ready. Upon obtaining a Litmus test result, the current congestion level is estimated by comparing the measured slowdown to the pre-studied slowdowns in the congestion tables. Then, Litmus pricing conjectures a possible slowdown due to the estimated congestion by using the congestion level as an index to the performance table. However, while congestion levels vary continuously, the tables only contain slowdowns at discrete intervals. Therefore, providers need a model that estimates the slowdown for any given congestion level. In our tests, we employ linear regression to develop the model.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/interpolation}\\
\caption{Estimating a function's slowdown with logarithmic interpolation}
\label{fig:interpolation}
\end{figure}

% Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding references' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). We employed two traffic generators to extrapolate a more precise congestion level, yielding two sub-tables in both the congestion and the performance tables. Consequently, the figure presents two linear regression models, each associated with a different traffic generator. 
Our experiments employ linear regression analysis to draw Figure~\ref{fig:referenceStartupSlowdownRev}, which shows the correlation between the two slowdowns. The X-axis shows the startup's slowdown, while the Y-axis shows the corresponding reference applications' slowdowns at the same congestion level. From left to right, the figure shows normalized \(T_{private}\), \(T_{shared}\), and \(T_{total}\). To extrapolate a precise congestion level, we created two sub-tables within both the congestion and performance tables using two distinct traffic generators. As a result, the figure depicts two linear regression lines (red and blue dotted lines), each associated with a different traffic generator.

% The provider needs to estimate the function's slowdown to uncover its price. However, the above two regression models return two vastly different slowdowns. Then, the providers need to determine which model is close to the current environment. We think the two models reflect two extreme congestions that the traffic generators create, one before the L3 and one after the L3. CT-Gen creates massive traffic from the core to the L3 cache, which filters the traffic, preventing the operations from consuming the memory bandwidth. MB-Gen also creates huge traffic but consumes the memory bandwidth and replaces L3 blocks. Since each traffic generator creates an extreme case, the machine state could be intermediate with congestion in the range between the two congestions created by CT-Gen and MB-Gen. However, Litmus pricing cannot answer this question with only the startup's slowdown. 

% To address this question, we note that the system's L3 misses are a critical indicator closely related to a function's performance. Functions suffer more when the system experiences more L3 misses, which stresses the cache space and off-chip memory bandwidth. Accordingly, Litmus test collects the system's L3 miss count as a supplementary index, which tells more about the crowdedness of shared resources.

These regression models return two different slowdowns. To estimate a function's slowdown, providers must determine which model reflects the current environment more accurately. The traffic generators create two extreme congestion scenarios: one before the L3 cache and one after. CT-Gen generates substantial traffic from the core to the L3 cache that filters the traffic and prevents operations from consuming memory bandwidth. Conversely, MB-Gen also generates massive traffic but consumes memory bandwidth and repeatedly evicts L3 cache blocks. Because each traffic generator represents a distinct extreme case, the actual machine state could fall somewhere between the two congestion levels created by CT-Gen and MB-Gen. However, Litmus pricing requires more than just the startup slowdown to identify the machine's state in these models. Thus, we have enabled Litmus tests to gather the system's L3 miss count as a supplementary metric that offers deeper insights into the crowdedness of shared resources.


% \hl{Figure 1} shows how to use the L3 cache misses with the performance sub-tables. The two traffic generators make the upper and lower boundary of the L3 miss rates. When performing a Litmus test, if the test's L3 miss rate is XXX, close to the L3 misses with CT-Gen, we can conclude that the congestion occurs before the L3 cache and select the expected slowdown of XXX. On the contrary, we choose XXX, in case the L3 miss rate is XXX, close to the L3 misses with MB-Gen. If the test's L3 miss rate is in-between, we interpolate the two slowdowns based on the L3 misses, assuming congestion in both resources. 
% Finally, we determine the Rprivate and Rshared based on the expected slowdown from its performance table. Calculating Rprivate and Rshared takes the same steps. The final discount price is computed using the equation with the computed rates. 

% Figure~\ref{fig:interpolation} shows how we employ the L3 misses when estimating the slowdown. The two traffic generators make the upper and lower boundary of the L3 misses. If a Litmus test reports the L3 miss count is 10, close to the L3 misses with CT-Gen, \textcircled{1}Litmus pricing estimates the discount (=expected slowdown) of the function to be near 1\%. This indicates that the congestion happens before the L3, as what CT-Gen creates. On the contrary, in case the L3 misses are 1000, close to the L3 misses with MB-Gen, \textcircled{2}Litmus pricing estimates the function's discount rate close to 6\%. Meanwhile, if the Litmus test reports the L3 misses as 100, we interpolate the two extreme discounts, 1 and 6, based on the L3 misses, assuming current congestion to stand in between the two extreme congestions. The congestion model in the figure shows how we interpolate with logarithmic interpolation. In this figure, \textcircled{3}applying the logarithmic interpolation to the L3 miss count returns the half-point between CT-Gen's 1\% and MB-Gen's 6\%, which is 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 
Figure~\ref{fig:interpolation} shows our approach to using L3 misses to estimate slowdowns. We created two figures illustrating separate regression models. The left figure (a) is derived from the startup slowdowns and L3 misses with logarithmic regression, indicating L3 misses at specific congestion levels. The right figure (b) is derived from the performance table with linear regression, displaying discounts at specific congestion levels. Each figure depicts two regression lines associated with different traffic generators.

The two traffic generators set the upper and lower boundaries for L3 misses. For instance, if a Litmus test reports 10 L3 misses, close to what CT-Gen generates: \textcircled{1}This suggests congestion occurs before reaching the L3 cache, similar to CT-Gen's scenario. Thus, Litmus pricing estimates the function's discount to be around 1\%. Conversely, if the Litmus test reports 1000 L3 misses, close to MB-Gen's results: \textcircled{2}Litmus pricing estimates the function's discount rate to be approximately 6\%, indicating congestion similar to MB-Gen, where memory bandwidth is heavily consumed and L3 cache blocks are frequently evicted. When the Litmus test reports 100 L3 misses, an interpolation between these extremes is applied: \textcircled{3}Using logarithmic interpolation, Litmus pricing estimates the function's discount rate to be midway between CT-Gen's 1\% and MB-Gen's 6\%, resulting in approximately 3.5\%. Upon obtaining the discount rates, Litmus pricing computes the final price, as discussed in Section~\ref{pricing model}. 



==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/07_litmus_test.tex <==
\section{Testing System Congestion}
\label{sec:congestion}

Before estimating a function's slowdown, Litmus needs to analyze the slowdowns of the language runtimes and reference functions. One challenge is that the functions and the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from both congestion types but differently, drawing two other figures. However, the service providers need to guess either system state when reading their startup's slowdown. That is to say, the service provider may estimate the system state incorrectly. 

To handle this, we developed two traffic generators discussed in section 3 to create their slowdowns. Our traffic generators separately create two different types of congestion in the system. CT-gen creates large traffic from the core to the L3 cache, which filters the traffic, preventing the traffic from consuming the memory bandwidth. MB-gen also creates large traffic that consumes the memory bandwidth and replaces the L3 cache blocks. We observed that functions suffer more when there is congestion in the L3 cache or after compared to when having congestion before the cache. Accordingly, our two generators create two extreme congestions, one before the L3 and one after the L3, and we expect most system congestions to belong in the range between these two. 

Before estimating system congestion, Litmus studies the impact of system crowdedness. However, estimating the system state using the limited records collected with the two generators is still another challenge. In our case, the startup may suffer the same slowdown under different system states. Figure X shows the startup's slowdowns with the two traffic generators. The two traffic generators create congestion in different resources, resulting in different congested systems. The startup suffers from each congestion type differently, drawing two other lines. However, Litmus needs to guess either system state when reading the startup's slowdown. That is to say, Litmus may evaluate the system state incorrectly. 

\begin{figure}[h]
\centering
\vspace{-0.8em}
\includegraphics[width=1\columnwidth]{./fig/startup_l3MPKI_slowdown}\\
\vspace{-1em}
\caption{The correlation between the l3MPKI and slowdowns of Python's startup phase}
\vspace{-0.5em}
\label{fig:startup_l3MPKI_slowdown}
\end{figure}

\textbf{Congestion Level Interpolation:} One solution is to look up another stat that contains additional information to unriddle the question. In our case, where we split the shared resources into resources before and after the L3 cache, the number of L3 cache misses can be a supplementary index, telling more specifics about the congestion. Figure~\ref{fig:startup_l3MPKI_slowdown} illustrates the correlation between the startup's L3 MPKI and \(T_{uncore}PerInst\). The X and Y axes are \(T_{uncore}PerInst\) and L3 MPKI, respectively. Each dot is measured in varying congestion levels and normalized to the congestion-free environment. 

When testing the system state, Litmus gets two points representing the congestion levels created by the two traffic generators and a range of congestion levels between the two points. The first solution employs linear interpolation to find a particular point in the range. The point with CT-gen has minimum L3 misses, making the bottom of the range. The interpolation assumes that extra L3 misses from the congestion by CT-gen raise slowdowns more severely until reaching the worst congestion by MB-gen. 

\begin{figure}[h]
\centering
\vspace{-0.5em}
\includegraphics[width=1\columnwidth]{./fig/charging_rates}\\
\vspace{-1em}
\caption{The normalized charging rates based on stressor l3, stressor l2, gap migration and current charging rage}
\vspace{-1em}
\label{fig:charging_rates}
\end{figure}

Figure~\ref{fig:charging_rates} shows the Tcore and Tuncore charging rates change as congestion level increases. The red and blue are the charging rates for the L2 MPKI and L3 MPKI. The black line represents the charging rates based on the current pricing model used by major serverless platforms. Notably, the charging rates for the current platforms remain the same as congestion levels increases. This is because the charging rates only depend on the memory spaces that the customers reserve for the application before the application starts. However, both of our charging rates, XXX and XXX, decrease as the congestion level increase. Our pricing model can dynamically adjust the charging rate based on the current system's impacts on the applications. 




==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/08_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \textbf{Litmus price \& error:}
% We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, and the other consists of selected reference applications to obtain the linear regression models for Litmus pricing. The discount models plug into the Litmus pricing used in our tests. For this experiment, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown.
We split our functions into two groups: as listed in Table~\ref{tb:benchmarks}, one consists of functions to test Litmus pricing, while the other consists of chosen reference applications to derive linear regression models for Litmus pricing. The discount models plug into the Litmus pricing employed in the tests. In this study, we estimate a function's price in three ways: the price using the Litmus pricing, a commercial price that offers no discounts, and an ideal price that provides an exact discount proportional to its slowdown. 

% % original version
% We maintain the congestion state consistent across all tests, co-running each function with 26 other functions. Using Perf~\cite{perfWiki}, we collect the three key stats: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup, which implies the congestion level in these tests, as well as the discount rates that every function receives. We execute every function 100 times and collect the average of the function's \(T_{private}\) and \(T_{shared}\). Finally, we compute each function's \(P_{private}\), \(P_{shared}\), and \(P\), the total price, by summing \(P_{private}\) and \(P_{shared}\).  

\subsection{One Function Per Core}

% revision version
% We maintain consistent congestion states across all tests by co-running each function with 26 other functions. Using Perf, we collect the three key statistics: \(T_{private}\), \(T_{shared}\), and system L3 misses during the first 45 million instructions of the Python startup. These metrics hint at the congestion level during the tests as well as the discount rates that a function receives. Each function is executed 30 times, and the average of its \(T_{private}\) and \(T_{shared}\) is collected. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).
We maintain consistent congestion levels across all tests by co-running each function with 26 other functions. As outlined in Section~\ref{sec:motivation}, whenever a function finishes, another is randomly launched to keep a total of 26 co-running functions. Using Perf~\cite{perfWiki}, we collect three key statistics: \(T_{private}\), \(T_{shared}\), and the machine's L3 misses during the first 45 million instructions of the Python startup. Through these metrics, Litmus pricing estimates the level of system congestion and the discount rates a function receives. Each function is executed 30 times, and we average its \(T_{private}\) and \(T_{shared}\) values. Subsequently, we calculate each function's \(P_{private}\), \(P_{shared}\), and total price (P) by summing \(P_{private}\) and \(P_{shared}\).

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice26Rev}\\
% \caption{The total price for functions computed via Litmus pricing and ideal prices when co-running with 26 other functions normalized to the commercial price that offers no discount}
\caption{Prices computed via Litmus pricing and ideal prices when co-running with 26 other functions, normalized to the commercial price that offers no discount}
\label{fig:normalizedPrice26Rev}
\end{figure}

% In Figure~\ref{fig:normalizedPrice26}, we can see a minimal difference in the discount rate between the Litmus price and the Ideal price. The average Litmus discount rate stands at 11.5\%, which is only marginally larger by 0.6\% than the average Ideal discount rate of 10.9\%. Also, we can see that the difference between the Litmus price and Ideal price are different among the applications. Certain applications exhibit higher Litmus prices compared to the Ideal price, while conversely, some applications demonstrate smaller Litmus prices. 
 %Figure~\ref{fig:priceErrorRunwith26} shows further details, analyzing the errors in each pricing component. 

% Figure~\ref{fig:normalizedPrice26Rev} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{10.66\%}, which is only marginally larger by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{10.28\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice26Rev} illustrates estimated prices derived from Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices to offset delays in a congested execution environment. The figure shows minimal disparities between the two prices, implying that Litmus pricing offers a reasonable discount. The average discount from Litmus pricing across all functions is 10.7\%, which is only marginally higher by 0.4\% compared to the average slowdown experienced by functions, which stands at 10.3\%, as depicted by the ideal price.

% However, the discount rates per slowdown differ among functions. For instance, float-py's ideal discount rate is \hl{0.05\%}, but it enjoys a \hl{4.31\%} discount with the Litmus pricing. Meanwhile, pager-py's performance drops by \hl{15.63\%} while receiving a \hl{13.87\%} discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more easily affected than the reference when congested. In contrast, float-py runs mostly with private resources, receiving a minor impact from the execution environment. Figure~\ref{fig:priceErrorRunwith26Rev} shows further details, analyzing the differences in each pricing component.
However, the discounts per slowdown differ among functions. For instance, float-py's ideal discount rate is 0.05\%, but it benefits from a 4.3\% discount with Litmus pricing. Conversely, pager-py encounters a 15.6\% performance decline while receiving only a 13.9\% discount. As shown in Figure~\ref{fig:TpriTshardDistriRev}, pager-py relies more on shared resources with a longer \(T_{shared}\), implying that pager-py's execution time is more susceptible to congestion than the references. In contrast, float-py predominantly utilizes private resources, resulting in minimal impact from the execution environment. Further insights into these variations in each pricing component are presented in Figure~\ref{fig:priceErrorRunwith26Rev}.


% From figure~\ref{fig:tcore\(T_{private}\)Distr}, we know that \(T_{private}\) dominates the execution time among all applications. The impact from \(T_{private}\) error has a bigger impact on the overall error. The slowdowns due to congestion in private resources are small. Theoretically, there should be no slowdowns when using private resources, but we observed that the congestion still influences it. The observed slowdown is 000, a small difference from an ideal slowdown. Meanwhile, the slowdowns in shared resources are significant. We observe that 

% % \[  Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}}\]

% \[Weighted Private Price Error = \frac{R_{privateLitmus} * T_{core}}{TotalIdealPrice}\]
% \[TotalIdealPrice = R_{privateIdeal} * T_{core}  + R_{sharedIdeal} * T_{uncore}\]

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/priceErrorRunwith26Rev}\\
\caption{Weighted errors in prices derived from Litmus pricing, which are compared to ideal prices}
% \vspace{-1em}
\label{fig:priceErrorRunwith26Rev}
\end{figure}

%%% We discuss error
% In figure~\ref{fig:priceErrorRunwith26} we can see that there are some applications receive positive errors and some receive negative errors.  A negative error indicates that our estimated slowdown for that application is higher than its actual slowdown, resulting in greater compensation than the observed performance losses. On the other hand, a positive error indicates that the compensation is smaller than its real slowdown. For most applications, the Litmus price is slightly higher than the Ideal price, with minimal differences. The highest price error is 0.0389 for auth-nj, while the lowest error is 0.007 for dyn-py. The geometric mean of the absolute error is 0.018. 
% Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors that each function experiences. The error rate is computed as the difference between the estimated and the ideal prices over the ideal price. The first two bars show the errors in \(P_{private}\) and \(P_{shared}\), which are weighted by their corresponding ratio in the execution time, considering their impacts, as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. The functions can have two different errors: positive and negative. A positive error indicates that the Litmus-estimated price is higher than its ideal price, implying that it receives smaller compensation than its performance losses. In other words, Litmus pricing estimates its slowdown to be less than its actual slowdown. A negative error implies the opposite; a function's compensation is higher than its slowdown. This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others. Meanwhile, the tenants need to acknowledge the consequences if their functions differ vastly from the reference workloads, heavily relying on shared memory.
Figure~\ref{fig:priceErrorRunwith26Rev} depicts the weighted errors each function experiences. The error rate is computed by comparing the estimated prices with the ideal prices and dividing the difference by the ideal prices. The first two bars show errors in \(P_{private}\) and \(P_{shared}\), weighted by their corresponding ratios in execution time, reflecting their impacts as shown in Figure~\ref{fig:TpriTshardDistriRev}. The last bar shows the error in their total execution time. Functions may have two types of errors: positive and negative. A positive error means that the estimated price exceeds its ideal price, implying that the compensation received is less than the performance loss incurred. In other words, Litmus pricing underestimates the slowdown relative to the actual slowdown. Conversely, a negative error indicates the opposite; a function's compensation exceeds its slowdown. This discrepancy indicates Litmus pricing may offer varying advantages to different functions, favoring those with lesser slowdowns. Meanwhile, tenants must recognize the consequences if their functions differ vastly from the references, particularly those heavily reliant on shared resources.

% Delete the followings
% This result indicates that the Litmus pricing may reward each function differently, offering more advantages to functions that are slowed less than the others, such as visual-py and fib-go. Meanwhile, the tenants need to understand the consequences if their functions differ vastly from the reference workloads from the shared resource perspectives.

% The largest absolute error is \hl{0.0723} for rate-go, while the smallest absolute error is \hl{0.0039} for \hl{mst-py}. Overall, the Litmus pricing shows minor errors with an average of \hl{0.0231}. With further details, the Litmus pricing accurately estimates the slowdowns in \(P_{private}\) with \hl{0.0175} of an average weighted error rate. \(P_{private}\)'s highest weighted error rate is \hl{0.079}, yet minor, while the lowest rate is only \hl{0.0008}. The weighted error rate for the estimated \(P_{shared}\) is also small. The average error rate for \(P_{shared}\) is \hl{0.0068}, even lower than for \(P_{private}\). \(P_{shared}\)'s highest error rate is \hl{0.0404}.
% The largest absolute error is 0.072, which occurs with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, the Litmus pricing exhibits minor errors, averaging 0.023, \hl{with the estimated discount differing by 22.5\% over the ideal discount.} With more details, Litmus pricing accurately estimates slowdowns in \(P_{private}\), with an average weighted error rate of 0.018. \(P_{private}\)'s highest weighted error rate is 0.08, yet minor, while the lowest rate is only 0.0008. The weighted error rate for estimated \(P_{shared}\) is similarly small, averaging at 0.0068, even lower than for \(P_{private}\). The highest error rate for \(P_{shared}\) stands at 0.04.
The largest absolute error is 0.072, occurring with rate-go, while the smallest absolute error is 0.004 with mst-py. Overall, Litmus pricing exhibits minor errors, averaging 0.023. Thus, the estimated discount deviates by 22.5\% from the ideal discount. Note that Litmus pricing aims to match the average discount across all functions by applying a system-wide discount based on the system's congestion level rather than adjusting the discount for each function individually. Consequently, individual functions may experience either positive or negative errors. However, it is noteworthy that the average discount between Litmus and ideal pricing differs by just 0.4\%, as illustrated in Figure~\ref{fig:normalizedPrice26Rev}, satisfying its objectives.
% This policy may incentivize some functions while penalizing others based on shared resource usage. 
Specifically, Litmus pricing estimates slowdowns in \(P_{private}\) with an average weighted error rate of 0.018. The highest for \(P_{private}\) is 0.079, while the lowest is just 0.001. For \(P_{shared}\), the average weighted error rate is even lower, at 0.007. The highest for \(P_{shared}\) is 0.040.


% Litmus employs the average performance of applications to determine the discount rate applied universally. In this context, an application encounters a positive error when its speedup is less than the estimated average speedup across all applications. Also, the error rate depends on the difference between the actual speedup and the estimated average speedup, with larger differences resulting in more significant errors for the given application.
% As discussed in Figure~\ref{fig:TpriTshardDistri}, \(T_{private}\) dominates the execution time across all applications, implying that a small error in the estimated \(T_{private}\) largely influences the execution time. This explains why, for functions that demand little shared resources, such as float-py and chame-py, the error in P is almost identical to that in \(T_{private}\), and errors with \(T_{shared}\) can be overlooked. In contrast, for functions with a larger \(T_{shared}\) ratio, such as pager-py and mst-py, errors in \(T_{shared}\) meaningfully affect the total execution time. Note that the Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price.  

Litmus pricing estimates each pricing component separately with an individual discount rate. For functions that demand minimal shared resources, such as float-py, the errors in P are nearly identical to those in \(T_{private}\), and the errors in \(T_{shared}\) can be overlooked. As shown in Figure~\ref{fig:TpriTshardDistriRev}, \(T_{private}\) dominates the execution time across many applications. While even a small error in the estimated \(T_{private}\) influences the function's execution time, substantial errors in \(T_{shared}\) likely have limited impacts, except for functions that have a relatively meaningful \(T_{shared}\) ratio, such as pager-py and mst-py, whose errors in \(T_{shared}\) are observable in the total price. 

% We emphasize that Litmus pricing cannot avoid producing a certain degree of errors since it does not track each function's slowdown. However, the figure proves that the Litmus pricing can catch the congested environment well and reflect it in the price. We observe that functions have similar slowdowns in \(T_{private}\) with slight variation when congested. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, also estimating reliable total prices since \(T_{private}\) mostly dominates the execution time. The \(T_{shared}\) fluctuates more dynamically across functions with a relatively large error, but the error's impact is little, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}. 
We emphasize that Litmus pricing cannot avoid producing a certain degree of error since it relies on estimation using a few metrics. However, the figure proves that Litmus pricing effectively captures a congested environment and reflects that environment in the price. Under the same congestion level, \(T_{private}\) values of all functions are delayed similarly with a little variation. Thus, the Litmus pricing can precisely estimate the \(P_{private}\) with the Litmus test, leading to reliable total price estimates since \(T_{private}\) generally dominates execution time. \(T_{shared}\) fluctuates more dynamically across functions and has a relatively larger error, but the impact of this error is minimal, as shown in Figure~\ref{fig:priceErrorRunwith26Rev}.

\begin{figure}[h]
\centering
% \vspace{-5em}
 \includegraphics[width=1\columnwidth]{./fig/normTprivtTshared26Rev}\\
% \vspace{-5.5em}
\caption{\(T_{private}\) \& \(T_{shared}\) of applications when co-running with 26 others, normalized to those when they run alone. The top(black) and bottom(blue) lines are discount rates from Litmus pricing for \(T_{private}\) and \(T_{shared}\)}
% \vspace{-1em}
\label{fig:normTprivtTshared26Rev}
\end{figure}

% To further investigate the price error differences, in igure~\ref{fig:normTprivtTshared}, we explore the \(T_{private}\) speedups across various serverless applications.  
% Notably, the difference between the Litmus discount (L-Discount) and the average speedup is merely 0.006.  This minute difference explains why Litmus can attains such high accuracy. 
%Furthermore, when comparing with figure~\ref{fig:priceErrorRunwith26}, a correlation between the error rate and the speedup differences becomes apparent. 
%For instance, float-py, with the most substantial difference above the Litmus discount, also experiences the most significant negative error rate. 
%Conversely, aes-go, with the smallest speedup, experiences the highest positive error rate.
% % original version
% Figure~\ref{fig:normTprivtTshared} shows the execution time of the baseline normalized to the execution time of each run under congestion. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the functions spend only 3.67\% more time on private resources, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, resulting in precise estimation with a Litmus test. 

% Figure~\ref{fig:normTprivtTshared26Rev} shows the execution time of each function run under congestion normalized to the execution time of the baseline. The gap of the bar to 1 is the amount of slowdown that should be translated to a discount in ideal cases. The top (black) and the bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that the interferences in private resources extend the function execution time only by 5.3\%, indicating the performance of the private resources is marginally affected by congestion. Additionally, all functions show similar \(T_{private}\) times with little dispersion, enabling precise estimation with a Litmus test.
Figure~\ref{fig:normTprivtTshared26Rev} shows the \(T_{private}\) and \(T_{shared}\) of each function, normalized to the same time components of the baseline. The gap between the bar and 1 represents the amount of slowdown that should be translated into ideal discounts. The top (black) and bottom (blue) dotted lines, along with the last bars, represent the estimated slowdowns of \(T_{private}\) and \(T_{shared}\) with Litmus tests. The figure shows that interferences in private resources extend the function execution time by only 5.3\%, implying the performance of the private resources is marginally affected by congestion. Additionally, all functions exhibit similar \(T_{private}\) values with little dispersion, helping precise estimation with Litmus tests.

% Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors are still in an acceptable range since their impacts are small. Functions that have a considerable \(T_{shared}\) ratio become more sensitive to system congestion. Instead, a function, such as float-py, with negligible \(T_{shared}\) ratio gains huge benefits with high discounts while its performance remains firm. This shows that Litmus pricing reflects the dynamically changing values of shared resources when the congestion level alters and encourages functions to be developed to use more private resources. 
Meanwhile, shared resources are more significantly affected than what the Litmus test estimates. However, the errors remain within an acceptable range as their impacts are minor. Functions that have a considerable \(T_{shared}\) ratio are more sensitive to system congestion. Conversely, a function like float-py, which has a negligible \(T_{shared}\) ratio, gains huge benefits from high discounts while maintaining stable performance under congestion. This shows that Litmus pricing accurately reflects the dynamic values of shared resources when the congestion level changes and incentivizes functions to be developed to use less shared resources. 

% \textbf{Litmus pricing under high congestion:} We test our Litmus pricing under a heavily congested environment to verify its pricing of functions with large slowdowns. To create a crowded environment, we concurrently execute 60 instances of Fibonacci-go, which produces the most L2 misses among our tested functions. 
% We raise the congestion level significantly with 60 co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo} shows the results from the same tests of Figure 11. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.8\%, which is only a 1.7\% difference from the ideal discount of 27.1\% with 2.48\% of an average absolute error. In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.151 and 4.299, which are only 2.45\% and 7.83\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. 
% \textbf{Litmus pricing under high congestion:} We raise the congestion level significantly with \hl{500} co-running Fibonacci-go, which produces the most L2 misses among the tested functions, to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceFibGo500} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. Again, the Litmus pricing shows a nearly ideal price, discounting the price by 28.1\%, which is only a 1\% difference from the ideal discount of 27.1\% with 0.088\% of an average absolute error. Litmus pricing discounts slightly more than an actual slowdown, leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% % \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
% \caption{The normalized total price for the applications calculated by using Litmus pricing and ideal prices when co-running with 500 Fibonacci-go}
% \label{fig:normalizedPriceCongested320}
% \end{figure}



%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure}[h]
%\centering
%\includegraphics[width=1\columnwidth]{./fig/diffStartupPortion-2Rev}\\
%\caption{The slowdown of Python's startup with 25 and 15 million instructions (X-axis) and the slowdown of reference applications (Y-axis). From left, \(T_{private}\), \(T_{shared}\), and \(T_{total}\), normalized to those when running alone}
%\label{fig:diffStartupPortion}
%\end{figure}

% \textbf{Instructions in Startup:} Litmus tests react differently to congestion when performed with different numbers of instructions from the startup phase. For example, Python's startup involves about 45 million instructions. While we have conducted Litmus tests using all these instructions, Figure~\ref{fig:diffStartupPortion} shows the response of these tests when running with the first 15 and 25 million instructions from this set. The figure shows the startups' \(T_{private}\), \(T_{shared}\), and \(T_{total}\) with two traffic generators, as depicted in Figure~\ref{fig:referenceStartupSlowdownRev}. Tests with fewer instructions are more sensitive to cold cache misses but less to interference in the L3 cache. Therefore, as the instruction count in Litmus tests decreases, they become less susceptible to conflicts in shared resources, especially from traffic by MB-Gen. As a result, tests with 25 million instructions exhibit reduced slowdowns. This trend becomes more apparent when running the tests with 15 million instructions, depicting that slowdowns when co-running with MB-Gen become nearly identical to those with CT-Gen. 

%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%







% \textbf{Instructions in Startup:} Python's whole startup phase contains about 45 million instructions. We can further divide the startup phase into smaller pieces with 10 million instructions code chunks. And each code chunk would have its characteristics. They react differently in the same congested environment. In section XXX we use the whole Python's startup portion's slowdown to indexsing the serverless application's slowdown. But, since the co-relationship between these two slowdown in different congestion source are different, one startup \(T_{private}\) slowdown may indicate two application's slowdown. By carefully picking the code chunks we can mitigate the difference between the two normalized slowdowns of the guidance application that correlated to the same startup phase slowdown. 

% Figure~\ref{fig:diffStartupPortion} depicts the correlation between the performance changes in the reference applications and distinct segments of Python's startup phase. From the figure, we see that selecting the first 15 million instructions as our startup phase results in the normalized \(T_{uncore}PerInst\) of the guidance application aligning nearly into a singular trendline. However, there are substantial gaps in the case of \(T_{core}PerInst\) with this code segment. Thus, we should pick xxx-xxx as our startup phase representation code for the normalized \(T_{core}PerInst\). We think that this can be used to mitigate the differences. But, we should be careful to use the small code chunks for the following reasons: First, only measuring the small portion can be a problem. The results might be too dynamic. Second, since we only measure this small portion there might be a huge execution period that cannot be covered.

% Continue to work from here

\subsection{Temporal CPU Sharing}
\label{sec:temporalCPUSharing}

The previous evaluation assumes an isolated environment where a CPU is assigned exclusively to an active function during execution, disallowing temporal sharing between functions through context-switching. While this setup ensures strict performance isolation, it inherently limits resource utilization. Conversely, enhancing utilization by permitting temporal CPU sharing among functions complicates price estimation. We explore how Litmus pricing can be applied in a less restrictive environment that permits sharing, where functions can temporarily share the same CPU and are not bound exclusively to specific cores. 

In this section, we deploy a testing function to co-run with 160 other functions across 16 cores without exclusive core assignments, assuming an average of 10 functions share a core. The reduction in the number of cores tested was necessitated by our system's memory limitations, as certain functions require significant memory space.

% \textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, the subsequent function clears the displaced one's cached data. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, the slowdown with extra sharing financially benefits the provider; we thereby argue that the extent of sharing should be factored into Litmus pricing as another discount factor.
\textbf{Method 1, Modeling Switching Overhead:} When a function is switched out, a subsequent function evicts the cached data of the displaced one. We noticed that this overhead grows as the number of co-running functions increases. Consequently, permitting more concurrent functions results in slower function execution. However, delayed execution due to extra sharing financially benefits the providers. Thus, we argue that the extent of temporal sharing should be incorporated into Litmus pricing as another discount factor.

Figure~\ref{fig:csImpactor} depicts the switching overheads as concurrently running functions increase. The figure demonstrates that the sharing overhead follows a logarithmic growth pattern and stabilizes at around 20 co-running functions. Furthermore, we discovered that the switching overheads predominantly affect \(T_{private}\). Consequently, Litmus pricing needs to calibrate \(T_{private}\) to account for the impacts of sharing before estimating the slowdown using the performance table.

Figure~\ref{fig:normalizedPrice160Method1} illustrates the discounted price reflecting this adjustment. In our configuration, with an average of 10 functions per core, we divide \(T_{private}\) by 1.025 before estimating the slowdown. In this figure, Litmus pricing estimates an average discount of 14.5\%, which falls 2.9\% short of the ideal discount of 17.4\%. While most benchmarks receive discounts lower than ideal, aes-py stands out with the largest error of 9.9\%, which is 6.9\% less than its ideal discount of 16.8\%.

\begin{figure}
\centering
% \includegraphics[width=1\columnwidth]{./fig/csImpactor}\\
\includegraphics[width=1\columnwidth]{./fig/csImpactor2}\\
\caption{\(T_{private}\) of functions over different co-running counts in the same core, normalized to when running alone}
% \vspace{-1em}
\label{fig:csImpactor}
\end{figure}

\begin{figure}
\centering
% \vspace{-1.2em}
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160Method1}\\
\caption{Prices derived from Litmus pricing (Method 1) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
% \vspace{-0.5em}
\label{fig:normalizedPrice160Method1}
\end{figure}

% In Figure~\ref{fig:normalizedPrice160Method1} we use the the same congestion and performance tables that we collected in the restricted environment. When checking the tables instead of using the original startup slowdown of tcore we use an adjusted slowdown by dividing the context switch impact factor. From figure~\ref{fig:normalizedPrice160Method1} we can see that the average Litums discount is 14.65\%, 3.01\% less than what they should receive compared to the ideal discount of 17.67\%. Most applications receive a smaller discount than the ideal price. The largest error is on aes-py with Litmus discount of 9.85\%, 6.87\% smaller than the ideal discount of 16.72\%. The smallest error is on dyn-py. It's Litmus discount is 22.45\%, only 0.47\% larger than the ideal discount of 21.97\%.

\textbf{Method 2, Updating Performance Tables:} Rather than reusing the performance/congestion tables designed for restrictive environments, arranging new tables for the sharing-enabled environments returns better accuracy. Although the notion of preparing separate tables for various sharing levels may seem challenging, we argue that only one or a few extra tables for heavily crowded systems would suffice, given that commercial systems are typically heavily crowded. Again, we emphasize that the impact of function co-placement stabilizes above a certain co-placement count, as shown in Figure~\ref{fig:csImpactor}.

For this test, we prepared new performance/congestion tables for the environment described above, where a testing function is assumed to co-locate and compete for a core with 9 other functions. Moreover, considering the scenario where a switched-out function has a low chance of being rescheduled to the same core, instead of assigning 10 functions to a specific core, we ran 50 functions across 5 dedicated cores; each can run on any of the 5 cores. We managed the congestion levels in shared resources using traffic generators on the other cores, as outlined in Section~\ref{sec:designDetails}.

\begin{figure}[h]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPrice160}
% \vspace{-0.6em}
\end{figure}

% Figure~\ref{fig:normalizedPrice160} illustrates the estimated prices derived from the Litmus pricing and ideal prices; both are normalized to the price from commercial pricing. The functions receive discounted prices as compensation for slowdowns in a congested execution environment. The figure shows minor differences between the two prices, implying that the Litmus pricing offers a reasonable discount. The average discount from the Litmus pricing across all functions is \hl{17.29\%}, which is only marginally smaller by \hl{0.38\%} than the average slowdown that the functions experience, which is \hl{17.67\%}, also shown as the ideal price.
Figure~\ref{fig:normalizedPrice160} shows the prices obtained from Litmus pricing with the new tables, which are normalized to those from commercial sources. Once more, as in Figure~\ref{fig:normalizedPrice26Rev}, the figure reveals marginal distinctions between the two price points, suggesting that Litmus pricing continues to offer a reasonable discount. Across all functions, the average discount provided by Litmus pricing stands at 17.2\%, merely 0.2\% less than the ideal discount of 17.4\%.


==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/09_sensitivity.tex <==
\section{Sensitivity}
\label{sec:sensitivity}

While the aforementioned tests highlight Litmus's potential, we recognize the need for more compelling results. This section expands our analysis and examines Litmus pricing from various angles across diverse system environments.

% \textbf{Heavy Congestions:} We raise the congestion level significantly with 320 co-running applications to verify its pricing of functions with substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} shows the results from the same tests of Figure~\ref{fig:normalizedPrice160}. The Litmus pricing is still close to the ideal price, discounting the price by 20.00\%, which is only a 1.46\% difference from the ideal discount of 21.46\%. The highest Litmus discount is 26.01\% for dyn-py. It has an error of 2.83\% compared with the ideal discount.
\textbf{Heavy Congestion:} We significantly escalate the congestion level to verify Litmus pricing under conditions of substantial slowdowns. Figure~\ref{fig:normalizedPriceCongested320} presents the outcomes of the same tests depicted in Figure~\ref{fig:normalizedPrice160} but with 320 co-running functions. Not only did we increase the function count, but we also specifically selected 8 memory-intensive functions, aes-py, compre-py, thum-py, bfs-py, auth-py, fib-go, geo-go, and profile-go, that produce the most L2 cache misses among the tested functions to create heavy congestion in shared resources deliberately. Even under such intensified congestion, Litmus pricing produces results remarkably close to the ideal price, discounting the price by 20.0\%, which deviates by merely 1.5\% from the ideal discount of 21.5\%. The highest discount by Litmus pricing is 26.0\% for dyn-py, a minor error of 2.8\% compared to the ideal discount.


% leaving no financial benefits for providers when the providers make the system overly crowded by scheduling excessively many tasks. Meanwhile, the tenants experience poor service with a slowed system. 
% \hl{Meanwhile, the tenants may leave negative feedback about their experiences with the slow system}. 

% In further detail, Litmus tests estimate slowdowns for \(T_{private}\) and \(T_{shared}\) are 1.148 and 3.946, only 2.10\% and 15.37\% different from the actual applications' slowdowns, 1.124 and 4.663, respectively. Additionally, we observe the functions that suffer from slowdowns more in Figure~\ref{fig:normalizedPrice26} also suffer more in Figure~\ref{fig:normalizedPriceFibGo}. For example, the least and most discounted functions in Figure~\ref{fig:normalizedPrice26} are float-py and dyn-py, which received 4.5\% and 14.8\% discounts, respectively. In Figure~\ref{fig:normalizedPriceFibGo}, they remain the least and most discounted functions with 13.2\% and 33.7\%. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCongested320}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 320 others, both normalized to commercial prices that offer no discount}
\label{fig:normalizedPriceCongested320}
% \vspace{-1em}
\end{figure}

\textbf{CPU Frequency:} Modern CPUs feature dynamic CPU frequency adjustments, which are controlled via software or hardware. A hardware technique like Intel Turbo Technology autonomously adjusts the CPU frequency based on the CPU's power and thermal budgets, allowing the CPU to operate at higher frequencies when conditions permit and lower frequencies under heavy load. Prior tests assumed that the frequencies were fixed and strictly managed by service providers who had knowledge of when and to what extent frequency adjustments were necessary. Also, we evaluated Litmus pricing under the other scenarios where CPU frequencies were not fixed, providing more dynamic perspectives.

% Figure~\ref{fig:normalizedPrice160unset} illustrates the prices from the Litmus pricing and the ideal price, which are normalized to commercial prices. We tested it under the configuration in Section 7.2 with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, the Litmus pricing's discount is lowered from 17.16\% to 16.84\%, while the ideal discount rate is decreased from 17.42\% to 17.31\%. Still, the discount rate difference from the ideal price is only 0.47\% without setting the CPU frequency. We observed that the CPU frequency changes rarely when the system runs with 160 functions. Overall, the varying frequency made a minor impact on performance as well as the pricing scheme. 
Figure~\ref{fig:normalizedPrice160unset} illustrates the prices derived from Litmus pricing alongside the ideal prices, both normalized to commercial prices. This evaluation was conducted under the configuration outlined in Section~\ref{sec:temporalCPUSharing} with 160 other functions. Compared with Figure~\ref{fig:normalizedPrice160}, we observe a slight decrease in Litmus pricing's discount, from 17.2\% to 16.8\%, while the ideal discount rate decreases from 17.4\% to 17.3\%. Still, even without fixed CPU frequencies, the difference in the discount rate from the ideal price is only 0.5\%. We noted that CPU frequency changes were infrequent when the system operated with 160 functions. Overall, the variation in frequency had a negligible impact on Litmus pricing.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPrice160unset}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others with unfixed CPU frequencies, both normalized to commercial prices}
\label{fig:normalizedPrice160unset}
% \vspace{-1em}
\end{figure}

% All the above experiments are done on Intel Xeon Gold 5218(Cascade Lake). We also perform our scheme on another CPU architecture, Intel Xeon Silver 4314(Ice Lake-SP). 
\textbf{CPU Architecture:} Ensuring the validity of Litmus pricing across different architectures is crucial. Our Litmus tests rely on the performance counter that measures a stall count due to L2 cache misses (cycle\_activity.stalls\_L2\_miss)~\cite{perfMonEvents}, supported by Intel's CPUs. Unfortunately, other vendors like AMD do not yet offer the same performance counter~\cite{amdPMC}, restricting our tests to Intel CPUs. Alternatively, we conducted tests on another Intel CPU based on the Ice Lake architecture, Xeon Silver 4314, to broaden the scope of our analysis.

\begin{figure}[b]
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun70kiwi}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 70 others on Xeon Silver 4314, both normalized to commercial prices}
\label{fig:normalizedPriceCorun70kiwi}
\end{figure}

% Because of the limitation of our memory size, we test Limtmus with 70 co-running applications. In this test, we use method 2 introduced in section~\ref{sec:temporalCPUSharing}. We first conduct the congestion and performance tables with 50 applications running in the first 5 cores. Then for the evaluation, we run 70 applications in the first 7 cores to let our testing application compete with 9 other applications for a core.  Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus discounting the tenant only pays 82.52\% commercial price. It's 0.696\% less than with the ideal discount.
Once again, this evaluation was conducted following the configuration outlined in Section~\ref{sec:temporalCPUSharing}, albeit with 70 co-running functions, limited by the main memory capacity of 128GB. Following Method 2, we constructed new congestion and performance tables with 50 functions running across 5 cores. Then, we ran 70 functions across 7 cores to match the competition count, averaging 10 functions per core. Figure~\ref{fig:normalizedPriceCorun70kiwi} presents the results. On average, with Litmus pricing, the tenant only pays 82.5\% of the commercial prices, which is merely 0.7\% less than the ideal price.

% \textbf{Per-core Function Count:} When altering the co-located applications in each core the performance of the application can also be influenced. In this test, we put 240 applications in the first 16 cores. The testing application is competing with 14 other applications. We used the same congestion and performance tables from section~\ref{sec:temporalCPUSharing} method 2. Figure~\ref{fig:normalizedPriceCorun15} presents the results. The error of Litmus pricing is 1.23\% with The average discount of 16.69\%. The ideal discount is 17.92\%. The mean price of Litmus is larger than the ideal price because we are using the tables that are made based on 10 applications per-core. The context-switching overhead is larger. But, from figure~\ref{fig:csImpactor} we know that there is a diminishing impact of per-core application count. The error of the Litmus pricing is still under control when we increase the per-core application count.
\textbf{CPU Sharing Overhead:} The co-located function count determines the level of interference, impacting a function's performance differently. To assess Litmus pricing under various co-running function counts, we increased the function count to 240 from the configuration outlined in Section~\ref{sec:temporalCPUSharing}, making an average of 15 functions running on each core. However, we reused the performance and congestion tables generated in Section~\ref{sec:temporalCPUSharing}. Figure~\ref{fig:normalizedPriceCorun15} illustrates the results, where the Litmus pricing's error is 1.2\% with an average discount of 16.7\%, compared to the ideal of 17.9\%. Despite reusing the tables constructed for 10 co-running functions per core, the error remains negligible. This outcome aligns with Figure~\ref{fig:csImpactor}, which highlights the diminishing impact of temporal sharing when running more than 10 co-running functions. Given the perpetual overcrowding of commercial systems, any configuration gap between the environment where constructing the tables and where conducting tests is expected to remain minor and easily manageable.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun15}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 15 functions per core and reusing tables, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun15}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
\caption{Prices derived from Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, both normalized to commercial prices}
% \vspace{-0.5em}
\label{fig:normalizedPriceCorun160smt}
\end{figure}

\textbf{Simultaneous Multithreading (SMT):} SMT is a technique aimed at maximizing resource utilization by enabling multiple threads to execute concurrently on the same core, extending the shared resource domain across the entire processor. However, while SMT enhances resource utilization, it significantly complicates the measurement of interference impact. Moreover, SMT introduces additional side channels, thereby increasing the processor's vulnerability to security attacks. Due to these concerns, serverless platforms like Amazon Lambda disable SMT in their systems~\cite{schall2023warming,agache2020firecracker,schall2022lukewarm}. Nonetheless, we have conducted a study to assess the impact of SMT on our Litmus pricing methodology.

% \begin{figure}
% \centering
% \includegraphics[width=1\columnwidth]{./fig/normalizedPriceCorun160smt}\\
% \caption{Prices computed via Litmus pricing (Method 2) and ideal prices when co-running with 160 others in an SMT-enabled system, normalized to the commercial prices}
% \vspace{-0.5em}
% \label{fig:normalizedPriceCorun160smt}
% \end{figure}

% To generate the performance/congestion tables, we executed 50 applications across 5 dedicated physical cores. In this way, the testing function is co-located with 9 other applications in the same virtual core and 19 other applications in the same physical core. Fiugre~\ref{fig:normalizedPriceCorun160smt} illustrates the results. The first thing we notice is that the normalized price is much smaller compared with the setups without SMT turned on. The average discount of Litmus is 45.42\% which is 1.9\% smaller than the average ideal discount of 47.32\%.
To construct the performance and congestion tables, we executed 50 applications across 5 physically separated cores, allowing an average of 10 functions to share two virtual cores. Figure~\ref{fig:normalizedPriceCorun160smt} illustrates the results,  presenting prices derived from Litmus pricing and ideal prices, both normalized to commercial prices without discounts. The normalized price experiences a significant drop compared to other configurations, highlighting the impact of heavy congestion within a physical core. The ideal price, which assumes no interference, stands at 47.3\% of the commercial price. Meanwhile, Litmus pricing offers a discount of 45.4\%, which is only 1.9\% less, confirming the effectiveness of Litmus pricing.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Node JS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Nodejs Startup:}NodeJs is another well-adopted language in serverless platforms besides Python. It's one of the earliest languages to be supported by AWS Lambda ~\cite{serverless1}. From Section~\ref{sec:designDetails} we see that NodeJs has a long startup phase which makes it a great candidate when we need to pick a language startup phase for the Litmus test. 

%\begin{figure}[h]
%\centering
%\vspace{-0.5em}
%\includegraphics[width=1\columnwidth]{./fig/njReferenceStartupSlowdown}\\
%\vspace{-1em}
%\caption{The correlation between the normalized NodeJs's startup phase and the normalized reference applications.}
%\vspace{-0.5em}
%\label{fig:njReferenceStartupSlowdown}
%\end{figure}

%Figure~\ref{fig:njReferenceStartupSlowdown} shows the correlation between NodeJs startup phases and reference applications. After applying the Litmus test with NodeJs applications, with this figure, we can use the slowdown of the NodeJs startup phase to find the corresponding system congestion level and the discount rate for both private and shared resources. NodeJs has a longer startup phase compared with Python. It gives us more room when picking the most suitable portions of the startup phase. We can choose the language to be used for the Litmus test based on the density of the startup phase. 


==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/10_related.tex <==
\section{Related Work}
\label{sec:related}

% \textbf{Serverless:} Many works address the performance bottleneck of serverless execution~\cite{du2020catalyzer}~\cite{agarwal2021reinforcement}~\cite{roy2022icebreaker}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Schall et al.~\cite{schall2022lukewarm} record and reload the instructions to reduce the front-end stalls when reaccessing the same application. Jovan et al.~\cite{stojkovic2023specfaas} focus on the performance of an application chain. They break the execution flow and speculative execute the functions. However, we are focusing on the price which is one of the most important potions of the cloud ecosystem.

% For the cloud providers, accommodating more tenants in a machine is a key strategy, gaining higher profits by maximizing the utilization of their machines. However, the approach inevitably introduces interference between tenants, slowing down applications unpredictably. Thus, prior researchers solved this challenge by allowing the tenants more non-biased, predictable, quality services~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed a clustering-based cache partitioning to remove unfairness between tenants. Rohan et al.~\cite{roy2021satori} simultaneously control multiple architectural resources to aim for both fairness and throughput. However, offering fairness inevitably sacrifices resource utilization. Thus, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} solve the unfairness uniquely by adjusting their prices while leaving the unfairness at a certain degree. This paper follows this direction but explores a more practical solution in serverless computing. 

Cloud providers strive to maximize profits by accommodating more tenants on their machines, which inevitably introduces interference between tenants, leading to unpredictable application slowdowns. To address this challenge, prior researchers have focused on providing tenants with a more unbiased and predictable quality of service~\cite{kannanproctor,zhao2021understanding,lee2009mcc,jin2015hardware,kannan2019caliper,vicent2017AppClustering,lavanya2015AppSlowdown}. Vicent et al.~\cite{vicent2017AppClustering} proposed clustering-based cache partitioning to mitigate unfairness between tenants. Rohan et al.~\cite{roy2021satori} aimed for both fairness and throughput by simultaneously controlling multiple architectural resources. However, achieving fairness comes at the cost of sacrificing resource utilization. In contrast, Alex et al.~\cite{alex2013ScFairPrice,tiwari2013enabling} addressed the unfairness by adjusting their prices while accepting a certain degree of unfairness. Our study follows a similar direction but explores a more practical solution within the context of serverless computing.

% delete the following section: the approaches are against our scheme. 
% \textbf{Serverless Computing:} Many studies focus on reducing the latencies of serverless applications~\cite{cadden2020seuss,oakes2018sock,wang2019replayable,jia2021boki}. Dong et al.~\cite{du2020catalyzer} proposed Catalyzer, a new serverless sandbox that restarts the application from a checkpoint image to reduce the cold start cost. Ustiugov et al.~\cite{ustiugov2021benchmarking} record and prefetches the functions’ stable working set of guest memory pages to further reduce the function's startup time. Wei et al.~\cite{wei2023no} remote forking the serverless functions to reduce the cold start latency while limiting the resource usage. Schall et al. record and reload the instructions~\cite{schall2022lukewarm} or the BTB entries ~\cite{schall2023warming} to reduce the front-end stalls when reaccessing the same application. 
% \hl{Litmus is orthogonal to these approaches and can be adopted together.}

==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Serverless computing is a key technology in present cloud computing, offering numerous advantages. One primary advantage is its effective cost-saving, as tenants only pay for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion. While tenants suffer slowdowns, they also have to pay more for the slowdowns. Unlike prior approaches that aim to maintain quality of service, this paper discounts the tenant's cost to compensate for the loss. Litmus pricing proposed in this work monitors the machine states and adjusts the tenants' costs. The congestion level can be frequently gauged before every function using the proposed Litmus test, an effectively lightweight testing approach. Our tests show that Litmus offers near-ideal prices with a 0.38\% difference, compared to the ideal price that discounts proportional to its slowdown. 
Serverless computing is a key technology in contemporary cloud computing, offering a range of benefits. One primary advantage is effective cost-saving, as tenants are billed only for the resources they use. However, the time-based fees on commercial platforms can unfairly charge tenants during periods of high congestion, which not only results in slowdowns but also higher costs for tenants. Rather than aiming to maintain service quality, this paper suggests discounting tenants' costs to compensate for performance losses. Litmus pricing proposed in this work monitors machine states through Litmus tests and adjusts tenant costs accordingly. The Litmus test is a lightweight testing approach for serverless platforms, which assesses the machine's congestion level before starting a user's function. Our tests prove that Litmus pricing offers nearly ideal prices in heavily congested environments, with an average deviation of just 0.2\% from the ideal price that adjusts discounts in proportion to the slowdown experienced.


==> smmwbfjzgbfsdyszxjtzpxpjqzmtbmkk/12_ack.tex <==
\section{Acknowledgment}
\label{ack}

We would like to thank our reviewers for their valuable feedback to improve this paper. This work was supported by NSF CAREER Award CCF-2146475.

